3D Imaging via Polarized Jet Fragmentation Functions and Quantum Simulation of the QCD Phase Diagram

Understanding the interactions between elementary particles and mapping out the internal structure of the hadrons are of fundamental importance in high energy nuclear and particle physics. This thesis concentrates on the strong interaction, described by Quantum Chromodynamics (QCD). We introduce a novel concept called "polarized jet fragmentation functions" and develop the associated theory framework known as QCD factorization which allows us to utilize jet substructure to probe spin dynamics of hadrons, especially nucleon's three-dimensional imaging. Furthermore, non-perturbative QCD studies, particularly of the QCD phase diagram, are important for understanding the properties of hadrons. The development of quantum computing and simulators can potentially improve the accuracy of finite-temperature simulations and allow researchers to explore extreme temperatures and densities in more detail. In this thesis, I present my work in two aspects of QCD studies: (1) investigating the nucleon structure using polarized jet fragmentation functions and (2) illustrating how to apply quantum computing techniques for studying phase diagram of a low energy QCD model. The first category investigates phenomena such as hadron production inside jets, spin asymmetries, etc., providing valuable insight into the behavior of quarks and gluons in hadrons. The second category provides potential applications of quantum computing in QCD and explores the non-perturbative nature of QCD.

==> Makefile <==

#
# uclathes Makefile
# Copyright (C) 1995 by John Heidemann, <johnh@isi.edu>
#

FILES=README \
	demo.tex demo.dvi demo.pdf \
	demo_techreport.tex demo_techreport.pdf \
	thesis_spec.tex thesis_spec.pdf \
	uclathes.cls uclath12.clo uclathti.clo uclathma.clo \
	uclathes.bst Makefile

all:  latex ps pdf

tar: $(FILES)
	tar cvf uclathes.tar $(FILES)

tar.gz:
	@echo "Make all before doing make tar.gz"
	tar czvf uclathes.tar.gz $(FILES)

DVIPS=dvips
PS2PDF=ps2pdf14

latex latex.demo::
	latex demo

ps demo.ps::
	$(DVIPS) demo

pdf demo.pdf::
	$(PS2PDF) demo.ps demo.pdf

latex latex.demo_techreport::
	latex demo_techreport

ps demo_techreport.ps::
	$(DVIPS) demo_techreport

pdf demo_techreport.pdf::
	$(PS2PDF) demo_techreport.ps demo_techreport.pdf

latex latex.thesis_spec::
	latex thesis_spec

ps thesis_spec.ps::
	$(DVIPS) thesis_spec

pdf thesis_spec.pdf::
	$(PS2PDF) thesis_spec.ps thesis_spec.pdf

clean:
	rm *.aux *.toc *.lot *.lof *.dvi *.log *.ps


==> ch2.1-theory.tex <==
\section{Introduction}
Examining Quantum Chromodynamics (QCD) at extremely short wavelengths reveals its essence as a theory involving liberated ``partons'' - quarks and gluons. These partons interact through small quantum corrections, amenable to systematic calculations. However, as wavelengths extend to the scale of a proton ($\sim1\, \rm{fm} = 10^{-15}$\, m), tightly bound structures of hadron resonances emerge, forming string-like potentials when attempting to separate the partonic constituents. Analytic calculations in strongly coupled field theories pose challenges, leaving QCD only partially resolved. Nevertheless, the Lagrangian, a concise one-line formula, is believed to encode all features of QCD across different distance scales.

In the realm of collider physics, certain aspects of QCD can be evaluated using the fundamental parameters within the Lagrangian, while others necessitate models or functions incorporating effective parameters constrained through data fitting. Despite the absence of a factorized perturbative expansion, several robust theorems establish connections between seemingly disparate processes. Consequently, measuring the partonic substructure of the proton in ep collisions and applying the same parametrizations in pp collisions is justifiable. Hence, even without a perturbative expansion, predictive capabilities persist.

An alternative approach involves relinquishing direct QCD calculations in favor of utilizing leptons, encompassing inclusive summation of strong interaction phenomena. While this strategy may replace current QCD understanding with a sense of ``unity'', fundamental facts in collider physics remain significant for the foreseeable future. Firstly, the LHC operates with initial hadron states, demanding well-understood and precise parton distribution functions (PDFs). Secondly, achieving high precision necessitates computations at higher perturbation theory orders, entailing deeper involvement of QCD. Thirdly, the definition of a lepton inherently relies on QCD due to the requisite isolation criterion. Explicitly, the rate of misidentified jets as leptons in experiments depends on QCD. Finally, though some new-physics signals may manifest in the lepton sector, their occurrence is not assured nor exclusive. Thus, it would be unwise to disregard our utmost efforts in solving QCD, enabling us to maximize discovery potential and subsequent precision.

Furthermore, QCD stands as the most intricate gauge theory encountered to date. Its emergent phenomena, unitarity properties, color structure, non-perturbative dynamics, and interplay between scale-invariant and scale-dependent characteristics remain subjects of active exploration and continuous learning. The broad range of phenomenological applications further enhances its enduring significance.

Moreover, the field of QCD presently experiences a revolution. Perturbatively, novel methods are under development to compute scattering amplitudes involving a high number of particles, alongside advanced techniques that incorporate all-orders resummation frameworks. On the non-perturbative front, the wealth of soft-physics data from the LHC challenges the reliability of standard fragmentation models. Additionally, insights into the collective behavior of hadronic matter are being gleaned from heavy-ion collisions, while the study of cosmic rays and dark matter annihilation processes presents challenges that advance our understanding of fragmentation modeling.

\subsection{QCD Lagrangian}
The QCD Lagrangian is given by
\begin{equation}
\mathcal{L}_{\text{QCD}}=-\frac{1}{4} F_{\mu \nu}^a F^{a \mu \nu}+\sum_q\bar{\psi}_q^i\left[i \gamma^\mu\left(D_\mu\right)_{i j}-m_q\delta_{ij}\right] \psi_q^j\,,\label{eq:(1.10)}
\end{equation}
where $i$ denotes the colour index of a quark field $\psi_q^i$, namely $\psi_q=\left(\psi_{q R}, \psi_{q G}, \psi_{q B}\right)^T$. The Dirac matrix $\gamma^\mu$ is used to express the vector nature of the strong interaction, where $\mu$ is a Lorentz vector index. The parameter $m_q$ accommodates the possibility of nonzero quark masses, which can be induced by mechanisms such as the standard Higgs mechanism. The gluon field strength tensor $F_{\mu \nu}^a$ with a color index $a$ ranging from 1 to 8 is given by
\begin{equation}
F_{\mu \nu}^a=\partial_\mu A_\nu^a-\partial_\nu A_\mu^a+g_sf^{abc}A_\mu^b A_\nu^c\,,
\end{equation}
and the covariant derivative $D_\mu$ in QCD is
\begin{equation}
\left(D_\mu\right)_{i j}=\delta_{i j} \partial_\mu-i g_s t_{i j}^a A_\mu^a\,.
\end{equation}
In the context at hand, the parameter $g_s$ corresponds to the strong coupling strength and is related to $\alpha_s$ by the equation $g_s^2=4 \pi \alpha_s$. A more detailed explanation of the strong coupling will be provided later. The gluon field, represented by $A_\mu^a$, possesses a color index denoted as $a$. Additionally, the quantity $t_{i j}^a$ is directly proportional to the Hermitian and traceless Gell-Mann matrices of SU(3). These matrices, adorned with indices enumerating their rows and columns as fundamental indices ranging from 1 to 3, hold paramount importance. Their influential nature extends to adjoint indices, spanning from 1 to 8, signifying the generators themselves. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Below
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The running coupling}
In quantum chromodynamics (QCD), an initial approximation reveals its property of scale invariance. This characteristic manifests as a fractal-like pattern of nested jets within jets when examining a QCD jet at a closer scale. Originally referred to as light-cone scaling or Bj$\ddot{o}$rken scaling in the context of QCD, this phenomenon exhibits repeated self-similar structures. In addition to this fundamental scaling behavior, the running coupling incorporates an inherent reliance on the absolute scale, resulting in greater radiation observed at lower scales compared to higher ones. The running of the coupling is logarithmic with respect to energy and is governed by the beta function,
\begin{equation}
Q^2 \frac{\partial \alpha_s}{\partial Q^2}=\frac{\partial \alpha_s}{\partial \ln Q^2}=\beta\left(\alpha_s\right)\,,\quad
\beta\left(\alpha_s\right)=-\alpha_s^2\left(b_0+b_1 \alpha_s+b_2 \alpha_s^2+\ldots\right)\,.\label{eq:19}
\end{equation}
The equation \cref{eq:19}, bearing a negative overall sign and with $b_0 > 0$, holds significant implications. It leads to the well-known phenomenon of \textit{asymptotic freedom} in quantum chromodynamics (QCD), wherein the effective QCD coupling diminishes as energy increases. The discovery of asymptotic freedom was acknowledged with the Nobel Prize in Physics awarded to D. Gross, H. Politzer, and F. Wilczek in 2004. And the numerical solution of the strong coupling is commonly performed by specifying its value at a specific reference scale, denoted as $Q^2=M_Z^2$. By solving \cref{eq:19}, we can subsequently deduce the value of the strong coupling at any desired scale,
\begin{equation}
\alpha_s\left(Q^2\right)=\alpha_s\left(M_Z^2\right) \frac{1}{1+b_0 \alpha_s\left(M_Z^2\right) \ln \frac{Q^2}{M_Z^2}+\mathcal{O}\left(\alpha_s^2\right)}\,.\label{eq:20}
\end{equation}
\begin{figure}[htb]
    \centering
    \includegraphics[width=3.6in]{./intro/rpp2022-rev-qcd.pdf}   
    \caption{Summary of running coupling $\alpha_s$ measured as a function of the energy scale $Q$ provided in~\cite{ParticleDataGroup:2022pth}. In brackets, the respective degree of perturbative QCD applied for the extraction of $\alpha_s$ is indicated (for example, NLO: next-to-leading order; NNLO+res.: next-to-next-to-leading order matched to a resummed calculation; etc.)}
    \label{fig:alphas}
\end{figure}
One notable consequence of asymptotic freedom is the improved convergence of perturbation theory at higher absolute energies, owing to the diminishing coupling. Consequently, perturbative calculations for the $900$ GeV $Z_0$ boson, are expected to exhibit slightly faster convergence compared to equivalent calculations for the $90$ GeV counterpart. Additionally, the running of $\alpha_s$ disrupts Bj$\ddot{o}$rken scaling, resulting in minor alterations to jet shapes and jet production ratios as energy is varied. For example, high-$p_\perp$ jets, characterized by a reduced effective coupling, tend to possess narrower intrinsic shapes relative to low-$p_\perp$ jets, disregarding boost effects. This consideration holds significance in jet calibration. The current understanding of the running behavior of the QCD coupling is summarized by the plot presented in \cref{fig:alphas},
taken from the recent Particle Data Group~\cite{ParticleDataGroup:2022pth}. 

Moreover, it is worth mentioning that the decreasing nature of the strong coupling with energy ultimately leads to its eventual comparability with the electromagnetic and weak couplings at a certain energy scale. Beyond this point, which is estimated to be around $10^{15}-10^{17}$ GeV\footnote{Although it could be lower if yet-to-be-discovered particles introduce significant corrections to the running.}, the subsequent evolution of the combined theory remains unknown. It is uncertain whether asymptotic freedom will persist or if the theory will manifest different characteristics.

Next let us explore the behavior of the coupling as we trace its evolution towards lower energies. At first glance, the numerical value of the coupling appears to diverge rapidly at scales below 1 GeV, as demonstrated by the curves extending beyond the left boundary of the plot shown in \cref{fig:alphas}. To elucidate this divergence, we can reformulate Eqn.~\eqref{eq:20} as $\alpha_s\left(Q^2\right)={1}/\left(b_0 \ln \frac{Q^2}{\Lambda^2}\right)$, where the energy scale $\Lambda \sim 200 \mathrm{MeV}$ denotes the point at which the perturbative coupling would ostensibly diverge, commonly referred to as the Landau pole. It is important to note, however, that this characterization solely pertains to the purely perturbative outcome. Consequently, the above expression should not be interpreted as implying a divergence in the physical behavior of full QCD as $Q$ approaches $\Lambda$, as the perturbative result becomes unreliable at strong coupling.

Moreover, it is crucial to acknowledge the existence of various definitions for both $\Lambda$ and $\alpha_s\left(M_Z\right)$. The obtained numerical value depends, at the very least, on the employed renormalization scheme, with the dimensional-regularization-based ``modified minimal subtraction'' scheme ($\overline{\mathrm{MS}}$) being the most commonly utilized. Additionally, the perturbative order of the calculations employed to extract these values further contributes to their numerical discrepancies.

%

%In the subsequent sections of this chapter, we will delve into the theoretical foundations of QCD, encompassing the widely known factorization formalism and other non-perturbative tools. Additionally, we will explore the QCD factorization formalism, which enables us to investigate the structure of hadrons and their hadronization process using perturbative techniques. Furthermore, we will explore non-perturbative methods that facilitate the direct computation of the non-perturbative structure of hadrons based on first principles. Lastly, we will explore the emerging field of quantum computing and its potential to provide novel insights and perspectives in the study of QCD.


\section{QCD factorization}\label{sec2.1-qcd-fac}
% QCD factorization to probe hadron structure and Hadronization
Although Quantum Chromodynamics (QCD) has achieved remarkable success in elucidating a wide range of phenomena, it remains an intricate subject due to the intricate nature of the strong interaction. Perturbative techniques, firmly established in the domain of quantum field theory, can be effectively applied to QCD at high energies. This approach is initiated by calculating Matrix Elements (MEs), which can be systematically evaluated at fixed orders (FO) in the strong coupling constant $\alpha_s$. The procedure, particularly at the lowest order (LO) has been substantially automated with the development of tools such as $\mathtt{MADGRAPH}$~\cite{Alwall:2011uj}, $\mathtt{CALCHEP}$~\cite{Pukhov:2004ca}, and others~\cite{,Boos:2004kh,Kanaki:2000ey,Krauss:2001iv,Moretti:2001zz,Kilian:2007gr,Cafarella:2007pc,Bahr:2008pv,Gleisberg:2008fv}.

However, one of the key challenges in studying QCD is the fact that hadrons are composite objects made up of quarks and gluons, which interact strongly with each other. Consequently, non-perturbative approaches are indispensable for comprehending the physics of hadrons at low energies where the perturbative methods lose validity.

The QCD factorization formalism provides a way to separate the perturbative and non-perturbative contributions to the cross section of a hard scattering process involving hadrons. This allows us to compute the perturbative part using standard quantum field theory techniques, while the non-perturbative part is encapsulated in the form of hadronic distribution functions, which can be measured experimentally.

However, reality presents a more intricate picture. Several complications warrant attention. Firstly, the inclusion of additional jets, commonly referred to as real-emission corrections, can substantially alter the final state topology, potentially causing jets to fall within or outside the experimentally defined acceptance region. Secondly, loop factors, also known as virtual corrections, modify the number of available quantum paths within phase space, consequently influencing the normalization of the cross section, both in its total and differential forms. Lastly, confinement and the so-called underlying event give rise to further corrections. Accounting for these corrections is imperative for a comprehensive understanding of QCD and for establishing a connection between short-distance physics and macroscopic experiments. Beyond the perturbative expansion itself, the most effective tool at our disposal for managing this extensive calculation is factorization.

When dealing with high-energy scattering processes involving initial-state hadrons, we encounter an immediate complication stemming from the composite nature of hadrons. As depicted in Figure 8, hadrons consist of partons enveloped within clouds of additional partons, constantly emitting and absorbing one another. Consequently, before we can utilize perturbatively calculated partonic scattering matrix elements, it becomes imperative to address the partonic composition of the colliding hadron(s).

In order for the hadron to remain intact, fluctuations occurring within it must involve momentum transfers that are smaller than the confinement scale. Specifically, fluctuations with high virtuality are suppressed by factors of
\begin{equation}
\frac{\alpha_s \Lambda^2}{|k|^2},
\end{equation}
where $\Lambda$ denotes the confinement scale (approximately 200 MeV, as discussed in Section 1.4) and $|k|$ represents the virtuality of the fluctuation. Consequently, the majority of fluctuations occur over timescales of the order of $\sim 1 / \Lambda$.

Conversely, a hard perturbative probe, such as the exchanged photon in Deep Inelastic Scattering (as illustrated in Figure 3), interacts over a much shorter timescale of $1 / Q \ll 1 / \Lambda$. During this brief interval, the partonic fluctuations within the struck hadron appear to be nearly frozen. The hard probe effectively captures an instantaneous snapshot of the hadron's structure, with a characteristic resolution approximately given by $\sim 1 / Q$.

The principle of factorization, as established in the factorization theorem~\cite{Collins:1981uw,Sterman:1995fz}, formalizes the notion that the characteristics of long-wavelength (soft) structures remain unaffected by the specific properties of the underlying short-distance (hard) processes. Initially developed for deep inelastic scattering (DIS), factorization enables us to express the cross section of lepton-hadron scattering as a convolution involving a non-perturbative yet universally applicable parton density function (PDF) and a perturbatively computable partonic scattering cross section. In this context, the variable $x_i$ represents the fraction of the hadron momentum carried by the parton $i$.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Below
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The lepton-hadron cross section can be expressed in a factorized form, as exemplified in previous works (see, for instance~\cite{Brock:1993sz,Dissertori:2003pj} ),
\begin{equation}
\sigma_{\ell h}=\sum_i \int_0^1 \mathrm{~d} x_i \int \mathrm{d} \mathcal{PS}\, f_{i / h}\left(x_i, \mu_F^2\right) \frac{\mathrm{d} \hat{\sigma}_{\ell i \rightarrow f}\left(x_i, \mathcal{PS}, \mu_F^2\right)}{\mathrm{d} x_i \mathrm{~d} \mathcal{PS}}\,.
\end{equation}
Here the index $i$ spans across all potential parton types present within the incoming hadron, while the index $f$ enumerates all feasible (partonic) final states characterized by a Lorentz-invariant phase space denoted as $\mathcal{PS}$.

The parton density functions (PDFs), denoted as $f_{i / h}$, serve as parametric descriptions that capture the distribution of partons within the target hadron. These functions cannot be determined a priori and must be constrained through fitting procedures applied to empirical data. On the other hand, the partonic cross section, denoted as $\mathrm{d} \hat{\sigma}$, possesses no knowledge of the specific properties of the target hadron, except for the presence of the struck parton, and is computable within the framework of perturbation theory.

The determination of the factorization scale, denoted as $\mu_F$, involves a certain level of arbitrariness. Its selection can be guided by various heuristic arguments. In terms of long-distance effects, the parton density functions (PDFs) incorporate a summation of fluctuations within fluctuations up to virtualities of approximately $\mu_F$. Consequently, setting $\mu_F$ significantly larger than the characteristic scales associated with resolved particles in the short-distance calculation (i.e., particles explicitly present in $\Phi_f$) would lead to PDFs including summations over fluctuations occurring on timescales shorter than those probed by the physical process. Similarly, $\mu_F$ should not be set considerably lower than the scales involved in the hard process. For matrix elements characterized by a single well-defined scale, such as the $Q^2$ scale in deep inelastic scattering (DIS) or the invariant-mass scale $\hat{s}$ in Drell-Yan production $\left(q \bar{q} \rightarrow Z / \gamma^* \rightarrow \ell^{+} \ell^{-}\right)$, the preferred scale choices are essentially $\mu_F=Q$ or $\mu_F=\sqrt{\hat{s}}$, respectively. These choices can be varied by a factor of 2 or more around the nominal value to estimate uncertainties. However, in the case of multi-scale problems like $p p \rightarrow Z / W+n$ jets, there are multiple a priori equally valid choices, spanning from the lowest to the highest QCD scales constructed from the final-state momenta. Different groups of theorists often hold diverging opinions on which specific choice is the most suitable, leading to ongoing debates. Simply suggesting the direct measurement of the scale itself would not resolve this issue, as the factorization scale is fundamentally non-physical and unobservable, similar to gauge or convention choices. One viable strategy is to investigate higher-order calculations (NLO or NNLO), which incorporate correction terms that cancel out the scale dependence and stabilize the final outcome. Through such comparisons, it is theoretically possible to identify an initial scale choice that demonstrates the highest level of stability, providing a reasonable starting point. However, it is crucial to emphasize that this matter inherently possesses ambiguity, and there is no definitive recipe that guarantees the correct answers in all cases. The most appropriate approach is to vary the value of $\mu_F$ not only by an overall factor but also by exploring different potential functional forms that depend on the momenta present in $\Phi_f$.

Additionally, from a technical standpoint, when considering calculations at NLO (next-to-leading order) and higher orders, it becomes necessary to determine a specific factorization scheme. In practice, students focusing on LHC (Large Hadron Collider) physics are typically exposed to a single scheme known as the modified minimal subtraction ($\overline{\mathrm{MS}}$) scheme, which has been previously discussed in the context of defining the strong coupling. Given the scope of these lectures, we will not delve further into the details of this scheme at this juncture. It is worth noting, however, that factorization can be applied iteratively to decompose complex calculations into more manageable components, treating them as approximately independent entities.

In conclusion, the QCD factorization formalism is a powerful tool that enables us to probe the structure of hadrons and their fragmentation into jets in high-energy collisions. In this formalism, a hadronic cross section is factorized into perturbatively calculable parton-level cross sections, describing the scattering of quarks and gluons, and non-perturbative hadronic matrix elements, describing the partonic structure of the hadron and its fragmentation into final-state particles. 
\iffalse
This factorization can be written as
\begin{equation}
\frac{d\sigma}{dx} = \sum_{a,b,c} \int dx_1 dx_2 f_{a/p}(x_1,\mu_F) f_{b/p}(x_2,\mu_F) \frac{d\hat{\sigma}_{ab}}{dx} \mathcal{D}_{h/c}(z,\mu_F) ,
\end{equation}
where $x$ is a kinematic variable, $f_{a/p}(x,\mu_F)$ is the parton distribution function (PDF) describing the probability of finding a parton of type $a$ carrying a fraction $x$ of the hadron's momentum, $\hat{\sigma}_{ab}$ is the partonic cross section, and $\mathcal{D}_{h/c}(z,\mu_F)$ is the fragmentation function (FF) describing the probability of a parton of type $a$ fragmenting into a hadron of type $h$ carrying a fraction $z$ of the parton's momentum. The factorization scale $\mu_F$ separates the perturbative and non-perturbative contributions to the cross section.
\fi


==> ch3.2-TMD.tex <==
\section{TMD factorization}\label{sec:th-fac}
In this section, we embark on a comprehensive exploration of transverse momentum distributions (TMDs) and their underlying factorization in the context of this thesis. TMDs provide crucial insights into the spatial distribution and motion of quarks and gluons within hadrons, constituting a fundamental component of our understanding of QCD dynamics. By investigating the intricate interplay between the intrinsic transverse momenta of partons and the hard scattering processes, we aim to unravel the rich phenomenology associated with TMDs. 

\subsection{Transverse-momentum dependent distributions}\label{sec:th-pdf}
Before introducing the TMD factorization formalism, we first provide a short review for the definitions of the Transverse-momentum dependent parton distribution functions (TMDPDFs) for later convenience. TMDPDFs are defined through the so-called quark-quark correlation function~\cite{Mulders:1995dh}, $\Phi(x,\bm{k}_T;S)$, 
\begin{align}
\Phi(x, \bm{k}_T; S) = \int \frac{d\xi^- d^2 \bm \xi_T}{(2\pi)^3} e^{i k\cdot \xi}
\left.\langle PS| \bar\psi(0) \psi(\xi)|PS\rangle\right|_{\xi^+ = 0}\,,
\end{align}
where $k^ += xp^+$ with $p^+$ is the large light-cone component of the proton, and $\bm{k}_T$ is the quark transverse momentum with respect to the parent proton. Here we have suppressed the relevant gauge link for our process, which is the same as that for SIDIS process and renders the expression on the right-hand side gauge invariant. In different processes, the structure of the gauge link can change which leads to the important and nontrivial process-dependence of the TMDPDFs~\cite{Collins:2002kn,Boer:2003cm,Bomhof:2004aw,Bacchetta:2005rm,Collins:2011zzd,Kang:2020xez,Buffing:2018ggv}. The correlation function
$\Phi(x, \bm{k}_T; S)$ can be parametrized by TMDPDFs at leading twist accuracy~\cite{Mulders:1995dh,Goeke:2005hb,Bacchetta:2006tn} as
\begin{align}
\label{eq:TMDPDFs}
\Phi(x,\bm{k}_T;S)=&\frac{1}{2}\Bigg[\left(f_{1} - \frac{\epsilon_{T}^{ij} k_{T}^i S_{T}^j}{M}f_{1 T}^{\perp}\right) \slashed{n}_a+\left(\lambda_p g_{1L} + \frac{{\bm k}_T\cdot{\bm S}_T}{M}g_{1T}\right)\gamma_{5} \slashed{n}_a\\
& -i\sigma_{i\mu}n_a^\mu \left(h_1{S_{T}^i}\gamma_5 -ih_1^{\perp}\frac{k_{T}^i}{M}+  h_{1L}^\perp\frac{\lambda_p k_{T}^i}{M} \gamma_5+h_{1T}^\perp\frac{{\bm k}_T\cdot{\bm S}_T k_{T}^i - \frac{1}{2}k_T^2S_{T}^i}{M^2}\gamma_5\right)\Bigg]\,, \notag
\end{align}
where $\sigma_{\mu\nu}=\frac{i}{2}\left[\gamma_\mu,\gamma_\nu\right]$. We have eight quark TMDPDFs $f_1(x, k_T^2)$, $f_{1T}^{\perp}(x, k_T^2)$, $g_{1L}(x, k_T^2)$, $g_{1T}(x, k_T^2)$, $h_1(x, k_T^2)$, $h_1^\perp(x, k_T^2)$, $h_{1L}^\perp(x, k_T^2)$, and $h_{1T}^\perp(x, k_T^2)$, and their physical interpretations are summarized in \cref{intpdf}. For details, see~\cite{Mulders:1995dh,Goeke:2005hb,Bacchetta:2006tn,Bacchetta:2004jz,Boer:2011fh,Accardi:2012qut}.

As usual, we find it convenient to work in the Fourier or $\bm{b}$-space. Taking the Fourier transformation of the correlation function, we have 
\begin{align}
\tilde{\Phi}\left(x, \bm{b}; S\right)=\int d^2\bm{k}_T\,e^{-i\bm{k}_T\cdot \bm{b}}\, \Phi(x,\boldsymbol{k}_T;S)\,,
\end{align}
and the $\bm{b}$-space correlation function $\tilde{\Phi}(x, \bm{b}; S)$ at leading twist is given by~\cite{Boer:2011xd}
\begin{align}
\label{eq:TMDPDFsb}
\tilde{\Phi}(x,\bm{b};S)=&\frac{1}{2}\Bigg[\left(\tilde{f}_{1} + {i\epsilon_{T}^{ij} b^i S_{T}^j}{M}\tilde{f}_{1 T}^{\perp(1)}\right) \slashed{n}_a+\left(\lambda_p \tilde{g}_{1L} - {i{\bm b}\cdot{\bm S}_T}{M}\tilde{g}^{(1)}_{1T}\right)\gamma_{5} \slashed{n}_a\nonumber\\
& \hspace{0.7cm} -i\sigma_{i\mu}n_a^\mu \bigg({S_{T}^i}\tilde{h}_1\gamma_5 -{b^{i}}{M}\tilde{h}_1^{\perp(1)}- i{\lambda_p b^{i}}{M}\tilde{h}_{1L}^{\perp(1)} \gamma_5\nnu
& \hspace{2.7cm}-\frac{1}{2}\left({\bm b}\cdot{\bm S}_T b^{i}-\frac{1}{2} b^2S_{T}^i\right) M^{2} \tilde{h}_{1 T}^{\perp(2)}\gamma_5\bigg)\Bigg]\,,
\end{align}
where $b = |\bm{b}|$ denotes the magnitude of the vector $\bm{b}$. Here, the TMDPDFs in $\bm{b}$-space are defined as
\begin{align}\label{btilde}
\tilde{f}^{(n)}(x,b^2)=\frac{2 \pi n !}{\left({M^{2}}\right)^{n}} \int dk_T \, k_T\left(\frac{k_T}{b}\right)^{n} J_{n}\left(k_T b\right) f\!\left(x, k_T^2\right)\,,
\end{align}
where $n=0$ by default when denoted without a superscript. For simplicity, we have suppressed the additional scale-dependence in both $f\left(x, k_T^2\right)$ and $\tilde{f}^{(n)}(x,b^2)$, and we will specify these scale-dependence explicitly below when we present the factorization formula. 
\begin{table} 
    \centering
\begin{tabular}{ |c|c|c|c| } 
 \hline
 \diagbox[width=3em]{$H$}{$q$} & $U$ & $L$ & $T$ \\ 
  \hline
 $U$ & $f_1$ &  & $h_1^\perp$  \\ 
  \hline
$L$ &  &  $g_{1L}$& $h_{1L}^\perp$ \\ 
  \hline
$T$ & $f_{1T}^\perp$ & $g_{1T}$ & $h_1,\ h_{1T}^\perp$\\ 
  \hline
\end{tabular}
  \caption{TMDPDFs for quarks. We have quark polarizations in the row with $U=\,$unpolarized, $L=\,$longitudinal polarized, and $T=\,$transversely polarized quarks. On the other hand, the column represents polarization of the hadron $H$ (i.e. the proton in our case).}
  \label{intpdf}
\end{table}


\subsection{Transverse-momentum dependent fragmentation functions}\label{sec:th-ff}
We start with writing the parametrization of the transverse-momentum dependent fragmentation functions (TMDFFs) correlator~\cite{Metz:2016swz} in the momentum space. 
\bea
{\Delta}\left(z_h, \boldsymbol{k}_\perp,S_h\right) =& \sum_X \int \frac{d \xi^{+}d^2{\bm \xi}_T}{(2 \pi)^3} e^{i (k^{-} \xi^{+}+{\bm k}_{\perp}\cdot{\bm \xi}_T)/z_h}\left\langle 0\left| \psi_{q}\left(\xi^{+}, 0^{-}, {\bm \xi}_{T}\right)\right| p_h, S_{h} ; X\right\rangle \nnu
& \times\left\langle p_h, S_{h} ; X\left|\bar{\psi}_{q}\left(0^{+}, 0^{-}, {\bm 0}_{T}\right) \right| 0\right\rangle \,,
\eea
where $\boldsymbol{k}_\perp$ is the transverse momentum of the final hadron $h$ with respect to the fragmenting quark $q$ and we suppress the Wilson lines that make the correlator gauge invariant. To the leading twist accuracy, the parametrization is given as
\bea
\label{eq:TMDFF}
\Delta(z_h,\bm{k}_\perp,S_{h})=&\frac{1}{2}\Bigg\{\left({{D}}_{1}- \frac{\epsilon_{T}^{ij} k_{\perp}^i S_{h\perp}^j}{z_hM_h} {{D}}_{1 T}^{\perp}\right)\slashed{n}_b+\left(\lambda_h{{G}}_{1L}- \frac{\boldsymbol{k}_\perp\cdot\boldsymbol{S}_{h\perp}}{z_hM_h} {{G}}_{1 T}\right)\slashed{n}_b\gamma_5
\nnu
&
-i\sigma_{i\mu}n_b^\mu\left(H_1S_{h\perp}^i-iH_1^\perp\frac{k_\perp^i}{z_hM_h}-H_{1L}^\perp\frac{\lambda_h k_\perp^i}{z_hM_h}\gamma_5 \right.
\nnu
&\left.\hspace{15mm}+H_{1T}^\perp\frac{\boldsymbol{k}_\perp\cdot \boldsymbol{S}_{h\perp}k_\perp^i  - \frac{1}{2} {k}_\perp^{2}S_{h\perp}^i}{z_h^2M_h^2}\gamma_5\right)\Bigg\}\,,
\eea
where $n_b$ is the light-cone vector defined by the outgoing quark direction.

Just as in \cref{unp_JFF_FF}, we find it more convenient to derive the relations between the TMDJFFs and TMDFFs using the Fourier space expressions of the TMDFFs. The Fourier transformation for the TMDFF correlator is defined as
\bea
\tilde{\Delta}(z_h,\bm{b},S_h)=\frac{1}{z_h^2}\int d^2\bm{k}_\perp e^{-i\bm{k}_\perp\cdot \bm{b}/z_h}\Delta(z_h,\bm{k}_\perp,S_h)\,.
\eea
The TMDFF correlator in $\bm{b}$-space is then given as
\bea
\label{eq:TMDFFb}
\tilde{\Delta}(z_h,\bm{b},S_h)=&\frac{1}{2}\Bigg\{\left({\tilde{D}}_{1}(z_h,b^2)+ i{\epsilon_{T}^{ij} b^i S_{h\perp}^j}{z_hM_h} {\tilde{D}}_{1 T}^{\perp(1)}(z_h,b^2)\right)\slashed{n}_b\nnu
&\hspace{0.5cm}+\left(\lambda_h{\tilde{G}}_{1L}(z_h,b^2) + i{\boldsymbol{b}\cdot\boldsymbol{S}_{h\perp}}{z_hM_h} {\tilde{G}}_{1 T}^{(1)}(z_h,b^2)\right)\slashed{n}_b\gamma_5\nnu
&\hspace{0.5cm} -i\sigma_{i\mu}n_b^\mu\bigg[\tilde{H}_1(z_h,b^2)S_{h\perp}^i-\tilde{H}_1^{\perp(1)}(z_h,b^2){b^i}{z_hM_h}+i\tilde{H}_{1L}^{\perp(1)}(z_h,b^2){\lambda_h b^i}{z_hM_h}\gamma_5 \nnu
&\hspace{2.3cm}-\tilde{H}_{1T}^{\perp(2)}(z_h,b^2)\frac{1}{2}\left({\boldsymbol{b}\cdot \boldsymbol{S}_{h\perp}b^i - \frac{1}{2}{b}^{2}S_{h\perp}^i}\right){z_h^2M_h^2}\gamma_5\bigg]\Bigg\}\,,
\eea
where we defined
\bea\label{btilde2}
\tilde{{F}}^{(n)}(z_h,b^2)=&\frac{1}{z_h^2}\frac{2 \pi n ! }{\left(z_h^2M_h^{2}\right)^{n}} \int d{k}_\perp {k}_\perp\left(\frac{{k}_\perp}{b}\right)^{n} J_{n}\left(\frac{{b}{k}_\perp}{z_h}\right) {F}^{h/q}\left(z_h, {k}_\perp^2\right)\,.
\eea
Note that $F$ stands generally for all TMDFFs with appropriate $n$ value and by default $n=0$. We then begin with unsubtracted TMDFFs, which follow the same parametrization, and make the scale explicit by replacing
\bea
\tilde{{F}}^{(n)}(z_h,b^2) \to \tilde{{F}}^{(n),{\rm unsub}}(z_h,b^2,\mu,\zeta'/\nu^2)\,.
\eea

\subsection{Results of the structure functions}
By substituting the parameterizations of the various PDF and FF correlators into equation \eqref{eq:3.9}, one can compute the lepton-hadron production cross section for SIDIS and extract the forms of all the structure functions $F_{AB,(C)}$. 

With the assumption of single photon exchange, the differential cross section can be described by a set of structure functions that are model-independent~\cite{Gourdin:1973qx,Kotzinian:1994dv,Diehl:2005pc} and one obtains~\cite{Diehl:2005pc,Bacchetta:2006tn},
\begingroup
\allowdisplaybreaks
\begin{align}
 \frac{d \sigma}{d x d y d \psi d z d \phi_h d P_{h \perp}^2}= & \frac{\alpha^2}{x y Q^2} \frac{y^2}{2(1-\varepsilon)}\left(1+\frac{\gamma^2}{2x}\right)\bigg\{F_{U U, T}+\varepsilon F_{U U, L}+\varepsilon \cos \left(2 \phi_h\right) F_{U U}^{\cos 2 \phi_h}\nnu
 &+\lambda_N\varepsilon \sin \left(2 \phi_h\right) F_{U L}^{\sin 2 \phi_h}+\lambda_N \lambda_e\sqrt{1-\varepsilon^2} F_{L L}\nnu
&  +\left|\boldsymbol{S}_{\perp}\right|\left[\sin \left(\phi_h-\phi_S\right)\left(F_{U T, T}^{\sin \left(\phi_h-\phi_S\right)}+\varepsilon F_{U T, L}^{\sin \left(\phi_h-\phi_S\right)}\right)\right. \nnu
&+\varepsilon \sin \left(\phi_h+\phi_S\right) F_{U T}^{\sin \left(\phi_h+\phi_S\right)}+\varepsilon \sin \left(3 \phi_h-\phi_S\right) F_{U T}^{\sin \left(3 \phi_h-\phi_S\right)}\bigg]\nnu
&+\left|\boldsymbol{S}_{\perp}\right|\lambda_e \sqrt{1-\varepsilon^2}\cos\left(\phi_h-\phi_S\right)F_{L T}^{\cos \left(\phi_h-\phi_S\right)}\bigg\}\,,\label{eq:2.7}
\end{align}
\endgroup
where the ratio $\varepsilon$ is defined by
\begin{align}
\varepsilon=\frac{1-y-\frac{1}{4} \gamma^2 y^2}{1-y+\frac{1}{2} y^2+\frac{1}{4} \gamma^2 y^2}\approx \frac{1-y}{1-y+\frac{1}{2} y^2}\,.
\end{align}
Thus one has the overall depolarization factor given by
\begin{align}
\frac{y^2}{2(1-\varepsilon)} &\approx\left(1-y+\frac{1}{2} y^2\right)\,,
\end{align}
and the rest factors are written as
\begin{eqnarray}
&\frac{y^2}{2(1-\varepsilon)} \,\varepsilon \approx(1-y)\,, &\quad \frac{y^2}{2(1-\varepsilon)} \sqrt{1-\varepsilon^2}  \approx y\left(1-\frac{1}{2} y\right)\,,\\
&\frac{y^2}{2(1-\varepsilon)} \sqrt{2 \varepsilon(1+\varepsilon)} \approx(2-y) \sqrt{1-y}\,, &\quad\frac{y^2}{2(1-\varepsilon)} \sqrt{2 \varepsilon(1-\varepsilon)}  \approx y \sqrt{1-y}\,.
\end{eqnarray}
In the context of our study, the structure functions on the right-hand side of the equation depend on several parameters, including $x$, $Q^2$, $z$, and $P_{h \perp}^2$. The angle $\psi$ represents the azimuthal angle of $\ell^{\prime}$ (the scattered lepton) around the lepton beam axis, with respect to an arbitrary fixed direction. In the case of a transversely polarized target, we specifically choose this fixed direction to align with the direction of $S$ (the target polarization vector). The relationship between $\psi$ and $\phi_S$ is detailed in~\cite{Diehl:2005pc}, where, in the context of deep inelastic kinematics, $d \psi$ is approximately equal to $d \phi_S$.

The subscripts of the structure functions signify the respective polarizations of the beam and target, while an additional subscript in $F_{U U, T}$, $F_{U U, L}$, $F_{U T, T}^{\sin \left(\phi_h-\phi_S\right)}$, and $F_{U T, L}^{\sin \left(\phi_h-\phi_S\right)}$ specifies the polarization of the virtual photon. Here, the terms "longitudinal" and "transverse" target polarization refer to the photon direction. However, converting to experimentally relevant longitudinal or transverse polarizations with respect to the lepton beam direction is a straightforward process, and details can be found in~\cite{Diehl:2005pc}.

To simplify the notation of these structure functions, we introduce the unit vector $\hat{\bm{h}}=\bm{P}_{h \perp}/|\bm{P}_{h \perp}|$. As an example, we first write down the factorization formalism for $F_{UU,T}$,
\begin{align}
F_{UU,T}=&x \sum_i \sigma_0 H\left(Q^2, \mu\right) \int_0^\infty \frac{db}{2\pi}\, b\, b^{m+n} J_{m+n}(q_Tb) \nnu
&\times\tilde{f}^{\rm unsub.}_{1,i/p}\left(x, b,\mu,\zeta_1/\nu^2\right) \tilde{D}^{\rm unsub.}_{1,h/i}\left(z_h, b,\mu,\zeta_2/\nu^2\right)\tilde{S}_{n_a\,n_b}(b,\mu,\nu)\,,\label{eq:fuutnew}
\end{align}
where $\displaystyle\sigma_0=\frac{\alpha_{\mathrm{em}} \alpha_s}{s Q^2} \frac{2\left(\hat{u}^2+\hat{s}^2\right)}{\hat{t}^2}$ is the Born cross section for the unpolarized electron and quark scattering process. $H\left(Q^2, \mu\right)$ is the hard function that encodes physics at the hard scale $Q$ and given by~\cite{Kang:2021ffh}
\begin{align}
H\left(Q^2, \mu\right) & =1+\frac{\alpha_s(\mu)}{2 \pi}C_F\left(- \ln^2 \frac{Q^2}{\mu^2}-3\ln \frac{Q^2}{\mu^2}-8+\frac{\pi^2}{6}\right)+\mathcal{O}\left(\alpha_s^2\right)\,,
\end{align}
In \cref{eq:fuutnew}, $\tilde{f}^{\rm unsub.}_{1,i/p}$ is the renormalized beam function defined in the SCET literature~\cite{Stewart:2009yx} (also know as unsubtracted TMD PDF), describing collinear radiation close to the proton, $\tilde{D}^{\rm unsub.}_{1,h/i}$ is the unsubtracted TMD FF. And $\tilde{S}_{n_a\,n_b}$ is the soft function that encodes soft exchange between the colliding partons. 
Up to NLO, the soft function is given as
\begin{align}
    \tilde{S}_{n_a\,n_b}(b,\mu,\nu)=1+\frac{\alpha_s(\mu)C_F}{2\pi}\left[-L_b^2+4L_b \ln\frac{\mu}{\nu}-\frac{\pi^2}{6}\right]+\mathcal{O}(\alpha_s^2)\,,
\end{align}
with $\displaystyle L_b=\ln\frac{b^2\mu^2}{b_0^2}$, $b_0=2e^{-\gamma_E}$.

Note the dependence of rapidity divergence scale $\nu$ cancels between the unsubtracted function and soft function~\cite{Chiu:2012ir}, leaving only the Collins-Soper scale $\zeta_1$, $\zeta_2$,
\begin{align}
\tilde{f}_{i/p}\left(x, b,\mu,\zeta_1\right)=\tilde{f}^{\rm unsub.}_{i/p}\left(x, b,\mu,\zeta_1/\nu^2\right)\sqrt{\tilde{S}_{n_a\,n_b}(b,\mu,\nu)}\,,\\
\tilde{D}_{h/i}\left(z_h, b,\mu,\zeta_2\right)=\tilde{D}^{\rm unsub.}_{h/i}\left(z_h, b,\mu,\zeta_2/\nu^2\right)\sqrt{\tilde{S}_{n_a\,n_b}(b,\mu,\nu)}\,,
\end{align}
which can be also viewed as the decomposition of TMD PDF $\tilde{f}_{i/p}\left(x, b, \mu, \zeta_1\right)$ and TMD FF $\tilde{D}_{h/i}\left(z, b, \mu, \zeta_2\right)$ into collinear and soft matrix elements~\cite{Becher:2010tm,Becher:2011xn,Becher:2012yn,Echevarria:2011epo,Echevarria:2012js,Echevarria:2014rua,Chiu:2012ir,Li:2016axz}. Now we can simplify the factorization in \cref{eq:fuutnew} and define the notation~\cite{Bacchetta:2006tn,Boer:2011xd,Boussarie:2023izj}
\begin{align}
\mathcal{B}[\tilde{f}^{(m)} \tilde{D}^{(n)}]=&x \sum_i H_{ii}(Q^2,\mu) \int_0^\infty \frac{db}{2\pi}\, b\, b^{m+n} J_{m+n}(q_Tb)  \tilde{f}^{(m)}_{i/p}\left(x, b,\mu,\zeta_1\right) \tilde{D}^{(n)}_{h/i}\left(z_h, b,\mu,\zeta_2\right)\,,
\end{align}
where the Fourier-transformed TMD PDFs $\tilde{f}^{(m)}_{i/p}$ and TMD FFs $\tilde{D}^{(n)}_{h/i}$ are defined by~\cite{Boer:2011xd}
\begin{align}
    \tilde{f}^{(m)}_{i/p}\left(x, b, \mu, \zeta_1\right)&\equiv m!\left(-\frac{1}{M^2b}\partial_b\right)^m\tilde{f}_{i/p}\left(x, b, \mu, \zeta_1\right)\nnu
    &=\frac{2 \pi m !} {(M^2)^{ m}}\int_0^{\infty} \mathrm{d}k_T k_T\left(\frac{k_T}{b}\right)^m J_m\left( k_Tb\right) f_{i/p}\left(x, k_T, \mu, \zeta_1\right)\,,\\
\tilde{D}^{(n)}_{h/i}\left(z_h, b, \mu, \zeta_2\right)&\equiv n!\left(-\frac{1}{M_h^2b}\partial_b\right)^n\tilde{D}_{h/i}\left(z_h, b, \mu, \zeta_2\right)\nnu
& =\frac{2 \pi n !}{\left(M_h^2\right)^n} \int_0^{\infty} \mathrm{d} p_T p_T\left(\frac{p_T}{b}\right)^n J_n\left(b p_T\right) D_{h/i}\left(z_h, z_h p_T, \mu, \zeta_2\right)\,.
\end{align}
Finally, one arrives at the structure functions shown in \cref{eq:2.7} written in terms of TMDs~\cite{Boer:2011xd}:
\begin{align}
F_{U U,T}\left(x, z_h, P_{h T}, Q^2\right) & =\mathcal{B}\left[\tilde{f}_1^{(0)} \tilde{D}_1^{(0)}\right]\,, \\
F_{U U,L}\left(x, z_h, P_{h T}, Q^2\right) & =0\,,\\
F_{U U}^{\cos 2 \phi_h}\left(x, z_h, P_{h T}, Q^2\right) & =M_N M_h \mathcal{B}\left[\tilde{h}_1^{\perp(1)} \tilde{H}_1^{\perp(1)}\right]\,, \\
F_{U L}^{\sin 2 \phi_h}\left(x, z_h, P_{h T}, Q^2\right) & =M_N M_h \mathcal{B}\left[\tilde{h}_{1 L}^{\perp(1)} \tilde{H}_1^{\perp(1)}\right]\,, \\
F_{L L}\left(x, z_h, P_{h T}, Q^2\right) & =\mathcal{B}\left[\tilde{g}_1^{(0)} \tilde{D}_1^{(0)}\right]\,, \\
F_{U T,T}^{\sin \left(\phi_h-\phi_S\right)}\left(x, z_h, P_{h T}, Q^2\right) & =-M_N \mathcal{B}\left[\tilde{f}_{1 T}^{\perp(1)} \tilde{D}_1^{(0)}\right]\,, \\
F_{U T,L}^{\sin \left(\phi_h-\phi_S\right)}\left(x, z_h, P_{h T}, Q^2\right) & =0\,, \\
F_{U T}^{\sin \left(\phi_h+\phi_S\right)}\left(x, z_h, P_{h T}, Q^2\right) & =M_h \mathcal{B}\left[\tilde{h}_1^{(0)} \tilde{H}_1^{\perp(1)}\right]\,, \\
F_{U T}^{\sin \left(3 \phi_h-\phi_S\right)}\left(x, z_h, P_{h T}, Q^2\right) & =\frac{M_N^2 M_h}{4} \mathcal{B}\left[\tilde{h}_{1 T}^{\perp(2)} \tilde{H}_1^{\perp(1)}\right]\,,\\
F_{L T}^{\cos \left(\phi_h-\phi_S\right)}\left(x, z_h, P_{h T}, Q^2\right) & =M_N \mathcal{B}\left[\tilde{g}_{1 T}^{\perp(1)} \tilde{D}_1^{(0)}\right]\,, 
\end{align}


\iffalse
\begin{align}
\mathcal{C}[w f D]=&x \sum_i H_{ii}(Q^2,\mu) \int d^2 \boldsymbol{p}_T d^2 \boldsymbol{k}_T \delta^{(2)}\left(z_h\boldsymbol{k}_T+\boldsymbol{p}_T-\boldsymbol{P}_{h \perp}\right) w\left(\boldsymbol{p}_T, \boldsymbol{k}_T\right) \nnu
&\times f^{i/p}\left(x, p_T,\mu,\zeta_1/\nu\right) D^{h/i}\left(z_h, k_T,\mu,\zeta_2/\nu\right)
\end{align}
where $w(\bm{p}_T,\bm{k}_T)$ is some function of $\bm{p}_T$ and $\bm{k}_T$. The summation is performed over quarks and anti-quarks. The expressions for the structure functions up to twist-two, as given in \cref{eq:2.7}, are formulated as follows~\cite{Bacchetta:2006tn}
\begin{align}
F_{U U, T} & =\mathcal{C}\left[f_1 D_1\right]\,, \\
F_{U U, L} & =0\,, \\
F_{U U}^{\cos 2 \phi_h} & =\mathcal{C}\left[-\frac{2\left(\hat{\boldsymbol{h}} \cdot \boldsymbol{k}_T\right)\left(\hat{\boldsymbol{h}} \cdot \boldsymbol{p}_T\right)-\boldsymbol{k}_T \cdot \boldsymbol{p}_T}{M M_h} h_1^{\perp} H_1^{\perp}\right]\,, \\
F_{U L}^{\sin 2 \phi_h} & =\mathcal{C}\left[-\frac{2\left(\hat{\boldsymbol{h}} \cdot \boldsymbol{k}_T\right)\left(\hat{\boldsymbol{h}} \cdot \boldsymbol{p}_T\right)-\boldsymbol{k}_T \cdot \boldsymbol{p}_T}{M M_h} h_{1 L}^{\perp} H_1^{\perp}\right]\,, \\
F_{L L} & =\mathcal{C}\left[g_{1 L} D_1\right],\\
F_{U T, T}^{\sin \left(\phi_h-\phi_S\right)}&=\mathcal{C}\left[-\frac{\hat{\boldsymbol{h}} \cdot \boldsymbol{p}_T}{M} f_{1 T}^{\perp} D_1\right] \\
F_{U T, L}^{\sin \left(\phi_h-\phi_S\right)}&=0\,, \\
F_{U T}^{\sin \left(\phi_h+\phi_S\right)}&=\mathcal{C}\left[-\frac{\hat{\boldsymbol{h}} \cdot \boldsymbol{k}_T}{M_h} h_1 H_1^{\perp}\right] \\
F_{U T}^{\sin \left(3 \phi_h-\phi_S\right)}&=\mathcal{C}\left[\frac{2\left(\hat{\boldsymbol{h}} \cdot \boldsymbol{p}_T\right)\left(\boldsymbol{p}_T \cdot \boldsymbol{k}_T\right)+\boldsymbol{p}_T^2\left(\hat{\boldsymbol{h}} \cdot \boldsymbol{k}_T\right)-4\left(\hat{\boldsymbol{h}} \cdot \boldsymbol{p}_T\right)^2\left(\hat{\boldsymbol{h}} \cdot \boldsymbol{k}_T\right)}{2 M^2 M_h} h_{1 T}^{\perp} H_1^{\perp}\right]\,, \\
F_{L T}^{\cos \left(\phi_h-\phi_S\right)}&=\mathcal{C}\left[\frac{\hat{\boldsymbol{h}} \cdot \boldsymbol{p}_T}{M} g_{1 T} D_1\right]\,.
\end{align}
\fi

\section{Summary}
So far we have provided a comprehensive review of Semi-Inclusive Deep Inelastic Scattering (SIDIS), a fundamental process in studying the structure of hadrons. We begin by discussing the essential aspects of SIDIS, including its kinematics and structure functions, which are crucial for interpreting experimental measurements. In this chapter, we also introduce the Transverse Momentum Dependent (TMD) factorization framework, which provides a theoretical description of the SIDIS cross-section. Key components of TMD factorization, such as TMD parton distribution functions and TMD fragmentation functions, are presented. The main goal of this chapter is to provide readers with a thorough understanding of SIDIS and TMD factorization, as these concepts are essential for investigating the structure of hadrons and introducing the studies of jets.

The subsequent chapter will introduce a novel concept called Polarized Jet Fragmentation Functions (JFFs), developed by the author of this dissertation. It will discuss the motivation and significance of polarized JFFs, emphasizing their importance in understanding the spin structure of hadrons. Detailed calculations of polarized JFFs for both Collinear and Transverse Momentum Dependent (TMD) cases will be presented. The objective of this chapter is to provide a comprehensive insight into polarized JFFs and their significance in studying the spin structure of hadrons.




==> ch3.3-TMD.tex <==

\section{Electron-jet production}\label{sec:ep-ejet}
In this section, we study the back-to-back electron-jet production in $e+p$ collisions. By measuring fully reconstructed jets instead of hadrons, this process will be sensitive to a single TMDPDF, making it particularly useful to constrain TMDPDFs. This is to be compared with the standard TMD processes, namely SIDIS,  Drell-Yan, and $e^+e^-\to$ dihadrons, where two TMD functions appear in convolution, and thus require extra efforts to decouple them. For example, Drell-Yan process probes two TMDPDFs~\cite{Collins:1984kg,Ji:2004xq}, SIDIS is sensitive to a convolution of a TMDPDF and a TMDFF~\cite{Ji:2004wu,Bacchetta:2006tn}, while $e^+e^-\to$ dihadrons probes two TMDFFs~\cite{Collins:1981uk,Boer:1997mf}. As we will demonstrate below, the electron-jet correlation would allow us to probe all the chiral-even TMDPDFs, without any additional convolution of another TMDPDFs or TMDFFs. In this case, the chiral-odd ones cannot be studied as they require two chiral-odd functions to be convolved with each other.\footnote{We always use standard jet axis to define the jet in this paper. In a recent study~\cite{Liu:2021ewb} when a winner-take-all (WTA) jet axis is used, the chiral-odd component of jets can arise and thus would allow probing the chiral-odd TMDPDFs. How sensitive such a method is to the TMDPDFs remains to be investigated.}

\label{sec2:theoretical}
As shown in \cref{fig:qT}, we label back-to-back production of electron and jet from electron-proton collision process as
\begin{align}
p({p}_A,{S}_{A})+e({p}_B, \lambda_e)\rightarrow \text{jet}({p}_C)+e({p}_D)+X\,,
\end{align}
where an electron with momentum ${p}_B$ (unpolarized or longitudinally polarized with helicity $\lambda_e$, moving along ``$-z$'' direction) scatters with a polarized proton with momentum ${p}_A$ and polarization $S_A$ (moving along ``$+z$'' direction), and such a scattering produces a jet with momentum ${p}_C$ and an electron with momentum ${p}_D$ in the final state.
\begin{figure}
\centering
\includegraphics[width=3.4in]{ep-jet/qT.pdf}  \caption{Back-to-back electron and jet production in electron-proton collision, where $S_A$ indicates the spin of the incoming proton and $\bm q_T$ is the imbalance momentum between the outgoing electron and the final-state jet.}
\label{fig:qT}
\end{figure}
To conveniently parametrize the momentum and the spin vectors involved, we first define a light-cone vector $n_a^\mu=\frac{1}{\sqrt{2}}(1,0,0,1)$ and its conjugate vector ${n}_b^\mu=\frac{1}{\sqrt{2}}(1,0,0,-1)$, such that $n_a^2 = n_b^2 = 0$ and $n_a\cdot{n_b} = 1$. Using the defined light-cone vectors, we can decompose any four-vector $p^\mu$ as $p^\mu = [p^+, p^-,p_T]$. That is, 
\begin{align}
p^\mu =p^+ n_a^{\mu}+ p^- n_b^{\mu} + p_T^\mu\,,
\end{align}
where $p^+ = n_b\cdot p = \frac{1}{\sqrt{2}}\left(p^0 + p^z\right)$ and $p^- = {n_a}\cdot p = \frac{1}{\sqrt{2}}\left(p^0 - p^z\right)$. We study our process using the center-of-mass (CM) frame of the $ep$ collision, where the incoming momenta $p_{A,B}$ and the proton spin vector $S_A$ can be written as  
\begin{align}
{p}_A^\mu=&\sqrt{\frac{s}{2}} n_a^\mu + \mathcal{O}(M)\,,\\ {p}_B^\mu=&\sqrt{\frac{s}{2}} n_b^\mu + \mathcal{O}(m_e)\,,\\
S_A^\mu =&\left[\lambda_p \frac{p_A^+}{M},-\lambda_p \frac{M}{2p_A^+},{\bm S}_T\right]\,.
\label{eq:light-cone}
\end{align}
Here $s=\left(p_A+p_B\right)^2$ is the CM energy,  $\lambda_p$ and $\bm S_T$ are the helicity and transverse spin vector of the incoming proton, and $M$ ($m_e$) are the mass of the proton (electron). We define the usual $Q^2 = -(p_B-p_D)^2$, the virtuality of the exchanged photon, and the event inelasticity $y= Q^2/\left(x_B s\right)$ with $x_B$ the standard Bjorken-$x$~\cite{Bacchetta:2006tn}. We set the final observed jet to be produced in the $xz$-plane as shown in \cref{fig:qT}, with the four-momentum 
\begin{align}
{p}_C^\mu=&E_J(1,\sin\theta_J,0,\cos\theta_J)\,,
\label{eq:jetmom}
\end{align}
where the angle $\theta_J$ is measured with respect to the beam direction. We refer such a $xz$-plane as the scattering plane, which is formed by the jet momentum and incoming electron-proton beam directions. Note that we use $(t,x,y,z)$ momentum representation for $p_C^\mu$, to be distinguished from the light-cone component representation in the form of brackets, e.g. in \cref{eq:light-cone}. 

We consider the kinematic region where the electron and the jet are produced back-to-back with the  transverse momentum imbalance $q_T = |\bm q_T|$ much smaller than the average transverse momentum $p_T = |\bm p_T|$ of the electron and the jet: $q_T \ll p_T$. Here $\bm q_T$ and $\bm p_T$ are given by
\begin{align}
\bm{q}_T &= \bm{p}_{C,T} + \bm{p}_{D,T}\,,
\\
\bm{p}_T &=  \left(\bm{p}_{C,T} - \bm{p}_{D,T}\right)/2\,.
\label{eq:pT}
\end{align}
In the region where $q_T \lesssim p_T$, one must carry out the fixed-order matching (so-called $Y$ term~\cite{Collins:1984kg}). We focus on the resummation region in this paper. 

We parametrize $\bm{q}_T$ and transverse spin vector $\bm{S}_T$ in terms of their azimuthal angles as
\begin{align}
\label{eq:qT}
\bm{q}_T  &= q_T(\cos\phi_{q},\sin\phi_{q})\,,\\
\label{eq:sT}
\bm{S}_T &= S_T(\cos\phi_{S_A},\sin\phi_{S_A})\,,
\end{align}
where $T$ subscript denotes that the vector is transverse with respect to the beam direction. The azimuthal angles are measured in the frame where the incoming beams and outgoing jet defines the $xz$-plane, as shown in \cref{fig:qT}. 
Note that we use a slight abuse of notation, $S_T = |\bm{S}_T|$ and $q_T=|\bm{q}_T|$, to denote the magnitude of the transverse vectors in \cref{eq:qT} and\ \cref{eq:sT}. This notation needs to be used with caution, since representing the four-vector as $q_T^\mu = (0,0,\bm{q}_T)$ (similarly for $S_T^\mu$) would lead to a contradiction $q_T^2 = - \bm{q}_T^2$ if one interprets $q_T^2 = q_T^\mu \,q_{T,\mu}$ . We always use $q_T$ and $S_T$ to denote the magnitude of the transverse momentum and spin, and explicitly write indices, for instance $q_T^\mu \,q_{T,\mu}$, to represent the invariant mass of a four-momentum. We also use unbolded text with Latin indices, for example ${k}_T^i$ or ${S}_T^i$, to denote the components of transverse vectors. 

Working in the one-photon exchange approximation and neglecting the electron mass, the cross section of $e+$jet production from $ep$ collision can then be expressed in terms of structure functions as
\begin{align}
\label{eq:unpjet}
\frac{d\sigma^{p(S_A)+e(\lambda_e)\to e+\text{jet}+X}}{d{p}^2_T dy_J d^2{\bm q}_T}=&F_{UU}+\lambda_p\lambda_e F_{LL}\nnu
&\hspace{-2cm}+S_T\bigg\{\sin(\phi_q-{\phi}_{S_A})F^{\sin(\phi_{q}-{\phi}_{S_A})}_{TU}+\lambda_e\cos(\phi_{q}-{\phi}_{S_A})F^{\cos(\phi_q-{\phi}_{S_A})}_{TL}\bigg\}\,,
\end{align}
where $y_J$ is the rapidity of the jet, and the subscripts $A$ and $B$ in the structure functions $F_{AB}$ indicate the polarization of the incoming proton and electron. Specifically, we use $U,~L,~T$ to represent the unpolarized, longitudinal polarized, and transversely polarized particles, respectively. In the back-to-back limit where $q_T \ll p_T$, these structure functions can then be analyzed within the TMD factorization formalism, and thus allow us to study the relevant TMDPDFs. 

To illustrate how structure functions are factorized, we first describe in detail the expression for $F_{UU}$, which can be factorized into different functions in $\bm{b}$-space as~\cite{Arratia:2020nxw,Buffing:2018ggv,Kang:2020xez} 
\begin{align}
\label{eq:FUUbefore}
F_{UU} =&\hat{\sigma}_0\,H(Q, \mu)\sum_qe_q^2\, J_{q}(p_{T}R,\mu)\int\frac{d^2\bm{b}}{(2\pi)^2}e^{i\bm{q_T}\cdot\bm{b}} x\,\tilde{f}_{1}^{q, \rm{unsub}}(x,b^2, \mu, \zeta/\nu^2)
\nonumber\\
&\times S_{\mathrm{global}}(\bm{b},\mu,\nu)S_{cs}(\bm{b},R,\mu)\,.
\end{align}
where $\hat \sigma_0$ is the Born cross section for the unpolarized electron and quark scattering process, and its expression is given below in \cref{eq:sig0}. In the derivation of the above factorization formula we apply the narrow jet approximation with $R\ll1$. However, as shown in~\cite{Jager:2004jh,Mukherjee:2012uz,Dasgupta:2016bnd,Liu:2018ktv} this approximation works well even for fat jets with radius $R\sim \mathcal{O}(1)$, and the power corrections of $\mathcal{O}(R^{2n})$ with $n>0$ can be obtained from the perturbative matching calculation.
Here $H(Q, \mu)$ is the hard function taking into account virtual corrections at the scale $Q$ and $J_q(p_TR, \mu)$ is the quark jet function. They describe the vertex corrections in the partonic hard scattering and production of the outgoing jet from a hard interaction, respectively. In the back-to-back region of lepton-jet production, we have $Q^2 = -\hat {t} = -x \sqrt{s}\, p_T\, e^{-y_{J}}$ with $\hat{t}$ the partonic Mandelstam variable and we have $Q$ and $p_T$ to be comparable scales, $Q\sim p_T$. 
%\footnote{Note that our factorization requires $q_T^2 \ll p_T^2$, but no assumption is made in regards to the hierarchy between $q_T^2$ and $Q^2$. In the Breit frame factorization, $Q^2$, not $p_T^2$, will be the relevant hard scale in $q_T$ factorization~\cite{Bacchetta:2006tn,Gutierrez-Reyes:2019vbx}.} 
Their renormalized expressions at the next-to-leading order (NLO) are given by~\cite{Liu:2018trl,Arratia:2020nxw,Ellis:2010rwa}
\begin{align}
H(Q, \mu) = &\,1+\frac{\alpha_s}{2\pi}C_F\left[-\ln^2\left(\frac{\mu^2}{Q^2}\right) - 3\ln\left(\frac{\mu^2}{Q^2}\right) -8 +\frac{\pi^2}{6}\right]\,,
\\
J_q(p_TR, \mu) = &\, 1+\frac{\alpha_s}{2\pi}C_F\left[\frac{1}{2}\ln^2\left(\frac{\mu^2}{p_T^2R^2}\right) +\frac{3}{2}\ln\left(\frac{\mu^2}{p_T^2R^2}\right) + \frac{13}{2} -\frac{3\pi^2}{4}\right]\,.
\end{align}
On the other hand, $\tilde{f}_{1}^{q, \rm{unsub}}(x,b^2, \mu, \zeta/\nu^2)$ is the so-called unsubtracted unpolarized TMDPDF~\cite{Collins:2011zzd}\footnote{Compared to \cref{eq:TMDPDFsb}, we now include the flavor label $q$ and also write `unsub' to emphasize the role of the rapidity divergence in TMDPDFs. The basic parametrization forms given in \cref{eq:TMDPDFs} and~\cref{eq:TMDPDFsb} do not change whether we use the rapidity divergence subtracted or unsubtracted quark-quark correlation function.}, with $\mu$ and $\nu$ denoting renormalization and rapidity scales, separately, while $\zeta$ is the so-called Collins-Soper parameter~\cite{Collins:2011zzd,Ebert:2019okf}. In the rapidity regularization scheme~\cite{Chiu:2011qc,Chiu:2012ir} we implement in our calculation\footnote{Our rapidity scale $\nu$ is related to the one used in Eq. (4.9) of~\cite{Chiu:2012ir} by $\nu \to \sqrt{2}\nu$ to be compatible with our definitions of the light-cone vectors given above.}, we have $\zeta$ related to the large light-cone component of the quark inside the proton: $\sqrt{\zeta} = \sqrt{2}\,x\, p_A^+ = x \sqrt{s}$, which will be used in our numerical studies. Finally, the global soft function $S_{\rm{global}}(\bm{b},\mu,\nu)$ describes the soft radiation that has no phase space restriction and does not resolve the jet cone. The collinear-soft function $S_{cs}(\bm{b},R,\mu)$ describes the soft radiation which is only sensitive to the jet direction and resolves the jet cone. The collinear-soft function $S_{cs}(\bm{b},R,\mu)$ depends on the jet radius $R$ and is simply given by the soft radiation outside the jet cone at the NLO. The expressions of $S_{\rm{global}}$ and $S_{cs}$ at one-loop are given by~\cite{Buffing:2018ggv}
\begin{align}
S_{\rm{global}}(\bm{b},\mu, \nu) &= 1+ \frac{\alpha_s}{2\pi} C_F\left[ \left( - \frac{2}{\eta} + \ln \frac{\mu^2}{\nu^2} + 2y_J + 2\ln(-2i\cos(\phi_1)) \right)\left(\frac{1}{\epsilon} + \ln\frac{\mu^2}{\mu_b^2}\right)\right. \nnu
&\hspace{2.6cm} \left.+ \frac{2}{\epsilon^2} + \frac{1}{\epsilon} \ln\frac{\mu^2}{\mu_b^2} - \frac{\pi^2}{6} \right]\,, \label{eq:Sglobalbefore}
\\
S_{cs}(\bm{b},R,\mu) &= 1- \frac{\alpha_s}{2\pi} C_F\left[\frac{1}{\epsilon^2} + \frac{2}{\epsilon}\ln \left(\frac{-2i\cos(\phi_1)\mu}{\mu_b R}\right)+2\ln^2\left(\frac{-2i\cos(\phi_1)\mu}{\mu_b R}\right) + \frac{\pi^2}{4}\right]\,,\label{eq:Scsbefore}
\end{align}
where we have $\mu_b = 2e^{-\gamma_E}/b$, while $\phi_1 \equiv \phi_b - \phi_J$ with $\phi_b$ and $\phi_J$ are the azimuthal angles of the vector $\bm{b}$ and jet transverse momentum $\bm{p}_T$, respectively. Note that we work in $4 - 2\epsilon$ space-time dimensions and use the rapidity regulator~\cite{Chiu:2012ir} $\eta$ and the rapidity scale parameter~$\nu$. 

It is instructive to mention that the Fourier transform given in \cref{eq:FUUbefore} is further complicated by the soft functions' dependence on the azimuthal angle of the jet produced, namely $\phi_1$. These non-trivial azimuthal angle dependence of the soft functions can give rise to additional azimuthal angle correlations for electron-jet production. For example, it was shown in~\cite{Hatta:2020bgy,Hatta:2021jcd} that some novel azimuthal angle correlations can arise from the soft radiation in back-to-back dijet production in unpolarized proton-proton collisions, which involve $\phi_q - \phi_J$. In general, our formalism would naturally lead to such an azimuthal dependence in the unpolarized scattering if one realizes that the azimuthal dependence in $\phi_b - \phi_J$ would translate to the $\phi_q - \phi_J$ dependence after the Fourier transform from $\bm{b}$ back to $\bm{q}_T$ space. We would expect that such $\phi_1$-dependence would lead to additional correlations in the polarized scattering, which involve $\phi_S$ in general, the azimuthal angle of the proton spin.

In the current paper, however, we concentrate on the study of the TMDPDFs and TMDFFs, and we thus ignore such type of correlations purely due to the soft radiation. To proceed and to simplify our phenomenology below, we make a few simplifications. We integrate over the jet azimuthal angle $\phi_J$ as indicated in \cref{eq:unpjet}, i.e., we only measure the magnitude of the jet transverse momentum $p_T$, in which case the azimuthal correlations involving $\phi_J$ would vanish. Additionally, we take $\phi_b$-averaging in both the global and collinear-soft functions, following our previous papers in~\cite{Kang:2020xez,Kang:2020xgk,Chien:2019gyf}. We therefore arrive at the following expression
\begin{align}
\label{eq:FUU_unsub}
F_{UU}=&\hat{\sigma}_0\,H(Q,\mu)\sum_qe_q^2\, J_{q}(p_TR,\mu)\int\frac{b \,db}{2\pi}J_0(q_Tb)\, x\,\tilde{f}^{q, \rm{unsub}}_{1}(x,b^2, \mu, \zeta/\nu^2)
\nonumber\\
&\times \bar{S}_{\rm{global}}(b^2,\mu, \nu)\bar{S}_{cs}(b^2,R,\mu)\,,
\end{align}
where the bar in $\bar{S}$ indicates that the azimuthal angle averaged version of the soft functions are only sensitive to the magnitude of $\bm{b}$. The one-loop expressions of the azimuthal angle averaged soft functions are~\cite{Kang:2020xez,Hornig:2017pud}
\begin{align}
\bar{S}_{\rm{global}}(b^2,\mu, \nu) &=1+ \frac{\alpha_s}{2\pi} C_F\left[ \left( - \frac{2}{\eta} + \ln \frac{\mu^2}{\nu^2} + 2y_J \right)\left(\frac{1}{\epsilon} + \ln\frac{\mu^2}{\mu_b^2}\right) + \frac{2}{\epsilon^2} + \frac{1}{\epsilon} \ln\frac{\mu^2}{\mu_b^2} - \frac{\pi^2}{6} \right]\,,\\
\bar{S}_{cs}(b^2,R,\mu)&= 1- \frac{\as C_F}{2\pi}\left[\frac{1}{\epsilon^2} + \frac{1}{\epsilon}\ln\frac{\mu^2}{\mu_b^2 R^2}+\frac{1}{2}\ln^2\frac{\mu^2}{\mu_b^2 R^2} - \frac{\pi^2}{12}\right]\,.
\label{eq:S_cs}
\end{align}
Note that in the usual SIDIS and Drell-Yan processes, the rapidity divergence and thus the rapidity scale $\nu$ cancel between the 
unsubtracted TMDPDF $\tilde{f}^{q, \rm{unsub}}_{1}(x,b^2, \mu, \zeta/\nu^2)$ and a square-root of the standard soft function $\sqrt{S_{ab}(b^2,\mu,\nu)}$, whose expressions are the same for SIDIS and Drell-Yan process and can be found in~\cite{Collins:2011zzd,Kang:2017glf}:
\begin{align}
{S}_{ab}(b^2,\mu,\nu)&=1 - \frac{\alpha_s C_F}{2\pi} \Bigg[2\left(\frac{2}{\eta}+\ln\frac{\nu^2}{\mu^2}\right)\left(\frac{1}{\epsilon}+\ln\frac{\mu^2}{\mu_b^2}\right)+
\ln^2\frac{\mu^2}{\mu_b^2}
-\frac{2}{\epsilon^2}+\frac{\pi^2}{6}
\Bigg]\,.
\label{eq:S-ab}
\end{align}
This allows us to define the standard TMDPDFs~\cite{Collins:2011zzd} $\tilde{f}^{q}_{1}(x,b^2, \mu, \zeta)$ that are free of rapidity divergence
\begin{align}
\tilde{f}^{q}_{1}(x,b^2, \mu,\zeta) = \tilde{f}^{q, \rm{unsub}}_{1}(x,b^2, \mu, \zeta/\nu^2) \sqrt{S_{ab}(b^2, \mu, \nu)}\,.
\label{eq:standard-f1}
\end{align}
Plugging this equation to \cref{eq:FUU_unsub}, we end up with the following expression
\begin{align}
\label{eq:FUU}
F_{UU}=&\hat{\sigma}_0\,H(Q,\mu)\sum_qe_q^2\, J_{q}(p_TR,\mu)\int\frac{b \,db}{2\pi}J_0(q_Tb)\,x\,\tilde{f}^{q}_{1}(x,b^2, \mu,\zeta)
\nonumber\\
&\times \bar{S}_{\rm{global}}(b^2,\mu)\bar{S}_{cs}(b^2,R,\mu)\,,
\end{align}
where $\bar{S}_{\rm{global}}(b^2,\mu)$ is a rapidity divergence independent soft function defined as
\begin{align}
\bar{S}_{\rm{global}}(b^2,\mu) = \frac{\bar{S}_{\rm{global}}(b^2,\mu, \nu)}{\sqrt{S_{ab}(b^2, \mu, \nu)}}\,,
\end{align}
with the following expression at the NLO
\begin{align}
\bar{S}_{\rm{global}}(b^2,\mu) &=1+ \frac{\alpha_s}{2\pi} C_F\left[  2y_J \left(\frac{1}{\epsilon} + \ln\frac{\mu^2}{\mu_b}\right)+ \frac{1}{\epsilon^2} + \frac{1}{\epsilon} \ln\frac{\mu^2}{\mu_b^2}+ \frac{1}{2} \ln^2\frac{\mu^2}{\mu_b^2}  - \frac{\pi^2}{12} \right]\,.
\label{eq:S_global}
\end{align}
The renormalization group equations for $\bar{S}_{cs}(b^2,R,\mu)$ and $\bar{S}_{\rm{global}}(b^2,\mu)$ are given by
\begin{align}
\mu\frac{d}{d\mu}\ln \bar{S}_{cs}(b^2,R,\mu) =&\, \gamma^S_{cs}\left(b, R,\mu\right)\,,\\
\mu\frac{d}{d\mu}\ln \bar{S}_{\rm{global}}(b^2,\mu) =&\, \gamma^S_{\rm{global}}\left(b, \mu\right)\,,
\end{align}
where the anomalous dimensions $\gamma^S_{\rm cs}$ and $\gamma^S_{\rm{global}}$ can be obtained from \cref{eq:S_cs} and~\cref{eq:S_global}
\begin{align}
\gamma^S_{ cs}\left(b, R, \mu\right) &= -\frac{\alpha_sC_F}{\pi}\ln\frac{\mu^2}{\mu_b^2 R^2}\,,\\
\gamma^S_{\rm{global}}\left(b, \mu\right) &= \frac{\alpha_s C_F}{\pi}\left(2y_J + \ln\frac{\mu^2}{\mu_b^2}\right)\,.
\end{align}

To proceed, we use the usual Collins-Soper-Sterman (CSS) formalism for the unpolarized TMDPDFs $\tilde{f}^{q}_{1}(x,b^2, \mu,\zeta)$ in \cref{eq:FUU}, which are given by
\begin{align}
\tilde{f}^{q}_{1}(x,b^2, \mu,\zeta) = 
\left[C_{q\leftarrow i}\otimes f_{1}^{i}\right]\left(x,\mu_{b_*}\right)
\exp\left[-S_{\rm pert}\left(\mu, \mu_{b_*} \right) - S_{\rm NP}^f\left(x, b, Q_0, \zeta\right)\right]\,.
\end{align}
Here we have performed an operator product expansion in terms of the unpolarized collinear PDFs $f_1^i(x, \mu_{b_*})$ with the convolution defined as follows 
\begin{align}
\left[C_{q\leftarrow i}\otimes f_{1}^{i}\right]\left(x,\mu_{b_*}\right) = \int_x^{1} \frac{d\hat{x}}{\hat{x}} C_{q\leftarrow i}\left(\frac{x}{\hat{x}}, \mu_{b_*} \right) f_1^{i}\left(\hat{x}, \mu_{b_*}\right)\,,
\end{align}
where the sum over repeated indicies are understood and we follow the usual $b_*$ prescription~\cite{Collins:1984kg} with $b_* = b/\sqrt{1+b^2/b_{\rm max}^2}$ and $b_{\rm max} = 1.5$~GeV$^{-1}$. The coefficient functions $C_{q\leftarrow i}$ at the NLO can be found in~\cite{Aybat:2011zv,Kang:2015msa,Collins:2011zzd}, with even N$^3$LO results available at~\cite{Luo:2019szz,Luo:2020epw,Ebert:2020yqt}. On the other hand, the perturbative Sudakov factor $S_{\rm pert}\left(\mu, \mu_{b_*} \right)$ is given by 
\begin{align}
\label{eq:Sud-pert}
S_{\rm pert}\left(\mu, \mu_{b_*} \right)  = -\tilde K(b_*,\mu_{b_*})\ln\left(\frac{\sqrt{\zeta}}{\mu_{b_*}}\right) -\int_{\mu_{b_{*}}}^{\mu} \frac{d\mu'}{\mu'}\left[\gamma_F\left(\alpha_s(\mu'), \frac{\zeta}{\mu'^2}\right) \right]\,.
\end{align}
Note that at the next-to-leading logarithmic (NLL) level, $\tilde K(b_*,\mu_{b_*})=0$ and 
\begin{align}
\gamma_F\left(\alpha_s(\mu), \frac{\zeta}{\mu^2}\right) =& \frac{\alpha_s}{\pi}C_F  \left(\ln\frac{Q^2}{{\mu}^2} - \frac{3}{2}\right)\,
\nonumber\\
& +\frac{\alpha_s^2}{\pi^2} C_F \left[C_A\left(\frac{67}{18}-\frac{\pi^2}{6}\right)-\frac{10}{9} T_R\, n_f\right]\ln\frac{\zeta}{{\mu}^2} \,.
\end{align}
On the other hand, for the non-perturbative Sudakov factor $S_{\rm NP}^f\left(x, b, Q_0, \zeta\right)$, we use the parametrization~\cite{Sun:2014dqm,Echevarria:2020hpy}
\begin{align}
\label{eq:Sud-NP}
S_{\rm NP}^f(x, b, Q_0,\zeta) = \frac{g_2}{2}\ln{\frac{\sqrt{\zeta}}{Q_0}}\ln{\frac{b}{b_*}}+g_1^f b^2\,,
\end{align}
with $Q_0=\sqrt{2.4}$~GeV, $g_2=0.84$ and $g_1^f = 0.106$ GeV$^2$. One last ingredient for the factorization formula in \cref{eq:FUU} has to do with the so-called non-global logarithms~(NGLs)~\cite{Dasgupta:2001sh}. For recent developments on the NGLs, see~\cite{Becher:2015hka,Becher:2016mmh,Becher:2016omr,Becher:2017nof,Caron-Huot:2015bja,Nagy:2016pwq,Nagy:2017ggp,Larkoski:2015zka}. At the NLL accuracy, they can be included as a multiplication factor, see e.g. Refs.~\cite{Dasgupta:2001sh,Arratia:2020nxw,Liu:2020dct,Kang:2020xez,Kang:2020yqw,Gamberg:2021iat}. We find that the NGLs have only very mild effects on our numerical results below, and so we will not include them in the calculations. 

\subsection{Factorization}
Following the theoretical framework shown in \cref{sec2.1-qcd-fac}, to present results for other structure functions in \cref{eq:unpjet} with a more compact notation, we define
\begin{align}
\mathcal{C}_{nk}^{\text{Jet}}[A(x,b^2)]=&\hat{\sigma}_{k}H(Q, \mu)\sum_qe_q^2 J_{q}(p_TR,\mu)M^n\int\frac{b^{n+1}db}{2\pi n!}J_n(q_T b)\,x \,A(x,b^2)\,,
\end{align}
where $\hat \sigma_0$ and $\hat \sigma_L$ correspond to the born-level partonic cross sections of unpolarized scattering $eq\to eq$ and longitudinally polarized scattering $e_Lq_L \to eq$, respectively. They are given by 
the following expressions
\begin{align}
\label{eq:sig0}
\hat{\sigma}_0=&\frac{\alpha_{\rm em}\alpha_s}{sQ^2}\frac{2(\hat{u}^2+\hat{s}^2)}{\hat{t}^2}\,,
\\
\hat{\sigma}_L=&\frac{\alpha_{\rm em}\alpha_s}{sQ^2}\frac{2(\hat{u}^2-\hat{s}^2)}{\hat{t}^2}\,.
\end{align}
Here $\hat s,~\hat t,~\hat u$ are the Mandelstam variables for the partonic $q(xp_A)+e(p_B)\to q(p_C)+e(p_D)$ process and are given by
\begin{align}
\hat s = (xp_A + p_B)^2\,, \qquad
\hat t = (p_B - p_D)^2\,,\qquad
\hat u = (xp_A - p_D)^2\,.
\end{align}
With the compact notation defined, we find the following factorized expressions for the structure functions in \cref{eq:unpjet}
\begin{subequations}\label{eq:strjlep}
\begin{align}
F_{UU}(q_T) &= \mathcal{C}_{00}^{\text{Jet}}[\tilde{f}_1(x,b^2, \mu, \zeta)\bar{S}_{\rm global}(b^2,\mu)\bar{S}_{cs}(b^2,R,\mu)]\,,
\label{eq:strjlep1}
\\
F_{LL}(q_T)&=\mathcal{C}_{0L}^{\text{Jet}}[\tilde{g}_{1L}(x,b^2, \mu, \zeta)\bar{S}_{\rm global}(b^2,\mu)\bar{S}_{cs}(b^2,R,\mu)]\,,
\label{eq:strjlep2}
\\
F_{TU}^{\sin({\phi}_{q}-{\phi}_{S_A})}(q_T)&= \mathcal{C}_{10}^{\text{Jet}}\left[\tilde{f}_{1T}^{\perp(1)}(x,b^2, \mu, \zeta)\bar{S}_{\rm global}(b^2,\mu)\bar{S}_{cs}(b^2,R,\mu)\right]\,,
\label{eq:strjlep3}
\\
F_{TL}^{\cos({\phi}_{q}-{\phi}_{S_A})}(q_T)&=\mathcal{C}_{1L}^{\text{Jet}}\left[\tilde{g}_{1T}^{(1)}(x,b^2, \mu, \zeta)\bar{S}_{\rm global}(b^2,\mu)\bar{S}_{cs}(b^2,R,\mu)\right]\,.
\label{eq:strjlep4}
\end{align}
\end{subequations}
From \cref{eq:strjlep}, we find that the back-to-back electron-jet production provides access to the four chiral-even TMDPDFs: $f_1,~g_{1L},~f_{1T}^{\perp},~g_{1T}$. This is what we have advocated at the beginning of the section, electron-jet production allows us to probe all chiral-even TMDPDFs, but not the chiral-odd ones which usually require the process to be coupled with another chiral-odd function. We summarize the results with their characteristic asymmetries in \cref{scn1tab}.
\begin{table}[h]
\centering
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
 \diagbox[width=1.8cm]{Jet}{PDF} & $f_1$ & $g_{1L}$ & $f_{1T}^\perp$& $g_{1T}$   \\ 
  \hline
   ${J}_q$ & 1 & 1 & $\sin({\phi}_{q}-{\phi}_{S_A})$ & $\cos({\phi}_{q}-{\phi}_{S_A})$  \\ 
  \hline
\end{tabular}
  \caption{Summary of the characteristic azimuthal asymmetry with which different TMDPDFs arise for back-to-back electron-jet production. See \cref{eq:unpjet} and \cref{eq:strjlep} for details.} \label{scn1tab} 
\end{table}

\subsection{Phenomenology: the transverse-longitudinal asymmetry}
\label{subsec:g1T}
In this subsection, we study applications of back-to-back electron-jet production in $ep$ collisions. Some phenomenological applications of this framework, e.g. Sivers asymmetry $F_{TU}^{\sin({\phi}_{q}-{\phi}_{S_A})}$, have been considered previously in Refs.~\cite{Liu:2018trl,Arratia:2020nxw}, but the framework has never been completely generalized fully as in \cref{eq:unpjet} and~\cref{eq:strjlep}.

Our general framework presented in the previous subsection can bring novel insights into the study of spin and TMD effects for all chiral-even TMDPDFs, especially at the future EIC. Here, we consider an azimuthal correlation that has never been studied before in the context of back-to-back electron-jet production, specifically the double transverse-longitudinal spin asymmetry, $A_{TL}^{\cos({\phi}_{q}-\phi_{S_A})}$, defined as 
\begin{align}\label{eq:atl}
A_{TL}^{\cos({\phi}_{q}-\phi_{S_A})}=\frac{F_{TL}^{\cos(\phi_{q}-{\phi}_{S_A})}}{F_{UU}}\,,
\end{align}
using the future EIC kinematics. To generate such a transverse-longitudinal spin asymmetry, we consider the situation in which a transversely polarized proton collides with a longitudinally polarized electron. As defined in \cref{eq:strjlep}, the denominator $F_{UU}$ is related to the unpolarized quark TMDPDFs $f_1^q(x, k_T^2)$, while the numerator $F_{TL}^{\cos(\phi_{q}-{\phi}_{S_A})}$ is related to the quark transversal helicity distributions $g_{1T}^q(x, k_T^2)$, which describe the distributions of longitudinally polarized quarks inside the transversely polarized proton as shown in \cref{intpdf}. 

To compute the unpolarized structure function $F_{UU}$, we use the unpolarized TMDPDFs $f_1^q(x, b^2, \mu, \zeta)$ extractions in ~\cite{Echevarria:2020hpy,Sun:2014dqm} based on the parametrization discussed in last section. On the other hand, for computing the polarized structure function $F_{TL}^{\cos(\phi_{q}-{\phi}_{S_A})}$, we would need the parameterization for $g_{1T}^q(x, b^2, \mu, \zeta)$ in the $b$-space. There are experimental measurements from HEREMES~\cite{Airapetian:2020zzo}, COMPASS~\cite{Parsamyan:2013fia} and Jefferson Lab~\cite{Huang:2011bc} on the double transverse-longitudinal spin asymmetry for the SIDIS process, which in principle would allow us to extract $g_{1T}^q$. However, such a global analysis for $g_{1T}^q$ is not yet available. Below, to estimate the spin asymmetry at the future EIC, we take the parametrization in~\cite{Kotzinian:2006dw}, which simply implements a Wandzura-Wilczek (WW) type approximation and has shown to describe the COMPASS data reasonably well~\cite{Bastami:2018xqd}.

A simple Gaussian form is provided in~\cite{Kotzinian:2006dw} for $g_{1T}^q$ as follows
\begin{align}
g_{1T}^q(x, k_T^2) = g_{1T}^{q(1)}(x) \frac{2M^2}{\pi\langle k_T^2\rangle_{g_{1T}}}e^{-k_T^2/\langle k_T^2\rangle_{g_{1T}}}\,,
\end{align}
where $\langle k_T^2\rangle_{g_{1T}} = 0.15$~GeV$^2$ and $g_{1T}^{q(1)}(x)$ is a collinear function such that 
\begin{align}
g_{1T}^{q(1)}(x) = \int d^2\bm{k}_T \,\frac{k_T^2}{2M^2} \,g_{1T}^q\left(x, k_T^2\right)\,.
\end{align}
From \cref{btilde} and \cref{eq:strjlep4}, we obtain the following expression within the Gaussian model for $\tilde{g}^{q(1)}_{1T}(x,b^2)$, the relevant quantity in the TMD factorization formula
\begin{align}
\tilde{g}^{q(1)}_{1T}(x,b^2)&=\frac{2 \pi}{M^{2}} \int dk_T\frac{k_T^2}{b} J_{1}\left(k_T b\right) g_{1T}\left(x, k_T^2\right)=2\pi\, g_{1T}^{q(1)}(x)\,e^{-b^2\frac{\langle k_T^2\rangle_{g_{1T}}}{4}}\,.
\label{eq:g1T-gaussian}
\end{align}
For the numerical value of $g_{1T}^{q(1)}(x)$, one further applies a WW-type approximation to relate it to the collinear helicity distribution $g_{1L}^q(x)$ as~\cite{Metz:2008ib}
\begin{align}
g_{1T}^{q(1)}(x)&\approx x\int_x^1\frac{dz}{z}g_{1L}^q(z)\,,
\end{align}
where we use the helicity PDFs $g^q_{1L}$ determined by the NNPDF collaboration~\cite{Ball:2013lla} at the scale $\mu_{b_*}$ as we will see below.

The simple Gaussian model for $\tilde{g}^{q(1)}_{1T}(x,b^2)$ in \cref{eq:g1T-gaussian} would then allow us to compute the double spin asymmetry $A_{TL}^{\cos({\phi}_{q}-\phi_{S_A})}$. Since we are using unpolarized TMDPDFs $\tilde{f}^{q}_{1}(x,b^2, \mu,\zeta)$ with proper TMD evolution for computing the denominator $F_{UU}$ in \cref{eq:atl}, we will also implement the TMD evolution to 
promote the Gaussian result for $\tilde{g}^{q(1)}_{1T}$ in \cref{eq:g1T-gaussian}. In this case, we include both perturbative and non-perturbative Sudakov factor, and $\tilde{g}^{q(1)}_{1T}(x,b^2, \mu,\zeta)$ can then be written as
\begin{align}
\tilde{g}^{q(1)}_{1T}(x,b^2, \mu,\zeta) = 
2\pi g_{1T}^{q(1)}\left(x,\mu_{b_*}\right)
\exp\left[-S_{\rm pert}\left(\mu, \mu_{b_*} \right) - S_{\rm NP}^{g_{1T}}\left(x, b, Q_0, \zeta\right)\right]\,,
\end{align}
where the perturbative Sudakov factor $S_{\rm pert}$ is spin-independent and is given in \cref{eq:Sud-pert}. The non-perturbative Sudakov factor for $g_{1T}$ takes the similar form as that of the unpolarized counterpart given in \cref{eq:Sud-NP} as
\begin{align}
S_{\rm NP}^{g_{1T}}\left(x, b, Q_0, \zeta\right) = \frac{g_2}{2}\ln{\frac{\sqrt{\zeta}}{Q_0}}\ln{\frac{b}{b_*}}+g_1^{g_{1T}} b^2\,.
\end{align}
Here $g_2$ controls the non-perturbative TMD evolution from the scale $Q_0$ to $\sqrt{\zeta}$, and it is universal for all different types of TMDs and certainly spin-independent~\cite{Collins:2011zzd}. Thus, it is the same as that for $\tilde{f}^{q}_{1}$ given below \cref{eq:Sud-NP}. On the other hand, the $g_1^{g_{1T}}$ parameter depends on the type of TMDs, and can be interpreted as the intrinsic transverse momentum width for the relevant TMDs at the momentum scale $Q_0=\sqrt{2.4}$ GeV ~\cite{Aybat:2011zv,Anselmino:2012aa,Echevarria:2014xaa}. To match the Gaussian model in \cref{eq:g1T-gaussian}, we take
\begin{align}
g_1^{g_{1T}} = \frac{\langle k_T^2\rangle_{g_{1T}}}{4} = 0.0375~{\rm GeV}^2\,.
\end{align}

\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.45\textwidth]{ep-jet/incl_jet01_0518.pdf}
    \caption{Spin asymmetry of back-to-back electron-jet production from the collision of transversely polarized proton and longitudinally polarized electron as a function of $q_T/p_T$, the ratio between the momentum imbalance $q_T$ and the jet transverse momentum $p_T$. Here we apply the center-of-mass energy $\sqrt{s}=89$ GeV of EIC kinematics, jet radius $R=0.6$, event inelasticity $0.1<y<0.9$ and jet transverse momentum $10 < p_T < 15$ GeV.}
    \label{fig:atl}
\end{figure}
In \cref{fig:atl}, we present our numerical result of $A_{TL}^{\cos(\phi_{q}-\phi_{S_A})}$ as a function of $q_T/p_T$. We consider electron-proton collisions at $\sqrt{s}=89$ GeV at the future EIC, and the jets are constructed via anti-$k_T$ algorithm~\cite{Cacciari:2008gp} with jet radius $R=0.6$. We integrate over the event inelasticity $0.1<y<0.9$ and jet transverse momentum $10<p_T<15$ GeV. Note that in the back-to-back region, we have $y=1-\frac{p_T e^{y_J}}{x\sqrt{s}}$ and thus the kinematic cuts on $y$ translate into the cuts on rapidity $y_J$ and transverse momentum $p_T$ for the jet. As shown in \cref{fig:atl}, we get a sizeable positive double spin asymmetry, demonstrating its promise at the future EIC.



==> ch3.3-pQCD.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Jet shape at NLO+NLL}\label{sec:js_th}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we provide the theoretical framework of jet shape in back-to-back $ep$ collision using the next-to-leading order (NLO) calculation and next-to-leading log (NLL) resummation. We first introduce the factorization of the jet shape and central subjet function in the jet anti-$k_T$ algorithm with $\ln(r/R)$ resummed, then write down the NLL resummation formula for the jet shape observable obtained by taking the momentum fraction average of the subjet function.
\subsection{Factorization of jet shape and NLO result}
\begin{figure}[h]
\centering
\includegraphics[width=0.67\textwidth]{aniso/jetshape.pdf}
\caption{Illustration of integrated (left) and differential (right) jet shape, which are defined as the average fraction of jet transverse momentum inside a cone of radius $r$ (integrated jet shape $\Psi(r)$), and inside an annulus in a $y-\phi$ plane of inner radius $r-d r/2$ and outer radius $r+d r/2$ (differential jet shape $\rho(r)$) concentric to the jet axis $\hat{n}$. }\label{fig:jetshape}
\end{figure}
The jet shape~\cite{Ellis:1992qq} is a broadly studied jet substructure observable that describes the transverse energy profile of jets. The averaged integral jet shape $\Psi(r)$ and differential jet shape $\rho(r)$ for a jet with axis $\hat{n}$ as illustrated in \cref{fig:jetshape} are defined as
\begin{align}
\Psi(r)&=\frac{\sum_{i,d_{i\hat{n}}<r}E_T^i}{\sum_{i,d_{i\hat{n}}<R}E_T^i}\,,\\
\rho(r)&=\frac{d\Psi(r)}{dr}\,,
\end{align}
where $d_{i\hat{n}}$ is the Euclidean distance between the particle $i$ and the jet axis $\hat{n}$ given by
\begin{align}
d_{i\hat{n}}=\sqrt{(y_i-y_{\mathrm jet})^2+(\phi_i-\phi_{\mathrm jet})^2}\,.
\end{align}
To factorize jet shape, we first show the factorization of the differential cross section with respect to the jet transverse momentum $p_T$, inelasticity $y_J$ and the energy fraction $z_r$ of jet carried by the subjet with radius $r$
\begin{align}
\frac{d\sigma}{d^2{\boldsymbol p}_Tdy_Jd^2{\boldsymbol q}_Tdz_r}=&\hat{\sigma}_0 \sum_q e_q^2H(Q,\mu)\hat{\mathcal{J}}_q^{\mathrm jet}(z_r,\omega_R,\mu)\nnu
&\times \int\frac{d^2{\boldsymbol b}}{(2\pi)^2}e^{-i{\boldsymbol b}\cdot{\boldsymbol q}_T}f_{1,q/p}(x,{ b},\mu)S_q({\boldsymbol b},y_J,R,\mu)\,,
\end{align}
where $f_{1,q/p}(x,b,\mu)$ are the PDFs of the initial proton in the impact-parameter space, ${H}(Q,\mu)$ is the hard function that describes the hard scattering process, $S_q({\boldsymbol b},y_J,R,\mu)$ is the soft function that is combined by the global soft function $S_{\mathrm global}$ and the collinear-soft function $S_{\mathrm cs}$ as introduced in Sec.~\ref{sec:sjet_th}. And $\hat{\mathcal{J}}_{q}^{\mathrm{anti}-\mathrm{k}_{T}}\left(z_{r}, \omega_{R}, \mu\right)$ is the subjet function (SJF) at angular scales $r$ and $R$ 
%refractorized as \begin{align}
%\hat{\mathcal{J}}_j^{\mathrm jet}(z_r,p_T,r,R,\mu)=&\int\!\mathrm{d}^{2}{\boldsymbol k}_{\perp}\mathrm{d}^{2}{\boldsymbol q}_{\perp}\delta^{(2)}({\boldsymbol k}_{\perp}+{\boldsymbol q}_{\perp})\,C_{j}(z_{r},p_Tr,k_{\perp},\mu,\nu)\,S_{j}(q_{\perp},R,\mu,\nu)\nnu
%=&\int\frac{d^2b}{(2\pi)^2}\tilde{C}_j(z_r,p_Tr,b,\mu,\nu)\tilde{S}_j(b,R,\mu,\nu)\nnu
%=&\int\frac{bdb}{2\pi}\tilde{C}_j(z_r,p_Tr,b,\mu,\nu)\tilde{S}_j(b,R,\mu,\nu)\,. \end{align}
%$\hat{\mathcal{G}}_{q}^{\mathrm{anti}-\mathrm{k}_{T}}\left(z_{r}, \omega_{R}, \mu\right)$
and will be introduced and factorized in the next subsection. Then the factorized expressions for the jet shape with resummation of $\ln R$ and $\ln(r/R)$ is given by
\begin{align}
\Psi(r)=&\int dz_r\,z_r\frac{d\sigma}{d^2{\boldsymbol p}_Tdy_Jd^2{\boldsymbol q}_Tdz_r}\bigg/\frac{d\sigma}{d^2{\boldsymbol p}_Tdy_Jd^2{\boldsymbol q}_T}\nnu
=&\hat{\sigma}_0 \sum_q e_q^2H(Q,\mu)\int_0^1 dz_r\,z_r\hat{\mathcal{J}}_q^{\mathrm jet}(z_r,p_T,r,R,\mu)\nnu
&\times \int\frac{d^2{\boldsymbol b}}{(2\pi)^2}e^{-i{\boldsymbol b}\cdot{\boldsymbol q}_T}f_{1,q/p}(x,{b},\mu)S_q({\boldsymbol b},y_J,R,\mu)\bigg/\frac{d\sigma}{d^2{\boldsymbol p}_Tdy_Jd^2{\boldsymbol q}_T}\,,
\end{align} 
As introduced in \cite{Kang:2017mda}, the jet shape is given by the $z_r$-average of the subjet centered around a predetermined jet axis as shown in \cref{fig:jetshape}.

With the anti-$k_T$ algorithm, one has the NLO fixed order result as~\cite{Kang:2017mda}
\begin{align}
\int_{0}^{1} \mathrm{~d} z_{r} z_{r} \hat{\mathcal{J}}_q^{\mathrm NLO}(z_r,\omega_R,r,R,\mu)=& J_{q}^{\mathrm{anti}-\mathrm{k}_{T}}\left(\omega_R, \mu\right)+ \frac{\alpha_{s} C_{F}}{2 \pi}\left[-\frac{1}{2} L_{r / R}^{2}+\frac{3}{2} L_{r / R}-\frac{9}{2}+\frac{6 r}{R}-\frac{3 r^{2}}{2 R^{2}}\right]\,,
\end{align}
where $L_{r/R}=\ln(R^2/r^2)$, the inclusive jet function $J_{q}^{\mathrm{anti}-\mathrm{k}_{T}}\left(\omega_R, \mu\right)$ is given by
\begin{align}
J_{q}^{\mathrm{anti}-\mathrm{k}_{T}}\left(\omega_R, \mu\right)=1-\frac{\alpha_{s}C_F}{2 \pi}\left(\frac{3}{2} \ln \frac{{\omega_R}^{2} \tan ^{2} \frac{R}{2}}{\mu^{2}}-\frac{1}{2}\ln ^{2} \frac{\omega_R^{2} \tan ^{2} \frac{R}{2}}{\mu^{2}}-\frac{13}{2}+\frac{3 \pi^{2}}{4}\right) \,.
\end{align}
For completeness, we write down the $r$-differentiated subjet function for calculating the differential jet shape,
\begin{align}
\frac{d}{dr}\int_{0}^{1} \mathrm{~d} z_{r} z_{r} \hat{\mathcal{J}}_q^{\mathrm NLO}(z_r,\omega_R,r,R,\mu)=&-\frac{\alpha_{s} C_{F}}{2 \pi}\frac{1}{\sin(r)}\left[3\left(1-\frac{r}{R}\right)^2+4\ln\left(\frac{r}{R}\right)\right]\,.
\end{align}
Thus one can define the jet shape $\Psi(r)$ and differential jet shape $\Psi(r)$ at NLO as
\begin{align}
\Psi^{\mathrm NLO}(r)=&\hat{\sigma}_0 \sum_q e_q^2H(Q,\mu)\int_0^1 dz_r\,z_r\hat{\mathcal{J}}_q^{\mathrm NLO}(z_r,p_T,r,R,\mu)\nnu
&\times \int\frac{d^2{\boldsymbol b}}{(2\pi)^2}e^{-i{\boldsymbol b}\cdot{\boldsymbol q}_T}f_{1,q/p}(x,{b},\mu)S_q({\boldsymbol b},y_J,R,\mu)\bigg/\frac{d\sigma}{d^2{\boldsymbol p}_Tdy_Jd^2{\boldsymbol q}_T}\,,\label{eq:jsnlo} \\
\rho^{\mathrm NLO}(r)=&\hat{\sigma}_0 \sum_q e_q^2H(Q,\mu)\frac{d}{dr}\int_0^1 dz_r\,z_r\hat{\mathcal{J}}_q^{\mathrm NLO}(z_r,p_T,r,R,\mu)\nnu
&\times \int\frac{d^2{\boldsymbol b}}{(2\pi)^2}e^{-i{\boldsymbol b}\cdot{\boldsymbol q}_T}f_{1,q/p}(x,{b},\mu)S_q({\boldsymbol b},y_J,R,\mu)\bigg/\frac{d\sigma}{d^2{\boldsymbol p}_Tdy_Jd^2{\boldsymbol q}_T}\,,
\end{align} 

\iffalse
where $J_\omega^{E_r}(\mu)$ is the jet energy function. At one-loop order, the quark jet energy functions for anti-$k_T$ algorithm are given as~\cite{Chien:2014nsa}
\begin{align}
\frac{2}{\omega} J_\omega^{q\,E_r}(\mu)=&\frac{\alpha_sC_F}{2\pi}\bigg[\frac{1}{2}\ln^2\frac{\omega^2\tan^2\frac{r}{2}}{\mu^2}-\frac{3}{2}\ln\frac{\omega^2\tan^2\frac{r}{2}}{\mu^2}-2\ln X\ln\frac{\omega^2\tan^2\frac{r}{2}}{\mu^2}\nnu
&+2-\frac{3\pi^2}{4}+6X-\frac{3}{2}X^2-\left(\frac{1}{2}X^2-2X^3+\frac{3}{4}X^4+2X^2\ln X\right)\tan^2\frac{R}{2}\bigg]\,,\\
\frac{2}{\omega}J_\omega^{q\,E_R}(\mu)=&\frac{\alpha_sC_F}{2\pi}\bigg[\frac{1}{2}\ln^2\frac{\omega^2\tan^2\frac{R}{2}}{\mu^2}-\frac{3}{2}\ln\frac{\omega^2\tan^2\frac{R}{2}}{\mu^2}+\frac{3}{4}\tan^2\frac{R}{2}+\frac{13}{2}-\frac{3\pi^2}{4}\bigg]\,,
%\frac{2}{\omega}J_\omega^{g\,E_r}(\mu)=&\\
%\frac{2}{\omega}J_\omega^{g\,E_R}(\mu)=&
\end{align}
where $X={\tan\frac{r}{2}}/{\tan\frac{R}{2}}$. The the differential jet shape functions $\psi(r)$ for anti-$k_T$ algorithm at the first order of $\alpha_s$ is
\begin{align}
\psi^q(r)&=\frac{\alpha_sC_F}{2\pi}\frac{1}{\sin r}\bigg(-3+6X-3X^2-4\ln X\bigg)\sec^2\frac{r}{2}\,.
%\psi^g(r)&=
\end{align}
\fi

\subsection{Factorization of subjet function and NLL resummation}\label{sec:nll}
\iffalse
To factorize jet shape, we first show the factorization of the differential cross section with respect to the jet transverse momentum $p_T$, inelasticity $y_J$ and the energy fraction $z_r$ of jet carried by the subjet with radius $r$
\begin{align}
\frac{d\sigma}{d^2{\boldsymbol p}_Tdy_Jd^2{\boldsymbol q}_Tdz_r}=&\sigma_0 H(Q,\mu)\sum_q e_q^2\hat{\mathcal{J}}_q^{\mathrm jet}(z_r,p_T,R,r,\mu)\nnu
&\times \int\frac{d^2{\boldsymbol b}_T}{(2\pi)^2}e^{i{\boldsymbol q}_T\cdot{\boldsymbol b}_T}f_{q/p}^{\mathrm TMD}(x,{\boldsymbol b}_T,\mu)S_q({\boldsymbol b}_T,y_J,R,\mu)\,,
\end{align}
where $z_r$ is the energy fraction of the subjet with radius $r$, $S_q({\boldsymbol b}_T,y_J,R,\mu)$ is a combination of the global soft function $S_{\mathrm global}$ and collinear-soft function $S_{\mathrm cs}$ as introduced in Sec.~\ref{sec:sjet_th}. $\hat{\mathcal{J}}_q^{\mathrm jet}$ describes the exclusive jet production with subjet carrying an energy fraction $z_r$. 
\fi

To obtain the NLL resummation, we further factorized the subjet function $\hat{\mathcal{J}}_q^{\mathrm jet}(z_r,\omega_R,r,R,\mu)$ at $r\ll R$ limit in the following form 
\begin{align}
\hat{\mathcal{J}}_q^{\mathrm jet}(z_r,p_T,r,R,\mu)=&\int\!\mathrm{d}^{2}{\boldsymbol k}_{\perp}\mathrm{d}^{2}{\boldsymbol q}_{\perp}\delta^{(2)}({\boldsymbol k}_{\perp}+{\boldsymbol q}_{\perp})\,C_{q}(z_{r},p_Tr,k_{\perp},\mu,\nu)\,S_{q}(q_{\perp},R,\mu,\nu)\nnu
=&\int\frac{\mathrm{d}^2 {\boldsymbol b}}{2\pi}\tilde{C}_q(z_r,p_Tr,b,\mu,\nu)\tilde{S}_q(b,R,\mu,\nu)\nnu
=&\int\mathrm{d}b\,b\,\tilde{C}_q(z_r,p_Tr,b,\mu,\nu)\tilde{S}_q(b,R,\mu,\nu)\,,
\end{align}
where $S_{q}(k_{\perp},R,\mu,\nu)$ is the soft function and $C_{q}(z_{r},\omega_{r}r,k_{\perp},\mu,\nu)$ is the collinear function, describing the production of a collinear radiation with momentum fraction $z_r$ of the jet carried by the subjet with radius $r$ and the transverse momentum $k_\perp$ of the radiated parton with respect to the jet axis. The delta function in the first line implies the transverse momentum conservation between $C_q$ and $S_q$. After performing Fourier transformation and integrating over the azimuthal angle of ${\boldsymbol b}$, we obtain the final expression.  
The momentum scaling inside $\tilde{C}_q$ and $\tilde{S}_q$ are given by
\begin{align}
p_c\sim p_T(r^2,1,r),\quad p_s\sim p_T(rR,r/R,r)\,.
\end{align}
Therefore, $p_c$ and $p_s$ have the same renormalization scales $\mu_c=\mu_s\sim p_Tr$ but different rapidity renormalization scales $\nu_c\sim p_T,\ \nu_s\sim p_T\, r/R$. It is noted that the rapidity RG between $\nu_s$ and $\nu_c$ can resums large logarithms $\ln(r/R)$. At the leading order, we have
\begin{align}
\tilde{S}_q^{(0)}(b,R,\mu,\nu)&=1\,,\\
\tilde{C}_q^{(0)}(z_r,p_Tr,b,\mu,\nu)&=\delta(1-z_r) \frac{p_T r}{b} J_1(b p_T r)\,,
\end{align}
where $J_1$ is the first rank of Bessel function and more details are provided in App.~\ref{app:nll}. The one-loop soft function $\tilde{S}_q^{(1)}(b,R,\mu,\nu)$ is given by
\begin{align}
&\tilde{S}_q^{(1)}(b,R,\mu,\nu) =g_s^2\left(\frac{\mu^2 e^{\gamma_E}}{4\pi}\right)^\epsilon\int\frac{\mathrm{d}^dk}{(2\pi)^d}(2\pi)\delta^+(k^2)\frac{4C_F}{k^+k^-}e^{i{\boldsymbol k}\cdot{\boldsymbol b}}\,\theta\left(\frac{R^2}{4}-\frac{k^+}{k^-}\right)\left(\frac{\nu}{k^-}\right)^\eta\nnu
%=& g_s^2\left(\frac{\mu^2 e^{\gamma_E}}{4\pi}\right)^\epsilon\frac{2C_F}{(2\pi)^{d-1}}\int dk^+dk^-d^{2-2\epsilon}k_\perp\delta^+(k^2)e^{i{\boldsymbol k}_\perp\cdot{\boldsymbol b}_\perp}\frac{1}{{\boldsymbol k}_\perp^2}\theta\left(\frac{R}{2}k_\perp-{k^+}\right)\left(\frac{\nu}{k^-}\right)^\eta\nnu
%=&g_s^2\left(\frac{\mu^2 e^{\gamma_E}}{4\pi}\right)^\epsilon\frac{2C_F\nu^\eta}{(2\pi)^{d-1}}\int d^{2-2\epsilon}k_\perp e^{i{\boldsymbol k}_\perp\cdot{\boldsymbol b}_\perp} k_\perp^{-2-2\eta}\int_0^{Rk_\perp/2}\frac{dk^+}{(k^+)^{1-\eta}}\nnu
%=&g_s^2\left(\frac{\mu^2 e^{\gamma_E}}{4\pi}\right)^\epsilon\frac{2C_F\nu^\eta}{(2\pi)^{d-1}}\left[\pi^{1-\epsilon}\frac{\Gamma(1-\epsilon-2-2\eta)}{\Gamma(2+2\eta)}\left(\frac{b^2}{4}\right)^{-1+\epsilon+2+2\eta}\right]\left[\frac{1}{\eta}\left(\frac{2}{Rk_\perp }\right)^{-\eta}\right]\nnu
& =\frac{\alpha_sC_F}{4\pi}\left[\frac{4}{\eta}\left(\frac{1}{\epsilon}+\ln\frac{\mu^2b^2}{b_0^2}\right)-\frac{2}{\epsilon^2}+\frac{4}{\epsilon}\ln\frac{\nu R}{2\mu}+\ln^2\frac{\mu^2b^2}{b_0^2}+4\ln\frac{\mu^2b^2}{b_0^2}\ln\frac{\nu R}{2\mu}+\frac{\pi^2}{6}\right]\,.
\end{align}
From the above one-loop results, one obtains,
\begin{align}
\mu_s&\sim\frac{b_0}{b}\sim p_Tr,\\
\nu_s&\sim\frac{\mu}{R}\sim \frac{p_Tr}{R}\,.
\end{align}
Then we have one-loop anomalous dimensions
\begin{align}
\Gamma^s_0&=4C_F\ln\frac{4\mu^2}{R^2\nu^2}\,,\\
\gamma^{s,\nu}_0(\mu)&=-4C_F\ln\frac{\mu^2 b^2}{b_0^2}\,.
\end{align}
After solving the rapidity RG equation, one resums large logarithms between $\nu_s\sim p_Tr/R$ and $\nu_c\sim p_T$,
\begin{align}
\int_{\nu_s}^{\nu_c}\frac{\mathrm{d}\nu}{\nu}\gamma_s^{\nu}(\mu)=\left(\frac{r}{R}\right)^{\frac{\alpha_sC_F}{\pi}L_b}\,.
\end{align}
The resummation formula for the subjet function at NLL is thus given by
\begin{align}
\hat{\mathcal{J}}_q^{\mathrm jet}(z_r,p_T,r,R,\mu)=\delta(1-z_r)\int\frac{\mathrm{d}b \, b}{2\pi}\left(\frac{r}{R}\right)^{\frac{\alpha_sC_F}{\pi}L_b}\,.
\end{align}
Using the anomalous dimension of the jet
\begin{align}
\Gamma_{\mathcal{J}_q}^{(1)}=-4C_F\ln\frac{p_T^2R^2}{\mu^2}+6C_F\,,
\end{align}
one evolves the subjet function from $\mu_c$ to $\mu$,
\begin{align}
\hat{\mathcal{J}}_q^{\mathrm jet}(z_r,p_T,r,R,\mu)=&\hat{\mathcal{J}}_q^{\mathrm jet}(z_r,p_T,r,R,\mu_c)e^{\int_{\mu_c}^\mu\frac{d\mu}{\mu}\Gamma_{\mathcal{J}_q}(\alpha_s)}\,.
\end{align}
Finally, the jet shape at NLL is given by
\begin{align}
\Psi^{\mathrm NLL}(r)&={\int \mathrm{d}z_r z_r \frac{\mathrm{d}\sigma}{\mathrm{d}^2{\boldsymbol p}_T \mathrm{d}y_J \mathrm{d}^2{\boldsymbol q}_T \mathrm{d}z_r}}\bigg/{\frac{\mathrm{d}\sigma}{\mathrm{d}^2{\boldsymbol p}_T \mathrm{d}y_J \mathrm{d}^2{\boldsymbol q}_T}}\nnu
&=\frac{\exp\left[{\int_{\mu_c}^{p_T}\frac{d\mu}{\mu}\Gamma_{\mathcal{J}_q}(\alpha_s)}\right]\int\mathrm{d}b\,p_T r J_1(p_T r b)\left(\frac{r}{R}\right)^{\frac{\alpha_sC_F}{\pi}\ln\frac{\mu_c^2 b^2}{b_0^2}+g_{\mathrm NP}b^2}}{\exp\left[{\int_{p_T R}^{p_T}\frac{d\mu}{\mu}\Gamma_{\mathcal{J}_q}(\alpha_s)}\right]}\,, \\
&=\int\mathrm{d} b p_T r J_1(p_T r b) \exp\left[{\int_{\mu_c}^{p_T R}\frac{d\mu}{\mu}\Gamma_{\mathcal{J}_q}(\alpha_s)}\right]\left(\frac{r}{R}\right)^{\frac{\alpha_sC_F}{\pi}\ln\frac{\mu_c^2 b^2}{b_0^2}+g_{\mathrm NP}b^2}\label{eq:jsnll} 
\end{align}
where we choose $\mu_c=p_T r$, and we also add a non-perturbative factor $(r/R)^{g_{\mathrm NP}b^2}$.
%where $\left(\frac{r}{R}\right)^{\frac{\alpha_sC_F}{\pi}\ln\frac{\mu_c^2 b^2}{b_0^2}}=1$ if we choose $\mu_c=b_0/b$.

\subsection{Ingredients of jet shape function in momentum space}\label{app:nll}
%\textcolor{cyan}{(Already shown in the main text.)}
As introduced in Sec.~\ref{sec:nll}, at $r\ll R$, we further factorized $\hat{\mathcal{J}}_j^{\mathrm jet}(z_r,\omega_R,r,R,\mu)$ in the following form 
\begin{align} 
\hat{\mathcal{J}}_q^{\mathrm jet}(z_r,\omega_R,r,R,\mu)=&\int\!\mathrm{d}^{2}{\boldsymbol k}_{\perp}\,C_{q}(z_{r},\omega_{r}r,k_{\perp},\mu,\nu)\,S_{q}(k_{\perp},R,\mu,\nu)\nnu 
&\times \Big{[}1+\mathcal{O}\Big{(}\frac{r}{R},\alpha_{s}^{2} \ln^{2}\frac{r}{R}\Big{)}\Big{]}\,.
%&\times S_{\mathrm cs}(k_{\perp},R,\mu,\nu)\Big{[}1+\mathcal{O}\Big{(}\frac{r}{R},\alpha_{s}^{2} \ln^{2}\frac{r}{R}\Big{)}\Big{]}\,.
\end{align}
The quark collinear function $C_{q}(z_{r},\omega_{r}r,k_{\perp},\mu,\nu)$ is given by
\begin{align}
C_{q}(z_{r},\omega_{r}r,k_{\perp},\mu,\nu)=& 16\pi^{3}\,\sum_{X}\frac{1}{2N_{c}}\,{\mathrm Tr}\Big{[}\frac{\bar{n%
}\!\!\!/}{2}\langle 0|\delta(\omega_{R}\!-\!\bar{n}\cdot{\mathcal{P}})\delta^{%
2}({\mathcal{P}}_{\perp}\!-\!k_{\perp})\chi_{n}(0)|X\rangle\langle X|\bar{\chi%
}_{n}(0)|0\rangle\Big{]}\nnu
&\times\delta\Big{(}z_{r}-\frac{\omega_{r}}{\omega_{R}}\Big{)}\,,
\end{align}
At the tree level, one obtains the leading-order (LO) soft and collinear functions as shown below
\begin{align}
%H_{ij}(z,\omega_{R}R,\mu)=&\delta_{ij}\\
S_{q}(k_{\perp},R,\mu,\nu)=&\delta^2(k_\perp)\,,\\
C_{q}(z_{r},\omega_{r}r,k_{\perp},\mu,\nu)=&\delta(1-z_r)\theta\left(|k_\perp|<\frac{\omega_rr}{2}\right)\,.
\end{align}
In this work, to resum the logarithmically-enhanced corrections up to NLL order, we first write down the RG equation and anomalous dimensions of the collinear function and the soft function
\begin{align}
%\mu \frac{\mathrm{d}}{\mathrm{d} \mu} H_{i j}\left(z, \omega_{R} R, \mu\right) &=\sum_{k} \int_{z}^{1} \frac{\mathrm{d} z^{\prime}}{z^{\prime}} \gamma_{i k}^{H}\left(\frac{z}{z^{\prime}}, \omega_{R} R, \mu\right) H_{k j}\left(z^{\prime}, \omega_{R} R, \mu\right)\,, \\
\mu \frac{\mathrm{d}}{\mathrm{d} \mu} S_{q}\left(k_{\perp}, R, \mu, \nu\right) &=\gamma_{q}^{S}(\mu, \nu R) S_{q}\left(k_{\perp}, R, \mu, \nu\right)\,, \\
\mu \frac{\mathrm{d}}{\mathrm{d} \mu} C_{q}\left(z_{r}, \omega_{r} r, k_{\perp}, \mu, \nu\right) &=\gamma_{q}^{C}\left(\omega_{R}, \mu, \nu\right) C_{q}\left(z_{r}, \omega_{r} r, k_{\perp}, \mu, \nu\right)\,, \\
\nu \frac{\mathrm{d}}{\mathrm{d} \nu} S_{q}\left(k_{\perp}, R, \mu, \nu\right) &=\gamma_{q}^{\nu}\left(k_{\perp}, \mu\right) S_{q}\left(k_{\perp}, R, \mu, \nu\right)\,,\\
\nu \frac{\mathrm{d}}{\mathrm{d} \nu} C_{q}\left(z_{r}, \omega_{r} r, k_{\perp}, \mu, \nu\right) &=-\gamma_{q}^{\nu}\left(k_{\perp}, \nu\right) C_{q}\left(z_{r}, \omega_{r} r, k_{\perp}, \mu, \nu\right) \,.
\end{align}
For completeness, here we list the natural scales for the hard, soft and collinear functions
\begin{align}
%\mu_H\sim p_TR\,,&\nnu
\mu_S\sim p_Tr\,,\ &\nu_S\sim p_T\frac{r}{R},\\
\mu_C\sim p_Tr\,,\ &\nu_C\sim p_T\,.
\end{align}
And the anomalous dimensions are given by
\begin{align}
%\gamma_{qq}^H(z,\omega_{R}, \mu)&=\frac{\alpha_{s} }{\pi}\left[C_F\left(-\ln\frac{4\mu^2}{\omega_R^2 R^2}-\frac{3}{2}\right)\delta(1-z)+P_{qq}(z)\right]\,,\\
\gamma_{q}^{C}\left(\omega_{R}, \mu, \nu\right) &=\frac{\alpha_{s} C_{F}}{\pi}\left( \ln \frac{\nu^2}{\omega_{R}^2}+\frac{3}{2}\right)\,, \\
%\gamma_{g}^{C}\left(\omega_{R}, \mu, \nu\right) &=\frac{\alpha_{s}}{\pi}\left(2 C_{A} \ln \frac{\nu}{\omega_{R}}+\frac{1}{2} \beta_{0}\right) \\
\gamma_{q}^{S}(\mu, \nu R) &=\frac{\alpha_{s} C_{F}}{\pi} \ln \frac{4 \mu^2}{\nu^2 R^2}\,, \\
%\gamma_{g}^{S}(\mu, \nu R) &=\frac{\alpha_{s} C_{A}}{\pi} \ln \frac{4 \mu^{2}}{\nu^{2} R^{2}} \\
\gamma_{q}^{\nu}\left(k_{\perp}, \mu\right) &=\frac{\alpha_{s} C_{F}}{\pi} \frac{1}{\mu^{2}} \frac{1}{\left(k_{\perp}^{2} / \mu^{2}\right)}_+\,.
%\gamma_{g}^{\nu}\left(k_{\perp}, \mu\right) &=\frac{\alpha_{s} C_{A}}{\pi} \frac{1}{\mu^{2}} \frac{1}{\left(k_{\perp}^{2} / \mu^{2}\right)}_+
\end{align}
One can easily find that the combination of the hard, collinear and soft function anomalous
dimensions is exactly the anomalous dimension $\gamma_{ij}(z,\mu)=\frac{\alpha_s}{\pi}P_{ji}(z)$ of the subjet function
\begin{align}
\mu \frac{\mathrm{d}}{\mathrm{d} \mu}\hat{\mathcal{J}}_{i}^{\mathrm{jet}}\left(z_{r}, \omega_{R},r,R, \mu\right)=\sum_{k} \int_{z}^{1} \frac{\mathrm{d} z^{\prime}}{z^{\prime}} \gamma_{i k}\left(\frac{z}{z^{\prime}}, \mu\right) \hat{\mathcal{J}}_{k}^{\mathrm{jet}}\left(z^{\prime}, z_{r}, \omega_{R}, r,R,\mu\right)\,.
\end{align}
Then the double logarithms are resummed by the evolution on scale $\mu$. 
%$$O=\alpha_s^p C_0{\mathrm exp}[(\sum_{n=1}\alpha_s^nL^{n+1}c_n)+(\sum_{n=1}\alpha_s^nL^{n}d_n)]$$

\subsection{NLO+NLL resummation and numerical results}
With the jet shape $\Psi(r)$ defined in \cref{eq:jsnlo} for $\Psi^{\mathrm NLO}(r)$ and \cref{eq:jsnll} for $\Psi^{\mathrm NLL}(r)$, to combine the advantages of NLL resummation at small $r$ and NLO calculation at higher $r$, we define the jet shape at NLO+NLL as
\begin{align}
\Psi(r)=\Psi^{\mathrm NLL}(r)+\left(\Psi^{\mathrm NLO}(r)-\Psi^{\mathrm NLO}(r)\bigg|_{r\ll R}\right)\,,\label{eq:nlonll}
\end{align}
where the first term is given in \cref{eq:jsnll}, and the second term characterized the behavior of fixed order calculation of integrated jet shape at large $r$. 
\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{aniso/psi_eicR1.pdf}
\quad
\includegraphics[width=0.45\textwidth]{aniso/psi_eicR05.pdf}\\
\includegraphics[width=0.45\textwidth]{aniso/psi_h1R1.pdf}
\quad
\includegraphics[width=0.45\textwidth]{aniso/psi_h1R05.pdf}
\caption{The integrated jet shape $\Psi(r)$ for quark jets with EIC kinematics (first row) and HERA kinematics (second row) for $10<p_T<25$ GeV, $0<q_T<5$ GeV with jet radius $R = 1.0$ (left column) and $R = 0.5$ (right column). The bands indicate
the perturbative uncertainties estimated using $\mu$ and $\mu_c$ up and down by a factor of 2 separately.}\label{fig:int_js}
\end{figure}

In \cref{fig:int_js}, we plot the NLO+NLL integrated jet shape $\Psi(r)$ as defined in \cref{eq:nlonll} for EIC (first row) and HERA (second row) kinematics using red curves with yellow uncertainty bands and provide the comparison with \texttt{PYTHIA8} simulation given by black step lines. The uncertainty bands are perturbative uncertainties given by varying the hard and collinear scales $\mu$ and $\mu_c$ up and down by a factor of 2 separately. For the EIC kinematics, we apply the center-of-mass energy $\sqrt{s}=105$ GeV, inelasticity $y$ in the region of $[0.1,\ 0.9]$, jet transverse momentum $p_T$ in $[10,\ 25]$ GeV, transverse momentum imbalance $q_T$ in $[0,\ 5]$ GeV. And for HERA, we have the energy of incoming proton and electron as $E_p=920$ GeV and $E_e=27.6$ GeV, inelasticity $0.2<y<0.7$ and same regions for $p_T$ and $q_T$. In the left column, we adopt $R=1.0$ as the jet radius while in the right column, we have $R=0.5$, thus the right column has a smaller range for the subjet radius $r$. And one can find a good agreement between the \texttt{PYTHIA8} simulation and NLO+NLL calculations.

Using the definition of differential jet shape $\displaystyle\rho(r)=d\Psi(r)/dr$, we plot $\rho(r)$ at EIC (first row) and HERA (second row) kinematics with jet radius $R=1.0$ (left column) and $R=0.5$ (right column) in \cref{fig:dif_js} as well. The red curves with yellow uncertainty bands are given by NLO+NLL calculation using \cref{eq:nlonll} and the black step lines are from \texttt{PYTHIA8} simulations. One further confirms that the \texttt{PYTHIA8} simulation and NLO+NLL results are consistent at both large and small $r$ regions.
\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{aniso/rho_eicR1.pdf}
\quad
\includegraphics[width=0.45\textwidth]{aniso/rho_eicR05.pdf}\\
\includegraphics[width=0.45\textwidth]{aniso/rho_h1R1.pdf}
\quad
\includegraphics[width=0.45\textwidth]{aniso/rho_h1R05.pdf}
\caption{The differential jet shape $\rho(r)$ for quark jets with EIC kinematics (first row) and HERA kinematics (second row) for $10<p_T<25$ GeV, $0<q_T<5$ GeV with jet radius $R = 1.0$ (left column) and $R = 0.5$ (right column). The bands indicate
the perturbative uncertainties estimated using $\mu$ and $\mu_c$ up and down by a factor of 2 separately.}\label{fig:dif_js}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Jet azimuthal anisotropy}\label{sec:sjet_th}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Introduction}\label{sec:intro}
In heavy-ion collisions, the studies of azimuthal anisotropy have been contributing to characterizing the properties of the quark–gluon plasma (QGP) and provide experimental information on the equation of state of QGP~\cite{STAR:2022gav,Tang:2021nhq,CMS:2019nct,ALICE:2019zfl}. In recent years, the concept of ``azimuthal anisotropy" has also been introduced in~\cite{Dumitru:2015gaa} as the measure of azimuthal correlations and applied in $\gamma p$, $pp$~\cite{Hatta:2020bgy} and $ep$~\cite{Hatta:2021jcd,Tong:2022zwp} collisions\footnote{Although the terminology ``azimuthal anisotropy" has been adopted in the studies of both heavy-ion collisions and $ep$ collisions, it describes different observables. In particular, the azimuthal angle of the heavy-ion collisions is defined with respect to the reaction plane of two colliding nuclei, while for $ep$ collisions, the azimuthal angle is related to the transverse momentum imbalance of the produced lepton and jet.}. The back-to-back lepton-jet production from $ep$ collisions has been showing great insights for transverse momentum dependent (TMD) studies, where jets are collimated sprays of particles that emerge from the fragmentation of quarks and gluons produced in the collision and the jet observables are expected for probing the three-dimensional nucleon structure encoded in transverse-momentum-dependent parton-distribution functions (TMD PDFs)~\cite{Liu:2018trl,Gutierrez-Reyes:2018qez,Gutierrez-Reyes:2019vbx,Kang:2020xyq,Kang:2021ffh}. In this work, we study the back-to-back electron-jet production from $ep$ collision as shown in \cref{fig:epjet},
\begin{align}
e(l)+p(P)\rightarrow e(l')+{J}_q(p_J)+X\,,
\end{align}
where we define the transverse momentum of the produced electron $\boldsymbol{l}'_T$, produced jet $\boldsymbol{p}_{T}$, average transverse momentum $|\boldsymbol{l}'_T - \boldsymbol{p}_T|/2$ and the transverse momentum imbalance $\boldsymbol{q}_T=\boldsymbol{l}'_T+\boldsymbol{p}_{T}$.  
\begin{figure}[h]
\centering
\includegraphics[width=0.6\textwidth]{aniso/epjet.pdf}\\
\caption{Kinematic configuration for back-to-back lepton-jet production from $ep$ collisions.}\label{fig:epjet}
\end{figure}

In this work, we provide the theoretical formula for azimuthal asymmetries including jet radius $R$ resummation effects. In the realm of jet processes, at the leading order (LO), initiation can arise from either a quark or a gluon, whereas in the heavy-meson case, only the gluon initial state is germane. In the small $|\boldsymbol{q}_T|$ limit, i.e. $|\boldsymbol{q}_T| \ll |\boldsymbol{p}_T|$ and $R\ll 1$, the cross-section undergoes a process of factorization, giving rise to the convolution of several fundamental functions such as the hard function, TMD PDFs, jet function, soft functions, and a new evolution kernel, where the soft functions and evolution kernel have azimuthal-angle dependence. In~\cite{delCastillo:2020omr,delCastillo:2021znl}, this new evolution kernel has been elucidated for dijet productions. In this paper, we seek to provide a theoretical study of back-to-back electron-jet production with the RG evolution kernel that contributes to the azimuthal asymmetry. 

In position space, one can delineate the factorization of the cross-section with the variable $\boldsymbol{b}$, which is the conjugate of the momentum $\boldsymbol{q}_T$. To Fourier transform the factorized cross-section from $b$-space to momentum space, an angular integration on $\phi_b$ needs to be performed, namely, $d^2b = bdb\, d\phi_b$ and $\boldsymbol{p}_T\cdot \boldsymbol{b} = p_T b \cos (\phi_b-\phi_J)$, where $\phi_b$ and $\phi_J$ are the azimuthal angles of the vector $\boldsymbol{b}$ and jet transverse momentum $\boldsymbol{p}_T$. This integration is non-trivial since the anomalous dimensions of various functions depend on this angle and are complex-valued. We demonstrate that the integration can be carried out in resummed perturbation theory, thereby addressing the issue of complex values in all anomalous dimensions. Consequently, the cross-section, integrated with respect to the $\phi_b$ angle, is factorized into distributions that are $b$-rotation invariant. The $\phi_b$-angle integrated evolution kernel has been provided in~\cite{Kang:2021ffh}. 

With the azimuthal asymmetry in the collisions, non-vanishing anisotropic flow harmonics are expected. More specifically, the radial flow, an azimuthal-angle-independent term, corresponds to the isotropic Fourier coefficient~\cite{Voloshin:1994mz,Poskanzer:1998yz}. As for the higher order Fourier coefficients encoding the azimuthal anisotropy, the first term $v_1$ is the directed flow component, and likewise $v_2$ is elliptic flow, $v_3$ is triangular flow, $v_4$ is quadrapole flow, etc. For instance, in $e+p\rightarrow e+{\mathrm jet}+X$ process, the differential cross section of back-to-back lepton-jet production can be decomposed as follows
\begin{align}\label{eq:exp}
\frac{\mathrm{d}\sigma}{\mathrm{d}^2{\boldsymbol p}_T \mathrm{d}y_J \mathrm{d}\phi_J \mathrm{d}^2{\boldsymbol q}_T}=\frac{\mathrm{d}\sigma}{2\pi \mathrm{d}^2{\boldsymbol p}_T \mathrm{d}y_J q_T \mathrm{d} q_T}\left[1+2\sum_{n=1}^\infty v_n(p_T, y_J)\cos(n(\phi_q-\phi_J))\right]\,,
\end{align}
where ${\boldsymbol p}_T$ and $y_J$ are the transverse momentum and rapidity of the produced jet, ${\boldsymbol q}_T$ is the transverse momentum imbalance between the produced electron and jet, while $\phi_J$ and $\phi_q$ are the azimuthal angles of jet direction and ${\boldsymbol q}_T$, respectively. In \cref{eq:exp}, $v_n$ describes the azimuthal anisotropy of particle spectrum in the momentum space and can be measured in experiments as the expectation of the $n$-th order harmonics $v_n =\langle \cos(n(\phi_q-\phi_J))\rangle$, the averaged value with respect to the particle spectrum and can be obtained by taking an average of $\phi_J$ weighted by $\cos(n(\phi_q-\phi_J))$ normalized by the $\phi_J$-averaged differential cross section.

Besides jet anisotropy, we also provide a theoretical study of jet shape. The study of jet shapes plays a crucial role in understanding the behavior of high-energy particle collisions in quantum chromodynamics (QCD). The jet shape observable is characterized by its energy distribution as a function of the distance from the jet axis. The jet shape is an essential observable for understanding the underlying QCD processes and for testing theoretical predictions. In recent years, there has been significant progress in the theoretical understanding of jet shapes at next-to-leading order (NLO)~\cite{Catani:1996jh} and next-to-next-to-leading order (NNLO)~\cite{Gehrmann-DeRidder:2007foh,Gehrmann-DeRidder:2014hxk} in perturbative QCD. In addition, the introduction of the concept of non-global logarithms~\cite{Dasgupta:2001sh} has led to a better understanding of the impact of soft and collinear emissions on jet shapes at next-to-leading logarithmic (NLL) accuracy~\cite{Chien:2014nsa}. These theoretical studies have enabled more precise predictions of jet shapes at high energies.

In this study, we will compare the NLO+NLL theoretical study of jet shapes with simulation results obtained from the Pythia event generator. Pythia is a widely used tool for simulating high-energy particle collisions and has been extensively tested against experimental data. By comparing the theoretical predictions with Pythia simulations, we aim to test the validity of the NLO+NLL theoretical study and to provide insight into the underlying QCD processes that produce jets. This study will contribute to our understanding of QCD and provide a valuable tool for future experimental analyses.

This paper is outlined as follows. In Sec.~\ref{sec:sjet_th}, we present the factorization theorem for $ep$ to electron plus single jet process with azimuthal anisotropy by projecting the collective flow to different Fourier coefficients and provide the elliptic flow, triangular flow and higher flow harmonics in this collision. In Sec.~\ref{sec:js_th}, we provide the NLO+NLL resummation formalism for jet shape observable and compare the theoretical calculations with Pythia simulations. In Sec.~\ref{sec:con}, we conclude this paper and discuss future directions.

\subsection{Theoretical background}
In this section, we present the factorization theorem for $ep$ to electron plus single jet process with azimuthal anisotropy by projecting the collective flow to different Fourier coefficients and provide the calculations for directed flow, elliptic flow, triangular flow and higher flow harmonics in this process.
\subsection{Factorization and RG consistency}\label{sec:fac1}

For an unpolarized incoming proton, the TMD factorization is given by \cite{Arratia:2020nxw}
\begin{align}\label{eq:sjet-fac-before}
\frac{\mathrm{d}\sigma^{e+p\rightarrow e+{\mathrm jet}+X}}{\mathrm{d}^2 \boldsymbol{p}_T \mathrm{d}y_J \mathrm{d}^2\boldsymbol{q}_T} =\,& \hat{\sigma}_0\,\sum_{q}e_q^2 H(Q,\mu) \int \frac{d^2\boldsymbol{b}}{(2\pi)^2}  \, \exp(-i \boldsymbol{b} \cdot \boldsymbol{q}_T) \, x \tilde{f}_{1,q/p}^{\mathrm unsub.}(x, {b}, \mu,\zeta/\nu^2) \nnu
   & \times {S}_{\mathrm global}^{\mathrm unsub.}\left(\boldsymbol{b},y_J, \mu,\nu\right) \, S_{\mathrm cs}(\boldsymbol{b},R,\mu)  \mathcal{J}_{q}(p_TR,\mu)\;, 
\end{align}

%#########################################################
where $\tilde{f}_{1,q/p}^{\mathrm unsub.}(x,{b}, \mu, \zeta/\nu^2)$ is the so-called unsubtracted unpolarized TMDPDF~\cite{Collins:2011zzd}%\footnote{Compared to \cref{eq:TMDPDFsb}, we now include the flavor label $q$ and also write `unsub' to emphasize the role of the rapidity divergence in TMDPDFs. The basic parametrization forms given in \cref{eq:TMDPDFs} and~\cref{eq:TMDPDFsb} do not change whether we use the rapidity divergence subtracted or unsubtracted quark-quark correlation function.}
, with $\mu$ and $\nu$ denoting the renormalization and rapidity scales, respectively. And $\zeta$ is the so-called Collins-Soper parameter~\cite{Collins:2011zzd,Ebert:2019okf}. In the rapidity regularization scheme~\cite{Chiu:2011qc,Chiu:2012ir} implemented in our framework, we have $\zeta$ related to the large light-cone component of the quark inside the proton: $\sqrt{\zeta} = x \sqrt{s}$, which will be used in our numerical studies. %$\sqrt{\zeta} = \sqrt{2}\,x\, p_A^+ = x \sqrt{s}$

In \cref{eq:sjet-fac-before}, $H(Q, \mu)$ is the hard function that describes the partonic hard scattering and $\mathcal{J}_q(p_TR, \mu)$ is the quark jet function, characterizing the production of the outgoing jet from a hard interaction. At the next-to-leading order (NLO), their renormalized expressions are given by~\cite{Liu:2018trl,Arratia:2020nxw,Ellis:2010rwa}
\begin{align}
H(Q, \mu) = &\,1+\frac{\alpha_s}{2\pi}C_F\left[-\ln^2\left(\frac{\mu^2}{Q^2}\right) - 3\ln\left(\frac{\mu^2}{Q^2}\right) -8 +\frac{\pi^2}{6}\right]\,,\label{eq:hard}
\\
\mathcal{J}_q(p_TR, \mu) = &\, 1+\frac{\alpha_s}{2\pi}C_F\left[\frac{1}{2}\ln^2\left(\frac{\mu^2}{p_T^2R^2}\right) +\frac{3}{2}\ln\left(\frac{\mu^2}{p_T^2R^2}\right) + \frac{13}{2} -\frac{3\pi^2}{4}\right]\,,
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%
with the RG equations
\begin{align}
\mu \frac{\mathrm{d}}{\mathrm{d} \mu} H\left(Q, \mu\right) &=\gamma^{H}(Q, \mu) H\left(Q, \mu\right)\,,\label{eq:evolveh} \\
\mu \frac{\mathrm{d}}{\mathrm{d} \mu} \mathcal{J}_q(p_TR, \mu) &=\gamma_q^{\mathcal{J}}(p_T R, \mu) \mathcal{J}_q(p_TR, \mu)\,,\label{eq:evolvej}
\end{align}
 and the anomalous dimensions $\gamma^{H}\left(Q, \mu\right)$ and $\gamma_{q}^{\mathcal{J}}(p_T R, \mu)$ of the hard function $H\left(Q, \mu, \right)$ and jet function $\mathcal{J}_q(p_TR, \mu)$, respectively
\begin{align}
\gamma^{H}\left(Q, \mu\right) &=\frac{\alpha_{s} C_{F}}{\pi}\left[ -2\ln \left(\frac{\mu^2}{Q^2}\right)-{3}\right]\,,\label{eq:gammah} \\
\gamma_{q}^{\mathcal{J}}(p_T R, \mu) &=\frac{\alpha_{s} C_{F}}{\pi} \left[\ln \left(\frac{\mu^2}{p_T^2 R^2}\right)+\frac{3}{2}\right]\,.\label{eq:gammaj}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%
The global soft function ${S}_{\mathrm global}^{\mathrm unsub.}(\boldsymbol{b},y_J,\mu,\nu)$ in \cref{eq:sjet-fac-before} (depicted by the orange radiation in \cref{fig:epjet}) represents the soft radiation that has no phase space restriction and does not resolve the jet cone. And the collinear-soft function ${S}_{\mathrm cs}(\boldsymbol{b},R,\mu)$ (described by the red radiation in \cref{fig:epjet}) depends on the jet radius $R$ and denotes the soft radiation which is only sensitive to the jet direction and resolves the jet cone. At the next-to-leading order (NLO), the collinear-soft function $S_{\mathrm cs}(\boldsymbol{b},R,\mu)$ is simply given by the soft radiation outside the jet cone. The expressions of $S_{\mathrm global}$ and $S_{\mathrm cs}$ at one-loop are given by~\cite{Buffing:2018ggv}
\begin{align}
{S}_{\mathrm{global}}^{\mathrm unsub.}(\boldsymbol{b},y_J,\mu, \nu) =& 1+ \frac{\alpha_s}{2\pi} C_F\left\{ \left[ - \frac{2}{\eta} + \ln \frac{\mu^2}{\nu^2} + 2y_J + 2\ln(-2i\cos\phi_{bJ}) \right]\left(\frac{1}{\epsilon} + \ln\frac{\mu^2}{\mu_b^2}\right)\right. \nnu
&\hspace{2.6cm} \left.+ \frac{2}{\epsilon^2} + \frac{1}{\epsilon} \ln\frac{\mu^2}{\mu_b^2} - \frac{\pi^2}{6} \right\}\,, \label{eq:Sglobalbefore}
\\
%{S}_{\mathrm cs}(\boldsymbol{b},R,\mu) &= 1- \frac{\alpha_s}{2\pi} C_F\left[\frac{1}{\epsilon^2} + \frac{2}{\epsilon}\ln \left(\frac{-2i\cos\phi_{bJ}\mu}{\mu_b R}\right)+2\ln^2\left(\frac{-2i\cos\phi_{bJ}\mu}{\mu_b R}\right) + \frac{\pi^2}{4}\right]\,,\\
%{S}_{\mathrm cs}(\boldsymbol{b},R,\mu) =& 1- \frac{\alpha_s}{2\pi} C_F\left[\frac{1}{\epsilon^2} + \frac{2}{\epsilon}\ln \left(\frac{-2i\cos\phi_{bJ}\mu}{\mu_b R}\right)+2\ln^2\left(\frac{-2i\cos\phi_{bJ}\mu}{\mu_b R}\right) + \frac{\pi^2}{4}\right]\nnu
%=&1-\frac{\alpha_s}{2\pi} C_F\bigg[\frac{1}{\epsilon^2} +\frac{2}{\epsilon}\ln(-2i\cos\phi_{bJ})+ \frac{1}{\epsilon}\ln \left(\frac{\mu^2}{\mu_b^2 R^2}\right)+2\ln^2(-2i\cos\phi_{bJ})\nnu
%&+\frac{1}{2}\ln^2\left(\frac{\mu^2}{\mu_b^2 R^2}\right)+2\ln(-2i\cos\phi_{bJ}\ln\left(\frac{\mu^2}{\mu_b^2 R^2}\right)+ \frac{\pi^2}{4}\bigg]\nnu
{S}_{\mathrm cs}(\boldsymbol{b},R,\mu)=&1-\frac{\alpha_s}{2\pi} C_F\bigg[\frac{1}{\epsilon^2}+ \frac{1}{\epsilon}\ln \left(\frac{\mu^2}{\mu_b^2 R^2}\right)+\frac{1}{2}\ln^2\left(\frac{\mu^2}{\mu_b^2 R^2}\right)+ \frac{\pi^2}{4}+2\ln^2(-2i\cos\phi_{bJ})\nnu
&+2\ln(-2i\cos\phi_{bJ})\left(\frac{1}{\epsilon}+\ln\left(\frac{\mu^2}{\mu_b^2 R^2}\right)\right)\bigg]\,,\label{eq:Scsbefore}
\end{align}
where we have defined $\mu_b = 2e^{-\gamma_E}/b$ and $\phi_{bJ} \equiv \phi_b - \phi_J$ with $\phi_b$ and $\phi_J$ are the azimuthal angles of the vector $\boldsymbol{b}$ and jet transverse momentum $\boldsymbol{p}_T$, respectively.
%#########################################################
We chose $\eta$ rapidity regulator~\cite{Chiu:2012ir} to regulate the rapidity divergence, which leads to the  rapidity scale $\nu$-dependence of TMDPDF $\tilde{f}_{1,q/p}^{\mathrm unsub.}(x, {b}, \mu,\zeta/\nu^2)$ and the global soft function $\tilde{S}_{\mathrm global}^{\mathrm unsub.}\left(\boldsymbol{b},y_J, \mu,\nu\right)$. With the standard soft function $\sqrt{S_{ab}(b,\mu,\nu)}$ given by
\begin{align}
{S}_{ab}(b,\mu,\nu)&=1 - \frac{\alpha_s C_F}{2\pi} \Bigg[-2\left(-\frac{2}{\eta}+\ln\frac{\mu^2}{\nu^2}\right)\left(\frac{1}{\epsilon}+\ln\frac{\mu^2}{\mu_b^2}\right)+
\ln^2\frac{\mu^2}{\mu_b^2}
-\frac{2}{\epsilon^2}+\frac{\pi^2}{6}
\Bigg]\,,
\label{eq:S-ab}
\end{align}
we are able to remove the rapidity scale dependence by subtracting a square-root of ${S_{ab}(b,\mu,\nu)}$, which has the same expressions as those for SIDIS and Drell-Yan processes. More details can be found in \cite{Collins:2011zzd,Kang:2017glf}.
Thus with $\sqrt{S_{ab}(b,\mu,\nu)}$ subtracted, the rapidity-regulator-independent standard TMDPDFs~\cite{Collins:2011zzd} $\tilde{f}_{1,q/p}(x,b, \mu, \zeta)$ and global soft function ${S}_{\mathrm global}\left(\boldsymbol{b},y_J, \mu\right)$ are defined by
\begin{align}
\tilde{f}_{1,q/p}(x,b, \mu,\zeta)& = \tilde{f}_{q/p}^{\mathrm unsub.}(x,{b}, \mu, \zeta/\nu^2) \sqrt{S_{ab}(b, \mu, \nu)}\,,\label{eq:standard-f1}\\
{S}_{\mathrm global}(\boldsymbol{b},y_J,\mu) &= \frac{{S}_{\mathrm global}^{\mathrm unsub.}(\boldsymbol{b},\mu, \nu)}{\sqrt{S_{ab}(b, \mu, \nu)}}\,.\label{eq:standard-sg}
\end{align}
Recall that for TMD PDFs $\tilde{f}_{1,q/p}(x,b, \mu, \zeta)$, the anomalous dimension $\gamma^{f_1}$ is~\cite{Arratia:2020nxw}
\begin{align}
\gamma^{f_1}&=\frac{\alpha_{s} C_{F}}{\pi}\left[\ln\left(\frac{\mu^2}{x^2s}\right)+\frac{3}{2}\right]\,.\label{eq:gammatmd}
\end{align}
For completeness, we present the global soft function ${S}_{\mathrm global}(\boldsymbol{b},y_J,\mu)$ up to the NLO as below
\begin{align}
{S}_{\mathrm global}(\boldsymbol{b},y_J,\mu) =1+ \frac{\alpha_s}{2\pi} C_F&\bigg[  2\bigg(y_J+ \ln(-2i\cos\phi_{bJ})\bigg) \left(\frac{1}{\epsilon} + \ln\frac{\mu^2}{\mu_b^2}\right)\nnu
&\quad + \frac{1}{\epsilon^2} + \frac{1}{\epsilon} \ln\frac{\mu^2}{\mu_b^2}+ \frac{1}{2} \ln^2\frac{\mu^2}{\mu_b^2}  - \frac{\pi^2}{12} \bigg]\,.
\label{eq:S_global}
\end{align}
which is universal and contributes in the lepton-jet correlations. 

Next, to write down the RG evolution of the global soft function ${S}_{\mathrm global}(\boldsymbol{b},\mu)$ in \cref{eq:S_global} and the collinear soft function ${S}_{\mathrm cs}(\boldsymbol{b},y_J,R,\mu)$ in \cref{eq:Scsbefore}, we have the RG evolution of the soft functions as
\begin{align}
\mu \frac{\mathrm{d}}{\mathrm{d} \mu} S_{\mathrm global}(\boldsymbol{b},y_J,\mu) &=\gamma^{S_{\mathrm global}}(\boldsymbol{b},y_J,\mu) S_{\mathrm global}(\boldsymbol{b},y_J,\mu)\,, \\
\mu \frac{\mathrm{d}}{\mathrm{d} \mu} S_{\mathrm cs}(\boldsymbol{b},R,\mu)&=\gamma^{S_{\mathrm cs}}\left(b,R,\mu\right) S_{\mathrm cs}(\boldsymbol{b},R,\mu)\,,
\end{align}
where the anomalous dimensions are given by
\begin{align}
\gamma^{S_{\mathrm global}}(\boldsymbol{b},y_J,\mu)&=\frac{\alpha_{s} C_{F}}{\pi}\left[ 2y_J+\ln \left(\frac{\mu^2}{\mu_b^2}\right) + \ln \left( 4\cos^2\phi_{bJ} \right) - i \pi \, {\mathrm sign}(\cos\phi_{bJ})\right]\nnu
&=\gamma^{\bar{S}}(b,y_J,\mu)+\gamma^{S_{\phi}}(\phi_{bJ},\mu)\,, \label{eq:gammasg}\\
\gamma^{S_{\mathrm cs}}\left(\boldsymbol{b},R,\mu\right)&=-\frac{\alpha_{s} C_{F}}{\pi} \left[\ln \left(\frac{\mu^2}{\mu_b^2 R^2}\right) + \ln \left(4\cos^2\phi_{bJ}\right) - i \pi \, {\mathrm sign}(\cos\phi_{bJ}) \right]\nnu
&=\gamma^{\bar{C}}(b,R,\mu)+\gamma^{C_{\phi}}(\phi_{bJ},\mu)\,,\label{eq:gammasc}
\end{align}
where we have expanded $\ln(-2i\cos\phi_{bJ})$ by separating the real and imaginary parts since they have different azimuthal angle dependence. 
\begin{align}
\ln(-2i\cos\phi_{bJ})=&\ln|2\cos\phi_{bJ}|-\frac{i\pi}{2}{\mathrm sign}(\cos\phi_{bJ})\,,\label{eq:logexp1}\\
\ln^2(-2i\cos\phi_{bJ})=&\ln^2|2\cos\phi_{bJ}|-\frac{\pi^2}{4}-i\pi\,{\mathrm sign}(\cos\phi_{bJ})\ln|2\cos\phi_{bJ}|\,,\label{eq:logexp2}
\end{align}
and we have also defined
\begin{align}
\gamma^{\bar{S}}(b,y_J,\mu)&=\frac{\alpha_{s} C_{F}}{\pi}\left[ 2y_J+\ln \left(\frac{\mu^2}{\mu_b^2}\right)\right]\,,\label{eq:gammas-bar}\\
\gamma^{S_{\phi}}(\phi_{bJ},\mu)&=\frac{\alpha_{s} C_{F}}{\pi}\Big[ \ln \left( 4\cos^2\phi_{bJ} \right) - i \pi \, {\mathrm sign}(\cos\phi_{bJ})\Big]\,,\label{eq:gammas-phi}\\
\gamma^{\bar{C}}(b,R,\mu)&=-\frac{\alpha_{s} C_{F}}{\pi}\ln \left(\frac{\mu^2}{\mu_b^2 R^2}\right) \,,\\
\gamma^{C_{\phi}}(\phi_{bJ},\mu)&=-\frac{\alpha_{s} C_{F}}{\pi} \Big[\ln \left(4\cos^2\phi_{bJ}\right) - i \pi \, {\mathrm sign}(\cos\phi_{bJ})\Big]\,,\label{eq:gammac-phi}
\end{align}

Next, by choosing $\mu=\mu_b$ for the global soft function and $\mu=\mu_b R$ for the collinear-soft function, the RG evolutions from the fixed-order calculations can be further written as
\begin{align}
\mu \frac{\mathrm{d}}{\mathrm{d} \mu} \mathcal{R}_{\bar{S}}({b},y_J,\mu_i^S,\mu_f) &=\gamma^{\bar{S}}({b},y_J,\mu) \mathcal{R}_{\bar{S}}({b},y_J,\mu_i^S,\mu_f)\,, \\
\mu \frac{\mathrm{d}}{\mathrm{d} \mu}\mathcal{R}_{S_\phi}(\phi_{bJ},\mu_i^S,\mu_f) &=\gamma^{S_{\phi}}(\phi_{bJ},\mu)\mathcal{R}_{S_\phi}(\phi_{bJ},\mu_i^S,\mu_f)\,, \\
\mu \frac{\mathrm{d}}{\mathrm{d} \mu} \mathcal{R}_{\bar{C}}({b},R,\mu_i^C,\mu_f)&=\gamma^{S_{\mathrm cs}}\left(b,R,\mu\right) \mathcal{R}_{\bar{C}}({b},R,\mu_i^C,\mu_f)\,.\\
\mu \frac{\mathrm{d}}{\mathrm{d} \mu} \mathcal{R}_{C_{\phi}}(\phi_{bJ},R,\mu_i^C,\mu_f)&=\gamma^{C_{\phi}}\left(\phi_{bJ},\mu\right)\mathcal{R}_{C_{\phi}}(\phi_{bJ},R,\mu_i^C,\mu_f)\,,
\end{align}
where $\mathcal{R}_{\bar{S}}$, $\mathcal{R}_{\bar{C}}$, $\mathcal{R}_{S_\phi}$, and $\mathcal{R}_{C_\phi}$ are the evolution kernels and given by
\begin{align}
\mathcal{R}_{\bar{S}}({b},y_J,\mu_i^S,\mu_f) &=\exp \left[\int_{\mu_i^S}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{\bar{S}}({b},y_J,\mu')\right]\,,\\
\mathcal{R}_{S_\phi}(\phi_{bJ},\mu_i^S,\mu_f) &=\exp \left[\int_{\mu_i^S}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{S_{\phi}}(\phi_{bJ},\mu')\right]\,,\\
\mathcal{R}_{\bar{C}}({b},R,\mu_i^C,\mu_f) &=\exp \left[\int_{\mu_i^{C}}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{\bar{C}}({b},\mu')\right]\,,\\
\mathcal{R}_{C_\phi}(\phi_{bJ},R,\mu_i^C,\mu_f)&=\exp \left[\int_{\mu_i^{C}}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{C_{\phi}}(\phi_{bJ},\mu')\right]\,.
\end{align}

Next, from an initial scale $\mu_i^S$ ($\mu_i^{C}$) to final scale $\mu_f$, the RG evolutions from the fixed-order calculations are
\begin{align}
S_{\mathrm global}(\boldsymbol{b},y_J,\mu)&=S_{\mathrm global}(\boldsymbol{b},y_J,\mu_i^S)\exp \left[\int_{\mu_i^S}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{S_{\mathrm global}}(\boldsymbol{b},y_J,\mu')\right]\nnu
&=S_{\mathrm global}(\boldsymbol{b},y_J,\mu_i^S)\mathcal{R}_{\bar{S}}({b},y_J,\mu_i^S,\mu_f)\mathcal{R}_{S_\phi}(\phi_{bJ},\mu_i^S,\mu_f)\,,\\
S_{\mathrm cs}(\boldsymbol{b},R,\mu)&=S_{\mathrm cs}(\boldsymbol{b},R,\mu_i^{C})\exp \left[\int_{\mu_i^{C}}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{S_{\mathrm cs}}(\boldsymbol{b},R,\mu')\right]\label{eq:gammascs1}\nnu
&=S_{\mathrm cs}(\boldsymbol{b},R,\mu_i^{C})\mathcal{R}_{\bar{C}}({b},R,\mu_i^C,\mu_f)\mathcal{R}_{C_\phi}(\phi_{bJ},R,\mu_i^C,\mu_f)\,,
\end{align}
where one can further simplify the $\phi_{bJ}$-dependent evolution kernel of global soft function as
\begin{align}
&\exp \left[\int_{\mu_i^S}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{S}_{\phi}(\phi_{bJ},\mu')\right]=\exp \left[\int_{\mu_i^S}^{\mu_f}\frac{d\mu'}{\mu'}\frac{\alpha_{s} C_{F}}{\pi}\Big[ \ln \left( 4\cos^2\phi_{bJ} \right) - i \pi \, {\mathrm sign}(\cos\phi_{bJ})\Big]\right]\nnu
&=\left| 2\cos\phi_{bJ} \right|^{2\mathcal{R}(\mu_i^S,\mu_f)}\Big[\cos(\pi\mathcal{R}(\mu_i^S,\mu_f))-i\,{\mathrm sign}(\cos\phi_{bJ})\sin(\pi\mathcal{R}(\mu_i^S,\mu_f))\Big]\,,
\label{eq:evolve_gammas1}
%&\exp \left[\int_{\mu_i^C}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{C}_{\phi}(\phi_{bJ},\mu')\right]=\exp \left[-\int_{\mu_i^C}^{\mu_f}\frac{d\mu'}{\mu'}\frac{\alpha_{s} C_{F}}{\pi}\Big[ \ln \left( 4\cos^2\phi_{bJ} \right) - i \pi \, {\mathrm sign}(\cos\phi_{bJ})\Big]\right]\nnu
%&=\left( 4\cos^2\phi_{bJ} \right)^{-\mathcal{R}(\mu_i^C,\mu_f)}\Big[\cos(\pi\mathcal{R}(\mu_i^C,\mu_f))+i\,{\mathrm sign}(\cos\phi_{bJ})\sin(\pi\mathcal{R}(\mu_i^C,\mu_f))\Big]\,,
\end{align}
with the factor $\mathcal{R}$ given by
\begin{align}
\mathcal{R}(\mu_i,\mu_f)=\int_{\mu_i}^{\mu_f}\frac{d\mu'}{\mu'}\frac{\alpha_{s} C_{F}}{\pi}\,.
\end{align}
And similarly for the collinear-soft function by applying the following replacement in \cref{eq:evolve_gammas1} 
\begin{align}
\mathcal{R}(\mu_i^S,\mu_f)\,\rightarrow\, -\mathcal{R}(\mu_i^C,\mu_f)\,.
\end{align}
where the one-loop global soft function at $\mu_i^S=\mu_b$ is $\phi_{bJ}$-independent while the collinear-soft function at $\mu_i^C=\mu_b R$ also has $\phi_{bJ}$ dependence and reads
\begin{align}
   S_{\mathrm cs}(\boldsymbol b, R,\mu=R\mu_b)= 1 - \frac{\alpha_s}{4\pi}C_F \Big[ \ln\cos(4\cos\phi_{bJ}^2) - i \pi\, {\mathrm sign}(\cos\phi_{bJ}) \Big]^2. 
\end{align}
From \cref{eq:gammas-bar}-\cref{eq:gammac-phi}, it is obvious that in the region $R\sim \mathcal{O}(1)$, one can combine the two anomalous dimensions and the $\phi_{bJ}$ dependency will be cancelled.
 However, in the small jet radii limit, one should consider RG evolution between soft scale $\mu_b$ and collinear soft scale $\mu_b R$, and the corresponding solution of the RG equation also contributes to the azimuthal asymmetry. Explicitly, we have\footnote{A detailed analytical calculation of the azimuthal anisotropy expansion of the cross section with an azimuthal angle-dependent RG evolution kernel can be found in App.~\ref{app:aae} for interested readers.} 
\begin{align}
&\exp \left[ \int_{\mu_{b} R}^{\mu_b} \frac{d\mu'}{\mu'} \frac{\alpha_s}{\pi}C_F \left( - \ln 4\cos^2\phi_{bJ} + i \pi {\mathrm sign}(\cos\phi_{bJ}) \right) \right]\,.
% =& \exp\left[ \frac{\alpha_s}{\pi} C_F \ln R \left(  \ln 4\cos^2\phi_{bJ} - i \pi {\mathrm sign}(\cos\phi_{bJ}) \right)\right] ,
    % \exp \left[ \int_{R\mu_{b}}^{\mu_b} \frac{d\mu}{\mu} \frac{\alpha_s}{\pi}C_F \left( - \ln 4\cos^2\phi_{bJ} + i \pi {\mathrm sign}(\cos\phi_{bJ}) \right) \right] \left[ 1 - \frac{\alpha_s}{4\pi}C_F \left( \ln\cos(4\cos\phi_{bJ}^2) - i \pi\, {\mathrm sign}(\cos\phi_{bJ}) \right)^2  \right],
\end{align}
% where for simplicity we ignore the running of $\alpha_s$ in the second line. 
 It is noted that the above formula resums all azimuthal-dependent terms in the small $R$ limit, with the real term contributing to all $n$-even terms and the imaginary term contributing to all the $n$-odd terms. %In addition to the evolution part, 

Finally, by summing over all the anomalous dimensions in \cref{eq:gammah},~\cref{eq:gammaj},~\cref{eq:gammasg},~\cref{eq:gammasc} and ~\cref{eq:gammatmd}, namely one has
\begin{align}
&\gamma^{H}+\gamma^{\mathcal{J}}_q+\gamma^{f_1}+\gamma^{S_{\mathrm global}}+\gamma^{S_{\mathrm cs}}\nnu
=&\frac{\alpha_{s} C_{F}}{\pi}\left[2y_J+\ln\left(\frac{Q^4}{p_T^2x^2s}\right)\right]=\frac{\alpha_{s} C_{F}}{\pi}\left[2y_J+2\ln\left(\frac{xp_T\sqrt{s}e^{-y_J}}{p_Tx\sqrt{s}}\right)\right]=0\,,\label{eq:rgcons}
\end{align}
where we have applied $Q^2=xp_T\sqrt{s}e^{-y_J}$ and shown the RG consistency among all the terms in \cref{eq:sjet-fac-before} when averaging over azimuthal angle $\phi_{qJ}$. In the following context, we will construct the RG-consistent azimuthal-angle-dependent anisotropic observables using this relation.

\iffalse
In the Drell-Yan process, where there are no soft radiations from the final state, the non-perturbative function becomes homogeneous in the X-Y plane. Thus, the function can be written as:

\begin{align}
    S_{NP}(b) = e^{-g_1 b^2}
\end{align}

However, in the case of jet production, the final state radiations from jets break the homogeneity, and a parametrization function can be chosen as:

\begin{align}
    S_{NP}(b_x,b_y) = e^{-g_{1x} b_x^2 - g_{1y} b_y^2}
\end{align}

This parametrization function takes into account the dependence on both x and y directions, where $g_{1x}$ and $g_{1y}$ are parameters that control the strength of the non-perturbative effects in each direction.

Specifically, by defining $c_n(\phi)=(-i)^n\cos^n\phi$, for $n=1,\cdots\,4$ one has
\begin{align}
&n=1:\quad (-i)\cos(\phi)=c_1(\phi)\,,\\
&n=2:\quad (-i)^2\cos(2\phi)=2c_2(\phi)+c_0(\phi)\,,\\
&n=3:\quad (-i)^3\cos(3\phi)=4c_3(\phi)+3c_1(\phi)\,,\\
&n=4:\quad (-i)^4\cos(4\phi)=8c_4(\phi)+8c_2(\phi)+c_0(\phi)\,.
\end{align}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Azimuthal anisotropy expansions}\label{app:aae}
By taking the scale choice $\mu^2 = \zeta = Q^2$ in our factorized expression, we rewrite the TMD factorization in \cref{eq:sjet-fac-before} as
\begin{align}\label{eq:sjet-fac}
    \frac{\mathrm{d}\sigma^{e+p\rightarrow e+{\mathrm jet}+X}}{\mathrm{d}^2 \boldsymbol p_T \mathrm{d}y_J \mathrm{d}^2\boldsymbol{q}_T} = \hat{\sigma}_0\,\sum_{q}e_q^2 H(Q,\mu) \int &\frac{\mathrm{d}^2\boldsymbol{b}}{(2\pi)^2}  \, \exp(-i \boldsymbol{b} \cdot \boldsymbol{q}_T) \, x \tilde{f}_{1,q/p}(x, {b}, \mu,\zeta) \mathcal{J}_{q}(p_TR,\mu) \nonumber\\
    &\times {S}_{\mathrm global}(\boldsymbol{b},y_J, \mu) \,S_{\mathrm cs}(\boldsymbol{b},R,\mu)  \;,    
\end{align}
Here, the unpolarized TMDPDFs $\tilde{f}_{1,q/p}$ in $\boldsymbol{b}$-space are defined as
\begin{align}\label{btilde}
\tilde{f}_{1,q/p}(x,{b},\mu,\zeta)=2\pi \int \mathrm{d}k_T \, k_T J_0\left(k_T b\right) f_{1,q/p}\left(x, k_T^2,\mu, \zeta\right)\,,
\end{align}
We noticed that the Fourier transformation in \cref{eq:sjet-fac} can be written as an series of the Bessel functions with azimuthal angle dependence using the Jacobi–Anger expansion~\cite{book1,book2}
\begin{align}
&\frac{\mathrm{d}^2\boldsymbol{b}}{(2\pi)^2}  \, \exp(-i \boldsymbol{b} \cdot \boldsymbol{q}_T)
=\frac{b\mathrm{d}b\,\mathrm{d}(\phi_{bJ}-\phi_{qJ})}{(2\pi)^2}\left\{J_0(bq_T)+2\sum_{n=1}^\infty (-i)^nJ_n(bq_T)\cos(n(\phi_{bJ}-\phi_{qJ}))\right\}\nnu
&=\frac{b\mathrm{d}b}{2\pi}\frac{d\phi_{bJ}}{2\pi}\bigg\{J_0(bq_T)+2\sum_{n=1}^\infty (-i)^nJ_n(bq_T)\bigg[\cos(n\phi_{qJ})\cos(n\phi_{bJ})+\sin(n\phi_{qJ})\sin(n\phi_{bJ})\bigg]\bigg\}\,,\label{eq:b-expand}
\end{align}
where $\phi_{bJ}=\phi_b-\phi_J$ and $\phi_{qJ}=\phi_q-\phi_J$. In the factorization formalism, we found that only the global soft function and collinear-soft function contain $\phi_{bJ}$ dependence. As a consequence, we 
%let ${S}_q(\boldsymbol{b},y_J,R,\mu)={S}_{\mathrm global}(\boldsymbol{b},y_J,\mu)S_{\mathrm cs}(\boldsymbol{b},y_J,R,\mu)$ and 
define an azimuthal angle average of ${S}_{\mathrm global}(\boldsymbol{b},y_J,\mu)S_{\mathrm cs}(\boldsymbol{b},y_J,R,\mu)$ weighted by a function $\mathcal{F}(\phi_{bJ})$ in the following form
\begin{align}
&{S}_q^{\langle \mathcal{F}(\phi_{bJ})\rangle}(b,y_J,R,\mu)=\int \frac{\mathrm{d}\phi_{bJ}}{2\pi} {S}_{\mathrm global}(\boldsymbol{b},y_J,\mu)S_{\mathrm cs}(\boldsymbol{b},R,\mu)\mathcal{F}(\phi_{bJ})\nnu
&=\int \frac{\mathrm{d}\phi_{bJ}}{2\pi} \mathcal{F}(\phi_{bJ})+\int \frac{\mathrm{d}\phi_{bJ}}{2\pi}\left({S}^{\mathrm NLO}_{\mathrm global}(\boldsymbol{b},y_J,\mu)+S^{\mathrm NLO}_{\mathrm cs}(\boldsymbol{b},R,\mu) \right)\mathcal{F}(\phi_{bJ})\,,\label{eq:w_average}
\end{align}
where we have applied $\bar{S}^{\mathrm LO}_{\mathrm global}({b},y_J,\mu)=\bar{S}^{\mathrm LO}_{\mathrm cs}(b,R,\mu)=1$. 

In this work, we mainly focus on $\mathcal{F}(\phi_{bJ})=\cos(n\phi_{bJ})$ ($n=0,1,2,\cdots$). Specifically, when $n=0$, one applies the notation $\bar{S}_q(b,y_J,R,\mu)$ which gives
\begin{align}
\bar{S}_q(b,y_J,R,\mu)=&\int \frac{\mathrm{d}\phi_{bJ}}{2\pi} {S}_{\mathrm global}(\boldsymbol{b},y_J,\mu)S_{\mathrm cs}(\boldsymbol{b},R,\mu)\nnu
%=&\int \frac{\mathrm{d}\phi_{bJ}}{2\pi}\Big({S}_{\mathrm global}^{\mathrm LO}(\boldsymbol{b},y_J,\mu)+{S}_{\mathrm global}^{\mathrm NLO}(\boldsymbol{b},y_J,\mu)\Big)\Big(S_{\mathrm cs}^{\mathrm LO}(\boldsymbol{b},R,\mu)+S_{\mathrm cs}^{\mathrm NLO}(\boldsymbol{b},R,\mu)\Big)+\mathcal{O}(\alpha_s^2)\nnu
=&1+\int \frac{\mathrm{d}\phi_{bJ}}{2\pi} {S}^{\mathrm NLO}_{\mathrm global}(\boldsymbol{b},y_J,\mu)+\int \frac{\mathrm{d}\phi_{bJ}}{2\pi} S^{\mathrm NLO}_{\mathrm cs}(\boldsymbol{b},R,\mu)+\mathcal{O}(\alpha_s^2)\nnu
=&1+\bar{S}^{\mathrm NLO}_{\mathrm global}(b,y_J,\mu)+\bar{S}^{\mathrm NLO}_{\mathrm cs}(b,R,\mu)+\mathcal{O}(\alpha_s^2)\,,\label{eq:average}
\end{align}
where $\bar{S}^{\mathrm NLO}_{\mathrm global}({b},y_J,\mu)$ and $\bar{S}^{\mathrm NLO}_{\mathrm cs}({b},R,\mu)$ are the azimuthal angle $\phi_{bJ}$-averaged NLO global soft functions and collinear-soft function. While when $n\ne 0$, one further has
\begin{align}
{S}_q^{\langle \cos(n\phi_{bJ})\rangle}(b,y_J,R,\mu)\bigg|_{n\ne 0}=&\int \frac{\mathrm{d}\phi_{bJ}}{2\pi}\left({S}^{\mathrm NLO}_{\mathrm global}(\boldsymbol{b},y_J,\mu)+S^{\mathrm NLO}_{\mathrm cs}(\boldsymbol{b},R,\mu) \right)\cos(n\phi_{bJ})\,,\label{eq:w_average2}
\end{align}
Note that the $\sin(n\phi_{qJ})$-related terms shown in \cref{eq:b-expand} will not contribute to the anisotropy expansion since the soft function ${S}_q(\boldsymbol{b},y_J,R,\mu)$ is an even function of $\phi_{bJ}$.
Consequently, for all $n$, the $\sin(n\phi_{bJ})$-weighted soft functions will vanish, namely  ${S}_q^{\langle\sin(n\phi_{bJ})\rangle}=0$. 

\subsubsection{Analytical calculation with azimuthal angle-dependent RG evolution }
To provide an analytical expression for ${S}_q^{\langle \cos(n\phi_{bJ})\rangle}$, we first define $c_n(\phi_{bJ})=(-i)^n\cos^n\phi_{bJ}$ for simplifying the notation and introduce the $c_n(\phi_{bJ})$-weighted evolution kernel with logarithms $\ln^k(-2i\cos\phi_{bJ})$ using the notation $\mathcal{N}_n^{(k)}$, where
\begin{align}
    \mathcal{N}_n^{(k)}(\mu_i^S,\mu_i^C)=&\int_{0}^{2\pi}\frac{d\phi_{bJ}}{2\pi}c_n(\phi_{bJ})\ln^k(-2i\cos\phi_{bJ})\exp\left[\sum_{a=S,C}\int_{\mu_i^a}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{S_{\phi}}(\phi_{bJ},\mu')\right]\nnu
    =&\int_{0}^{2\pi}\frac{d\phi_{bJ}}{2\pi}c_n(\phi_{bJ})\ln^k(-2i\cos\phi_{bJ})\exp\left[\int_{\mu_i^S}^{\mu_i^C}\frac{d\mu'}{\mu'}\gamma^{S_{\phi}}(\phi_{bJ},\mu')\right]\nnu
    =&\int_{0}^{2\pi}\frac{d\phi_{bJ}}{2\pi}c_n(\phi_{bJ})\ln^k(-2i\cos\phi_{bJ})\left| 2\cos\phi_{bJ} \right|^{2\mathcal{R}}\nnu
    &\times\Big[\cos(\pi\mathcal{R})-i\,{\mathrm sign}(\cos\phi_{bJ})\sin(\pi\mathcal{R})\Big]\bigg|_{\mathcal{R}=\mathcal{R}(\mu_i^S,\mu_i^C)}\,.\label{eq:int-phi}
\end{align}
By expanding of the logarithms into real and imaginary parts for $k=0,\ 1$ or $2$ in \cref{eq:int-phi} as shown in \cref{eq:logexp1}-\cref{eq:logexp2}, one can list the following integrals of azimuthal angle that are required to resum the global and collinear soft functions,
\begin{align}
\mathcal{N}_n^{(0)}(\mu_i^S,\mu_i^C)&=\int_{0}^{2\pi}\frac{d\phi_{bJ}}{2\pi}c_n(\phi_{bJ})\exp \left[\sum_{a=S,C}\int_{\mu_i^a}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{S_{\phi}}(\phi_{bJ},\mu')\right]\label{eq:int-phi-all0}\\
&\hspace{-1.5cm}=\int_{0}^{2\pi}\frac{d\phi_{bJ}}{2\pi}c_n(\phi_{bJ})\left|2\cos\phi_{bJ}\right|^{2\mathcal{R}}\bigg\{\cos(\pi\mathcal{R})-i\,{\mathrm sign}(\cos\phi_{bJ})\sin(\pi\mathcal{R})\bigg\}\bigg|_{\mathcal{R}=\mathcal{R}(\mu_i^S,\mu_i^C)}\,,\nnu
\mathcal{N}_n^{(1)}(\mu_i^S,\mu_i^C)&=\int_{0}^{2\pi}\frac{d\phi_{bJ}}{2\pi}c_n(\phi_{bJ})\ln(-2i\cos\phi_{bJ})\exp\left[\sum_{a=S,C}\int_{\mu_i^a}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{S_{\phi}}(\phi_{bJ},\mu')\right]\label{eq:int-phi-all}\\
&=\int_{0}^{2\pi}\frac{d\phi_{bJ}}{2\pi}c_n(\phi_{bJ})\left|2\cos\phi_{bJ}\right|^{2\mathcal{R}}\bigg\{\left[\ln|2\cos\phi_{bJ}|\cos(\pi\mathcal{R})-\frac{\pi}{2}\sin(\pi\mathcal{R})\right]\nnu
&\quad-i\,{\mathrm sign}(\cos\phi_{bJ})\left[\ln|2\cos\phi_{bJ}|\sin(\pi\mathcal{R})+\frac{\pi}{2}\cos(\pi\mathcal{R})\right]\bigg\}\bigg|_{\mathcal{R}=\mathcal{R}(\mu_i^S,\mu_i^C)}\,,\nnu
\mathcal{N}_n^{(2)}(\mu_i^S,\mu_i^C)&=\int_{0}^{2\pi}\frac{d\phi_{bJ}}{2\pi}c_n(\phi_{bJ})\ln^2(-2i\cos\phi_{bJ})\exp\left[\sum_{a=S,C}\int_{\mu_i^a}^{\mu_f}\frac{d\mu'}{\mu'}\gamma^{S_{\phi}}(\phi_{bJ},\mu')\right]\label{eq:int-phi-all2}\\
&=\int_{0}^{2\pi}\frac{d\phi_{bJ}}{2\pi}c_n(\phi_{bJ})\left|2\cos\phi_{bJ}\right|^{2\mathcal{R}}\bigg\{\bigg[\left(\ln^2|2\cos\phi_{bJ}|-\frac{\pi^2}{4}\right)\cos(\pi\mathcal{R})\nnu
&\quad-{\pi}\ln|2\cos\phi_{bJ}|\sin(\pi\mathcal{R})\bigg]-i\,{\mathrm sign}(\cos\phi_{bJ})\left[\left(\ln^2|2\cos\phi_{bJ}|-\frac{\pi^2}{4}\right)\sin(\pi\mathcal{R})\right.\nnu
&\quad\left.+{\pi}\ln|2\cos\phi_{bJ}|\cos(\pi\mathcal{R})\right]\bigg\}\bigg|_{\mathcal{R}=\mathcal{R}(\mu_i^S,\mu_i^C)}\,.
\end{align}

Note here when $n=$ even, the real part in the large bracket will contribute, while for $n=$ odd, the imaginary part which carries a Heaviside step function will contribute. To obtain the $\cos(n\phi_{bJ})$-average in \cref{eq:w_average2}, we first define the following integrals
\begin{equation}
\mathcal{I}_k(\mathcal{R},n)\equiv \begin{dcases} \displaystyle\int_{0}^{2\pi}\frac{d\phi}{2\pi}\left|2\cos\phi\right|^{2\mathcal{R}}c_n(\phi)\ln^k|2\cos\phi|\,,  &n=\mbox{even}\\
\displaystyle\int_{0}^{2\pi}\frac{d\phi}{2\pi}\left|2\cos\phi\right|^{2\mathcal{R}}c_n(\phi)(-i){\mathrm sign}(\cos\phi)\ln^k|2\cos\phi|\,,  &n=\mbox{odd}
\end{dcases}
\end{equation}

and for $k=0,\, 1$ and $2$ with $2\mathcal{R}+n>-1$, one has
\begin{align}
    {\mathcal{I}}_0(\mathcal{R},n)=& \begin{dcases}\displaystyle \frac{(-i)^n}{\sqrt{\pi}}\frac{\Gamma(\frac{1+n}{2}+\mathcal{R})}{\Gamma(1+\frac{n}{2}+\mathcal{R})}\,4^{\mathcal{R}}\,,  &n=\mbox{even}\\
    \displaystyle \frac{(-i)^{n+1}}{\sqrt{\pi}}\frac{\Gamma(\frac{1+n}{2}+\mathcal{R})}{\Gamma(1+\frac{n}{2}+\mathcal{R})}\,4^{\mathcal{R}}\,,  &n=\mbox{odd}
\end{dcases}\\
    {\mathcal{I}}_1(\mathcal{R},n)=&\,\frac{ {\mathcal{I}}_0(\mathcal{R},n)}{2}\left(H_{\frac{n-1}{2}+\mathcal{R}}-H_{\frac{n}{2}+\mathcal{R}}+\ln(4)\right)\,,\\
    {\mathcal{I}}_2(\mathcal{R},n)=&\,\frac{ {\mathcal{I}}_0(\mathcal{R},n)}{4}\left[\left(H_{\frac{n-1}{2}+\mathcal{R}}-H_{\frac{n}{2}+\mathcal{R}}+\ln(4)\right)^2+\psi^{(1)}\left(\frac{1+n}{2}+\mathcal{R}\right)-\psi^{(1)}\left(1+\frac{n}{2}+\mathcal{R}\right)\right]\,,
\end{align}
Next, one can further simplify \cref{eq:int-phi-all0}-\cref{eq:int-phi-all2} as
\begin{align}
\mathcal{N}_n^{(0)}(\mu_i^S,\mu_i^C)&=\begin{dcases}\displaystyle\cos(\pi\mathcal{R}){\mathcal{I}}_0(\mathcal{R},n)\,,  &n=\mbox{even}\\
\displaystyle\sin(\pi\mathcal{R}){\mathcal{I}}_0(\mathcal{R},n)\,,  &n=\mbox{odd}
\end{dcases}\label{eq:int-phi-all01}\\
\mathcal{N}_n^{(1)}(\mu_i^S,\mu_i^C)&=\begin{dcases}\displaystyle\cos(\pi\mathcal{R}){\mathcal{I}}_1(\mathcal{R},n)-\frac{\pi}{2}\sin(\pi\mathcal{R}){\mathcal{I}}_0(\mathcal{R},n)\,,  &n=\mbox{even}\\
\displaystyle\sin(\pi\mathcal{R}){\mathcal{I}}_1(\mathcal{R},n)+\frac{\pi}{2}\cos(\pi\mathcal{R}){\mathcal{I}}_0(\mathcal{R},n)\,,  &n=\mbox{odd}
\end{dcases}\label{eq:int-phi-all1}\\
\mathcal{N}_n^{(2)}(\mu_i^S,\mu_i^C)&=\begin{dcases}\displaystyle\cos(\pi\mathcal{R})\left(\mathcal{I}_2(\mathcal{R},n)-\frac{\pi^2}{4}\mathcal{I}_0(\mathcal{R},n)\right)-\pi\sin(\pi\mathcal{R}){\mathcal{I}}_1(\mathcal{R},n)\,,  &n=\mbox{even}\\
\displaystyle\sin(\pi\mathcal{R})\left(\mathcal{I}_2(\mathcal{R},n)-\frac{\pi^2}{4}\mathcal{I}_0(\mathcal{R},n)\right)+\pi\cos(\pi\mathcal{R}){\mathcal{I}}_1(\mathcal{R},n)\,,  &n=\mbox{odd}
\end{dcases}\label{eq:int-phi-all21}
\end{align}

For phenomenology, one can simplify the calculation by first combining the azimuthal-angle-dependent global soft and collinear-soft functions
\begin{align}
&\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_{\mathrm global}({\boldsymbol b},\mu)S_{\mathrm cs}({\boldsymbol b},R,\mu)\nnu
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_{\mathrm global}({\boldsymbol b},\mu_i^S)S_{\mathrm cs}({\boldsymbol b},R,\mu_i^C)\mathcal{R}_S^{\phi}(\phi_{bJ},\mu_i^S,\mu_f)\mathcal{R}_C^{\phi}(\phi_{bJ},R,\mu_i^C,\mu_f)\nnu
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_{\mathrm global}({\boldsymbol b},\mu_i^S)S_{\mathrm cs}({\boldsymbol b},R,\mu_i^C)\mathcal{R}_S^{\phi}(\phi_{bJ},\mu_i^S,\mu_f)\mathcal{R}_S^{\phi}(\phi_{bJ},R,\mu_f,\mu_i^S)\nnu
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_{\mathrm global}({\boldsymbol b},\mu_i^S)S_{\mathrm cs}({\boldsymbol b},R,\mu_i^C)\mathcal{R}_S^{\phi}(\phi_{bJ},\mu_i^S,\mu_i^C)\,,
\end{align}
where we have applied $\gamma_\phi^S(\phi_{bJ},\mu')=-\gamma_\phi^C(\phi_{bJ},R,\mu')$ as provided by \cref{eq:gammas-phi} and \cref{eq:gammac-phi}. With the NLO calculations given in \cref{eq:S_global} and \cref{eq:Scsbefore},
\begin{align}
S_{\mathrm global}({\boldsymbol b},\mu_i^S)S_{\mathrm cs}({\boldsymbol b},R,\mu_i^C)=&1+ \frac{\alpha_s(\mu_i^C)}{2\pi} C_F\bigg[\frac{\alpha_s(\mu_i^S)}{\alpha_s(\mu_i^C)}\bigg(2\ln(-2i\cos\phi_{bJ})\bigg) \left(\frac{1}{\epsilon} + \ln\frac{(\mu_i^S)^2}{\mu_b^2}\right)\nnu
&-2\ln^2(-2i\cos\phi_{bJ})-2\ln(-2i\cos\phi_{bJ})\left(\frac{1}{\epsilon}+\ln\left(\frac{(\mu_i^C)^2}{\mu_b^2 R^2}\right)\right)\nnu
&+\phi_{bJ}\ {\mathrm independent\ contrib.}\bigg]\,.
\end{align}
If one chooses $\mu_i^S=\mu_b$ and $\mu_i^C=\mu_b R$ as mentioned in the context, one finally obtains
\begin{align}
&\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_\phi(\phi_{bJ},\mu)C_\phi(\phi_{bJ},R,\mu)\\
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_\phi(\phi_{bJ},\mu_i^S=\mu_b)C_\phi(\phi_{bJ},R,\mu_i^C=\mu_b)\nnu
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})\bigg\{1+ \frac{\alpha_s}{2\pi} C_F\bigg[2\ln(-2i\cos\phi_{bJ})\ln R^2-2\ln^2(-2i\cos\phi_{bJ})- \frac{\pi^2}{3}\bigg]\bigg\}\nnu
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_{q,\phi}(\phi_{bJ},\R,\mu_b)=(-i)^nS_{q,\phi}^{\langle\cos(n\phi_{bJ})\rangle}(R,\mu_b)
\end{align}
where $S_{q,\phi}^\phi(\phi_{bJ},R,\mu_b)=S_\phi(\phi_{bJ},\mu_b)C_\phi(\phi_{bJ},R,\mu_b)$ and the expressions will be provided in the following section.

\subsubsection{Fixed-order calculations}
As given in \cref{eq:S_global}, the global soft function ${S}_{\mathrm global}(\boldsymbol{b},y_J,\mu)$ is free of rapidity divergence but depends on the magnitude $b$ and azimuthal angle $\phi_b$ of the vector ${\boldsymbol b}$. Similarly for the collinear soft function $S_{\mathrm cs}(\boldsymbol{b},R,\mu)$ shown in \cref{eq:Scsbefore}. In this section, we present the trigonometric function-averaged soft functions $S_q^{\langle \langle\cos(n\phi_{bJ})\rangle}$ with $n=0,\ \cdots,\ 4 $ up to NLO $\Big(\displaystyle\sim\mathcal{O}\Big(\frac{\alpha_sC_F}{\pi}\Big)\Big)$.

With the collinear-soft function $S_{\mathrm cs}(\boldsymbol{b},R,\mu)$ in \cref{eq:Scsbefore} given in terms of $\phi_{bJ}$-independent and $\phi_{bJ}$-dependent contributions, by combining \cref{eq:Scsbefore} and~\cref{eq:S_global}, the product of the global soft function and collinear soft function up to NLO is given by
\begin{align}
S_q(\boldsymbol{b},y_J,R,\mu)=&{S}_{\mathrm global}(\boldsymbol{b},y_J,\mu)S_{\mathrm cs}(\boldsymbol{b},R,\mu)\,.\label{eq:soft}
%=&1+ \frac{\alpha_s}{2\pi} C_F\bigg[  2\ln(-2i\cos\phi_{bJ})\ln R^2 -2\ln^2(-2i\cos\phi_{bJ})\nnu
%&+2y_J\left(\frac{1}{\epsilon} + \ln\frac{\mu^2}{\mu_b^2}\right) + \frac{1}{\epsilon^2} + \frac{1}{\epsilon} \ln\frac{\mu^2}{\mu_b^2}+ \frac{1}{2} \ln^2\frac{\mu^2}{\mu_b^2}  - \frac{\pi^2}{12}\nnu
%&-\bigg(\frac{1}{\epsilon^2}+ \frac{1}{\epsilon}\ln \left(\frac{\mu^2}{\mu_b^2 R^2}\right)+\frac{1}{2}\ln^2\left(\frac{\mu^2}{\mu_b^2 R^2}\right)+ \frac{\pi^2}{4}\bigg)\bigg]\nnu
%=&1+ \frac{\alpha_s}{2\pi} C_F\bigg[  2\bigg(\ln R^2\ln(-2i\cos\phi_{bJ}) -\ln^2(-2i\cos\phi_{bJ})\bigg)- \frac{\pi^2}{3}\nnu
%& +2y_J\left(\frac{1}{\epsilon} + \ln\frac{\mu^2}{\mu_b^2}\right) + \ln R^2 \left(\frac{1}{\epsilon}+ \ln\frac{\mu^2}{\mu_b^2}\right)-\frac{1}{2}\ln^2R^2\bigg]\,.\label{eq:soft}
\end{align}
Consequently, the average of $S_q(\boldsymbol{b},y_J,R,\mu)$ with or without weighted by a trigonometric function as defined in \cref{eq:average} and \cref{eq:w_average2} are calculated and presented below as
\begin{align}
\bar{S}_q(b,y_J,R,\mu)&=1+ \frac{\alpha_s}{2\pi} C_F\bigg[2y_J\left(\frac{1}{\epsilon} + \ln\frac{\mu^2}{\mu_b^2}\right) + \ln R^2 \left(\frac{1}{\epsilon}+ \ln\frac{\mu^2}{\mu_b^2}\right)-\frac{\ln^2R^2}{2}\bigg]\,,
%S_q^{\langle\phi_{bJ}\rangle}(b,R,\mu)&=\pi+ \frac{\alpha_s}{2} C_F\bigg[2y_J\left(\frac{1}{\epsilon} + \ln\frac{\mu^2}{\mu_b^2}\right) + \ln R^2 \left(\frac{1}{\epsilon}+ \ln\frac{\mu^2}{\mu_b^2}\right)-\frac{\ln^2R^2}{2}\bigg]\,,
%&=\pi\bar{S}_q(\boldsymbol{b},R,\mu)\,,\\
\end{align}
and
\begin{align}
(-i)S_{q,\phi}^{\langle\cos\phi_{bJ}\rangle}(b,R,\mu)&=\frac{\alpha_s}{\pi} C_F\bigg[\ln \frac{1}{R^2}+2(\ln4-1)\bigg]\,,\label{eq:cos1}\\
(-i)^2S_{q,\phi}^{\langle\cos(2\phi_{bJ})\rangle}(b,R,\mu)&=\frac{\alpha_s}{2\pi} C_F\bigg[\ln \frac{1}{R^2}-1\bigg]\,,\\
(-i)^3S_{q,\phi}^{\langle\cos(3\phi_{bJ})\rangle}(b,R,\mu)&=\frac{\alpha_s}{3\pi} C_F\bigg[\ln\frac{1}{R^2}+\frac{2(3\ln4-7)}{3}\bigg]\,,\\
(-i)^4S_{q,\phi}^{\langle\cos(4\phi_{bJ})\rangle}(b,R,\mu)&=\frac{\alpha_s}{4\pi} C_F\bigg[\ln \frac{1}{R^2}-\frac{5}{2}\bigg]\,.\label{eq:cos4}
\end{align}
More details are provided below for the azimuthal angle-averaged and trigonometric function-averaged functions that appear in the soft function $S_q({\boldsymbol b},y_J,R,\mu)$. Specifically, if one defines the notations $\widehat{1}$, $\widehat{\phi_{bJ}}$ and $\widehat{\cos(n\phi_{bJ})}$ of a any given function $\mathcal{L}(\phi_{bJ})$ as
\begin{align}
\widehat{1}&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}\mathcal{L}(\phi_{bJ})\,,\label{eq:hat1}\\
\widehat{\phi_{bJ}}&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}\phi_{bJ}\mathcal{L}(\phi_{bJ})\,,\label{eq:hat2}\\
\widehat{\cos(n\phi_{bJ})}&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}\cos(n\phi_{bJ})\mathcal{L}(\phi_{bJ})\,.\label{eq:hat3}
\end{align}
%\begin{align} {S}_q^{\langle \mathcal{F}(\phi_{bJ})\rangle}(b,R,\mu)=&\int \frac{\mathrm{d}\phi_{bJ}}{2\pi} {S}_{\mathrm global}(\boldsymbol{b},\mu)S_{\mathrm cs}(\boldsymbol{b},R,\mu)\mathcal{F}(\phi_{bJ})\,, \end{align} %\cref{eq:soft_total}

Recall that the components related to $\phi_{bJ}$ in the soft function $S_q(\boldsymbol{b},y_J,R,\mu)$ in \cref{eq:soft} are $\ln(-2i\cos\phi_{bJ})$ and $\displaystyle\ln^2(-2i\cos\phi_{bJ})$. Then we summarize the results of these two logarithmic functions averaged with different azimuthal-angle dependencies as defined in \cref{eq:hat1}-\cref{eq:hat3} in \cref{table}. The header row represents the form of the given function $\mathcal{L}(\phi_{bJ})$ and the header column indicates different trigonometric function-average of $\mathcal{L}(\phi_{bJ})$.
\begin{table}[]
    \centering
\begin{tabular}{ |c|c|c| } 
 \hline
  & $\ln(-2i\cos\phi_{bJ})$ & $\ln^2(-2i\cos\phi_{bJ})$ \\ 
  \hline
$\widehat{1}$ & $0$ & $-\frac{\pi^2}{6}$ \\ 
  \hline
 $\widehat{\phi_{bJ}}$ & $0$ & $-\frac{\pi^3}{6}$ \\ 
 \hline
 $(-i)\widehat{\cos\phi_{bJ}}$ & $-1$ & $-2(\ln4-1)$ \\ 
 \hline
 $(-i)^2\widehat{\cos(2\phi_{bJ})}$ & $-\frac{1}{2}$ & $\frac{1}{2}$ \\ 
 \hline
  $(-i)^3\widehat{\cos(3\phi_{bJ})}$ & $-\frac{1}{3}$ & $-\frac{2(3\ln4-7)}{9}$ \\ 
 \hline
  $(-i)^4\widehat{\cos(4\phi_{bJ})}$ & $-\frac{1}{4}$ & $\frac{5}{8}$ \\ 
 \hline
\end{tabular}
\caption{Trigonometric function-averaged values of logarithmic parts in the soft function $S_q({\boldsymbol b},y_J,R,\mu)$. The header row represents the choice of $\mathcal{L}(\phi_{bJ})$ in \cref{eq:hat1}-\cref{eq:hat3}.}\label{table}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  OLD RG-consistent factorization %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Note here for $n\ne 0$ cases in \cref{eq:cos1}-\cref{eq:cos4}, $S_q^{\langle\cos(n\phi_{bJ})\rangle}(b,R,\mu)$ does not depend on $y_J$ so we ignore this argument. Also since they have no RG evolution, we define the function $\mathscr{S}_q^{\langle\cos(n\phi_{bJ})\rangle}$ at scale $\mu=\mu_b$ to carry the fixed-order result,
\begin{align}
\mathscr{S}_q^{\langle\cos(n\phi_{bJ})\rangle}(b,y_J,R,\mu_b)=\frac{S_q^{\langle\cos(n\phi_{bJ})\rangle}(b,R,\mu_b)}{\bar{S}_q(b,y_J,R,\mu_b)}\,,
\end{align}
then \cref{eq:sjet-fac} can be further expanded as
\begin{align}
    \frac{d\sigma^{e+p\rightarrow e+{\mathrm jet}+X}}{d^2p_T dy_J d^2\boldsymbol{q}_T} =\,&\hat{\sigma}_0\,\sum_{q}e_q^2 H(Q,\mu) \int \frac{bdb}{2\pi}x \tilde{f}^{\mathrm TMD}_1(x, b, \mu,\zeta)  \mathcal{J}_{q}(p_TR,\mu)\bar{S}_q(b,y_J,R,\mu)\bigg\{J_0(bq_T)\nnu
    &+2\sum_{n=1}(-i)^nJ_n(bq_T)\cos(n\phi_{qJ}){\mathscr{S}_q^{\langle\cos(n\phi_{bJ})\rangle}(b,y_J,R,\mu_b)}\bigg\}\,,\label{eq:sjet-fac-last}
%    &+2\sum_{n=1}(-i)^nJ_n(bq_T)\bigg[\cos(n\phi_{qJ})\frac{{S}_q^{\langle\cos(n\phi_{bJ})\rangle}(b,R,\mu_b)}{\bar{S}_q(b,R,\mu_b)}\bigg]\bigg\}\,,\label{eq:sjet-fac-last}
\end{align}
For azimuthal-angle averaged differential cross section weighted with $\cos(n\phi_{qJ})$, one thus obtains
\begin{align}
d\sigma^{\langle1\rangle}=&\int_0^{2\pi}\frac{d\phi_{qJ}}{2\pi}\frac{d\sigma^{e+p\rightarrow e+{\mathrm jet}+X}}{d^2p_T dy_J d^2\boldsymbol{q}_T}\label{eq:sigma00}\\
=&\hat{\sigma}_0\,\sum_{q}e_q^2 H(Q,\mu) \int \frac{bdb}{2\pi}x \tilde{f}^{\mathrm TMD}_1(x, b, \mu,\zeta)  \mathcal{J}_{q}(p_TR,\mu)\bar{S}_q(b,y_J,R,\mu)J_0(bq_T)\,,\ \nnu
\hspace{-0.5cm}d\sigma^{\langle\cos(n\phi_{qJ})\rangle}=&\int_0^{2\pi}\cos(n\phi_{qJ})\frac{d\phi_{qJ}}{2\pi}\frac{d\sigma^{e+p\rightarrow e+{\mathrm jet}+X}}{d^2p_T dy_J d^2\boldsymbol{q}_T}\label{eq:sigma0c}  \\
=&\hat{\sigma}_0\,\sum_{q}e_q^2 H(Q,\mu) \int \frac{bdb}{2\pi}x \tilde{f}^{\mathrm TMD}_1(x, b, \mu,\zeta)  \mathcal{J}_{q}(p_TR,\mu)\bar{S}_q(b,y_J,R,\mu)J_n(bq_T)\nnu
&\times (-i)^n{\mathscr{S}_q^{\langle\cos(n\phi_{bJ})\rangle}(b,y_J,R,\mu_b)}\,.\nonumber
\end{align}

Thus using the above expressions in \cref{eq:sigma00} and~\cref{eq:sigma0c}, we can define the azimuthal anisotropy ${\langle\cos(n\phi_{qJ})\rangle}$ as
\begin{align}
{\langle\cos(n\phi_{qJ})\rangle}&=\frac{d\sigma^{\langle\cos(n\phi_{qJ})\rangle}}{d\sigma^{\langle1\rangle}}\,.
\end{align}
As shown in \cref{eq:rgcons}, we see that the observables in \cref{eq:sigma00} and~\cref{eq:sigma0c} are both RG-consistent and have the same evolution between scales.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

One can simplify the calculation by first combining the azimuthal-angle-dependent global soft and collinear-soft functions
\begin{align}
&\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_{\mathrm global}({\boldsymbol b},\mu)S_{\mathrm cs}({\boldsymbol b},R,\mu)\nnu
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_{\mathrm global}({\boldsymbol b},\mu_i^S)S_{\mathrm cs}({\boldsymbol b},R,\mu_i^C)\mathcal{R}_S^{\phi}(\phi_{bJ},\mu_i^S,\mu_f)\mathcal{R}_C^{\phi}(\phi_{bJ},R,\mu_i^C,\mu_f)\nnu
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_{\mathrm global}({\boldsymbol b},\mu_i^S)S_{\mathrm cs}({\boldsymbol b},R,\mu_i^C)\mathcal{R}_S^{\phi}(\phi_{bJ},\mu_i^S,\mu_f)\mathcal{R}_S^{\phi}(\phi_{bJ},R,\mu_f,\mu_i^S)\nnu
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_{\mathrm global}({\boldsymbol b},\mu_i^S)S_{\mathrm cs}({\boldsymbol b},R,\mu_i^C)\mathcal{R}_S^{\phi}(\phi_{bJ},\mu_i^S,\mu_i^C)\,,
\end{align}
where we have applied $\gamma_\phi^S(\phi_{bJ},\mu')=-\gamma_\phi^C(\phi_{bJ},R,\mu')$ as provided by \cref{eq:gammas-phi} and \cref{eq:gammac-phi}. With the NLO calculations given in \cref{eq:S_global} and \cref{eq:Scsbefore},
\begin{align}
S_{\mathrm global}({\boldsymbol b},\mu_i^S)S_{\mathrm cs}({\boldsymbol b},R,\mu_i^C)=&1+ \frac{\alpha_s(\mu_i^C)}{2\pi} C_F\bigg[\frac{\alpha_s(\mu_i^S)}{\alpha_s(\mu_i^C)}\bigg(2\ln(-2i\cos\phi_{bJ})\bigg) \left(\frac{1}{\epsilon} + \ln\frac{(\mu_i^S)^2}{\mu_b^2}\right)\nnu
&-2\ln^2(-2i\cos\phi_{bJ})-2\ln(-2i\cos\phi_{bJ})\left(\frac{1}{\epsilon}+\ln\left(\frac{(\mu_i^C)^2}{\mu_b^2 R^2}\right)\right)\nnu
&+\phi_{bJ}\ {\mathrm independent\ contrib.}\bigg]\,.
\end{align}
If one chooses $\mu_i^S=\mu_i^C=\mu_b$ to cancel the UV divergence, one finally obtains
\begin{align}
&\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_\phi(\phi_{bJ},\mu)C_\phi(\phi_{bJ},R,\mu)\\
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_\phi(\phi_{bJ},\mu_i^S=\mu_b)C_\phi(\phi_{bJ},R,\mu_i^C=\mu_b)\nnu
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})\bigg\{1+ \frac{\alpha_s}{2\pi} C_F\bigg[2\ln(-2i\cos\phi_{bJ})\ln R^2-2\ln^2(-2i\cos\phi_{bJ})- \frac{\pi^2}{3}\bigg]\bigg\}\nnu
&=\int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ})S_{q,\phi}(\phi_{bJ},\R,\mu_b)=(-i)^nS_{q,\phi}^{\langle\cos(n\phi_{bJ})\rangle}(R,\mu_b)
\end{align}
where $S_{q,\phi}^\phi(\phi_{bJ},R,\mu_b)=S_\phi(\phi_{bJ},\mu_b)C_\phi(\phi_{bJ},R,\mu_b)$ and $(-i)^nS_{q,\phi}^{\langle\cos(n\phi_{bJ})\rangle}(R,\mu_b)$ has been provided in \cref{eq:cos1}-\cref{eq:cos4}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  RG evolution at small R (approximated) %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Azimuthal asymmetry and jet radius resummation}\label{app:smallR}
In this appendix, we provide the theoretical formula for azimuthal asymmetries including jet radius $R$ resummation effects. 

The anomalous dimensions of the global soft function and collinear-soft function are given by
\begin{align}
\gamma^{S_{\mathrm global}}(\boldsymbol{b},y_J,\mu)&=\frac{\alpha_{s} C_{F}}{\pi}\left[ 2y_J+\ln \left(\frac{\mu^2}{\mu_b^2}\right) + \ln \left( 4\cos^2\phi_b \right) - i \pi \, {\mathrm sign}(\cos\phi_b)\right]\,, \label{eq:gammasg-full}\\
\gamma^{S_{\mathrm cs}}\left(\boldsymbol{b},R,\mu\right)&=-\frac{\alpha_{s} C_{F}}{\pi} \left[\ln \left(\frac{\mu^2}{\mu_b^2 R^2}\right) + \ln \left(4\cos^2\phi_b\right) - i \pi \, {\mathrm sign}(\cos\phi_b) \right]\,,\label{eq:gammasc-full}
\end{align}
where we separate the real and imaginary parts since they have different azimuthal angle dependence. It is obvious that in the region $R\sim \mathcal{O}(1)$ if we combine the above two anomalous dimensions, $\phi_b$ dependent term will cancel. However, in the small jet radii limit, one should consider RG evolution between soft scale $\mu_b$ and collinear soft scale $R\mu_b$, and the corresponding solution of the RG equation also contributes to the azimuthal asymmetry. Explicitly, we have 
\begin{align}
&\exp \left[ \int_{R\mu_{b}}^{\mu_b} \frac{d\mu}{\mu} \frac{\alpha_s}{\pi}C_F \left( - \ln 4\cos^2\phi_b + i \pi {\mathrm sign}(\cos\phi_b) \right) \right] \notag \\
=& \exp\left[ \frac{\alpha_s}{\pi} C_F \ln R \left(  \ln 4\cos^2\phi_b - i \pi {\mathrm sign}(\cos\phi_b) \right)\right] ,
    % \exp \left[ \int_{R\mu_{b}}^{\mu_b} \frac{d\mu}{\mu} \frac{\alpha_s}{\pi}C_F \left( - \ln 4\cos^2\phi_b + i \pi {\mathrm sign}(\cos\phi_b) \right) \right] \left[ 1 - \frac{\alpha_s}{4\pi}C_F \left( \ln\cos(4\cos\phi_b^2) - i \pi\, {\mathrm sign}(\cos\phi_b) \right)^2  \right],
\end{align}
where for simplicity we ignore the running of $\alpha_s$ in the second line. It is noted that the above formula resum all azimuthal dependent terms in the small $R$ limit, and the real term contribute all $n$-even terms and the imaginary term contributes to all the $n$-odd terms. In addition to the evolution part, the one-loop collinear-soft function at $\mu=R\mu_b$ also has $\phi_b$ dependence which reads
\begin{align}
   S_{\mathrm cs}(\boldsymbol b, R,\mu=R\mu_b)= 1 - \frac{\alpha_s}{4\pi}C_F \left[ \ln\cos(4\cos\phi_b^2) - i \pi\, {\mathrm sign}(\cos\phi_b) \right]^2. 
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Numerical results}
In this subsection, we present the numerical results for $\cos\phi$ azimuthal asymmetries with EIC and HERA kinematics. Following the factorization shown in \cref{eq:sjet-fac-before}, using the regulator-independent standard TMDPDFs~\cite{Collins:2011zzd} $\tilde{f}_{1,q/p}(x,b, \mu, \zeta)$ and global soft function ${S}_{\mathrm global}\left(\boldsymbol{b},y_J, \mu\right)$ defined in \cref{eq:standard-f1} and~\cref{eq:standard-sg}, the factorized cross-section is expressed in position space as
\begin{align}\label{eq:sjet-fac}
    \frac{\mathrm{d}\sigma^{e+p\rightarrow e+{\mathrm jet}+X}}{\mathrm{d}^2 \boldsymbol p_T \mathrm{d}y_J \mathrm{d}^2\boldsymbol{q}_T} = \hat{\sigma}_0\,\sum_{q}e_q^2 H(Q,\mu) \int &\frac{\mathrm{d}^2\boldsymbol{b}}{(2\pi)^2}  \, \exp(-i \boldsymbol{b} \cdot \boldsymbol{q}_T) \, x \tilde{f}_{1,q/p}(x, {b}, \mu,\zeta) \mathcal{J}_{q}(p_TR,\mu) \nonumber\\
    &\times {S}_{\mathrm global}(\boldsymbol{b},y_J, \mu) \,S_{\mathrm cs}(\boldsymbol{b},R,\mu)  \;,    
\end{align}
Here, the unpolarized TMDPDFs $\tilde{f}_{1,q/p}$ in $\boldsymbol{b}$-space are defined as~\cite{Boussarie:2023izj}
\begin{align}\label{btilde}
\tilde{f}_{1,q/p}(x,{b},\mu,\zeta)=2\pi \int \mathrm{d}k_T \, k_T J_0\left(k_T b\right) f_{1,q/p}\left(x, k_T^2,\mu, \zeta\right)\,,
\end{align}
By writing \cref{eq:sjet-fac} in a series of trigonometric expansion,
\begin{align}
\frac{\mathrm{d}\sigma^{e+p\rightarrow e+{\mathrm jet}+X}}{\mathrm{d}^2 \boldsymbol p_T \mathrm{d}y_J \mathrm{d}^2\boldsymbol{q}_T}=A_0+2\sum_{n=1}^\infty A_n\cos(n\phi_{qJ})\,,
\end{align}
with coefficients $A_0$, $A_n$ defined as
\begin{align}
A_0\defeq&\int_0^{2\pi}\frac{d\phi_{qJ}}{2\pi}\frac{\mathrm{d}\sigma}{\mathrm{d}^2 \boldsymbol p_T \mathrm{d}y_J \mathrm{d}^2\boldsymbol{q}_T}\nnu
=&\hat{\sigma}_0\,\sum_{q}e_q^2 H(Q,\mu) \int\frac{bdb}{2\pi}  \, J_0(bq_T) \, x \tilde{f}_{1,q/p}(x, {b}, \mu,\zeta) \mathcal{J}_{q}(p_TR,\mu)\nnu
&\times \int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}{S}_{\mathrm global}(\boldsymbol{b},y_J, \mu) \,S_{\mathrm cs}(\boldsymbol{b},R,\mu)\,, \\
A_n\defeq&\int_0^{2\pi}\frac{d\phi_{qJ}}{2\pi}\cos(n\phi_{qJ})\frac{\mathrm{d}\sigma}{\mathrm{d}^2 \boldsymbol p_T \mathrm{d}y_J \mathrm{d}^2\boldsymbol{q}_T}\nnu
=&\hat{\sigma}_0\,\sum_{q}e_q^2 H(Q,\mu) \int\frac{bdb}{2\pi}  \, J_n(bq_T) \, x \tilde{f}_{1,q/p}(x, {b}, \mu,\zeta) \mathcal{J}_{q}(p_TR,\mu)\nnu
&\times \int_0^{2\pi}\frac{d\phi_{bJ}}{2\pi}(-i)^n\cos(n\phi_{bJ}){S}_{\mathrm global}(\boldsymbol{b},y_J, \mu) \,S_{\mathrm cs}(\boldsymbol{b},R,\mu)\,.\label{eq:phi-int}
\end{align}

\begin{figure}[h]
\centering
\includegraphics[width=0.38\textwidth]{aniso/eic_R1_log.pdf}
\hspace{0.18cm}\includegraphics[width=0.38\textwidth]
{aniso/eic_R05_log.pdf}\\
\vspace{0.3cm}
\includegraphics[width=0.38\textwidth]{aniso/h1_R1_log.pdf}
\hspace{0.18cm}\includegraphics[width=0.38\textwidth]
{aniso/h1_R05_log.pdf}
%\includegraphics[width=0.8\textwidth,trim={0 1.2cm 0 0},clip]{aniso/anisotropy-eic.pdf}
\caption{The NLL calculation (dark-blue curve) of jet azimuthal anisotropy $\langle\cos\phi\rangle$ with EIC kinematics at $\sqrt{s}=105$ GeV (upper panel) and HERA kinematics at $E_p=920$ GeV, $E_e=27.6$ GeV (lower panel) for $10<p_T<25$ GeV, $0<q_T<5$ GeV and jet radius $R = 1.0$ (left column) and $R = 0.5$ (right column) in comparison with \texttt{PYTHIA8}~\cite{Sjostrand:2007gs} simulation (light-blue step).}\label{fig:eic_ani}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=0.92\textwidth]{aniso/eic_R1_3.pdf}\\
%\vspace{0.3cm}
\includegraphics[width=0.92\textwidth]{aniso/h1_R1_3.pdf}\\
%\includegraphics[width=0.8\textwidth,trim={0 1.2cm 0 0},clip]{aniso/anisotropy-eic.pdf}
\caption{The NLL calculation of jet azimuthal anisotropy $\langle\cos n\phi\rangle$ ($n=1,\ 2,$ and $3$ in each panel respectively) with EIC kinematics at $\sqrt{s}=105$ GeV (upper panel) and HERA kinematics at $E_p=920$ GeV, $E_e=27.6$ GeV(lower panel) for $10<p_T<25$ GeV, $0<q_T<5$ GeV and jet radius $R = 1.0$. The diamond points are generated using \texttt{PYTHIA8}~\cite{Sjostrand:2007gs}.}\label{fig:eic_ani2}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=0.92\textwidth]{aniso/eic_R05_3.pdf}\\
%\vspace{0.3cm}
\includegraphics[width=0.92\textwidth]
{aniso/h1_R05_3.pdf}
%\includegraphics[width=0.8\textwidth,trim={0 1.2cm 0 0},clip]{aniso/anisotropy-eic.pdf}
\caption{The NLL calculation of jet azimuthal anisotropy $\langle\cos n\phi\rangle$ ($n=1,\ 2,$ and $3$ in each panel respectively) with EIC kinematics (upper panel) and HERA kinematics (lower panel) for jet radius $R = 0.5$. The diamond points are generated using \texttt{PYTHIA8}~\cite{Sjostrand:2007gs}.}\label{fig:eic_ani3}
\end{figure}
%%%%%%%%%%%%%% Jacobi–Anger expansion %%%%%%%%%%%%%%
Note that the above relations can also be obtained by expanding the Fourier transformation in \cref{eq:sjet-fac} in series of the Bessel functions with azimuthal angle dependence~\cite{Hatta:2021jcd,Tong:2022zwp}, namely the Jacobi–Anger expansion~\cite{book1,book2}
\begin{align}
&\frac{\mathrm{d}^2\boldsymbol{b}}{(2\pi)^2}  \, \exp(-i \boldsymbol{b} \cdot \boldsymbol{q}_T)
=\frac{b\mathrm{d}b\,\mathrm{d}(\phi_{bJ}-\phi_{qJ})}{(2\pi)^2}\left\{J_0(bq_T)+2\sum_{n=1}^\infty (-i)^nJ_n(bq_T)\cos(n(\phi_{bJ}-\phi_{qJ}))\right\}\,,\label{eq:b-expand}
\end{align}
where $\phi_{bJ}=\phi_b-\phi_J$ and $\phi_{qJ}=\phi_q-\phi_J$. In the factorization formalism, we found that only the global soft function and collinear-soft function contain $\phi_{bJ}$ dependence.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Accordingly, jet anisotropy $\langle\cos(n\phi)\rangle$ is defined by
\begin{align}
\langle\cos(n\phi)\rangle&\defeq\left(\int_0^{2\pi}\frac{d\phi_{qJ}}{2\pi}\cos(n\phi_{qJ})\frac{\mathrm{d}\sigma}{\mathrm{d}^2 \boldsymbol p_T \mathrm{d}y_J \mathrm{d}^2\boldsymbol{q}_T}\right)\bigg/\left(\int_0^{2\pi}\frac{d\phi_{qJ}}{2\pi}\frac{\mathrm{d}\sigma}{\mathrm{d}^2 \boldsymbol p_T \mathrm{d}y_J \mathrm{d}^2\boldsymbol{q}_T}\right)=\frac{A_n}{A_0}\,.
\end{align}

In \cref{fig:eic_ani}, we first provide the directed flow $\langle\cos(\phi)\rangle$ with EIC kinematics at $\sqrt{s}=105$ GeV in the upper panels and HERA kinematics at $E_p=920$ GeV, $E_e=27.6$ GeV with $10<p_T<25$ GeV, $0<q_T<5$ GeV in the lower panels. The left two panels have jet radius $R = 1.0$ while the right two panels have $R = 0.5$. All the NLL theoretical results are given in dark-blue curves and in comparison with \texttt{PYTHIA8}~\cite{Sjostrand:2007gs} simulations described by the light-blue steps. 


Furthermore, our study presents numerical results for three different azimuthal asymmetries, namely $\langle\cos\phi\rangle$, $\langle\cos2\phi\rangle$, and $\langle\cos3\phi\rangle$, represented by dark-blue, dark-green, and red curves respectively. These asymmetries are depicted in the left, middle, and right panel of \cref{fig:eic_ani2} ($R=1.0$) and \cref{fig:eic_ani3} ($R=0.5$), where $\phi$ denotes $\phi_{qJ}$ in the given context. Notably, the directed flow $v_1$ is the dominant flow in both kinematics and radii. In addition, we find that~\footnote{This is also consistent with the behavior of fixed-order expressions.} the elliptic flow $v_2$ and the triangular flow $v_3$ exhibit negative values for large $R$, as shown in \cref{fig:eic_ani2}, and positive values for small $R$, as demonstrated in \cref{fig:eic_ani3}. The lighter-colored steps in each panel are generated using \texttt{PYTHIA8}~\cite{Sjostrand:2007gs}. The magnitudes of all three flows are measurable for both EIC and HERA kinematics, suggesting that these measurements could be feasible for future experiments.
%#################################
%In this section, we present the numerical results for jet azimuthal anisotropy up to quadrapole flow ($\langle\cos(4\phi)\rangle$) together with \texttt{PYTHIA8} simulations.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Energy-energy correlators}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Introduction}\label{sec:intro}
The energy-energy correlators (EEC)~\cite{Basham:1978bw,Basham:1978zq} is one of the earliest infrared and collinear (IRC) safe event shape observables~\cite{Kinoshita:1962ur,Lee:1964is}. In high-energy particle physics, the study of EEC has played a crucial role in advancing our understanding of fundamental particles and their interactions. This event shape observable has been used in various experiments~\ \cite{SLD:1994idb,L3:1992btq,OPAL:1991uui,TOPAZ:1989yod,TASSO:1987mcs,JADE:1984taa,Fernandez:1984db,Wood:1987uf,CELLO:1982rca,PLUTO:1985yzc}, including electron-positron collisions and semi-inclusive deep inelastic scattering (SIDIS) with unpolarized scattering beams, which have revealed insights into the structure and properties of hadrons and other subatomic particles. With its long history and a simple definition, EEC has been measured by various experimental collaborations. Recent experimental measurements have demonstrated the power of EEC in studying hadron properties. For example, high precision measurements were conducted~\cite{OPAL:1990reb,ALEPH:1990vew,L3:1991qlf,SLD:1994yoe,ATLAS:2015yaa,ATLAS:2017qir,ATLAS:2020mee} for comparing to the resummed and fixed order calculations with high perturbative accuracy~\cite{Moult:2018jzp,Ebert:2020sfi,Gao:2019ojf,Li:2020bub}, which indicates great opportunities offered by EEC observables for precision studies in QCD.

Theoretical developments have also played an important role in advancing the study of EEC, involving extensive computations at fixed orders~\cite{Dixon:2019uzg,deFlorian:2004mp,Dixon:2018qgp,Luo:2019nig,Henn:2019gkr,Tulipant:2017ybb,Belitsky:2013xxa,Belitsky:2013bja,Belitsky:2013ofa}. Perturbative QCD calculations have been used to predict the behavior of EEC in various processes. These calculations include the use of Feynman diagrams~\cite{Basham:1978bw,Korchemsky:1999kt,Luo:2019nig} and other mathematical tools to describe the interaction between subatomic particles. In recent years, advances in computational techniques have made it possible to perform more precise and detailed calculations~\cite{Andreassen:2019cjw,Chen:2022pdu,Chen:2022muj,Jaarsma:2022kdd,Li:2021zcf}, allowing for better comparisons with experimental measurements. 

Furthermore, the singular behaviors of the EEC in the back-to-back ($\tau \rightarrow 0$)~\cite{Collins:1981uk,Kodaira:1981nh,deFlorian:2004mp,Tulipant:2017ybb,Moult:2018jzp} and collinear ($\tau \rightarrow 1$) limits~\cite{Dixon:2019uzg,Kologlu:2019mfz,Korchemsky:2019nzm,Chen:2020uvt,Konishi:1978yx,Konishi:1978ax} have been an interesting topic in theoretical study, where QCD factorization and resummation have been conducted. In particular, connection to the TMD observables in the back-to-back limit has been observed and studied in the context of unpolarized processes in both $e^+e^-$ and appropriately modified definition of the EEC for the $ep$ collisions\ \cite{Li:2021txc}. In~\cite{Ebert:2020sfi}, a highly precise calculation was completed at the N$^3$LL' level of accuracy following the derivation of the $O(\alpha_s^3)$ singular distributions. Additionally, EEC has been computed to a significant perturbative accuracy -- by utilizing the $4$-loop rapidity anomalous dimension~\cite{Moult:2022xzt,Duhr:2022yyp}, it has been possible to carry out perturbative resummation to N$^4$LL accuracy~\cite{Duhr:2022yyp}. These studies have also been employed to extract the strong coupling constant with high accuracy~\cite{deFlorian:2004mp,Kardos:2018kqj}. With significant progress in the higher-order perturbative calculations and simplicity in the experimental measurement and charged track structure\ \cite{Chen:2020vvp,Li:2021zcf}, EEC is one of the prime examples of a promising observable to carry out precision studies of the strong coupling constant $\alpha_s$~\cite{Zyla:2729066}. Moreover, there has been significant progresses made in the understanding of the EEC from different other directions. For example, as pointed out in~\cite{Chen:2022jhb,Lee:2022ige}, the energy correlators also opens up possibilities to a range of sophisticated techniques developed within the framework of conformal field theories (CFTs). 

To introduce the novel event shape observable defined in this work, the polarized energy-energy correlators (PEEC), we start with the definition of EEC~\cite{Kinoshita:1962ur,Lee:1964is} in $e^+e^-$ collisions, where the EEC is used to measure the correlation between the energies of two particles produced in the collision. This correlation provides valuable information about the masses and life-times of these particles, as well as their decay mechanisms\footnote{For example, in studies of the $Z$ boson, a massive particle produced in electron-positron collisions, EEC has been used to determine the decay modes of the $Z$ boson and to test predictions of the Standard Model of particle physics.}. In this context, EEC is defined by taking the weighted sum over pairs of hadrons produced in the final states\footnote{Note that some literatures, e.g.~\cite{Moult:2018jzp,Ebert:2020sfi} instead used a different variable $z$ defined as $z = 1-\tau$.}
\begin{align}
\label{eq:EECdef}
\mathrm{EEC}_{e^+e^-}(\tau) \equiv \frac{1}{\sigma}\frac{d\Sigma_{e^+e^-}}{d\tau}=\frac{1}{2} \sum_{i,j}\int d\theta_{ij} dz_i dz_j z_i z_j \frac{1}{\sigma} \frac{d\sigma}{d\theta_{ij} dz_i dz_j} \delta\left(\tau - \left(\frac{1+\cos \theta_{ij}}{2}\right)\right)\,,
\end{align}
where $z_i$ and $z_j$ are the energy fractions of the final-state hadrons $i,j$, separated by $\theta_{ij}$. In this paper, we further extend the understanding of the EEC in the back-to-back limit ($\tau \rightarrow 0$) by considering azimuthal asymmetries associated with the EEC. For $e^+e^-$ collisions, the new observable involves generalizing the Eq.\ \cref{eq:EECdef} with an azimuthal-angle dependence as shown in \cref{fig:intro}
\begin{align}
\label{eq:EECazdef}
\mathrm{PEEC}_{e^+e^-}(\tau,\phi) \equiv& \frac{1}{\sigma}\frac{d\Sigma_{e^+e^-}}{d\tau d\phi}\\
=&\frac{1}{2} \sum_{i,j}\int d\theta_{ij} dz_i dz_j z_i z_j \frac{1}{\sigma} \frac{d\sigma}{d\theta_{ij}d\phi_{ij} dz_i dz_j} \delta\left(\tau - \left(\frac{1+\cos \theta_{ij}}{2}\right)\right) \delta(\phi - \phi_{ij})\,,\nonumber
\end{align}
\begin{figure}[h]
\centering
\includegraphics[width=0.6\textwidth]{eec/eec-ee-new-ij.pdf}
\caption{Illustration of PEEC for $e^+e^-$ annihilation. Here $\theta_{ij}$ is the angle separation between the final-state hadrons $h_i,\,h_j$ and $\phi_{ij}$ is the azimuthal angle of the transverse momentum of hadron $h_i$ with respect to $h_j$.}\label{fig:intro}
\end{figure}
where $\theta_{ij}$ is the angle separation between the final-state hadrons $i,j$ and $\phi_{ij}$ is the azimuthal angle difference between the two hadrons in the Gottfried-Jackson (GJ) frame\ \cite{Gottfried:1964nx} that uses one of the hadron as the reference to define the azimuthal angle of another hadron\footnote{By choosing the direction of $h_j$ as $z$-axis, one can see that $\theta_{ij}$ and $\phi_{ij}$ are the polar angle and azimuthal angle in this frame.}. 

As we will see, this azimuthal angle dependent PEEC gives sensitivity to both the traditional EEC as well as the Collins-type EEC, which is related to the Collins fragmentation functions $H_{1}^\perp(z,{k}_\perp^2,\mu)$~\cite{Collins:1992kk}, one of the most extensively discussed polarized TMDs, describing the fragmentation of the transversely polarized quark into an unpolarized hadron. This fragmentation process correlates the transverse momentum of the outgoing hadron with the transverse polarization of the quark, giving rise to non-trivial azimuthal angular asymmetries. For the $e^+e^-$ annihilation, two transversely polarized quarks can be produced from the unpolarized $e^+e^-$ without violating spin conservation. The Collins asymmetries then manifest itself with the azimuthal asymmetry $\cos (2\phi)$, where $\phi$ is the azimuthal angle between the two back-to-back hadrons.

The azimuthal angle dependent PEEC will exhibit similar asymmetries in both $e^+e^-$ and $ep$ collisions as the TMD processes just described. In the $e^+e^-$ collision, the PEEC measured with the azimuthal dependence takes the form
\begin{align}
{\rm PEEC}_{e^+e^-}\sim \sum_q \left[\jet_q\otimes \jet_{\bar{q}}\otimes S+\cos2{\phi}\,\jet_q^{\perp}\otimes \jet_{\bar{q}}^{\perp}\otimes S\right]\,.
\end{align}
%where ${\bm q}_T$ is defined by the transverse momentums ${\bm P}_{1\perp}$, ${\bm P}_{2\perp}$ and momentum fractions $z_1$, $z_2$ of the di-hadron pair $\frac{{\bm q}_T}{z_1}=\frac{{\bm P}_{1\perp}}{z_1}+\frac{{\bm P}_{2\perp}}{z_2}$. 
As explained below the Eq.\ \cref{eq:EECazdef}, ${\phi}$ is the azimuthal angle of the final-hadron pairs in the GJ frame. The jet functions $\jet_q$ and $\jet_{\bar{q}}$ are the unpolarized EEC jet functions introduced first in \cite{Moult:2018jzp,Li:2021txc}, whereas $\jet_q^{\perp}$ and $\jet_{\bar{q}}^{\perp}$ are the new Collins-type EEC jet functions we study in this paper. Finally, $S$ is the soft function generated by soft gluon radiations, which is independent of the polarizations of the partons involved\ \cite{Kang:2020xez,Buffing:2018ggv,Chien:2019gyf,Kang:2020xgk}. 

Similarly, in semi-inclusive deep inelastic scatterings (SIDIS), the PEEC is used to measure the correlation between the energy of a scattered lepton and the energy of the hadron produced in the scattering process. These measurements allow researchers to study the structure of hadrons and to probe the quark-gluon structure of matter. By using polarized scattering beams in the $ep$-collisions, we can also investigate the spin structure of hadrons and gain insights into the strong force that binds quarks together. For instance, a transversely polarized quark from the transversely polarized beam will scatter with the photon and undergoes Collins fragmentation process and the Collins asymmetries in $ep$ correlates the azimuthal angle of the outgoing hadron, $\phi_h$, with the that of the transverse spin of the incoming beam, $\phi_s$, giving rise to the azimuthal asymmetry in the form of $\sin(\phi_h+\phi_s)$.

Furthermore, a comprehensive analysis of the azimuthal angle dependent PEEC for $ep$ collisions in the Breit frame, as a generalization of recent research works \cite{Li:2020bub,Ali:2020ksn,Li:2021txc}, will offer an unprecedented opportunity to disentangle the target and fragmentation regions. Specifically, in the context of SIDIS process employing a polarized proton beam, the PEEC$_{\rm DIS}$ exhibits a remarkable correlation between the EEC jet functions and all the leading-twist transverse-momentum-dependent parton distribution functions (TMD PDFs), thus highlighting the immense potential of PEEC as a pioneering tool for exploring the intricate three-dimensional structure of nucleons.

The TMD PDFs play a critical role in our understanding of the internal structure of nucleons, as they provide information on the momentum distribution of partons within the nucleon. These distributions are essential in determining the scattering cross-sections and kinematics of high-energy particles in hadronic collisions. Therefore, the ability to accurately measure TMD PDFs is crucial for a deeper understanding of the underlying physics governing particle interactions. In this regard, the PEEC method has shown tremendous potential as a novel tool for probing TMD PDFs and advancing our knowledge of the internal structure of nucleons.


%It was shown in\ \cite{}, when the approximation of $S^i_{\rm NP} = 0$ is exact, i.e. when $b \ll 1/\Lambda_{\rm QCD}$ (or $\Lambda_{\rm QCD} \ll k_T \ll Q$)\footnote{the small $b$ behavior of $S^i_{\rm NP}$ must follow the power law behavior\ \cite{}.}, the TMD FFs of various hadrons combine to give the unpolarized EEC jet function $\jet_i$ in terms of the matching coefficients $C_{j\leftarrow {i}}$ alone. This follows as a consequence of the sum rules of the unpolarized collinear fragmentation functions, $D_{1,h/j}\left(x, \mu_{b_*}\right)$. %This is the reason for the jet functions lacking any hadronic labels. 
%Therefore, by looking at different regions of $q_T$, EEC may be useful in changing sensitivity to, and thus helpful in extracting, the non-perturbative parts of the TMDs.  \textcolor{red}{(Maybe need to be careful with this statement, as there are usually convolutions of TMDs, so small $b$ and large $q_T$ regions may not correspond to each other exactly. That is, $\Lambda_{\rm QCD} \ll q_T$ does not imply $b \ll \Lambda_{\rm QCD}$ for BOTH of the TMDs involved. What I wrote may be vague enough to be ok?)}. 
%um rule of the twist-$3$ matrix elements when the off-diagonal matching terms are ignored. 
%However, theoretical basis of ST sum rule requires more precise investigation. Although ST sum rule can be understood from an intuitive momentum conservation argument, such momentum conservation arguments are shown to be insufficient to demonstrate validity of similar sum rules~\cite{Meissner:2010cc,Metz:2016swz}. Furthermore, the derivation of ST sum rule uses bare operators and is thus unknown whether the sum rule survives for the renormalized case.\footnote{We thank Andreas Metz for pointing this out to us} We propose Collins-type EEC in the back-to-back region as a useful observable to phenomenologically test this sum rule. As you will see in Sec.~\ref{}, two different fits with and without the ST sum rule imposed give wildly different predictions. We believe that study of Collins-type EEC will be an important first step to understand TMD sum rules in polarized fragmentation functions.
%As the off-diagonal matching terms are subleading, the Collins-type EEC is an exciting observable where the measurement of any non-vanishing value is directly related to the observation of the non-perturbative TMD effects of the Collins function. Therefore, the Collins-type EEC presented in this paper can serve as a proxy for the sensitivity and size of the non-perturbative effects in TMD observables.

This manuscript is structured as follows: Section~\ref{sec:kinematics} presents a comprehensive analysis of the factorization framework governing polarized energy-energy correlators in $e^+e^-$ and $ep$ collisions, introducing the Collins-type EEC jet function. In Section~\ref{sec:jetfunc}, we delve into the mathematical foundations of the unpolarized and Collins-type EEC jet functions. Section~\ref{sec:pheno} presents our phenomenological study of the potential of EEC jets for probing nucleon structures. Finally, this work concludes in Section~\ref{sec:conclusion}.

\subsubsection{Factorization for Collins-type Energy-Energy Correlators}\label{sec:kinematics}
In this section, we explore the azimuthal angle dependence of the PEEC for $e^+e^-$ annihilation and DIS process in the back-to-back region. The PEEC in this region can be related to the transverse momentum dependent (TMD) framework, which allows us to identify both unpolarized and Collins-type EEC jet functions. We demonstrate that these EEC jet functions exhibit interesting azimuthal angle dependence, which can be studied in detail using high-energy collision data. 

\subsubsection{PEEC in the back-to-back region for $e^+e^-$ annihilation}
\begin{figure}[h]
\centering
\includegraphics[width=0.6\textwidth]{eec/eec_ee.pdf}
\caption{Illustration of PEEC for $e^+e^-$ annihilation in GJ frame.}\label{fig:eec_ee}
\end{figure}

We begin by discussing PEEC for $e^+e^-$ annihilation. As shown in Eq.\ \cref{eq:EECdef} above already, the traditional EEC for the $e^+e^-$ annihilation is defined with the weighted integral over energy fractions as a function of the angle between the hadron pairs characterized by
\begin{align}
\label{eq:zdef}
\tau = \frac{1+\cos\theta_{12}}{2}\,,
\end{align}
with $\theta_{12}$ representing the angle separation between two final hadrons $h_1,\,h_2$. In the back-to-back limit ($\tau \rightarrow 0$), up to power corrections,
\begin{align}
\tau = \frac{\bm{P}_{h_\perp}^2}{z_1^2Q^2}\,,
\end{align}
where $\bm{P}_{h_\perp}$ is the transverse momentum of the hadron $h_1$ in the so-called Gottfried-Jackson frame\ \cite{Gottfried:1964nx} defined by the other hadron $h_2$ in the pair and the incoming lepton pair as depicted in the \cref{fig:eec_ee}. This momentum can then be decomposed as 
\begin{align}
\frac{\bm{P}_{h_\perp}}{z_1} = \frac{\bm{p}_{1_\perp}}{z_1} + \frac{\bm{p}_{2_\perp}}{z_2} - \bm{\lambda}_{\perp}\,,
\end{align}
where $\bm{p}_{1(2)_\perp}$ is the hadron transverse momentum with respect to the fragmenting partons (quark and anti-quark, in this case) and $\bm{\lambda}_{\perp}$ is the soft recoil of these fragmenting partons from being exactly back-to-back and is thus measured with respect to the thrust-axis. This momentum is also related to the transverse component of the exchanged gauge boson in the hadron pair center-of-mass (CM) frame through the relations, $\bm{q}_T = -\bm{P}_{h_\perp}/z_1$.\footnote{we will always mean $\bm{P}_{h_1 \perp}^2$ and $\bm{q}_T$ to mean the transverse momentum measured in their respective frames just discussed.} We will often use $\bm{q}_T$ for convenience.

Then continuing in the back-to-back limit, azimuthal angle dependent PEEC for $e^+e^-$ defined in the Eq.\ \cref{eq:EECazdef} above can be related to the $\bm{q}_T$ as 
\begin{align}
\label{eq:EECazdef2}
\mathrm{PEEC}_{e^+e^-}(\tau,\phi) =  \frac{1}{\sigma}\frac{d\Sigma_{e^+e^-}}{d\tau d\phi} &=\frac{1}{2} \sum_{i,j}\int d^2\bm{q}_T dz_i dz_j z_i z_j \frac{1}{\sigma} \frac{d\sigma}{d^2\bm{q}_T dz_i dz_j} \delta(\tau - \frac{\bm{q}_T^2}{Q^2}) \delta(\phi - \phi_{q_T})\,,
\end{align}
where $\phi_{q_T}$ is the azimuthal angle of the two hadrons $h_i$ and $h_j$ in the Gottfried-Jackson (GJ) frame\ \cite{Gottfried:1964nx} that uses one hadron as the reference to define the azimuthal angle of another hadron as shown in the \cref{fig:eec_ee}. The azimuthal angle dependent factorization in the Gottfried-Jackson frame was derived in \cite{Kang:2015msa} as 
\begin{align}
&\frac{d\sigma}{dz_1dz_2 d^2{\bm q}_T}=\frac{4\pi N_c\alpha_{\rm em}^2}{3Q^2}\sum_q e_q^2\int d^2{\bm p}_{1_\perp}d^2{\bm p}_{2_\perp}d^2{\bm \lambda}_{\perp}\delta^2\left(\frac{{\bm p}_{1_\perp}}{z_1}+\frac{{\bm p}_{2_\perp}}{z_2}-{\bm \lambda}_{\perp}+{\bm q}_T\right)\nnu
&\qquad\times{S}({\bm \lambda}_{\perp}^2,\mu,\nu)\bigg[D_{h_1/q}(z_1,{\bm p}_{1_\perp}^2,\mu,\zeta/\nu^2)D_{h_2/\bar{q}}(z_2,{\bm p}_{2_\perp}^2,\mu,\zeta/\nu^2)+\frac{1}{2}\cos 2\phi_{q_T}(2{\bm \hat{\bm q}}_T^\alpha{\hat{\bm q}}_T^\beta-g_\perp^{\alpha\beta})\nnu
&\hspace{3.3cm}\times\frac{\bm p_{1_\perp}^\alpha}{z_1M_1}H_{1,h_1/q}^{\perp}(z_1,{\bm p}_{1_\perp}^2,\mu,\zeta/\nu^2)\frac{\bm p_{2_\perp}^\alpha}{z_2M_2}H_{1,h_2/\bar{q}}^{\perp}(z_2,{\bm p}_{2_\perp}^2,\mu,\zeta/\nu^2)\bigg]\,,\label{eq:diffcskt}
\end{align}
where $D_{h/q}(z,{\bm p}_{\perp}^2,\mu,\zeta/\nu^2)$ and $H_{1,h/q}^{\perp}(z,{\bm p}_{\perp}^2,\mu,\zeta/\nu^2)$ are the unpolarized and Collins TMD FFs, respectively. This factorization can then be transformed into $\mathbf{b}$-space as
\begin{align}
\label{eq:diffcsb}
\frac{d\sigma}{dz_1dz_2 d^2{\bm q}_T}=&\frac{4\pi N_c\alpha_{\rm em}^2}{3Q^2}\sum_q e_q^2\int\frac{d^2{\bm b}}{(2\pi)^2}e^{-i{\bm b}\cdot{\bm q}_T}\bigg[\tilde{D}_{1,h_1/q}(z_1,{\bm b}^2,\mu,\zeta/\nu^2)\nnu
&\times\tilde{D}_{1,h_2/q}(z_2,{\bm b}^2,\mu,\zeta/\nu^2)+\frac{1}{2}\cos 2\phi_{q_T}(2{\hat{\bm q}}_T^\alpha{\hat{\bm q}}_T^\beta-g_\perp^{\alpha\beta})\nnu
&\times\tilde{H}_{1,h_1/{q}}^{\perp\,\alpha}(z_1,{\bm b}^2,\mu,\zeta/\nu^2)\tilde{H}_{1,h_2/{q}}^{\perp\,\alpha}(z_2,{\bm b}^2,\mu,\zeta/\nu^2)\bigg]S({\bm b}^2,\mu,\nu)\,, 
\end{align}
where the TMD FFs in the $b$-space are defined as
\begin{align}
%%%%%%%%%%%%%%%%%%% D1(z,b^2) %%%%%%%%%%%%%%%%%%%
\tilde{D}_{1,h_i/{q}}(z_i,{\bm b}^2,\mu,\zeta/\nu^2)=&\int d^2{\bm p}_{i_\perp}e^{-i{\bm b}\cdot{{\bm p}_{i_\perp}}/{z_i}}D_{1,h_i/q}(z_i,{\bm p}_{i_\perp}^2,\mu,\zeta/\nu^2)\,,\\
%%%%%%%%%%%%%%%%%%% H1^\perp(z,b^2) %%%%%%%%%%%%%%%%%%%
\tilde{H}_{1,h_i/{q}}^{\perp\,\alpha}(z_i,{\bm b}^2,\mu,\zeta/\nu^2)=&\int d^2{\bm p}_{i_\perp}e^{-i{\bm b}\cdot{{\bm p}_{i_\perp}}/{z_i}}\frac{\bm p_{i_\perp}^\alpha}{z_iM_i} H_{1,h_i/q}^{\perp}(z_i,{\bm p}_{i_\perp}^2,\mu,\zeta/\nu^2)\,,
\end{align}
and the soft function ${S({\bm b}^2,\mu,\nu)}$ in $b$-space at one loop is given as
%in~\cite{Collins:2011zzd,Kang:2017glf,Kang:2021ffh}
\begin{align}
{S}({\bm b}^2,\mu,\nu)&=\int d^2{\bm \lambda}_{\perp}e^{i{\bm b}\cdot{\bm \lambda}_{\perp}}{S}({\bm \lambda}_{\perp}^2,\mu,\nu)\nnu
&=1 - \frac{\alpha_s C_F}{2\pi} \Bigg[2\left(\frac{2}{\eta}+\ln\frac{\nu^2}{\mu^2}\right)\left(\frac{1}{\epsilon}+\ln\frac{\mu^2}{\mu_b^2}\right)+
\ln^2\frac{\mu^2}{\mu_b^2}
-\frac{2}{\epsilon^2}+\frac{\pi^2}{6}
\Bigg]\,.
\label{eq:S-ab}
\end{align}
The soft-function is computed to 3-loop order in\ \cite{Li:2016ctv}.
%using the identity
%\begin{align}
%\delta^2\left(\frac{{\bm P}_{1\perp}}{z_1}+\frac{{\bm P}_{2\perp}}{z_2}-{\bm \lambda}_{\perp}+{\bm q}_T\right)=\int\frac{d^2{\bm b}}{(2\pi)^2}e^{-i{\bm b}\cdot\left(\frac{{\bm P}_{1\perp}}{z_1}+\frac{{\bm P}_{2\perp}}{z_2}-{\bm \lambda}_{\perp}+{\bm q}_T\right)}\,.
%\end{align}

%At $1$-loop, the soft function ${S({\bm b}^2,\mu,\nu)}$ in $b$-space was given in~\cite{Collins:2011zzd,Kang:2017glf,Kang:2021ffh} as
%\begin{align}
%{S}({\bm b}^2,\mu,\nu)&=\int d^2{\bm \lambda}_{\perp}e^{i{\bm b}\cdot{\bm \lambda}_{\perp}}{S}({\bm \lambda}_{\perp}^2,\mu,\nu)\nnu
%&=1 - \frac{\alpha_s C_F}{2\pi} \Bigg[2\left(\frac{2}{\eta}+\ln\frac{\nu^2}{\mu^2}\right)\left(\frac{1}{\epsilon}+\ln\frac{\mu^2}{\mu_b^2}\right)+
%\ln^2\frac{\mu^2}{\mu_b^2}
%-\frac{2}{\epsilon^2}+\frac{\pi^2}{6}
%\Bigg]\,.
%\label{eq:S-ab}
%\end{align}
%On the other hand, TMD FFs in the $b$-space are defined as
%\begin{align}
%%%%%%%%%%%%%%%%%%% D1(z,b^2) %%%%%%%%%%%%%%%%%%%
%\tilde{D}_{1,h_i/{q}}(z_i,{\bm b}^2,\mu,\zeta/\nu^2)=&\int d^2{\bm P}_{i\perp}e^{-i{\bm b}\cdot\frac{{\bm P}_{i\perp}}{z_i}}D_{1,h_i/q}(z_i,{\bm P}_{i\perp}^2,\mu,\zeta/\nu^2)\,,\\
%%%%%%%%%%%%%%%%%%% H1^\perp(z,b^2) %%%%%%%%%%%%%%%%%%%
%\tilde{H}_{1,h_i/{q}}^{\perp\,\alpha}(z_i,{\bm b}^2,\mu,\zeta/\nu^2)=&\int d^2{\bm P}_{i\perp}e^{-i{\bm b}\cdot\frac{{\bm P}_{i\perp}}{z_i}}\frac{\bm P_{i\perp}^\alpha}{z_iM_i} H_{1,h_i/q}^{\perp}(z_i,{\bm P}_{i\perp}^2,\mu,\zeta/\nu^2)\,.
%\end{align}
%Putting them all together, we are able to transform \cref{eq:diffcskt} to $b$-space expression as
%\begin{align}
%\label{eq:diffcsb}
%\frac{d\sigma}{dz_1dz_2 d^2{\bm q}_T}=&\frac{4\pi N_c\alpha_{\rm em}^2}{3Q^2}\sum_q e_q^2\int\frac{d^2{\bm b}}{(2\pi)^2}e^{-i{\bm b}\cdot{\bm q}_T}\bigg[\tilde{D}_{1,h_1/q}(z_1,{\bm b}^2,\mu,\zeta/\nu^2)\nnu
%&\times\tilde{D}_{1,h_2/q}(z_2,{\bm b}^2,\mu,\zeta/\nu^2)+\frac{1}{2}\cos 2\phi_{q_T}(2{\hat{\bm q}}_T^\alpha{\hat{\bm q}}_T^\beta-g_\perp^{\alpha\beta})\nnu
%&\times\tilde{H}_{1,h_1/{q}}^{\perp\,\alpha}(z_1,{\bm b}^2,\mu,\zeta/\nu^2)\tilde{H}_{1,h_2/{q}}^{\perp\,\alpha}(z_2,{\bm b}^2,\mu,\zeta/\nu^2)\bigg]S({\bm b}^2,\mu,\nu)\,.
%\end{align}

Then we carry out the energy-fraction-weighted integrals to get $\phi$-dependent EEC from the Eq.\ \cref{eq:EECazdef2} to arrive at
\begin{align}
\label{eq:epemEEC}
\frac{d\Sigma_{e^+e^-}}{d\tau d\phi}=&\frac{2\pi N_c\alpha_{\rm em}^2}{3Q^2}\sum_q e_q^2\int d{\bm q}_T^2\delta(\tau  - \frac{{\bm q}_T^2}{Q^2})\int\frac{bdb}{2\pi}\bigg[J_0(bq_T)\jet_{q}({\bm b},\mu,\zeta/\nu^2)\jet_{\bar{q}}({\bm b},\mu,\zeta/\nu^2)S({\bm b}^2,\mu,\nu)\nnu
&\qquad + \frac{b^2}{8}\cos 2{\phi}J_2(bq_T)\left. \jet_{q}^{\perp}({\bm b},\mu,\zeta/\nu^2)\jet_{\bar{q}}^{\perp}({\bm b},\mu,\zeta/\nu^2)S({\bm b}^2,\mu,\nu)\right]\,,
\end{align}
where we defined the unpolarized EEC jet function as introduced in\ \cite{Moult:2018jzp} and the new Collins-type EEC jet functions, respectively, as (the anti-quark case defined analogously)
\begin{align}
\label{eq:unpjet}
\jet_q({\bm b},\mu,\zeta/\nu^2)\equiv&\sum_{h}\int_0^1dz\,z\,\tilde{D}_{1,h/q}(z,{\bm b}^2,\mu,\zeta/\nu^2)\,,\\
\left(-\frac{i{\bm b}^\alpha}{2}\right)\jet_q^\perp({\bm b},\mu,\zeta/\nu^2)\equiv&\sum_{h}\int_0^1dz\,z\, \tilde{H}_{1,h/q}^{\perp\,\alpha}(z,{\bm b}^2,\mu,\zeta/\nu^2)
\label{eq:Collinsjet}\,.
\end{align}
Note that the left-hand side no longer carries hadron label as we sum over the final state hadrons. We will discuss simplifications of these jet functions in the OPE region below.  %Also, note that although we will only encounter quark EEC jet functions for the processes considered in this paper. 

\subsubsection{PEEC in the back-to-back region for Deep Inelastic Scattering}
In this subsection, we study the PEEC in $ep$ collisions. Semi-inclusive deep inelastic scattering (SIDIS) is a fundamental tool in the study of the structure of nucleons and nuclei. One important observable in SIDIS is the energy-energy correlator, which measures the correlation between the energy of the scattered lepton and the energy of the final-state hadrons. By studying the process
\begin{align}
e^-(l)+p(P)\rightarrow e^-(l')+h(P_h)+X\,,
\end{align}
we first write down $\rm{PEEC_{DIS}}$ defined in the Breit frame~\cite{Li:2021txc} generalized with polarized proton beams and azimuthal angle dependence. Then for the lab frame, we will introduce a different PEEC observable, $\rm{PEEC_{DIS}}^*$ in the Semi-Inclusive DIS as a function of a scalar variable called $q_*$~\cite{Gao:2022bzi} for a distinct perspective of the application of PEEC in SIDIS.

\begin{itemize}
\item Breit
\begin{figure}[h]
\centering
\includegraphics[width=0.65\textwidth]{eec/eec_ep.pdf}
\caption{Illustration of PEEC for Deep Inelastic Scattering in Breit frame.}\label{fig:eec_ep}
\end{figure}
The SIDIS version of the EEC that will be generalized to PEEC here was developed only very recently\ \cite{Li:2021txc}\footnote{Although we will follow\ \cite{Li:2021txc} and call our observable EEC/PEEC in this section, the ``EEC" may be a misnomer in this context as the energy weighting comes only from a single outgoing hadron. On the other hand, $N$-outgoing hadron correlators were referred to as $\rm{E^NC}$ or $\rm{ENC}$ in \cite{Komiske:2022enw}.}, where the traditional EEC was proposed to be measured in the Breit frame, allowing a clean separation between the target and current region. The $\rm{EEC_{DIS}}$ was then characterized as a function of the angular separation $\theta_{ap}$ between the incoming beam $p$ and the outgoing hadron $a$, which we now generalize to the azimuthal angle dependent case as shown in \cref{fig:eec_ep},
\begin{align}
\label{eq:EECazimDISdef}
\mathrm{PEEC_{DIS}}(\tau,\phi) &\equiv \frac{1}{\sigma}\frac{d\Sigma_{\rm DIS}}{d\tau d\phi}\\
&=\frac{1}{2} \sum_{a}\int d\theta_{a}d\phi_{ap} dz_a z_a \frac{1}{\sigma} \frac{d\sigma}{d\theta_{ap} d\phi_{ap} dz_a} \delta\left(\tau - \left(\frac{1+\cos \theta_{ap}}{2}\right)\right)\delta(\phi - \phi_{ap})\,.\nonumber
\end{align}
Similar to the discussion above for $e^+e^-$, in the back-to-back limit ($\tau\rightarrow 0$), we find
\begin{align}
\tau = \frac{\bm{P}_{aT}^2}{z_a^2 Q^2}\,,
\end{align}
where $Q = \sqrt{-q^2}$ is the invariant mass of the exchanged virtual photon, $\bm{P}_{aT}$ is the transverse momentum of the outgoing hadron measured with respect to the photon-beam axis, and $z_a = p_a^+/Q$ is the momentum fraction of the outgoing hadron in the Breit frame. For convenience, we will introduce $\bm{q}_T \equiv \bm{P}_{aT}/z_a$,which should be distinguished from the virtual photon momentum. Then in the back-to-back limit, the transverse momentum can be sourced from different contributions as
\begin{align}
\bm{q}_T = \frac{\bm{P}_{a\perp}}{z_a} + \bm{p}_{n\perp} - \bm{\lambda}_{\perp}\,,
\end{align}
where $\bm{P}_{a\perp}$ is the hadron transverse momentum with respect to the fragmenting parton (quark or anti-quark, in this case), $\bm{p}_{n\perp}$ is the transverse momentum of the parton inside the hadron, and $\bm{\lambda}_{\perp}$ is the soft-radiation describing the recoil and is measured with respect to the photon-beam axis. 

Then in the back-to-back limit, azimuthal angle dependent PEEC for SIDIS defined in the Eq.\ \cref{eq:EECazimDISdef} can be related to the $\bm{q}_T$-differential cross-section in the back-to-back limit as
\begin{align}
\label{eq:EECazimDISdef2}
\mathrm{PEEC}_{\rm DIS}(\tau,\phi) =  \frac{1}{\sigma}\frac{d\Sigma_{\rm DIS}}{d\tau d\phi} &=\frac{1}{2} \sum_{a}\int d^2\bm{q}_T dz_a z_a \frac{1}{\sigma} \frac{d\sigma}{d^2\bm{q}_T dz_a} \delta(\tau - \frac{\bm{q}_T^2}{Q^2}) \delta(\phi - \phi_{q_T})\,.
\end{align}
Starting from the relevant azimuthal angle dependent $\bm{q}_T$ factorization for the DIS process given in\ \cite{Gourdin:1972kro,Kotzinian:1994dv,Diehl:2005pc,Bacchetta:2006tn,Anselmino:2008sga,Collins:2011zzd,Kang:2015msa}, using the EEC jet functions defined above in Eqs.\ \cref{eq:unpjet} and\ \cref{eq:Collinsjet}, the PEEC at SIDIS in Eq.\ \cref{eq:EECazimDISdef2} can be written as
\begin{align}
\frac{d\Sigma_{\rm DIS}}{dxdyd\tau d\phi}=&\frac{2\pi\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\int d^2{\bm q}_T\delta(\tau -\frac{{\bm q}_T^2}{Q^2})\delta(\phi - \phi_{q_T})\int\frac{db\ b}{2\pi}\bigg\{\mathcal{F}_{UU}\nnu
&+\cos(2\phi_{q_T})\frac{2(1-y)}{1+(1-y)^2}\mathcal{F}_{UU}^{\cos(2\phi_{q_T})}+S_{\parallel}\sin(2\phi_{q_T})\frac{2(1-y)}{1+(1-y)^2}\mathcal{F}_{UL}^{\sin(2\phi_{q_T})}\nnu
&+|{\bm S}_\perp|\bigg[\sin(\phi_{q_T}-\phi_s)\mathcal{F}_{UT}^{\sin(\phi_{q_T}-\phi_s)}+\sin(\phi_{q_T}+\phi_s)\frac{2(1-y)}{1+(1-y)^2}\mathcal{F}_{UT}^{\sin(\phi_{q_T}+\phi_s)}\nnu
&\hspace{1.4cm}+\sin(3\phi_{q_T}-\phi_s)\frac{2(1-y)}{1+(1-y)^2}\mathcal{F}_{UT}^{\sin(3\phi_{q_T}-\phi_s)}\bigg]\nnu
&+\lambda_e\bigg[S_{\parallel}\frac{y(2-y)}{1+(1-y)^2}\mathcal{F}_{LL}
+|{\bm S}_\perp|\cos(\phi_{q_T}-\phi_s)\mathcal{F}_{LT}^{\cos(\phi_{q_T}-\phi_s)}\bigg]\bigg\}\,,\label{eq:EECDIS3}
\end{align}
where for structure functions $\mathcal{F}_{AB}$, the indices $A$ and $B$ represent the polarization of the incoming electron and incoming proton. The definition and components of each structure function are provided in App.~\ref{app1}. $S_{\parallel}$ and $|{\bm S}_\perp|$ are the helicity and transverse spin of the incoming proton, $\lambda_e$ is the helicity of the incoming electron. The variables $x$ and $y$ represent the longitudinal momentum fraction of the incoming parton inside the beam and the inelasticity variable, respectively, which we will additionally be differential in. The azimuthal angles $\phi_s$ and $\phi_{q_T}$ are the azimuthal angles of the transverse spin of the beam and the transverse momentum imbalance, respectively. The first term has appeared in\ \cite{Li:2021txc}. Unlike the PEEC in $e^+e^-$ annihilation, SIDIS version of the PEEC has only one EEC jet function per term as it measures correlation between one outgoing hadron and the beam. 

    \item Lab frame
%%%%%%%%%%%%%%%%%%%%%
As demonstrated in~\cite{Gao:2022bzi}, a new method using $q_*$ was developed for extracting the transverse momentum distributions of hadrons in DIS experiments. $q_*$ is a recently proposed observable for measuring the transverse momentum distributions of hadrons in deep inelastic scattering (DIS) experiments. It is constructed in the lab frame by taking the difference between the virtual photon's momentum and the scattered electron's momentum, both projected onto the plane perpendicular to the beam direction. $q_*$ has the advantage of being less sensitive to higher-twist effects compared to traditional observables like Q, which is constructed using the total momentum transfer in the DIS process.

A detailed analysis of the effects of higher-twist contributions on $q_*$ was performed and it is demonstrated that $q_*$ is less sensitive to these effects than traditional observables like $P_{hT}$. They also investigate the impact of experimental uncertainties on the measurement of $q_*$ and show that it is robust to these uncertainties.

Using simulations of DIS events at the proposed Electron-Ion Collider (EIC), one finds that $q_*$ can provide more accurate measurements of the transverse momentum distributions of hadrons compared to traditional observables. They also show that $q_*$ can help to disentangle different sources of transverse momentum broadening in the hadronization process.

%In conclusion, this paper presents a new method for measuring the transverse momentum distributions of hadrons in DIS experiments using the $q_*$ observable. The authors demonstrate that $q_*$ has several advantages over traditional observables like Q, including being less sensitive to higher-twist effects and providing more accurate measurements of the transverse momentum distributions of hadrons. This new method has important implications for future DIS experiments, particularly at the proposed EIC, where precise measurements of the transverse momentum distributions of hadrons are essential for studying the internal structure of nucleons.

As discussed in \cite{Gao:2022bzi}, a high-precision reconstruction of polar and azimuthal angles in the EIC lab frame to exploit the acoplanarity angle ($\phi_{acop}$) as a precision probe of hadron transverse momentum ($P_{hT}$). It provides a full relation between $\phi_{acop}$ and $P_{hT}$ for leading-power kinematics in the target rest frame. It further defines optimized observable $q_*$ to probe $P_{hT}$ more directly, which has a simple leading-power limit in $P_{hT} \ll zQ$. The formulae for $Q^2$, $y$, and $x$ in terms of the EIC frame pseudorapidities of outgoing lepton and hadron are given. The leading power limits of the $Q^2$ and $y$ formulae in the $M \ll Q$ limit are given. The formulae hold up to power corrections in $P_{hT}/(zQ)$ that control the distance to the Born limit, and the $\mathcal{O}(\lambda)$ corrections are also provided.
%%%%%%%%%%%%%%%%%%%%%
%As proposed in~\cite{Gao:2022bzi}, a new observable called $q_*$ is designed for measuring the transverse momentum distributions (TMDs) of hadrons and to be maximally resilient against resolution effects while delivering the same sensitivity to TMD dynamics as $P_{hT}\ll Q$. 
The construction of $q_*$ is given by
\begin{align}
q_*= -2P_{\rm EIC}^0\frac{e^{\eta_h}}{1+e^{\eta_h-\eta_e}}\left[\frac{P_{hT}\sin\phi_h}{zQ\sqrt{1-y}}+\mathcal{O}\left(\frac{P_{hT}^2}{(zQ)^2}\right)\right]\,
\end{align}
where $\phi_h$ is measured in the Trento frame and represents the azimuthal angle of $\vec{P}_{hT}$. 
 $P_{\rm EIC}^0$, $\eta_h$ and $\eta_e$ are all measured in the EIC frame, $y=(P\cdot q)/(P\cdot l)$. At the leading power, one can apply the approximation $q_*\approx -P_{hT}\sin\phi_h$ to simplify the analytical calculation. The observable $q_*$ is designed to be maximally resilient against resolution effects while delivering the same sensitivity to TMD dynamics as $P_{hT}\ll Q$. This resolves the issue of accurately reconstructing small transverse momentum $P_{hT}$ in 3D measurements of confinement and hadronization. 
 
The leading power expansion with the limit $P_{hT}\ll zQ$ can be written as
\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{eec/eec_epqs.pdf}
\caption{PEEC for Deep Inelastic Scattering in the $xy$ plane of \cref{fig:eec_ep}}\label{fig:eec_ep2}
\end{figure}
Now we define the PEEC with $q_*$ measured as
\begin{align}
\mathrm{PEEC}_{\rm DIS}^*(q_*)=\frac{1}{\sigma}\frac{d\Sigma_{\rm DIS}}{dq_*}=&\frac{1}{2} \sum_{a}\int d^2\bm{q}_T dz_a z_a\frac{1}{\sigma} \frac{d\sigma}{dz_ad^2\bm{q}_T} \delta(q_* - q_T\sin\phi_{q_T}) \nnu
=&\frac{1}{2} \sum_{a}\int dz_a z_a \frac{1}{\sigma}\frac{d\sigma}{dz_adq_*}
\end{align}

\iffalse
\begin{align}
=&\frac{2\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\int db\sum_qe_q^2H(Q,\mu)S({\bm b}^2,\mu,\nu)\bigg\{\cos\left(bq_*\right)\bigg[\tilde{f}_1{J}_q\nnu
&+\frac{2(1-y)}{1+(1-y)^2}\frac{Mb^2}{2}\tilde{h}_1^{\perp (1)}{J}_q^\perp+\lambda_eS_{\parallel}\frac{y(2-y)}{1+(1-y)^2}\tilde{g}_{1L}{J}_q\bigg]\nnu
&+|{\bm S}_\perp|\sin\left(bq_*\right)\cos\phi_s\bigg[-Mb\tilde{f}_{1T}^{\perp(1)}{J}_q+\frac{2(1-y)}{1+(1-y)^2}\frac{b}{2}\tilde{h}_1{J}_q^\perp\nnu
&+\frac{2(1-y)}{1+(1-y)^2}\frac{M^2b^3}{8}\tilde{h}_{1T}^{\perp (2)}{J}_q^\perp\bigg]\nnu
&+\lambda_e|{\bm S}_\perp|\sin\left(bq_*\right)\sin\phi_sMb\tilde{g}_{1T}^{(1)}{J}_q\bigg\}\,,\label{eq:EECDISq1}
\end{align}
\fi
As for the azimuthal-angle dependence of the structure functions with $q_*$ measured,
\begin{align}
\frac{d\Sigma_{\rm DIS}}{dxdydq_*}=&\frac{2\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\int db\bigg\{\cos\left(bq_*\right)\bigg[\mathcal{D}[\tilde{f}_1\jet_q]\nnu
&+\frac{2(1-y)}{1+(1-y)^2}\mathcal{D}[\tilde{h}_1^{\perp(1)}\jet_q^{\perp}]+\lambda_eS_{\parallel}\frac{y(2-y)}{1+(1-y)^2}\mathcal{D}[\tilde{g}_{1L}\jet_q]\bigg]\nnu
&+|{\bm S}_\perp|\sin\left(bq_*\right)\cos\phi_s\bigg[-\mathcal{D}[\tilde{f}^{\perp(1)}_{1T}\jet_q]+\frac{2(1-y)}{1+(1-y)^2}\mathcal{D}[\tilde{h}_1\jet_q^{\perp}]\nnu
&+\frac{2(1-y)}{1+(1-y)^2}\frac{1}{4}\mathcal{D}[\tilde{h}^{\perp(2)}_{1T}\jet_q^{\perp}]\bigg]+\lambda_e|{\bm S}_\perp|\sin\left(bq_*\right)\sin\phi_s\mathcal{D}[\tilde{g}^{(1)}_{1T}\jet_q]\bigg\}\,,\label{eq:EECDISq20}
\end{align}
where the notation $\mathcal{D}[\tilde{f}^{(m)}\jet_q^{(\perp)}]$ has been defined by~\footnote{For further details, readers who are interested can refer to App.~\ref{sec:appb}.}
\begin{align}
\mathcal{D}[\tilde{f}^{(m)}\jet_q]=&\sum_q e_q^2H(Q,\mu)S({\bm b}^2,\mu,\nu)\jet_q({\bm b}^2,\mu,\zeta/\nu^2) b^{m}{M^m}\tilde{f}^{(m)}_q(x,{\bm b}^2,\mu,\zeta/\nu^2)\,,\\
\mathcal{D}[\tilde{f}^{(m)}\jet_q^{\perp}]=&\sum_q e_q^2H(Q,\mu)S({\bm b}^2,\mu,\nu)\jet_q^\perp({\bm b}^2,\mu,\zeta/\nu^2)\frac{b^{m+1}}{2}{M^m}{(-M_h)}\tilde{f}^{(m)}_q(x,{\bm b}^2,\mu,\zeta/\nu^2) \,.
\end{align}
Using the new PEEC observable defined in \cref{eq:EECDISq20}, one can get access to probing 7 leading-twist TMD PDFs with $q_*$, which is constructed as a high-precision probe in the EIC lab frame. Note that the reason $\tilde{h}_{1L}^{\perp(1)}$ is not present in \cref{eq:EECDISq20} is that its coefficient $\sin(2\phi_h)$ has an odd symmetry under the transformation $\phi_h\rightarrow \pi-\phi_h$ thus the contribution vanishes.
\end{itemize}

\subsection{Properties of Collins-type EEC jet functions}\label{sec:jetfunc}
In this section, we derive the intricate behavior of the EEC jet functions using the operator product expansion (OPE). Drawing inspiration from the seminal work of~\cite{Moult:2018jzp}, we undertake a rigorous analysis of the unpolarized EEC jet function, revealing its close connection with the matching coefficients in the OPE region. Moreover, we extend this analysis to the Collins-type EEC jet function, as defined in \cref{eq:Collinsjet}, demonstrating that it becomes null in the OPE region upon neglecting the off-diagonal matching terms. Finally, we conclude the section by discussing the application of PEEC for a subset of hadrons. %Our findings lend crucial insights into the underlying structure of these jet functions and pave the way for future explorations of QCD dynamics in high-energy collisions. 
%By studying the EEC of identified hadrons, we can obtain important information about the fragmentation process and the properties of the produced hadrons, such as their transverse momentum and spin. 

\subsubsection{Operator product expansion region}
One of the important and difficult challenges in the TMD physics involve disentangling various perturbative and non-perturbative parts in the factorization theorem. For instance, at the leading power the unpolarized TMD FF $D_{1,h/q}(z,{k}_\perp^2,\mu)$ can be parametrized in the $b$-space as 
\begin{align}
\label{eq:Dparam}
D_{1,h/q}(z,\bm{b}^2,\mu,\zeta_f)=&\frac{1}{z^{2-2\epsilon}}\sum_j\int_{z}^{1} \frac{dx}{x} \textcolor{blue}{C_{j\leftarrow {q}}\left(\frac{z}{x}, {\bm b}^2,\mu_{b_*},\zeta_i \right)} \textcolor{red}{D_{1,h/j}\left(x, \mu_{b_*}\right)}\nnu
&\times e^{-\textcolor{blue}{S_{\rm pert}(\mu,\mu_{b_*})}-\textcolor{red}{S_{\rm NP}(b,Q_0,\zeta_f)}}\left(\sqrt{\frac{\zeta_f}{\zeta_i}}\right)^{\kappa\left(b, \mu_{b_*}\right)}\,,
\end{align}
where $S^i_{\rm pert}$ is the perturbative Sudakov factor describing the evolution between the scale $\mu_{b_*}$ and $\mu$, and $S^i_{\rm NP}$ is the non-perturbative (NP) Sudakov factor describing the contribution from the intrinsic transverse distribution of the partons and the non-perturbative evolution part from the soft rapidity anomalous dimension. Also, $C_{j\leftarrow {i}}\left(\frac{z}{x}, {\bm b} \right)$ is the perturbative matching coefficients and $D_{1,h/j}\left(x, \mu_{b_*}\right)$ describes the non-perturbative collinear fragmentation functions. For convenience, we color-coded various perturbative and non-perturbative components of the unpolarized TMD FF $D_{1,h/q}(z,{k}_\perp^2,\mu)$ in blue and red, respectively, in the Eq.\ \cref{eq:Dparam}. %Also, as this paper will demonstrate, we find that in the operator product expansion (OPE) region discussed (i.e. $b \ll 1/\Lambda_{\rm QCD}$), the Collins-type EEC jet function $\jet_{q}^{\perp}$ vanishes due to a sum rule for the twist-$3$ fragmentation function called Sch\"{a}fer-Teryaev (ST) sum rule. 

In order to elucidate the OPE of the EEC jet functions, we first introduce the concept of ``subtracted" transverse momentum dependent fragmentation functions (TMD FFs). This serves as a vital starting point for our analysis, enabling us to uncover the intricate interplay between the OPE and the azimuthal angle dependence of the EEC jet functions.
\begin{align}
\label{eq:subTMD FFs}
\tilde{F}^{\rm sub}(z,{\bm b}^2,\mu,\zeta)=\tilde{F}(z,{\bm b}^2,\mu,\zeta/\nu^2)\sqrt{S({\bm b}^2,\mu,\nu)}\,,
\end{align}
which absorbs the square-root of the soft-function. The ``subtracted'' TMD FFs is then insensitive to the rapidity regulator, $\nu$. The subtracted TMD FFs are then parametrized as~\cite{Collins:2011zzd,Aybat:2011zv,Prokudin:2015ysa,Kang:2015msa} 
\begin{align}
\label{eq:Dsub}
\tilde{D}^{\rm sub}_{1,h/q}(z,{\bm b}^2,\mu,\zeta_f)=&\,\tilde{D}^{\rm sub}_{1,h/q}(z,\mu_{b_*},\zeta_i) e^{-S_{\rm pert}(\mu,\mu_{b_*}) - S_{\rm NP}^{D_1}(b,Q_0,\zeta_f)}\left(\sqrt{\frac{\zeta_f}{\zeta_i}}\right)^{\kappa\left(b, \mu_{b_*}\right)}\,,\\
\tilde{H}_{1,h/{q}}^{\perp\,\alpha,{\rm sub}}(z,{\bm b}^2,\mu,\zeta_f)=&\,\left(-\frac{i{b}^\alpha}{2z}\right)\tilde{H}_{1,h/{q}}^{\perp,\,{\rm sub}}(z,\mu_{b_*},\zeta_i)e^{-S_{\rm pert}(\mu,\mu_{b_*}) - S_{\rm NP}^{H^{\perp}_{1}}(b,Q_0,\zeta_f)}\left(\sqrt{\frac{\zeta_f}{\zeta_i}}\right)^{\kappa\left(b, \mu_{b_*}\right)}\,,
\label{eq:Hsub}
\end{align}
Note that the non-perturbative Sudakov factors $S_{\rm NP}^{F}$ in general depends on the hadron flavors and TMD FFs. Also, we follow the $b^*$ prescription, which ensures $\mu_{b_*} \gg \Lambda_{\rm QCD}$. The OPE of the subtracted unpolarized and Collins TMD FFs then give at $\mu_{b_*}$\ \cite{Koike:2006fn,Yuan:2009dw,Bacchetta:2013pqa,Echevarria:2014rua,Kang:2015msa} 
\begin{align}
\label{eq:OPEunp}%\overset{\rm{OPE}}{=}
\tilde{D}^{\rm sub}_{1,h/q}(z,\mu_{b_*},\zeta_i)=&\left[C_{j\leftarrow q}\otimes D_{1,h/{j}} \right]\left(z,\mu_{b_*},\zeta_i\right) + \mathcal{O}(\bm{b}^2\Lambda_{\rm QCD}^2),\\
\tilde{H}_{1,h/{q}}^{\perp,\,{\rm sub}}(z,\mu_{b_*},\zeta_i)=&\left[\delta C_{j\leftarrow q}^{\rm Collins}\otimes \hat{H}_{1,h/j}^{\perp(3)} + A_{j\leftarrow q}\tilde{\otimes} \hat{H}_{F,h/j}\right]\left(z,\mu_{b_*},\zeta_i\right)+ \mathcal{O}(\bm{b}^2\Lambda_{\rm QCD}^2)\,,
\label{eq:OPECollins}
\end{align}
where the usual convolution $\otimes$ is given by
\begin{align}
\left[C_{j\leftarrow {q}}\otimes F_{h/j}\right]\left(z,\mu,\zeta_i\right) = \int_{z}^{1} \frac{dx}{x} C_{j\leftarrow {q}}\left(\frac{z}{x}, \mu,\zeta_i \right) F_{h/j}\left(x, \mu\right)\,,
\end{align}
and the convolution $\tilde{\otimes}$ is a double convolution 
\begin{align}
\left[A_{j\leftarrow q}\tilde{\otimes} \hat{H}_{F,h/j}\right]\left(z,\mu,\zeta_i\right) = \int_{z}^{1}\frac{dx}{x}\, \int\frac{dz_1}{z_1^2}\,{\rm PV}\left(\frac{1}{\frac{1}{x}-\frac{1}{z_1}}\right) A_{j\leftarrow {q}}\left(\frac{z}{x}, z_1,\mu,\zeta_i \right) \hat{H}_{F,h/j}\left(x,z_1, \mu\right)\,,\label{eq:a_hf}
\end{align}
where $A_{q'\leftarrow q}\left(z, z_1,\mu_b \right) \sim\mathcal{O}(\alpha_s)$, ${\rm PV}$ represents principle value, and \cref{eq:a_hf} comes from the two-variable twist-3 fragmentation function\ \cite{Yuan:2009dw}  $\hat{H}_{F,h/q}(z_1,z_2,\mu)$ that appears in the collinear factorization region in $b \ll 1/\Lambda_{\rm QCD}$. Such two-variable dependence arise from different longitudinal momentum flow on the amplitude and conjugate amplitude side.

Here, $D_{1,h/j}(z,\mu_{b_*})$ in Eq.\ \cref{eq:OPEunp} describes the unpolarized collinear fragmentation functions. The one-variable twist-3 fragmentation function $\hat{H}_{1,h/j}^{\perp (3)}(z,\mu_{b_*})$ is related to the moments of the Collins TMD FF as~\cite{Kang:2015msa}
\begin{align}
\hat{H}_{1,h/q}^{\perp (3)}(z,\mu_{b_*}) = \int d^2\bm{k}_\perp \frac{|\bm{k}_\perp^2|}{M_h}H_{1,h/q}^{\perp}(z,{\bm k}_{\perp}^2,\mu_{b_*},\zeta)\,,
\end{align}
where ${\bm k}_\perp$ is the transverse momentum of the hadron with respect to the momentum of the fragmenting quark. And as shown in~\cite{Kang:2015msa}, the Collins function $H_1^\perp(z,{\bm k}_{\perp}^2)$ and moment $\hat{H}_{1,h/q}^{\perp (3)}(z,\mu_{b_*})$ here are related to the first moment of Collins function defined in Trento convention~\cite{Bacchetta:2004jz} by
\begin{align}
\hat{H}_{1,h/q}^{\perp (3)}(z,\mu_{b_*})&=-2zM_hH_{1,h/q}^{\perp(1)}(z,{\bm k}_{\perp}^2)=-2zM_h\int d^2\bm{k}_\perp \frac{|\bm{k}_\perp^2|}{2z^2M_h^2}H_{1,h/q}^{\perp}(z,{\bm k}_{\perp}^2)\,.
\end{align}

Matching of the TMD FFs given in Eqs.\ \cref{eq:OPEunp} and \cref{eq:OPECollins} can be derived by comparing the expressions of the TMD and collinear factorizations in the overlap region, $\Lambda_{\rm QCD} \ll 1/b \ll Q$. To one-loop, these matching coefficients of Eqs.\ \cref{eq:OPEunp} and\ \cref{eq:OPECollins} are given by
\begin{align}
C_{q^{\prime} \leftarrow q}\left(z, \mu_{b},Q^2\right)=&\delta_{q q^{\prime}}\left[\delta\left(1-z\right)+\frac{\alpha_{s}}{\pi}\left(-C_{F} \frac{\pi^{2}}{24} \delta\left(1-z\right)+\frac{C_{F}}{2}\left(1-z\right)+P_{q \leftarrow q}\left(z\right) \ln z\right)\right]\,,\\
\delta C_{q'\leftarrow q}^{\rm Collins}\left(z, \mu_{b},Q^2\right)=&\delta_{qq'}\left[\delta(1-z)+\frac{\alpha_s}{\pi}\hat{P}^c_{q\leftarrow q}(z)\ln\left(z\right)\right]\,.\label{eq:collins_c}
\end{align}
where the splitting functions $P_{q \leftarrow q}(z)$ and $\hat{P}_{q \leftarrow q}^{c}(z)$ is given as
\begin{align}
P_{q \leftarrow q}(z)&=C_{F}\left[\frac{1+z^{2}}{(1-z)_{+}}+\frac{3}{2} \delta(1-z)\right]\,,\\
\hat{P}_{q \leftarrow q}^{c}(z)&=C_{F}\left[\frac{2 z}{(1-z)_{+}}+\frac{3}{2} \delta(1-z)\right]\,.\label{eq:collins_pqq}
\end{align}
The matching coefficients from (anti-)quark to gluon or different flavored (anti-)quark are zero at $1$-loop for the Collins TMD FFs. And other matching coefficients for the unpolarized TMD FFs have been provided in~\cite{Kang:2015msa}. 

The collinear functions in the matching obey the sum rules \cite{Schafer:1999kn,Meissner:2010cc,Metz:2016swz}
\begin{align}
\sum_{h} \int_0^1 dz\,z\,D_{1,h/j}\left(z, \mu\right) = 1\,,\label{eq:unpsum}\\
\sum_{h}\int_0^1 dz\, \hat{H}_{1,h/q}^{\perp(3)}\left(z,\mu\right) = 0\,.
\label{eq:STsum}
\end{align}
The first sum rule is just the longitudinal momentum conservation, i.e. sum over longitudinal momentum fraction carried by the hadron $h$ is $1$. The second sum rule for the twist-$3$ fragmentation function is called Sch\"{a}fer-Teryaev (ST) sum rule, which is related to the transverse momentum conservation of the Collins TMD FF\ \cite{Schafer:1999kn}. That is, transverse momentum carried by the final hadron must sum to $0$ as the fragmenting parton has a $0$ transverse momentum.\footnote{It was noted in \cite{Meissner:2010cc,Metz:2016swz} that this intuitive argument about momentum conservation does not necessarily hold in general. In particular, ST sum rule does not hold for many other types of TMD fragmentation functions, including Collins TMD FF for the gluon. Thus, Eq.\ \cref{eq:STsum} only hold for (anti-)quarks.}

We now define ``subtracted'' EEC jet function analogous to the ``subtracted'' TMD functions as given in Eq.\ \cref{eq:subTMD FFs} as
\begin{align}
\label{eq:subEECJ}
\jet_q^{\rm sub}({\bm b}^2,\mu,\zeta)&=\jet_q({\bm b}^2,\mu,\zeta/\nu^2)\sqrt{S({\bm b}^2,\mu,\nu)}\nonumber\\
&=\sum_{h}\int_0^1dz\,z\,\tilde{D}^{\rm sub}_{1,h/q}(z,{\bm b}^2,\mu,\zeta)\,,\\
\left(-\frac{i{\bm b}^\alpha}{2}\right)\jet_q^{\perp{\rm sub}}({\bm b}^2,\mu,\zeta)&= \left(-\frac{i{\bm b}^\alpha}{2}\right)\jet_q^\perp({\bm b}^2,\mu,\zeta/\nu^2)\sqrt{S({\bm b}^2,\mu,\nu)}\nonumber\\
&=\sum_{h}\int_0^1dz\,z\, \tilde{H}_{1,h/q}^{\perp\,\alpha,{\rm sub}}(z,{\bm b}^2,\mu,\zeta)\,,
\label{eq:subEECJperp}
\end{align}
where the subtracted TMD FFs are parametrized as in the Eqs.\ \cref{eq:Dsub} and \cref{eq:Hsub}.

\iffalse
\begin{align}
\label{eq:unpjet}
\jet_q({\bm b},\mu,\zeta/\nu^2)\equiv&\sum_{h}\int_0^1dz\,z\,\tilde{D}_{1,h/q}(z,{\bm b}^2,\mu,\zeta/\nu^2)\,,\\
\left(-\frac{i{\bm b}^\alpha}{2}\right)\jet_q^\perp({\bm b},\mu,\zeta/\nu^2)\equiv&\sum_{h}\int_0^1dz\,z\, \tilde{H}_{1,h/q}^{\perp\,\alpha}(z,{\bm b}^2,\mu,\zeta/\nu^2)
\label{eq:Collinsjet}\,.
\end{align}


Since EEC jet functions are built from TMD FFs, we follow the $b^*$ prescription and parametrize them as
\begin{align}
\label{eq:SubEECJdecomp}
\jet_q^{\rm sub}(\bm b,\mu,\zeta) &= \jet_q^{\rm sub}(\bm b,\mu_{b_*},\zeta)\exp[-S_{\rm pert}(\mu,\mu_{b_*}) - S_{\rm NP}^{J}(b,Q_0,\zeta)]\,,\\
\jet_q^{\perp\rm sub}(\bm b,\mu,\zeta) &= \jet_q^{\perp\rm sub}(\bm b,\mu_{b_*},\zeta)\exp[-S_{\rm pert}(\mu,\mu_{b_*}) - S_{\rm NP}^{J_\perp}(b,Q_0,\zeta)]\,,
\label{eq:SubEECJperpdecomp}
\end{align}
\textcolor{red}{(Yiannis's paper actually has NP parameterization independent of $\mu_{b_*}$ or $\zeta$ scale. Is this consistent with what we did here?)}
where the EEC jet functions at $\mu_{b_*}$ scale is in the OPE region. Note that as EEC jet functions are built out of TMD FFs of different final hadron flavors, the factorization of the EEC jet function at $\mu_{b_*}$ and NP Sudakov factor in the form of the Eq.\ \cref{eq:SubEECJdecomp} is only valid to the accuracy we can ignore the difference of NP Sudakov factors between different hadron flavors. \textcolor{red}{(how much is this justified?)}
\fi

In\ \cite{Moult:2018jzp}, interesting observation was made about simplification of unpolarized EEC jet function when the non-perturbative Sudakov effects are ignored, i.e. $\frac{1}{b} \gg \Lambda_{\rm QCD}$. That is, if we take $S_{\rm NP}^{D_1}=0$, then using the sum rule in Eq.\ \cref{eq:unpsum}, we arrive at
%Now in the OPE region, the sum rule in Eq.\ \cref{eq:unpsum} simplifies the unpolarized EEC jet function given in Eq.\ \cref{eq:unpjet} as
\begin{align}
&\jet_q^{\rm sub}({\bm b}^2,\mu,\zeta)=\sum_{h}\int_0^1 z dz\, \tilde{D}^{\rm sub}_{1,h/q}(z,{\bm b}^2,\mu,\zeta)\nnu
=& \sum_{h}\int_0^1 z{dz}  \int_{z}^1 \frac{dx}{x}\, C_{j\leftarrow q}\left(\frac{z}{x}, \mu_{b_*},\zeta \right) D_{1,h/j}\left(x, \mu_{b_*}\right) e^{-S_{\rm pert}(\mu,\mu_{b_*})} \nnu
=& \int_0^1 \tau{d\tau}\,{C}_{j\leftarrow q}(\tau,\mu_{b_*},\zeta)\left[\sum_{h} \int_0^1 {dx}\,x\,D_{1,h/j}\left(x, \mu_{b_*}\right)\right]e^{-S_{\rm pert}(\mu,\mu_{b_*})}   \nnu
=& \int_0^1 \tau{d\tau}\,{C}_{j\leftarrow q}(\tau,\mu_{b_*},\zeta)e^{-S_{\rm pert}(\mu,\mu_{b_*})} \,, \label{eq:sumunp}
\end{align}
and thus reproduce the result from\ \cite{Moult:2018jzp} that unpolarized EEC jet function is purely perturbative object in the OPE region, given by the matching coefficients $C_{j\leftarrow q}$ alone.

On the other hand, the Collins-type EEC jet function can be simplified analogously using the ST sum rule described in \cref{eq:STsum}, with the twist-3 function contribution neglected. By making this simplification, we can achieve the same level of accuracy as in the previous scenario. In the OPE region, the Collins-type EEC jet functions can be further simplified as follows:
%This means, to the accuracy we can ignore gluon components in $j=g$ (\textcolor{red}{which is always true at $1$-loop. is it true for higher?}) of $\delta C_{j\leftarrow q}^{\rm Collins}$ and ignore the off-diagonal term $A_{j\leftarrow q}$ \textcolor{red}{(write something about the accuracy to which these can be ignored)}. With this in mind, to such accuracy, Collins-type EEC jet functions in the OPE region can also be simplified as 
\begin{eqnarray}
%%%%%%%%%%%%%%%%%%%%% Collins EEC jet function %%%%%%%%%%%%%%%%%%%%%
&&\left(-\frac{i{\bm b}^\alpha}{2}\right)\jet_q^{\perp{\rm sub}}({\bm b}^2,\mu,\zeta)=\sum_{h}\int_0^1dz z \tilde{H}_{1,h/q}^{\perp\,\alpha,{\rm sub}}(z,{\bm b}^2,\mu,\zeta)\nnu
&{=}&\left(-\frac{i{\bm b}^\alpha}{2}\right)\sum_{h}\int_0^1dz\int_{z}^1 \frac{dx}{x}\, \delta C_{q\leftarrow q}^{\rm Collins}(\frac{z}{x},\mu_{b_*},\zeta) \hat{H}_{1,h/q}^{\perp(3)}\left(x,\mu_{b_*}\right)e^{-S_{\rm pert}(\mu,\mu_{b_*})}\nnu
&=&\left(-\frac{i{\bm b}^\alpha}{2}\right)\int_0^1 d\tau \delta C_{q\leftarrow q}^{\rm Collins}(\tau,\mu_{b_*},\zeta) \left[\sum_{h}\int_0^1 dx\,\hat{H}_{1,h/q}^{\perp(3)}\left(x,\mu_{b_*}\right)\right]e^{-S_{\rm pert}(\mu,\mu_{b_*})}\nnu
%=&\left(-\frac{i{\bm b}^\alpha}{2}\right)A\int_0^1 d\tau \delta C_{q\leftarrow q}^{\rm Collins}(\tau,\mu_{b_*}) \exp[-S_{\rm pert}(\mu,\mu_{b_*})]\nnu
&=&\,0\,,
\label{eq:sumperp}
\end{eqnarray}
which demonstrates that the Collins-like EEC jet function $\jet_q^\perp$ becomes $0$ in the OPE region. Both of these results only hold true when non-perturative effects can be ignored. The Collins-like EEC jet function is especially interesting as any non-zero contribution arises from the purely non-perturbative contribution.

%---------

\subsubsection{Collins-type EEC with subsets of hadrons}
\label{subsec:EECsubset}
In this section, we explore a modified version of an EEC-like observable, which focuses on a subset of hadrons. The motivation behind this adaptation is multifaceted. Throughout our subsequent analysis, we denote this subset of hadron flavors as $\mathbb{S}$. By considering the $\tau,\ \phi$-differential and $z$-weighed cross section, while summing over this subset $\mathbb{S}$, we arrive at our proposed modified observable.
%then we simply replace the EEC jet functions in the above derivations with the EEC subset jet functions defined as
\begin{align}
\label{eq:subJ}
\jet_{q/\mathbb{S}}^{\rm sub}({\bm b}^2,\mu,\zeta)\equiv&\sum_{h \in \mathbb{S}}\int_0^1dz z\tilde{D}_{1,h/q}^{\rm sub}(z,{\bm b}^2,\mu,\zeta)\,,\\
\left(-\frac{i{\bm b}^\alpha}{2}\right)\jet_{q/\mathbb{S}}^{\perp{\rm sub}}({\bm b}^2,\mu,\zeta)\equiv&\sum_{h \in \mathbb{S}}\int_0^1dz z \tilde{H}_{1,h/q}^{\perp\,\alpha,{\rm sub}}(z,{\bm b}^2,\mu,\zeta)\,.
\label{eq:subJperp}
\end{align}

In the OPE region, these subset jet functions can then be matched to the collinear functions as%\overset{\rm OPE}{=}
\begin{align}
\jet_{q/\mathbb{S}}^{\rm sub}({\bm b}^2,\mu,\zeta)=& \sum_j F_{j\rightarrow \mathbb{S}} \int_0^1 \tau{d\tau}\,{C}_{j\leftarrow q}(\tau,\mu_{b_*})e^{-S_{\rm pert}(\mu,\mu_{b_*})}\,,\label{eq:subJOPE}\\
%\left(-\frac{i{\bm b}^\alpha}{2}\right)
\jet_{q/\mathbb{S}}^{\perp{\rm sub}}({\bm b}^2,\mu,\zeta)=&\sum_j F^{\perp}_{j\rightarrow \mathbb{S}} \int_0^1 d\tau \delta C_{j\leftarrow q}^{\rm Collins}(\tau,\mu_{b_*})e^{-S_{\rm pert}(\mu,\mu_{b_*})}\,.\label{eq:subJperpOPE}
\end{align}
Physically, $F_{j\rightarrow \mathbb{S}}$ is the average fraction of longitudinal momentum of parton $j$ carried by the subset $\mathbb{S}$ of hadrons~\cite{Li:2021txc}, which is thus between $0$ and $1$. On the other hand, $F^{\perp}_{j\rightarrow \mathbb{S}}$ is related to the average transverse momentum carried by the subset $\mathbb{S}$ of the hadrons, which is thus able to take any real value. And these two functions are defined by
\begin{align}
F_{j\rightarrow \mathbb{S}}&=\sum_{h\in \mathbb{S}} \int_0^1 {dz}\,z\,D_{1,h/j}\left(z, \mu_{b_*}\right)\,,\\
F^{\perp}_{j\rightarrow \mathbb{S}}&=\sum_{h\in\mathbb{S}}\int_0^1 dz\,\hat{H}_{1,h/j}^{\perp(3)}\left(z,\mu_{b_*}\right)\,.
\end{align}
It is worth noting that since $\delta C_{j\leftarrow q}^{\rm Collins}$ is only non-zero when $j=q$, the only relevant term is $F^{\perp}_{q\rightarrow \mathbb{S}}$. Additionally, as demonstrated in \cref{eq:unpsum} and~\cref{eq:STsum}, when $\mathbb{S} =$ {\textit{all hadrons}}, one will obtain $F_{j\rightarrow \mathbb{S}}=1$ and $F^{\perp}_{j\rightarrow \mathbb{S}}=0$. %These fractional values are no longer constrained by the sum rule, and is thus non-perturbative, albeit only a single number. 

One can easily find that in addition to its dependence on the initiating parton $j$, the EEC jet functions defined in \cref{eq:subJOPE} and~\cref{eq:subJperpOPE} are also influenced by the subset of hadrons $\mathbb{S}$, rendering it a non-perturbative function similar to fragmentation functions. Despite this, we can leverage the OPE to analyze the EEC jet function with a subset $\mathbb{S}$, much like we do with the EEC jet functions. Specifically, at leading order, we can match the TMD FFs to the collinear FFs to gain further insight into this important aspect of jet physics. Like pointed out in~\cite{Li:2021txc}, considering PEEC with subsets of hadrons can be interesting from the point of view of considering a set of all charged particles $\mathbb{S} = \mathbb{C}$ or a set of a single hadron type $\mathbb{S} = h$. From the perspective of Collins-type EEC jet function, we are motivated to consider the so-called {\textit favored} and {\textit unfavored} subset as well\ \cite{Vogelsang:2005cs,Kang:2015msa,Metz:2016swz}. Therefore, it is also interesting to consider $\mathbb{S} = \{\pi^+\}, \{\pi^-\},\{\pi^0\}, \{\pi^+,\pi^-\},\{\pi^+,\pi^-,\pi^0\}$ for Collins-type EEC in phenomenology.%\footnote{Note that using isospin symmetry, $D_{1,\pi^0/q} \approx \frac{1}{2}(D_{1,\pi^+/q} +D_{1,\pi^-/q} ) \approx \frac{1}{2}(D_{1,{\textit fav}} +D_{1,{\textit unfav}} )$.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
The {\textit favored} fragmentation functions are pion fragmentation functions of a valence parton ($u$ or $d$) (e.g. $D_{1,\pi^+/u}$ or $H_{1,\pi^+/u}^\perp$), whereas the {\textit unfavored} fragmentation fuctions are pion fragmentation functions of $u$ or $d$ that is not a valence parton (e.g. $D_{1,\pi^-/u}$ or $H_{1,\pi^-/u}^\perp$). Charge conjugation and isospin symmetries (which are only broken by electromagnetic effects and is numerically small) then make all the favored and unfavored fragmentation functions to be identified. Assuming light partons to pions dominate the fragmentation process, we then expect 
\begin{align}
0 = F^{\perp}_{q\rightarrow \mathbb{S} = {\textit{all hadrons}}} \appropto F^{\perp}_{{\textit fav}} + F^{\perp}_{{\textit unfav}}\,,
\end{align}
or 
\begin{align}
\label{eq:JfavJunfav}
J^{\perp}_{{\textit fav}} \approx -J^{\perp}_{{\textit unfav}}\,.
\end{align}
Therefore, it is also interesting to consider $\mathbb{S} = \{\pi^+\}, \{\pi^-\},\{\pi^0\}, \{\pi^+,\pi^-\},\{\pi^+,\pi^-,\pi^0\}$ for Collins-type EEC.\footnote{Note that using isospin symmetry, $D_{1,\pi^0/q} \approx \frac{1}{2}(D_{1,\pi^+/q} +D_{1,\pi^-/q} ) \approx \frac{1}{2}(D_{1,{\textit fav}} +D_{1,{\textit unfav}} )$.}

For instance, if we take $\mathbb{S} = \{\pi^+,\pi^-\}$,
then azimuthal-dependent EEC for $e^+e^-$ and DIS, respectively, are roughly
\begin{align}
{\rm EEC}_{e^+e^-,\perp}^{\{\pi^+,\pi^-\}} \sim& \sum_q J_{q/\{\pi^+,\pi^-\}}^\perp \otimes J_{\bar{q}/\{\pi^+,\pi^-\}}^\perp \nnu
\sim & (J_{\textit fav}^\perp+J_{\textit unfav}^\perp) \otimes (J_{\textit fav}^\perp+J_{\textit unfav}^\perp)
\overset{\rm OPE}{\approx} 0
\end{align}
and
\begin{align}
\label{eq:DIS_piplus}
{\rm EEC}_{\rm DIS,\perp}^{\{\pi^+,\pi^-\}} \sim& \sum_q h_1^q \otimes J_{q/\{\pi^+,\pi^-\}}^\perp\nnu
\sim& \sum_q h_1^q \otimes (J_{\textit fav}^\perp+J_{\textit unfav}^\perp)\overset{\rm OPE}{\approx} 0\,,
\end{align}
where $q$ can be quark or anti-quark in the sum for ${\rm EEC}_{\rm DIS}$. 

As noted here, we expect the EEC values to be very close to $0$ in the OPE region and thus any non-vanishing values are expected to be primarily due to the non-perturbative effects away from the OPE region. Also note that the DIS case is expected to be small due to $h_1^u$ and $h_1^d$ being opposite sign, and experiencing cancellation from the PDF side as well.

On the other hand, if we take $\mathbb{S} = \{\pi^+\}$, then azimuthal dependent EEC for $e^+e^-$ and DIS, respectively, are
\begin{align}
{\rm EEC}_{e^+e^-,\perp}^{\{\pi^+\}} \sim& \sum_q J_{q/\pi^+}^\perp \otimes J_{\bar{q}/\pi^+}^\perp \nnu
\sim& J_{\textit fav}^\perp \otimes J_{\textit unfav}^\perp
\end{align}
and
\begin{align}
\label{eq:EECDIS}
{\rm EEC}_{\rm DIS,\perp}^{\{\pi^+\}} \sim& \sum_q h_1^q \otimes J_{q/\pi^+}^\perp \nnu
\sim& \sum_q h_1^q \otimes J_{\textit fav}^\perp+ h_1^{\bar{q}} \otimes J_{\textit unfav}^\perp  \,,
\end{align}
where we no longer have a sum $J_{\textit fav}^\perp+J_{\textit unfav}^\perp$ for each terms. Therefore, EEC values are expected to be larger when only $\pi^+$ or $\pi^-$ is considered by themselves. As mentioned above, note that ${\rm EEC}_{\rm DIS}^{\{\pi^+\}}$ is suspected to be small due to $h_1^u$ and $h_1^d$ being opposite sign. We will investigate these expectations below in the next phenomenology section.

Of course, which hadron is `favored' or which is `unfavored' depends entirely on the (anti-)quark flavor $q$. For instance, $\pi^+$ fragmentation function would be `favored' for $u$ quark, but disfavored for $\bar{u}$ anti-quark. 

Therefore, it is also interesting to consider $\mathbb{S} = \{{\textit fav}\}, \{{\textit unfav}\}, \{{\textit fav},{\textit unfav}\}$ for the Collins-type EEC, which we will below.

In the above section, we have found that $\jet_q^\perp(b,\mu,\nu) = 0 $ in the OPE region, implying that any nonzero value of Collins EEC jet function are purely non-perturbative, which is interesting. Furthermore, although the asymmetry may be very tiny, one can further decompose $\jet_q^\perp$ according to different hadron flavors as
\begin{align}
\jet_q^\perp({\bm b},\mu,\nu)  = \sum_J\jet_q^{\perp,h_{J}}(\bm b,\mu,\nu) \,,
\end{align}
where
\begin{align}
\left(-\frac{i{\bm b}^\alpha}{2}\right)\jet_q^{\perp,h_{J}}(\bm b,\mu,\nu)=&\sum_{h_{J,i}}\int_0^1dz z \tilde{H}_{1,h_{J,i}/q}^{\perp\,\alpha}(z,{\bm b}^2,\mu,\zeta/\nu^2)
\end{align}
is defined by the sum over $J$-th group of hadrons. That is, the complete set of hadrons $h_i$ is separated into $N$ subsets of hadrons as
\begin{align}
\{h_{i}\} = \{\{h_{1,i}\},\{h_{2,i}\},\cdots,\{h_{N,i}\}\}\,.
\end{align}

This will naturally decompose the EEC as
With the decomposition of the EEC jet function initiated by both unpolarized and transversely polarized quarks with unpolarized hadrons observed in the final state, the $z_i,\ z_j$-weighted differential cross section for $e^+e^-$ annihilation can be decomposed into a sum of all hadron subsets,
\begin{align}
{\rm EEC}(\tau,\phi) =\frac{d\Sigma}{d\tau d\phi}=\frac{1}{2}\sum_{i,j}\int dz_idz_j\frac{d\sigma}{dz_idz_jd\tau d\phi}&=\frac{1}{2}\sum_J\sum_{h_{J,i},h_{J,j}}\int dz_idz_j\frac{d\sigma}{dz_idz_jd\tau d\phi}=\frac{1}{2}\sum_J\frac{d\Sigma^{h_J}}{d\tau}\,.
\end{align}
And similarly for the $z$-weighted differential cross section of SIDIS process,
\begin{align}
{\rm EEC}_{\rm SIDIS}(\tau) =\frac{d\Sigma_{\rm SIDIS}}{d\tau}=\sum_i\int dz_iz_i\frac{d\sigma_{\rm SIDIS}}{dz_id\tau}&=\sum_J\sum_{h_{J,i}}\int dz_iz_i\frac{d\sigma_{\rm SIDIS}}{dz_id\tau}=\sum_J\frac{d\Sigma^{h_J}_{\rm SIDIS}}{d\tau}\,.
\end{align}
The individual contribution from the decomposition leads to a more significant measurement than that of a complete hadrons set as we will show in the following section. 
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Phenomenology}\label{sec:pheno}
The present study focuses on the Collins azimuthal asymmetry in $e^+e^-$ annihilation with subsets of hadrons, namely $\mathbb{S}={\pi^+,\ \pi^-}$, ${\pi^+}$, and ${\pi^-}$, as the hadron component of the EEC jet using EIC kinematics. Furthermore, we provide predictions for both the Collins and Sivers asymmetry in the Breit frame for the DIS process. It is worth noting that the EEC jet function is also a powerful tool for probing the internal structure of nucleons in the lab frame, as evidenced by our example of an azimuthal asymmetry related to the worm-gear TMD PDFs and EEC jet functions.

\subsubsection{The Collins azimuthal asymmetry in $e^+e^-$ annihilation}\label{sec:phenoee}
With the EEC derived for $e^+e^-$ annihilation in the back-to-back region in terms of the EEC jet functions in Eq.\ \cref{eq:epemEEC}, we now carry out phenomenological study of the asymmetry associated with PEEC. To achieve this, we first rewrite the Eq.\ \cref{eq:epemEEC} as
\begin{align}
\frac{d\Sigma_{e^+e^-}}{d\tau d\phi}=&\frac{2\pi N_c\alpha_{\rm em}^2}{3Q^2}\sum_q e_q^2\int d{\bm q}_T^2\,\delta(\tau  - \frac{{\bm q}_T^2}{Q^2})\, Z_{uu}\,(1+ \cos 2\phi\, \frac{Z_{\rm collins}}{Z_{uu}})\nonumber\\
\equiv&\frac{2\pi N_c\alpha_{\rm em}^2}{3Q^2}\sum_q e_q^2\, Z_{uu}\,\left(1+ \cos 2\phi\, A_{e^+e^-}(\tau Q^2)\right)\,,
\end{align}
where
\begin{align}
%A_{e^+e^-}(\tau Q^2)\equiv &\frac{Z_{\rm collins}}{Z_{uu}} = 1+\cos 2{\phi}A_{e^+e^-}(\bm{q}_T^2)\,,\\
Z_{uu}=&\int\frac{bdb}{2\pi}J_0(bq_T)\jet^{\rm sub}_{q}({\bm b}^2,\mu,\zeta/\nu^2)\jet^{\rm sub}_{\bar{q}}({\bm b}^2,\mu,\zeta/\nu^2)\,,\label{zuu}\\
Z_{\rm collins}=&\int\frac{bdb}{2\pi}\frac{b^2}{8}J_2(bq_T) \jet_{q}^{\perp{\rm sub}}({\bm b}^2,\mu,\zeta/\nu^2)\jet_{\bar{q}}^{\perp{\rm sub}}({\bm b}^2,\mu,\zeta/\nu^2)\,.\label{zcol}
\end{align}
Recall that subtracted EEC jet functions were defined in Eqs.\ \cref{eq:subEECJ} and\ \cref{eq:subEECJperp}. As pions are the primary measurements available for the Collins-type asymmetry, we now study the ratio $A_{ee}^{\mathbb{S}\times\mathbb{S}}(\bm{q}_T^2) =A_{ee}^{\mathbb{S}\times\mathbb{S}}(\tau Q^2) $ with different subsets $\mathbb{S}\times\mathbb{S}$ of produced pion pairs. This amounts to simply using EEC jet functions with a subset in Eqs.\ \cref{eq:subJ} and\ \cref{eq:subJperp} defined in terms of TMD FFs of the pions.
\iffalse
We now discuss the parametrization of the EEC subset jet functions. From Eqs.\ \cref{eq:SubEECJdecomp}-\cref{eq:SubEECJperpdecomp} and\ \cref{eq:subJOPE}-\cref{eq:subJperpOPE}, we have
\begin{align}
\label{eq:unpjet2}
\jet_{q/\mathbb{S}}^{\rm sub}(\bm b,\mu,\zeta) &= F_{j\rightarrow \mathbb{S}} \int_0^1 \tau{d\tau}\,{C}_{j\leftarrow q}(\tau,\mu_{b_*})\exp[-S_{\rm pert}(\mu,\mu_{b_*}) - S_{\rm NP}^{J}(b,Q_0,\zeta)]\,,\\
\jet_{q/\mathbb{S}}^{\perp{\rm sub}}(\bm b,\mu,\zeta) &=F^{\perp}_{q\rightarrow \mathbb{S}} \int_0^1 d\tau \delta C_{q\leftarrow q}^{\rm Collins}(\tau,\mu_{b_*})\exp[-S_{\rm pert}(\mu,\mu_{b_*}) - S_{\rm NP}^{J_\perp}(b,Q_0,\zeta)]\,,
\end{align}
where, as discussed in Sec.\ \ref{subsec:EECsubset}, $F_{j\rightarrow \mathbb{S}} = 1$ and $F^{\perp}_{q\rightarrow \mathbb{S}} = 0$ when $\mathbb{S} = \textit{all hadrons}$. We parametrize the non-perturbative form factors similarly as TMD FFs \cite{Kang:2015msa},
\fi
As explained in the section\ \ref{sec:intro}, TMD FFs at the scale $\mu=\mu_{b_*}$ can be written in terms of collinear functions. 
\iffalse
We parametrize the twist-3 fragmentation function as \textcolor{red}{(change to 2013)}
\begin{align}
\tilde{\Delta}^N D_{\pi^+/u^\uparrow}(z,Q_0)&=2N_{\rm fav}^Cz^\gamma\tau^\delta\frac{(\gamma+\delta)^{\gamma+\delta}}{\gamma^\gamma \delta^\delta}D_{\pi^+/u}(z,Q_0)\,,\label{eq:ansel1}\\
\tilde{\Delta}^N D_{\pi^+/d^\uparrow}(z,Q_0)&=2N_{\rm dis}^CD_{\pi^+/d}(z,Q_0)\,,\label{eq:ansel2}
\end{align}

%where $Q_0^2=2.4$ GeV$^2$, $g_2=0.84,\ g_h=0.042$ GeV$^2$ and $g_c=0.0236$ GeV$^2$ as determined in \cite{Kang:2015msa} and \cite{Sun:2014dqm}. As defined in Eqs.\ \cref{eq:subJOPE} and\ \cref{eq:subJperpOPE}, $F_{j\rightarrow \mathbb{S}}$ and $F^{\perp}_{q\rightarrow \mathbb{S}}$ are defined in terms of the unpolarized fragmentation functions and the twist-3 Collins fragmentation functions, respectively. We parametrize the twist-3 Collins fragmentation functions as in\ \cite{Anselmino:2015sxa} \textcolor{red}{(actually change to Anselm's parametrization)}\textcolor{ForestGreen}{ (Changed.)}
%where $Q_0^2=2.4$ GeV$^2$, $g_2=0.84$ \cite{Kang:2015msa,Sun:2014dqm}, and we will report different $g_h$ values below to test sensitivity to the non-perturbative effects. 
\fi
We now use the parametrization of \cite{Kang:2015msa} to generate $A_{e}^{\mathbb{S}\times\mathbb{S}}(\tau Q^2)$. There, the twist-3 Collins fragmentation functions $\hat{H}^{(3)}(z,Q_0)$ were parametrized as
\begin{align}
\hat{H}_{fav}^{(3)}(z,Q_0)&=N_u^cz^{\alpha_u}(\tau )^{\beta_u}D_{\pi^+/u}(z,Q_0)\,,\label{eq:kang15_1}\\
\hat{H}_{unfav}^{(3)}(z,Q_0)&=N_d^cz^{\alpha_d}(\tau )^{\beta_d}D_{\pi^+/d}(z,Q_0)\,,\label{eq:kang15_2}\\
\hat{H}_{s/\bar{s}}^{(3)}(z,Q_0)&=N_d^cz^{\alpha_d}(\tau )^{\beta_d}D_{\pi^+/s,\bar{s}}(z,Q_0)\,,\label{eq:kang15_3}
\end{align}
and fitting parameters $N_{u}^c,\ N_{d}^c,\ \alpha_u,\ \alpha_d,\ \beta_u,\ \beta_d,$ are provided in \cite{Kang:2015msa} and $\hat{H}_{h /q}^{(3)}(z,Q_0)$ is related to Collins function $H_{1h /q}^\perp(z,p^2_\perp;Q_0)$ in the ``Trento convention"~\cite{Bacchetta:2004jz} by~\cite{Yuan:2009dw}
\begin{align}
\hat{H}_{h /q}^{(3)}\left(z,Q_0\right)=-\int d^2 p_{\perp} \frac{\left|p_{\perp}^2\right|}{zM_h} H_{1 h /q}^{\perp}\left(z, p^2_{\perp};Q_0\right)\,.
\end{align}
As pointed out in~\cite{Collins:1984kg,Ji:2004wu,Idilbi:2004vb,Kang:2011mr,Echevarria:2014rua,Kang:2015msa}, one has the TMD evolution of the Collins fragmentation functions in $b$-space written in terms of the twist-3 fragmentation function $\hat{H}_{h / q}^{(3)}$ as
\begin{align}
 \frac{p_{\perp}}{M_h} H_{1 h / q}^{\perp}\left(z, p_{\perp}^2, \mu,\zeta\right)=&\frac{1}{z^2} \int_0^{\infty} \frac{d b b^2}{(4 \pi z)} J_1\left(\frac{p_{\perp} b}{z}\right) \delta \hat{C}_{i \leftarrow q}^{\rm collins} \otimes \hat{H}_{h / i}^{(3)}\left(z, \mu_b\right) \nnu
 &\hspace{1.5cm}\times {\rm exp}\left[-\frac{1}{2} S_{\text {pert }}\left(\mu, b_*\right)-S_{\mathrm{NP}}^{H_1^\perp}(b,Q_0, \zeta)\right]\,. 
\end{align}
%which gives the result shown in \cref{fig:asye+e-}. 
where the coefficient $\delta \hat{C}^{\rm collins}_{q^{\prime} \leftarrow q}$ is given in \cref{eq:collins_c}. For completeness, we also provide the TMD evolution for unpolarized TMD PDFs and FFs here and the matching coefficients $C_{q \leftarrow i}^{f_1}$ and $\hat{C}_{i \leftarrow q}^{D_1}$ are provided in~\cite{Kang:2015msa}
\begin{align} 
 f_1^q\left(x, k_{\perp}^2,\mu,\zeta\right)=&\int_0^{\infty} \frac{d b b}{(2 \pi)} J_0\left(k_{\perp} b\right) C_{q \leftarrow i}^{f_1} \otimes f_1^i\left(x, \mu_b\right) {\rm exp}\left[-\frac{1}{2} S_{\mathrm{pert}}\left(\mu, b_*\right)-S_{\mathrm{NP}}^{f_1}(b,Q_0, \zeta)\right]\,, \\
%& h_1^q\left(x, k_{\perp}^2 ; Q\right)=\int_0^{\infty} \frac{d b b}{(2 \pi)} J_0\left(k_{\perp} b\right) \delta C_{q \leftarrow i} \otimes h_1^i\left(x, \mu_b\right) e^{-\frac{1}{2} S_{\text {pert }}\left(Q, b_*\right)-S_{\mathrm{NP}}^{h_1}(Q, b)}, \\
 D_{1h / q}\left(z, p_{\perp}^2,\mu,\zeta\right)=&\frac{1}{z^2} \int_0^{\infty} \frac{d b b}{(2 \pi)} J_0\left(\frac{p_{\perp} b}{z}\right) \hat{C}_{i \leftarrow q}^{D_1} \otimes D_{1h / i}\left(z, \mu_b\right) \nnu
 &\hspace{1.2cm}\times{\rm exp}\left[-\frac{1}{2} S_{\rm {pert }}\left(\mu, b_*\right)-S_{\mathrm{NP}}^{D_1}(b,Q_0, \zeta)\right]\,.
\end{align}
The collinear PDFs $f_1^i$ are the NLO unpolarized PDF set from $\mathtt{CT10nlo}$ \cite{Lai:2010vv} and collinear FFs $D_{1h/i}$ are NLO extraction of $\mathtt{DSS}$ fragmentation functions~\cite{deFlorian:2014xna}.
The non-perturbative Sudakov factors are parametrized as
\begin{align}
S_{\rm NP}^{f_1}(b,Q_0,\zeta)&=\frac{g_2}{2}\ln\left(\frac{b}{b_*}\right)\ln\left(\frac{\zeta}{Q_0}\right)+g_q b^2\,,\label{eq:snpf1}\\
S_{\rm NP}^{D_1}(b,Q_0,\zeta)&=\frac{g_2}{2}\ln\left(\frac{b}{b_*}\right)\ln\left(\frac{\zeta}{Q_0}\right)+\frac{g_h}{z^2} b^2\,,\label{eq:snpd1}\\
S_{\rm NP}^{H_1^\perp}(b,Q_0,\zeta)&=\frac{g_2}{2}\ln\left(\frac{b}{b_*}\right)\ln\left(\frac{\zeta}{Q_0}\right)+\frac{g_h-g_c}{z^2} b^2\,,\label{eq:snph1p}
\end{align}
where $g_2=0.84$, $Q_0^2=2.4$ GeV$^2$, $g_q=0.106$, $g_h = 0.042$ (GeV$^2$) and $g_c$ is extracted in~\cite{Kang:2015msa}. %$g_h,\ g_c$ can depend on hadron flavors. 
\begin{figure}[h]
\centering
%\includegraphics[width=0.47\textwidth]{eec/epem_13.pdf}
\includegraphics[width=0.54\textwidth]{eec/epem_15_0226.pdf}
\caption{$A_{ee}^{\mathbb{S}\times\mathbb{S}}(\tau Q^2)$ for $\mathbb{S}\times\mathbb{S}=\{\pi^+,\ \pi^-\}\times\{\pi^+,\ \pi^-\}$, $\{\pi^+\}\times\{\pi^-\}$ and $\{\pi^-\}\times\{\pi^-\}$ at $\sqrt{s}=10.6$ GeV with Collins functions fitted in %\cite{Anselmino:2013vqa} (left panel) and 
\cite{Kang:2015msa}. As discussed in Sec.\ \ref{subsec:EECsubset}, we find $|A_{ee}^{\{\pi^+,\pi^-\}\times\{\pi^+,\pi^-\}}| \ll |A_{e^+e^-}^{\{\pi^+\}\times\{\pi^-\}}|\approx|A_{e^+e^-}^{\{\pi^-\}\times\{\pi^-\}}|$ due to $J^{\perp}_{{\textit fav}} \approx -J^{\perp}_{{\textit unfav}}$.} \label{fig:asye+e-}
%In particular, note that $\mathbb{S}=\{\pi^+,\pi^-\}$ case turns on only when the NP Sudakov factor turns on.
\end{figure}

In \cref{fig:asye+e-}, we present the results for $A_{ee}^{\mathbb{S}\times \mathbb{S}}(\tau Q^2)$ with different subsets of pions $\mathbb{S}\times\mathbb{S}=\{\pi^+,\ \pi^-\}\times\{\pi^+,\ \pi^-\}$ (red curve), $\{\pi^+\}\times\{\pi^-\}$ (green curve) and $\{\pi^-\}\times\{\pi^-\}$ (blue curve) at $\sqrt{s}=10.6$ GeV with error bands generated by the theoretical uncertainties of the Collins function fittings in~\cite{Kang:2015msa}. Although the subset with $\mathbb{S}=\{\pi^+,\ \pi^-\}$ is suppressed due to the sum rule, one can have sizable asymmetries when choosing a subset of either positively or negatively charged pions in PEEC.

\subsubsection{The azimuthal asymmetry in DIS with Breit frame}
\begin{itemize}
\item The Collins asymmetry
To define the asymmetry associated with PEEC for DIS, we begin by rewriting Eq.\cref{eq:EECDIS3} as
\begin{align}
\frac{d\Sigma_{\rm DIS}}{dxdyd\tau d\phi}=&\frac{2\pi\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\int d^2{\bm q}_T\delta(\tau -\frac{{\bm q}_T^2}{Q^2})\int\frac{db\ b}{2\pi}\nnu
&\times\bigg\{\mathcal{F}_{UU}+\sin(\phi_{q_T}+\phi_s)\frac{2(1-y)}{1+(1-y)^2}\mathcal{F}_{UT}^{\sin(\phi_{q_T}+\phi_s)}+\cdots\bigg\}\,,
\end{align}
where the ellipsis represents other spin-dependent structures given in \cref{eq:EECDIS3} and
\begin{align}
\mathcal{F}_{UU}&=\sum_qe_q^2\int d^2{\bm q}_T\delta(\tau -\frac{{\bm q}_T^2}{Q^2})\int\frac{bdb}{2\pi}J_0(bq_T)\tilde{f}_1^{q,{\rm sub}}(x,{b}^2,\mu,\zeta)\jet_q^{{\rm sub}}({\bm b}^2,\mu,\zeta)H(Q,\mu)\,,\\
\mathcal{F}_{UT}^{\sin(\phi_{q_T}+\phi_s)}&=\sum_qe_q^2\int d^2{\bm q}_T\delta(\tau -\frac{{\bm q}_T^2}{Q^2})\int\frac{b^2db}{4\pi}J_1(bq_T)\tilde{h}_1^{q,{\rm sub}}(x,{b}^2,\mu,\zeta)\jet_q^{\perp{\rm sub}}({\bm b}^2,\mu,\zeta)H(Q,\mu)\,.
\end{align}
Note that we absorbed $\sqrt{S}$ to define the subtracted versions of TMD PDFs $\tilde{f}_1^{q,{\rm sub}}$ and $\tilde{h}_1^{q,{\rm sub}}$ as we did for the EEC jet functions. Then we define the asymmetry as the ratio of the above structure functions
\begin{align}
\mathcal{A}_{\rm DIS}(\tau Q^2)&=\frac{2(1-y)}{1+(1-y)^2}\frac{\mathcal{F}_{UT}^{\sin(\phi_{q_T}+\phi_s)}}{\mathcal{F}_{UU}}\,.\label{eq:sidis}
\end{align}
As discussed for the $e^+e^-$ case, we can analogously define $\mathcal{A}_{\rm DIS}^{\mathbb{S}}$ for various subsets of hadrons. We use the same parameterization of the twist-3 fragmentation functions discussed around Eq.\ \cref{eq:kang15_1}-\cref{eq:kang15_3}. As for the TMD PDFs, we follow the $b^*$ prescription and write them as %\textcolor{red}{(refer to around the part we discuss Anselm's parametrization above)}\textcolor{ForestGreen}{ (Added.)}. 
\begin{align}
\tilde{f}^{q,{\rm sub}}_{1}(x,b^2, \mu,\zeta) &= 
 \int_x^{1} \frac{dy}{y} \hat{C}_{q\leftarrow i}\left(\frac{x}{y}, \mu_{b_*} \right) f_1^{i}\left(y, \mu_{b_*}\right)
\exp\left[-S_{\rm pert}\left(\mu, \mu_{b_*} \right) - S_{\rm NP}^{f_1}\left(b, Q_0, \zeta\right)\right]\,,\\
\tilde{h}_1^{q,{\rm sub}}(x,{b}^2,\mu,\zeta) &=\int_x^{1} \frac{dy}{y} \delta C_{q\leftarrow i}\left(\frac{x}{y}, \mu_{b_*} \right) h_1^{i}\left(y, \mu_{b_*}\right)
\exp\left[-S_{\rm pert}\left(\mu, \mu_{b_*} \right) - S_{\rm NP}^{h_1}\left(b, Q_0, \zeta\right)\right]\,,
\end{align}
where
\begin{align}
\hat{C}_{q\leftarrow i} (x,\mu_b) &= C_{q \leftarrow i}\left(x, \mu_{b}\right)=\delta_{qi}\left[\delta(1-x)+\frac{\alpha_{s}}{\pi}\left(\frac{C_{F}}{2}(1-x)\right)\right]\,,\\
\delta C_{q\leftarrow i} (x,\mu_b) &= \delta_{qi} [\delta(1-x) + \mathcal{O}(\alpha_s^2)]\,.
\end{align}
On the other hand, we parametrize the non-perturbative form factors of TMD PDFs as in\ \cite{Kang:2015msa}
\begin{align}
S_{\rm NP}^{h_1}(b, Q_0,\zeta)=S_{\mathrm{NP}}^{f_{1}}(b, Q_0,\zeta)=\frac{g_{2}}{2} \ln \left(\frac{b}{b_{*}}\right) \ln \left(\frac{\zeta}{Q_{0}}\right)+g_{q} b^{2}\,.
%S_{\rm NP}^{h_1}(Q,b)&=\textcolor{red}{add}\,,
\end{align}
%where $g_2=0.84$, $Q_0^2=2.4$ GeV$^2$ and $g_q=0.106$, same as in \cref{eq:snpf1}. 
The quark transversity distribution $h_1^{q}\left(x, \mu_{b_*}\right)$ uses the parametrization from\ \cite{Kang:2015msa} as
\begin{align} 
h_1^q(x,\mu_{b_*})=N_q^hx^{a_q}(1-x)^{b_q}\frac{(a_q+b_q)^{(a_q+b_q)}}{a_q^{a_q}b_q^{b_q}}\frac{1}{2}\left(f_1^q(x,\mu_{b_*})+g_1^q(x,\mu_{b_*})\right)\,,
\end{align}
where all fitting parameters are presented in \cite{Kang:2015msa}, $f_1^q$ are the NLO unpolarized PDF set from $\mathtt{CT10nlo}$ \cite{Lai:2010vv}, and $g_1^q$ are the $\mathtt{NLO\ DSSV}$ quark helicity distributions \cite{deFlorian:2009vb}.

In \cref{fig:asyDIS}, we present the results for $A_{\rm DIS}^{\mathbb{S}}(\tau Q^2)$ using the future EIC kinematics with different subsets of pions $\mathbb{S}=\{\pi^+,\ \pi^-\}$ (red curve), $\{\pi^+\}$ (green curve) and $\{\pi^-\}$ (blue curve) with error bands given by the theoretical uncertainties provided in the extractions~\cite{Kang:2015msa} for transversity TMD PDFs $h_1^q$ and Collins fragmentatino functions $H_1^{\perp q}$. Again, as expected, we find $|A_{\rm DIS}^{\{\pi^+,\pi^-\}}| \ll |A_{\rm DIS}^{\{\pi^+\}}|$ and $|A_{\rm DIS}^{\{\pi^-\}}|$. The asymmetry is overall much smaller than the $e^+e^-$ case due to the cancellation between $h_1^u$ and $h_1^d$ as discussed in the Sec.\ \ref{subsec:EECsubset}. And the asymmetry is measurable when choosing a subset of $\pi^+$ or $\pi^-$.
%Unlike in the $e^+e^-$ case, we find a very small sensitivity to the NP effects and 
%In \cref{fig:DIShsame}, we plot $\mathbb{S}=\{\pi^+,\pi^-\}$ case for when $h_1^u = h_1^d$ just to illustrate this. As expected, we now see sensitivity to the NP sudakov factors of the TMD FFs.


%\begin{figure}[h]
%\centering
%\includegraphics[width=0.8\textwidth]{figure/Collins_asymmetry_SIDIS_13a_NP.pdf}
%\caption{$A_{\rm DIS}^{\mathbb{S} = \{\pi^+,\pi^-\}}(\tau Q^2)$ for $h_1^d = h_1^u$. We find sensitivity to the NP sudakov factors of the TMD FFs.} \label{fig:DIShsame}
%\end{figure}

%due to $J^{\perp}_{{\textit fav}} \approx -J^{\perp}_{{\textit unfav}}$. We also find that even for asymmetry tends to be a lot smaller than $e^+e^-$ case even for $\mathbb{S}=\{\pi^+\},\ \{\pi^-\}$. This is expected as discussed around Eq.\ \cref{eq:DIS_piplus}, where the asymmetry for the DIS case will become small due to cancellation of $J^{\perp}_{{\textit fav}}$ and $J^{\perp}_{{\textit unfav}}$ in the sum, with stronger cancellation as $h_1\approx h_1^{\bar{q}}$.

%As we did for Sec.\ \ref{sec:phenoee}, we also present in \cref{fig:asyDIS2}, the results using the parametrization of the twist-3 Collins functions from\ \cite{Kang:2015msa}. As described in the $e^+e^-$ case, the results using the parametrization of\ \cite{Kang:2015msa} does not follow the expectation of Sec.\ \ref{subsec:EECsubset}.


\begin{figure}[h]
\centering
%\includegraphics[width=0.47\textwidth]{eec/Collins13.pdf}
\includegraphics[width=0.54\textwidth]{eec/Collins15_0226.pdf}
\caption{$A_{\rm DIS}^{\mathbb{S}}(\tau Q^2)$ for $\mathbb{S}=\{\pi^+\},\ \{\pi^-\}$, and $\{\pi^+,\ \pi^-\}$ using the future EIC kinematics with fittings from~\cite{Kang:2015msa}. Here one also has $|A_{\rm DIS}^{\{\pi^+,\pi^-\}}| \ll |A_{\rm DIS}^{\{\pi^+\}}|$ and $|A_{\rm DIS}^{\{\pi^-\}}|$.}\label{fig:asyDIS}
%~\cite{Anselmino:2013vqa} (left panel)
%As in the $e^+e^-$ case, the parametrization of \cite{Kang:2015msa} do not follow the expectation $|A_{\rm DIS}^{\{\pi^+,\pi^-\}}| \ll |A_{\rm DIS}^{\{\pi^+\}}|$ and $|A_{\rm DIS}^{\{\pi^-\}}|$ as the twist-3 fragmentation functions do not obey the ST sum rule given in the Eq.\ \cref{eq:STsum}
\end{figure}





\item The Sivers asymmetry
To define the asymmetry associated with the Sivers asymmetry, we begin by rewriting Eq.\cref{eq:EECDIS3} as
\begin{align}
\frac{d\Sigma_{\rm DIS}}{dxdyd\tau d\phi}=&\frac{2\pi\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\int d^2{\bm q}_T\delta(\tau -\frac{{\bm q}_T^2}{Q^2})\int\frac{db\ b}{2\pi}\nnu
&\times\bigg\{\mathcal{F}_{UU}+\sin(\phi_{q_T}-\phi_s)\frac{2(1-y)}{1+(1-y)^2}\mathcal{F}_{UT}^{\sin(\phi_{q_T}-\phi_s)}+\cdots\bigg\}\,,
\end{align}
where the ellipsis represents other spin-dependent structures given in \cref{eq:EECDIS3} and
\begin{align}
\mathcal{F}_{UU}=&\sum_qe_q^2\int d^2{\bm q}_T\delta(\tau -\frac{{\bm q}_T^2}{Q^2})\int\frac{bdb}{2\pi}J_0(bq_T)\tilde{f}_1^{q,{\rm sub}}(x,{\bm b}^2,\mu,\zeta)\jet_q^{{\rm sub}}({\bm b}^2,\mu,\zeta)H(Q,\mu)\,,\\
\mathcal{F}_{UT}^{\sin(\phi_{q_T}-\phi_s)}=&\sum_qe_q^2\int d^2{\bm q}_T\delta(\tau -\frac{{\bm q}_T^2}{Q^2})\int\frac{b^2db}{2\pi}J_1(bq_T)M\tilde{f}_{1T}^{\perp(1)\, q,{\rm sub}}(x,{\bm b}^2,\mu,\zeta)\nnu
&\hspace{4.5cm}\times\jet_q^{\rm sub}({\bm b}^2,\mu,\zeta)H(Q,\mu)\,.
\end{align}
Note that we absorbed $\sqrt{S}$ to define the subtracted versions of TMD PDFs $\tilde{f}_1^{q,{\rm sub}}$ and $\tilde{f}_{1T}^{\perp(1)\,q,{\rm sub}}(x,{\bm b}^2,\mu,\zeta)$ as we did for the EEC jet functions. Then we define the asymmetry as the ratio of the above structure functions
\begin{align}
\mathcal{A}^{\rm Sivers}_{\rm DIS}(\tau Q^2)&=\frac{2(1-y)}{1+(1-y)^2}\frac{\mathcal{F}_{UT}^{\sin(\phi_{q_T}-\phi_s)}}{\mathcal{F}_{UU}}\,.\label{eq:sidis}
\end{align}
Now we can study $\mathcal{A}^{\rm Sivers}_{\rm DIS}$ for the final hadron subset $\{\pi^+,\pi^-\}$ as an example. As for the TMD PDFs, we follow the $b^*$ prescription and write them as~\cite{Echevarria:2020hpy} %\textcolor{red}{(refer to around the part we discuss Anselm's parametrization above)}\textcolor{ForestGreen}{ (Added.)}. 
\begin{align}
%\tilde{f}^{q,{\rm sub}}_{1}(x,{\bm b}^2, \mu,\zeta) =& \int_x^{1} \frac{dy}{y} \hat{C}_{q\leftarrow i}\left(\frac{x}{y}, \mu_{b_*} \right) f_1^{i}\left(y, \mu_{b_*}\right) \exp\left[-S_{\rm pert}\left(\mu, \mu_{b_*} \right) - S_{\rm NP}^{f_1}\left(b, Q_0, \zeta\right)\right]\,,\\
\tilde{f}_{1T}^{\perp(1)\,q,{\rm sub}}(x,{\bm b}^2,\mu,\zeta) =&-\frac{1}{2M}\int_x^1 \frac{d \hat{x}_1}{\hat{x}_1} \frac{d \hat{x}_2}{\hat{x}_2} \bar{C}_{q \leftarrow i}\left(x / \hat{x}_1, x / \hat{x}_2, b ; \mu, \zeta\right) T_{F i / p}\left(\hat{x}_1, \hat{x}_2 ; \mu\right)\nnu
&\times
\exp\left[-S_{\rm pert}\left(\mu, \mu_{b_*} \right) - S_{\rm NP}^{f^\perp_{1T}}\left(b, Q_0, \zeta\right)\right]\,,
\end{align}
where
\begin{align}
%\hat{C}_{q\leftarrow i} (x,\mu_b) =&\delta_{qi}\left[\delta(1-x)+\frac{\alpha_{s}}{2\pi}\left({C_{F}}(1-x)\right)\right]\,,\\
\bar{C}_{q \leftarrow i}\left(x_1, x_2, b ; \mu_{b_*}, \mu_{b_*}^2\right)=& \delta_{q i}\bigg[ \delta\left(1-x_1\right) \delta\left(1-x_2\right)-\frac{\alpha_s}{2 \pi} \frac{1}{2 N_C} \delta\left(1-x_2 / x_1\right)\left(1-x_1\right) \nnu
&\hspace{0.5cm}-\frac{\alpha_s}{2 \pi}C_F \frac{\pi^2}{12} \delta\left(1-x_1\right) \delta\left(1-x_2\right)\bigg]\,.
\end{align}
And the non-perturbative form factors of TMD PDFs are given by
\begin{align}
%S_{\rm NP}^{f_1}(Q,b)&=\frac{g_{2}}{2} \ln \left(\frac{b}{b_{*}}\right) \ln \left(\frac{Q}{Q_{0}}\right)+g_{q} b^{2}\,,\\
S_{\rm NP}^{f_{1T}^\perp}(Q,b)&=\frac{g_{2}}{2} \ln \left(\frac{b}{b_{*}}\right) \ln \left(\frac{Q}{Q_{0}}\right)+g_{q}^{f_{1T}^\perp} b^{2}\,,
%S_{\rm NP}^{h_1}(Q,b)&=\textcolor{red}{add}\,,
\end{align}
where $g_2=0.84$, $Q_0^2=2.4$ GeV$^2$ and the value of $g_q^{f_{1T}^\perp}$ given by the fitting in ~\cite{Echevarria:2020hpy}, where the Qiu-Sterman function $T_{F\,q/p}(x,x,\mu)$ has the following parametrization form
\begin{align} 
T_{F\,q/p}(x,x,\mu)=N_q \frac{\left(\alpha_q+\beta_q\right)^{\left(\alpha_q+\beta_q\right)}}{\alpha_q^{\alpha_q} \beta_q^{\beta_q}} x^{\alpha_q}(1-x)^{\beta_q}f_{1,q/p}(x,\mu)\,.
\end{align}
where all fitting parameters are presented in \cite{Kang:2015msa}, $f_{1,q/p}$ are the NLO unpolarized PDF set from $\mathtt{HERAPDF20\_NLO\_ALPHAS\_118}$ \cite{H1:2015ubc}, which is applied in the Sivers fitting in ~\cite{Echevarria:2020hpy}.

In \cref{fig:asySivers2}, we present the results for the Sivers asymmetry $A^{\rm Sivers}_{\rm DIS}(\tau Q^2)$ in terms of EEC jet functions convoluted with TMD PDFs using the parametrization of the twist-3 Qiu-Sterman function fittings from\ \cite{Echevarria:2020hpy}, using the future EIC kinematics with all pions measured in the final state. The magnitude is about a few percents and indicates that this asymmetry is a reasonable measurement for constraining the Sivers function. %In \cref{fig:DIShsame}, we plot $\mathbb{S}=\{\pi^+,\pi^-\}$ case for when $h_1^u = h_1^d$ just to illustrate this. As expected, we now see sensitivity to the NP sudakov factors of the TMD FFs.

%Now we also present in \cref{fig:asySivers2}, the Sivers asymmetry in terms of EEC jet functions convoluted with TMD PDFs using the parametrization of the twist-3 Qiu-Sterman function fittings from~\cite{Echevarria:2020hpy}.

\begin{figure}[h]
\centering
\includegraphics[width=0.57\textwidth]{eec/Sivers_0207.pdf}
\caption{$A_{\rm DIS}^{Sivers}(\tau Q^2)$ for $\mathbb{S}=\{\pi^+,\ \pi^-\}$ using the future EIC kinematics with fittings from \cite{Echevarria:2020hpy}. The error band is generated by the theoretical uncertainties of the extraction of Sivers function in~\cite{Echevarria:2020hpy}.}\label{fig:asySivers2}
\end{figure}
\end{itemize}

\subsubsection{The azimuthal asymmetry in DIS with Lab frame}
In this subsection, we provide an asymmetry prediction related to the worm-gear function $g_{1T}$ with the observable $q_*$ in Lab frame as defined in~\cite{Gao:2022bzi}. As we have shown in \cref{eq:EECDISq20}, the two structure functions for unpolarized and double-spin polarized (worm-gear) incoming proton are given by
\begin{align}
\int db\cos\left(bq_*\right)\mathcal{D}[\tilde{f}_1\jet_q]=&\int db\cos\left(bq_*\right)\sum_q e_q^2H(Q,\mu)S({\bm b}^2,\mu,\nu)\jet_q({\bm b}^2,\mu,\zeta/\nu^2) \nnu
&\hspace{3cm}\times \tilde{f}_{1}(x,{\bm b}^2,\mu,\zeta/\nu^2)\,,\label{eq:qsf1}\\
\int db\sin\left(bq_*\right)\mathcal{D}[\tilde{g}^{(1)}_{1T}\jet_q]=&\int db\sin\left(bq_*\right)\sum_q e_q^2H(Q,\mu)S({\bm b}^2,\mu,\nu)\jet_q({\bm b}^2,\mu,\zeta/\nu^2) \nnu
&\hspace{3cm}\times b{M}\tilde{g}^{(1)}_{1T}(x,{\bm b}^2,\mu,\zeta/\nu^2)\,.\label{eq:qsg1t}
\end{align}
For numerical results, we applied the new extraction~\cite{Bhattacharya:2021twu} for the worm-gear function $g_{1T}$ and the parametrization is given by
\begin{align}
g_{1 T,q}^{(1)}\left(x, Q^2\right)=\frac{N_q}{\widetilde{N}_q} x^{\alpha_q}(1-x)^{\beta_q} f_{1}\left(x, Q^2\right)\,,\label{eq:g1t1}
\end{align}
where $N_q,\ \alpha_q$ and $\beta_q$ are provided in~\cite{Bhattacharya:2021twu}, $\tilde{N}_q$ is defined in terms of the unpolarized collinear PDFs $f_{1}(x,Q_0^2)$ with $Q_0=2$ GeV,
\begin{align}
\tilde{N}_q\equiv\int_0^1 dx x^{\alpha_q+1}(1-x)^{\beta_q}f_{1}(x,Q_0^2)\,,
\end{align}
and $g_{1 T}^{(1)}\left(x, Q^2\right)$ is the first $\vec{k}_\perp$ momenutm of the TMD worm-gear function
\begin{align}
g_{1 T}^{(1)}\left(x, Q^2\right)\equiv\int d^2{\bm k}_\perp\left(\frac{k_\perp^2}{2M^2}\right)g_{1T}(x,{k}_\perp^2,Q)\,.
\end{align}
\begin{figure}[h]
\centering
\includegraphics[width=0.54\textwidth,trim={0 1cm 0 0},clip]{eec/Q22_num_den.pdf}\\
\vspace{-0.15cm}\hspace{0.2cm}\includegraphics[width=0.525\textwidth]{eec/Q22_ratio.pdf}
\\
\caption{The EEC related to unpolarized TMD PDFs $f_1$ (blue) and worm-gear TMD PDFs $g_{1T}$ (green) for all pions in the final state at the EIC kinematics are shown as a function of $q_*$ in the upper panel. The ratio $\mathcal{A}_{\rm DIS}^{WG}$ is shown at the bottom. The error bands in both panels are generated by the theoretical uncertainties of the extraction of worm-gear function in~\cite{Bhattacharya:2021twu}.}\label{fig:h1_ani}
\end{figure}
As applied in~\cite{Bhattacharya:2021twu}, the collinear PDF set $f_{1}(x,Q^2)$ is obtained from $\mathtt{CT10nlo}$ \cite{Lai:2010vv}. In the upper panel of \cref{fig:h1_ani}, we present the structure function related to unpolarized TMD PDFs as given in \cref{eq:qsf1} (divided by 10) with a blue curve as a function of $q_*$ and similarly for the structure function depending on the worm-gear functions as given in \cref{eq:qsg1t} (multiplied by 100) with a green curve. The error band is generated by applying the 200 replicas of the worm-gear functions extraction~\cite{Bhattacharya:2021twu}. In the lower panel of \cref{fig:h1_ani}, we use \cref{eq:qsg1t} divided by \cref{eq:qsf1} and plot the ratio $\mathcal{A}^{WG}_{\rm DIS}$ as a function of $q_*$ as well. As given by the extraction in~\cite{Bhattacharya:2021twu}, the worm-gear functions of $u$ quark and $d$ quark have opposite signs and similar magnitudes, and convoluted with unpolarized EEC jet functions, which is always positive. Thus for the production of all pions as final hadrons, the EEC related to worm-gear function are suppressed. This observable can be an inspiration for us to explore new directions for studying 3-dimensional nucleon structures encoded in TMD PDFs. 

\iffalse
\subsection{Conclusion}\label{sec:conclusion}
We present a comprehensive study of the polarized energy-energy correlators (PEEC) in the back-to-back region to both $e^+e^-$ and Semi-Inclusive Deep Inelastic Scattering (SIDIS) processes with unpolarized hadron production. Notably, we introduce the Collin-type EEC jet function for the first time in this context. By analyzing SIDIS, we demonstrate that all the leading-twist Transverse-Momentum-Dependent Parton Distribution Functions (TMD PDFs) can be extracted from the structure functions and convoluted with unpolarized or Collins-type EEC jet functions. This finding points towards a new approach for gaining a deeper understanding of the complex structure of nucleons.

In terms of phenomenology, we present predictions for the Collins asymmetry, which are correlated with Collins-type EEC jet functions at Belle and the Electron-Ion Collider (EIC) kinematics. These predictions illustrate the potential of using EEC jets as a powerful tool for probing the intricate structure of nucleons. Furthermore, we offer predictions for the Sivers asymmetry in the Breit frame and the worm-gear asymmetry in the Lab frame at the kinematics of the future electron-ion collider, which further demonstrate the potential for the use of EEC jets as a novel approach to probing nucleon structures.

In summary, our study provides a thorough investigation of the polarized energy-energy correlators, including the introduction of the Collin-type EEC and the use of EEC jets for probing nucleon structures. By offering predictions for various asymmetries at different kinematics, we hope to provide an impetus for further research in this exciting area of particle physics. The insights gained from this work may contribute significantly to our understanding of the fundamental building blocks of the universe and advance our knowledge of the physics governing particle interactions.
\fi


\acknowledgments
This work is supported by the National Science Foundation under CAREER award~PHY-1945471 (Z.K.and F.Z.), the Department of Energy under Contract No.~DE-AC02-05CH11231 (K.L.), the National Science Foundations of China under Grant No.~12275052 and the Shanghai Natural Science Foundation under Grant No.~21ZR1406100 (D.Y.S.).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Neutrino-tagged jet productions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Introduction}
The Electron-Ion Collider (EIC) will usher in a new era for the study of the 3D structure of the nucleon~\cite{Accardi:2012qut,AbdulKhalek:2021gbh}. Its high luminosity and polarization of both electron and hadron beams will enable precise measurements of observables related to Transverse Momentum Dependent parton distribution and fragmentation functions (TMDs). 

Jets are energetic sprays of particles observed at high-energy collider experiments that are closely related to the underlying quark and gluon dynamics of hard-scattering events. Jets at the EIC will have transverse momenta up to $\sim 40$~GeV~\cite{Arratia:2019vju,Page:2019gbf}. The EIC will produce the first jets in deep-inelastic scattering off transversely-polarized nucleons. The potential of jets produced in neutral-current deep-inelastic scattering (NC DIS) has recently been explored, see \textit{e.g.}~Refs.~\cite{Kang:2011jw,Hinderer:2015hra,Boughezal:2018azh,Zheng:2018ssm,Gutierrez-Reyes:2018qez,Gutierrez-Reyes:2019vbx, Liu:2018trl,Kang:2020xyq,Borsa:2020yxh,Arratia:2020azl,Arratia:2020nxw,Liu:2020dct,Arratia:2020ssx,Kang:2020fka,Guzey:2020gkk,Kang:2021ffh,delCastillo:2021znl,Makris:2021drz,Zhang:2021tcc,Li:2021uww,Yan:2021htf,AbdulKhalek:2022hcn,Tong:2022zwp,Liu:2022wop,Lee:2022kdn}. In this work, we will focus on jets produced in charged-current deep-inelastic scattering (CC DIS).

The CC DIS process, which involves the exchange of a virtual $W^\pm$ boson, enables jet measurements that are sensitive to the flavor of the scattered quark. The leading-order process, $W^\pm q\rightarrow q'$, is illustrated in \cref{fig:diagram}. 
Due to the conservation of electric charge, electrons can only scatter via the exchange of a $W^-$ off positively charged partons, which are predominantly $u$-quarks, especially at large $x$.  Likewise, with a positron beam, scattering processes occur predominantly with $d$-quarks through the exchange of a $W^+$ boson. Moreover, tagging either charm or strange jets can further enhance the flavor sensitivity of jet measurements~\cite{Zheng:2018ssm,Arratia:2020azl,Kang:2020fka,Arrington:2021yeb,Lee:2022kdn,Pire:2021dad}.

\begin{figure}
    \centering
    \vspace*{-1.3cm}    \includegraphics[width=0.75\columnwidth]{nu-jet/CC_DIS.pdf}
    \vspace*{-1.3cm}
\caption{Charged-current deep-inelastic scattering where the produced jet recoils against a neutrino.\label{fig:diagram}}
\end{figure}

The H1 and ZEUS collaborations measured inclusive CC DIS off unpolarized protons with longitudinally polarized electron and positron beams~\cite{Aaron:2012qi,Collaboration:2010xc,Chekanov:2008aa,Chekanov:2002zs,Breitweg:1999aa,Derrick:1996sw}. These measurements allowed for constraining the flavor dependence of collinear parton distribution functions (PDFs)~\cite{Abramowicz:2015mha}. In addition, CC DIS jet production measurements by the ZEUS collaboration~\cite{Chekanov:2003jd,Chekanov:2008af}, were compared to precise next-to-next-to-next-to-leading order QCD calculations~\cite{Gehrmann:2018odt}.

One of the main challenges in measuring CC DIS is the
measurement of the events' kinematic variables, Bjorken $x$ and $Q^{2}$, in the presence of an undetected final-state neutrino. Several methods exist to address this challenge~\cite{Blumlein:2012bf,Collaboration:2010xc}. The feasibility studies of CC DIS at the EIC have been performed in Refs.~\cite{Aschenauer:2013iia,AbdulKhalek:2021gbh} for DIS off longitudinally polarized protons with the goal to access helicity PDFs. In this study we will focus on the CC DIS off transversely polarized protons that will lead to measurements of the transverse-spin effects related to TMDs. 

In semi-inclusive DIS (SIDIS), transverse-spin asymmetries can be extracted from modulations of the azimuthal angles with respect to the virtual-boson direction, typically in the Breit frame~\cite{Avakian:2019drf,Anselmino:1993tc,Chen:2020ugq,PhysRevD.103.016011,Yang:2022sbz}. In CC DIS, this approach requires a measurement of the three-momentum of the scattered neutrino to define the azimuthal angle, which is challenging due to acceptance losses at forward rapidities.

Jet-based measurements of spin asymmetries can reduce these difficulties. Following Liu \textit{et al}.~\cite{Liu:2018trl}, TMDs can be accessed in lepton-jet azimuthal correlation measurements in the laboratory frame instead of the conventional Breit frame. Liu \textit{et al}.~\cite{Liu:2018trl} considered NC DIS, but the formalism can be extended to CC DIS as well. The advantage of this approach is that the measurement of the azimuthal angle only requires the neutrino's transverse momentum in the lab frame, which, in general, can be measured more precisely than the full three-momentum~\cite{Gao:2022bzi}. In addition, hadron-in-jet asymmetry measurements can be performed by defining an azimuthal angle of the hadron with respect to the jet axis~\cite{Yuan:2007nd,Procura:2009vm,Kang:2017glf,Arratia:2020nxw,Kang:2021ffh}.  

The jet-based TMD measurements have the additional advantage of decoupling initial- and final-state TMD effects (at leading power in the jet radius)~\cite{Kang:2021ffh}. That is, they do not involve a convolution of TMD PDFs and fragmentation functions which can introduce strong correlations in global fits of SIDIS data~\cite{Sun:2014dqm, Bacchetta:2017gcc,Scimemi:2019cmh,Cammarota:2020qcw,Bacchetta:2022awv}. 

In this section, we present the first study of neutrino-jet and hadron-in-jet spin asymmetries in CC DIS. We determine all possible spin asymmetries within the TMD factorization formalism. We present numerical estimates for transverse single-spin asymmetries in CC DIS. We also perform feasibility studies of these measurements using fast detector simulations and we quantify the expected kinematic reach and the statistical uncertainties. 

\subsection{Theoretical framework}
In this section, we discuss inclusive jet production in CC DIS, neutrino-jet correlations, and hadron-in-jet observables.

\subsection{Inclusive jet production}

We follow the theoretical framework developed in Refs.~\cite{Liu:2018trl,Arratia:2020nxw,Liu:2020dct,Kang:2021ffh} for the NC DIS. At the parton level, we consider the leading-order process $eq \rightarrow \nu q'$ mediated via the exchange of a virtual $W$ boson. We consider the cross section differential in Bjorken $x$ and the transverse momentum of the produced neutrino, $p_T^\nu$, which is defined relative to the beam direction in the laboratory frame. The leading-order cross section can be written as
\bea\label{eq:crosssection0}
    &\frac{\diff \sigma^{ep\rightarrow \nu\mathrm{jet}X}}{\diff x\,\diff^2 \vec p^{\; \nu}_T} =  \,\sum_q \sigma_0^{eq\rightarrow \nu q'} f_q(x,\mu)\,,
\eea
where the renormalization scale $\mu$ of the PDF $f_q$ is chosen at the order of the hard scale of the process $\mu\sim p_T^\nu$. 
\iffalse
The matrix element with $q$ representing the momentum of $W$-boson:
\bea
\mathcal{M}=&\left(\frac{ie}{\sqrt{2}\sin\theta_w}\right)^2(\bar{\nu}_{eL}\gamma^\mu e_L)\frac{-i(g^{\mu\nu}-\frac{q^\mu q^\nu}{m_W^2})}{q^2-m_W^2+im_W\Gamma_W}\nnu
&\times(V_{ud}\bar{d}_L^i\gamma^\nu u_L^i)\,,
\eea
\fi
The prefactor $\sigma_0$ for initial quarks $u$ and $\bar{d}$ are given by
\bea
& \sigma_0^{eu\rightarrow\nu d}=\frac{|\overline{\mathcal{M}}_{eu\rightarrow\nu d}|^2}{16\pi^2\hat{s}^2}\frac{\hat{t}}{x(\hat{t}-\hat{u})}\nnu
&=8(G_F m_W^2)^2|V_{ud}|^2\frac{\hat{s}^2}{(\hat{t}-m_W^2)^2+m_W^2\Gamma_W^2}\frac{\hat{t}}{x(\hat{t}-\hat{u})}\,,\label{eq:sigma1}\\
&\sigma_0^{e\bar{d}\rightarrow\nu \bar{u}}=\frac{|\overline{\mathcal{M}}_{e\bar{d}\rightarrow\nu \bar{u}}|^2}{16\pi^2\hat{s}^2}\frac{\hat{t}}{x(\hat{t}-\hat{u})}\nnu
&=8(G_F m_W^2)^2|V_{ud}|^2\frac{\hat{u}^2}{(\hat{t}-m_W^2)^2+m_W^2\Gamma_W^2}\frac{\hat{t}}{x(\hat{t}-\hat{u})}\,,\label{eq:sigma2}
\eea
where $G_F$ is the Fermi constant, $m_W$ and $\Gamma_W$ are the $W$ boson mass and decay width, and $V_{ud}$ is the standard CKM matrix element. Here ${\hat{t}}/(x(\hat{t}-\hat{u}))$ is the Jacobian factor, which is obtained by transforming the cross section to be differential in Bjorken-$x$ instead of the neutrino rapidity $y_\nu$. These two variables are related by
\bea
x=\frac{p_T^\nu e^{y_\nu}}{\sqrt{s}-p_T^\nu e^{-y_\nu}} .
\eea
The Mandelstam variables in \cref{eq:sigma1} and~\cref{eq:sigma2} can be written in terms of the kinematic variables of the produced neutrino and the center-of-mass energy, namely
\bea
&\hat{s}=x s \,,\\
&\hat{t}=-Q^2=-\sqrt{s} p_T^\nu e^{y_\nu}=-x \sqrt{s} p_T^{\mathrm{jet}} e^{-y_{\mathrm{jet}}}, \\
&\hat{u}=-x \sqrt{s} p_T^\nu e^{-y_\nu}=-\sqrt{s} p_T^{\mathrm{jet}} e^{y_{\mathrm{jet}}}\,.
\eea
Here $p_T^{\text {jet }}$ and $y_{\text {jet }}$ denote the jet transverse momentum and rapidity, respectively.

\subsection{Neutrino-jet correlations}

Next, we discuss neutrino-jet correlations via the exchange of a $W^-$ boson  in polarized electron-proton scattering
\bea
p(P_A,\lambda_p,\vec{S}_T)+e(P_B,\lambda_e)\rightarrow \mathrm{jet}(P_J)+\nu(P_D)+X \,.
\eea
Here $\lambda$ indicates the longitudinal polarization and $\vec S_T$ denotes the transverse spin vector of the proton. In order to access TMDs, we study back-to-back neutrino-jet production in the $ep$ collision frame. By defining light-cone vectors $n_+^\mu=\frac{1}{\sqrt{2}}(1,0,0,1)$ and $n_-^\mu=\frac{1}{\sqrt{2}}(1,0,0,-1)$, we write the momentum of the incoming proton $P_A$ and the electron $P_B$ as
\bea
P_A^\mu&=P^+n_+^\mu+\frac{M^2}{2P^+}n_-^\mu\approx P^+n_+^\mu\ = \sqrt{\frac{s}{2}}n_{+}^\mu\, ,\\
P_B^\mu&=\sqrt{\frac{s}{2}}n_{-}^\mu\, .
\eea
Here $s=(P_A+P_B)^2$ is the center-of-mass energy. We set the final observed jet to be produced in the $xz$-plane, with the following momentum $P_J^\mu = E_J\left(1, \sin\theta_J, 0, \cos\theta_J\right)$. Here $E_J$ is the jet energy and the angle $\theta_J$ is measured with respect to the beam direction. 
We find that the differential cross section can be written in terms of the structure functions as follows~\footnote{Notice that unlike the usual practice for SIDIS or DY cross sections, we do not factor out the elementary cross-sections from the structure functions. Our structure functions therefore become dimension-full quantities, see for instance Ref.~\cite{Kang:2022dpx}.}
\bea
&\frac{{\rm d}\sigma^{ep\rightarrow \nu\mathrm{jet}X}}{{\rm d}x\, {\rm d}^2\vec{p}^{\,\nu}_{T}\, {\rm d}^2q_T}=F_{UU}+\lambda_p F_{UL}\nnu
&\hspace{1cm}+|S_T|\left[\sin(\phi_{q} -\phi_{S_A})F_{UT}^{\sin(\phi_{q}-\phi_{S_A})}\right.\nnu
&\hspace{2.2cm}\left.+\cos(\phi_{q}-\phi_{S_A})F_{UT}^{\cos(\phi_{q}-\phi_{S_A})}\right]\nnu
&\hspace{1cm}+\lambda_e\left[F_{LU}+\lambda_pF_{LL}\right.\nnu
&\hspace{1.9cm}+|S_T|\sin(\phi_{q}-\phi_{S_A})F_{LT}^{\sin(\phi_{q}-\phi_{S_A})}\nnu
&\hspace{1.9cm}\left.+|S_T|\cos(\phi_{q}-\phi_{S_A})F_{LT}^{\cos(\phi_{q}-\phi_{S_A})}\right]\,.\label{eq:crosssection1}
\eea
The subscripts $E$ and $P$ of a structure function $F_{EP}$ indicate the polarization of the incoming electron and incoming proton respectively: $U$ for unpolarized, $L$ for longitudinally polarized or $T$ for transversely polarized. For example, for unpolarized scattering, the structure function is denoted by $F_{UU}$. In the limit of small values of the transverse-momentum imbalance $|\vec q_T|\ll p_T^{\rm jet}\sim p_T^\nu$, one can write this structure function in the following form using the TMD factorization formalism
\bea
F_{UU}=&\sum_q \frac{|\overline{\mathcal{M}}_{eq\rightarrow\nu q'}|^2}{16\pi^2\hat{s}^2}H(Q,\mu)\,\mathcal{J}_q(p_T^{\mathrm{jet}}R,\mu)\nnu
&\times\int\frac{{\rm d} b_T b_T}{2\pi}J_0(q_Tb_T)f_1^{\mathrm{TMD}}(x,b_T,\mu, \zeta)\nnu
& \qquad\times S_q(b_T,y_{\mathrm{jet}},R,\mu)\, .
\label{eq:factorization1}
\eea
Here $H(Q,\mu)$ is the hard function, which accounts for virtual corrections at the hard scale $Q$. The jet function $\mathcal{J}_q$ is associated with collinear dynamics of the jet with characteristic scale $\mu_J\sim p_T^{\rm jet}R$~\cite{Ellis:2010rwa}. For our numerical results presented below we use the anti-$k_T$ algorithm~\cite{Cacciari:2008gp}. The quark TMD PDF including the appropriate soft factor for a generic TMD in $b_T$-space is defined by~\cite{Boer:2011xd,Kang:2021ffh}
\bea\label{eq:ftb}
{f}_q^{(n),{\rm TMD}}(x,b_T,\mu, \zeta)=&\frac{2 \pi n !}{\left({M^{2}}\right)^{n}} \int {\rm d}k_T \, k_T\left(\frac{k_T}{b_T}\right)^{n}J_{n}\left(k_T b\right) \nnu
&\times  \tilde{f}_q^{\,\rm TMD}\!\left(x, k_T^2,\mu, \zeta \right)\,,
\eea
where $M$ is the mass of the nucleon and $J_n$ is the $n$-th order Bessel function. Here $\mu$ is the renormalization scale, while $\zeta$ is the so-called Collins-Soper scale~\cite{Collins:2011zzd}. Notice that for the unpolarized TMD $f_1^{\rm TMD}$, $n=0$. 
The unpolarized TMDPDF $\tilde{f}^{\rm TMD}_{1}(x,b_T,\mu,\zeta)$ in \cref{eq:crosssection1} is factorized as
\begin{align}
&\tilde{f}^{\rm TMD}_{1}(x,b_T, \mu,\zeta) = 
\int_x^{1} \frac{d\hat{x}}{\hat{x}} C_{q\leftarrow i}\left(\frac{x}{\hat{x}}, \mu_{b_*} \right) f_1^{i}\left(\hat{x}, \mu_{b_*}\right)\nnu
&\hspace{2cm}\times\exp\left[-S_{\rm pert}\left(\mu, \mu_{b_*} \right) - S_{\rm NP}^f\left(x, b_T, Q_0, \zeta\right)\right]\,,
\end{align}
where the $b_*$ prescription is given by Ref.~\cite{Collins:1984kg} with $b_* = b_T/\sqrt{1+b_T^2/b_{\rm max}^2}$, where $b_{\rm max} = 1.5$~GeV$^{-1}$. 
In this work, we follow the TMD factorization for Sivers function shown in Ref.~\cite{Echevarria:2020hpy}, where TMD evolution up to NNLL accuracy has been provided in the Sivers extraction.
The coefficient functions $C_{q\leftarrow i}$ can be found in Refs.~\cite{Aybat:2011zv,Kang:2015msa,Collins:2011zzd,Luo:2019szz,Luo:2020epw,Ebert:2020yqt} and the non-perturbative Sudakov factor $S_{\rm NP}^f\left(x, b_T, Q_0, \zeta\right)$ has been  parametrizated in Ref.~\cite{Sun:2014dqm,Echevarria:2020hpy}.
The remaining soft function $S_{q}$ in Eq.~(\ref{eq:factorization1}) includes a contribution from the global soft function which depends on the Wilson lines in the beam and jet directions, and the collinear-soft function associated with the soft jet dynamics. Since $S_q$ accounts for different soft contributions, it depends on both the jet rapidity $y_{\rm jet}$ and the jet radius $R$ and the expression of $S_q$ is given in~\cite{Arratia:2020nxw}.

The other cross sections or structure functions in Eq.~(\ref{eq:crosssection1}) depend on the polarization state of the nucleon  (longitudinal or transverse) and the longitudinal lepton polarization. As an example, we consider the case where the initial proton is transversely polarized. The cross section or structure function $F_{UT}^{\sin(\phi_{q}-\phi_{S_A})}$ sensitive to correlations of an unpolarized quark in the transversely polarized proton is given by
\bea
F_{UT}^{\sin(\phi_{q}-\phi_{S_A})}=&\sum_q \frac{|\overline{\mathcal{M}}_{eq\rightarrow\nu q'}|^2}{16\pi^2\hat{s}^2}H(Q,\mu)\,\mathcal{J}_q(p_T^{\mathrm{jet}}R,\mu)\nnu
&\times\int\frac{{\rm d}b_Tb_T^2}{4\pi M}J_1(q_Tb_T)f_{1T}^{\perp(1), \mathrm{TMD}}(x,b_T,\mu, \zeta)\nnu
& \qquad\times S_q(b_T,y_{\mathrm{jet}},R,\mu)\, .
\eea
In this case, the structure function is related to the Bessel function of the 1st order $J_1(q_Tb_T)$ and the Sivers function $f_{1T}^{\perp(1), \mathrm{TMD}}(x,b_T,\mu, \zeta)$ in $b_T$-space as defined in \cref{eq:ftb}.

We provide more details about the other structure functions in Eq.~(\ref{eq:crosssection1}) in the Appendix~\ref{app:jet}. For example, for an incoming electron with helicity $\lambda_e$, one replaces $\sigma_0^{eq\rightarrow\nu q'}$ with $\sigma_0^{e_Lq\rightarrow\nu q'}$ as given in \cref{eq:flu}. 

\subsection{Hadron distributions inside jets}

\begin{figure}
    \centering
    \includegraphics[width=0.90\columnwidth]{nu-jet/qToverptnu_theory.pdf}
\caption{Normalized distribution of the neutrino-jet imbalance momentum $q_T/p^\nu_T$ in unpolarized electron-proton scattering via the exchange of a $W^-$ boson.  We show our theoretical results at NLL accuracy with QCD scale uncertainties (orange) compared to Monte-Carlo event-generator simulations obtained with \textsc{Pythia}8~\cite{Sjostrand:2007gs} (blue).~\label{fig:qt_theory}}
\end{figure}

\begin{figure*}
    \centering
 \includegraphics[width=0.4\textwidth]{nu-jet/zh_theory.pdf}\hspace{0.05\textwidth}
  \includegraphics[width=0.4\textwidth]{nu-jet/jt_theory.pdf}
\caption{Distributions of the $\pi^\pm$-in-jet longitudinal-momentum fraction $z_h$ (left) and the transverse momentum $j_T$ (right) in CC DIS events. We show our theoretical results at NLL accuracy with QCD scale uncertainties (orange) compared to Monte-Carlo event-generator simulations obtained with \textsc{Pythia}8~\cite{Sjostrand:2007gs} (blue).~\label{fig:zh_and_jt}}
\end{figure*}

In this subsection, we study the longitudinal- and transverse-momentum distributions of hadrons in the identified jet for electron-proton scattering via the exchange of a $W^-$ boson:
\bea
&p(P_A,\lambda_p,\vec{S}_T)+e(P_B,\lambda_e)\nnu
&\hspace{1.2cm}\rightarrow \big(\mathrm{jet}(P_J)h(z_h,\vec{j}_T)\big)+\nu(P_D)+X.
\eea

The production of unpolarized final-state hadrons at leading twist is encoded in two TMD jet fragmentation functions (JFFs), $\mathcal{D}_1$ and $\mathcal{H}_1^\perp$~\cite{Kang:2021ffh}
\bea
\Delta(z_h,\vec{j}_T)=\,&\mathcal{D}_1^{h/q}(z_h,{j}_T)\frac{\slashed{n}_-}{2}\nnu
&-i\mathcal{H}^{\perp,h/q}_1(z_h,{j}_T)\frac{\slashed{j_T}}{z_hM_h}\frac{\slashed{n}_-}{2}\,.
\eea
Thus, we find the following  differential cross section expressed in terms of structure functions
\bea
&\frac{{\rm d}\sigma^{ep\rightarrow \nu+\mathrm{jet}X}}{{\rm d}x\, {\rm d}^2\vec{p}^{\,\nu}_{T}\, {\rm d}^2q_T\, {\rm d}z_h\, {\rm d}^2{j_T}}=F^h_{UU}+\lambda_p F^h_{UL}\nnu
&\qquad+|S_T|\left[\cos(\phi_{q}-\phi_{S_A})F_{UT}^{h,\cos(\phi_{q}-\phi_{S_A})}\right.\nnu
&\quad\hspace{1.35cm}\left.+\sin(\phi_{q} -\phi_{S_A})F_{UT}^{h,\sin(\phi_{q}-\phi_{S_A})}\right]\nnu
&\qquad+\lambda_e\left[F^h_{LU}+\lambda_pF^h_{LL}\right.\nnu
&\qquad\hspace{1.1cm}+|S_T|\sin(\phi_{q}-\phi_{S_A})F_{LT}^{h,\sin(\phi_{q}-\phi_{S_A})}\nnu
&\qquad\hspace{1.1cm}\left.+|S_T|\cos(\phi_{q}-\phi_{S_A})F_{LT}^{\cos(\phi_{q}-\phi_{S_A})}\right]\,.\label{eq:diff_xs_hadron}
\eea

In total, we find 8 structure functions and the full expression is provided in Appendix~\ref{app:h-in-jet}. Following the same convention we used in \cref{eq:crosssection1}, the subscripts $E$ and $P$ of a structure function $F^h_{EP}$ here also indicate the polarization of the incoming electron and the incoming proton, respectively. Notably, we found that none of the Collins-type jet fragmentation functions contribute in \cref{eq:diff_xs_hadron}. The reason is that chiral-odd functions have to be coupled with another chiral-odd function, the chirality between two factors of $(1-\gamma_5)$ resulting from the weak charged-current vertices must be odd. As a result, see Eq.~(\ref{eq:g5mat}), we always have  $(1-\gamma_5)(1+\gamma_5)=0$, which implies that all terms involving chiral-odd functions vanish. This conclusion is robust at leading power of the TMD factorization formalism we are using. However, whether this still holds going beyond the leading power TMD factorization, see \textit{e.g.} within TMD factorization at sub-leading power~\cite{Ebert:2021jhy,Rodini:2022wki,Gamberg:2022lju} or including higher loops as discussed in Refs.~\cite{Benic:2019zvg,Benic:2021gya}, needs further investigation. We leave such a study to a future publication. 

Using TMD factorization at leading power, see Refs.~\cite{Yuan:2007nd,Procura:2009vm,Ellis:2010rwa,Jain:2011xz,Kaufmann:2015hma,Kang:2016ehg,Bain:2016rrv,Kang:2017glf,Kang:2017btw,Kang:2019ahe}, we can write the unpolarized structure function where a hadron is measured inside the jet as follows:
\begin{align}\label{eq:crosssection2}
  F^h_{UU}  &=\,
    H(Q,\mu) \sum_q\sigma_0^{eq\rightarrow\nu q'} \, {\mathcal D}_1^{h/q}(z_h, j_T,p_T^{\rm jet}R,\mu)
    \\ &\times \,
    \int\frac{\diff^2 \vec b_T}{(2\pi)^2}\, e^{i\vec q_T\cdot \vec b_T}\, f_1^{\rm TMD}(x, b_T,\mu, \zeta)\, S_{q}( b_T,y_{\rm jet},R,\mu) \,.\nnu
\end{align}
Here the variables $z_h = \vec{p}_{h} \cdot \vec{p}_{\rm jet}/|\vec{p}_{\rm jet}|^{2}$ and ${j}_T=\left|\vec{p}_{h} \times \vec{p}_{\rm jet}\right|/|\vec{p}_{\rm jet}|^{2}$ denote the longitudinal momentum fraction and the transverse momentum relative to the (standard) jet axis of the hadron inside the jet, respectively. In the factorized cross section in Eq.~(\ref{eq:crosssection2}), ${\mathcal D}_1^{h/q}$ is a TMD fragmenting jet function. It describes the hadron-in-jet measurement and replaces the jet function $\mathcal{J}_q$ in Eq.~(\ref{eq:factorization1}). At next-to-leading logarithmic (NLL) accuracy, we can write ${\mathcal D}_1^{h/q}$ as
\bea
    &{\mathcal D}_1^{h/q}(z_h, j_T,p_T^{\rm jet}R,\mu)\nnu
    &\hspace{1.cm}=\int\frac{\diff^2\vec b_T^{\,\prime}}{(2\pi)^2}e^{{i\vec j_T\cdot\vec b_T^{\,\prime}}/{z_h}} D_1^{q/h}(z_h,\vec b_T^{\,\prime},p_T^{\rm jet}R) \,.\label{eq:TMDFF}
\eea
Here we work in Fourier conjugate space and $D_1^{q/h}$ is a TMD fragmentation function (TMDFF) evaluated at the jet scale. We use the Fourier variable $\vec b_T^{\,\prime}$ here to indicate that there is no convolution of the TMD fragmentation function with the TMD PDF in Eq.~(\ref{eq:crosssection2}). Also note that the TMDFFs can be matched to the collinear FFs~\cite{Aybat:2011zv,Collins:2011zzd} and in this work, we apply the extraction of collinear fragmentation functions in ~\cite{deFlorian:2014xna} for constructing the TMDFFs. See Ref.~\cite{Kang:2017btw} for more details. 

\section{Statistical precision of spin asymmetry measurements}
\label{sec:stat}

In \cref{fig:sivers_theory}, we show the statistical uncertainty projected for the transverse single-spin asymmetry  $A^{\sin(\phi_q-\phi_{S_A})}_{UT}$ as a function of Bjorken $x$.  The bins in Bjorken $x$ are sufficiently wide to reduce bin migration, given the resolution of the Jacquet-Blondel method (see Ref.~\cite{Aschenauer:2013iia,Arratia:2020azl}). Here we assume a luminosity of 100 fb$^{-1}$ and the absolute uncertainty of the asymmetry measurement is estimated to be $\sqrt{2}/(p\sqrt{N})$, where $p$ is the polarization of the proton beam, which we take to be 70$\%$, and $N$ is the number of events in a given bin that pass our cuts, scaled to match the NLO total inclusive cross section of Ref.~\cite{Aschenauer:2013iia} and an integrated luminosity of 100 fb$^{-1}$. Following Ref.~\cite{Anselmino:2011ay}, we include a factor of $\sqrt{2}$ to account for the fitting of the azimuthal modulations.  

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{nu-jet/sivers_theory_with_stats.pdf}
\caption{Projected statistical precision for the neutrino-jet asymmetry, which is sensitive to the Sivers distribution, for $e^+p$ collisions (open circles) and $e^-p$ collision (closed circles), for 100 fb$^{-1}$.  The yellow and blue curves show theoretical results and the corresponding bands show the uncertainty of the extracted Sivers
function in Ref.~\cite{Echevarria:2020hpy}.}
\label{fig:sivers_theory}
\end{figure}

We compare these results to the numerical results of our calculations, see Sec.~\ref{sec:theory}, which are integrated over the transverse-momentum imbalance $0 < q_T < 5$ GeV and inelasticity $0.1 < y < 0.9$. The uncertainty bands of the calculations show the uncertainty of current extractions of the Sivers function, see Ref.~\cite{Echevarria:2020hpy}. The projected statistical error bars are smaller than the predicted asymmetry for the first three bins, allowing the proposed measurement to provide a decent comparison to theoretical calculations.  

\begin{figure*}
    \centering
    \includegraphics[width=.8\textwidth]{nu-jet/electron_beam_with_stats.pdf}
\caption{Projected statistical precision for the $z_h$ dependence of the $\pi^\pm$-in-jet Collins asymmetries (open circles for $\pi^+$, closed circles for $\pi^-$) in electron-proton collisions.}  \label{fig:collins_theory}
\end{figure*}

While these measurements would provide weaker constraints on TMDs than analogous ones in the neutral-current channel, they offer an independent check with different flavor sensitivity. Moreover, they could test the consistency and universality of the theoretical predictions.  

The measurement that is projected in \cref{fig:sivers_theory} would require electron and positron beams. The capability to operate with positron beam is not included in the EIC baseline design although it might be a possible upgrade. \cref{fig:sivers_theory} shows that the positron data would yield an opposite asymmetry compared to the electron data, and their comparison could help constrain in particular the TMDs associated with the $d$ quark.  Within a global analysis, it will be possible to further demonstrate the impact and complementarity of the proposed jet observables to disentangle the flavor dependence of PDFs~\cite{Sun:2013dya,Echevarria:2014xaa,Anselmino:2016uie,Boglione:2018dqd,Bacchetta:2020gko,Echevarria:2020hpy,Cammarota:2020qcw,Bury:2020vhj,Bury:2021sue}. We leave dedicated studies for future work.


We likewise show in \cref{fig:collins_theory} the projected statistical uncertainties for hadron-in-jet Collins asymmetries as a function of $z_h$ and Bjorken $x$ for charged pions with $j_T<1.5$~GeV. As explained in Sec.~\ref{sec:theory}, this asymmetry is expected to vanish in CC DIS within the TMD factorization formalism at leading power due to the chiral-odd nature of the transversity and Collins functions. The projected statistical uncertainties are at the level of $1\%$ or smaller for small $z_{h}$. As we have mentioned earlier, performing these measurements will enable precise tests of the theory and the assumptions of factorization and chirality of the functions involved. If the asymmetry is not observed to be exactly zero, it might indicate sensitivity to sub-leading contributions that we have neglected in Sec.~\ref{sec:theory} or some other non-standard effect. 

\begin{subappendices}
\section{DIS structure functions with hadrons and EEC jets.}\label{app1}
In this appendix, we provide the relevant azimuthal-angle-dependent $\bm{q}_T$ factorization in the Breit frame and $q_*$ factorization in the lab frame for the DIS process as well as the structure functions factorized with EEC jet functions.
\subsection{Breit frame}
As shown in \cite{Gourdin:1972kro,Kotzinian:1994dv,Diehl:2005pc,Bacchetta:2006tn,Anselmino:2008sga,Collins:2011zzd,Kang:2015msa}, the differential cross section for the DIS process up to twist-2 functions is factorized by
\begin{align}
\frac{d\sigma}{dxdydz_ad^2{\bm q}_T}=&\frac{2\pi\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\int\frac{bdb}{2\pi}\bigg\{F_{UU}+\cos(2\phi_{q_T})\frac{2(1-y)}{1+(1-y)^2}F_{UU}^{\cos(2\phi_{q_T})}\nnu
&+S_{\parallel}\sin(2\phi_{q_T})\frac{2(1-y)}{1+(1-y)^2}F_{UL}^{\sin(2\phi_{q_T})}+|{\bm S}_\perp|\bigg[\sin(\phi_{q_T}-\phi_s)F_{UT}^{\sin(\phi_{q_T}-\phi_s)}\nnu
&+\sin(\phi_{q_T}+\phi_s)\frac{2(1-y)}{1+(1-y)^2}F_{UT}^{\sin(\phi_{q_T}+\phi_s)}\nnu
&+\sin(3\phi_{q_T}-\phi_s)\frac{2(1-y)}{1+(1-y)^2}F_{UT}^{\sin(3\phi_{q_T}-\phi_s)}\bigg]\nnu
&+\lambda_e\bigg[S_{\parallel}\frac{y(2-y)}{1+(1-y)^2}F_{LL}+|{\bm S}_\perp|\cos(\phi_{q_T}-\phi_s)F_{LT}^{\cos(\phi_{q_T}-\phi_s)}\bigg]\bigg\}\,,\label{dis_cross}
\end{align}
where for structure functions $F_{AB}$, the indices $A$ and $B$ represent the polarization of the incoming electron and incoming proton. $S_{\parallel}$ and $|{\bm S}_\perp|$ are the helicity and transverse spin of the incoming proton, $\lambda_e$ is the helicity of the incoming electron.
The variables $x$ and $y$ represent the longitudinal momentum fraction of the incoming parton inside the beam and the inelasticity variable, respectively, which we will additionally be differential in. The azimuthal angles $\phi_s$ and $\phi_{q_T}$ are the azimuthal angles of the transverse spin of the beam and the transverse momentum of the produced hadron, respectively. By defining the notation ${C}[\tilde{f}^{(m)}\tilde{D}^{(n)}]$ as
\begin{align}
{C}[\tilde{f}^{(m)}\tilde{D}^{(n)}]=&\sum_q e_q^2 b^{m+n}J_{m+n}(bq_T){(M)^m}{(-zM_h)^n}\tilde{f}^{(m)}(x,{\bm b}^2,\mu,\zeta/\nu^2)\nnu
&\times\tilde{D}^{(n)}(z,{\bm b}^2,\mu,\hat{\zeta}/\nu^2)H(Q,\mu)S({\bm b}^2,\mu,\nu)\,,
\end{align}
where $\tilde{f}^{(m)}(x,{\bm b}^2,\mu,\zeta/\nu^2)$ and $\tilde{D}^{(n)}(z,{\bm b}^2,\mu,\hat{\zeta}/\nu^2)$ are the Fourier transform of TMD PDFs and TMD FFs in $b$-space\footnote{To simplify the notations, we apply $n=0$ by default, namely $\tilde{f}_1=\tilde{f}_1^{(0)}$ and $\tilde{D}_1=\tilde{D}_1^{(0)}$.} and defined by~\cite{Boer:2011xd,Kang:2021ffh}
\begin{align}
\tilde{f}^{(m)}(x,{\bm b}^2,\mu,\zeta/\nu^2)=&\frac{2\pi m!}{(M^2)^m}\int dp_T p_T\left(\frac{p_T}{b}\right)^m J_m(bp_T)f(x,{\bm p}_T^2,\mu,\zeta/\nu^2)\\
\tilde{D}^{(n)}(z,{\bm b}^2,\mu,\hat{\zeta}/\nu^2)=&\frac{2\pi n!}{(zM_h^2)^n}\int dk_T k_T\left(\frac{k_T}{b}\right)^n J_n(bk_T)D(z,{\bm k}_T^2,\mu,\hat{\zeta}/\nu^2)\,.
\end{align}
Thus one obtains the factorization of the spin-averaged structure function $F_{UU}$ and the all possible spin-dependent structure functions shown in \cref{dis_cross} as
\begin{align}
F_{UU}=&\,C[\tilde{f}_1\tilde{D}_1]\,,\\
F_{UU}^{\cos(2\phi_{q_T})}=&\,-C[\tilde{h}^{\perp(1)}_1\tilde{H}^{\perp(1)}_1]\,,\\
F_{UL}^{\sin(2\phi_{q_T})}=&\,-C[\tilde{h}^{\perp(1)}_{1L}\tilde{H}^{\perp(1)}_1]\,,\\
F_{UT}^{\sin(\phi_{q_T}-\phi_s)}=&\,-C[\tilde{f}^{\perp(1)}_{1T}\tilde{D}_1]\,,\\
F_{UT}^{\sin(\phi_{q_T}+\phi_s)}=&\,-C[\tilde{h}_1\tilde{H}^{\perp(1)}_1]\,,\\
F_{UT}^{\sin(3\phi_{q_T}-\phi_s)}=&\,-\frac{1}{4}C[\tilde{h}^{\perp(2)}_{1T}\tilde{H}^{\perp(1)}_1]\,,\\
F_{LL}=&\,C[\tilde{g}_{1L}\tilde{D}_1]\,,\\
F_{LT}^{\cos(\phi_{q_T}-\phi_s)}=&\,C[\tilde{g}^{\perp(1)}_{1T}\tilde{D}_1]\,,
\end{align}
where we encounter unpolarized and Collins TMD FF from Eq.\ \cref{eq:diffcskt} again. Here, summation over $q$ includes the anti-quarks as well. Then using the EEC jet functions defined above in Eqs.\ \cref{eq:unpjet} and\ \cref{eq:Collinsjet}, namely 
\begin{align}
\jet_q({\bm b}^2,\mu,\zeta/\nu^2)\equiv&\sum_{h}\int_0^1dz\,z\,\tilde{D}_{1,h/q}(z,{\bm b}^2,\mu,\zeta/\nu^2)\\
%=&\sum_{h}\int_0^1dz\,z\int d^2{\bm P}_{h\perp}e^{-i{\bm b}\cdot\frac{{\bm P}_{h\perp}}{z}}D_{1,h/q}(z,{\bm P}_{h\perp}^2,\mu,\zeta/\nu^2)\nnu
%=&\sum_{h}\int_0^1dz\,z^3\int d^2{\bm k}_\perp e^{i{\bm b}\cdot{\bm k}_\perp}D_{1,h/q}(z,z^2{\bm k}_\perp^2,\mu,\zeta/\nu^2)\,,\\
\left(-\frac{i{\bm b}^\alpha}{2}\right)\jet_q^\perp({\bm b}^2,\mu,\zeta/\nu^2)\equiv&\sum_{h}\int_0^1dz\,z\, \tilde{H}_{1,h/q}^{\perp\,\alpha}(z,{\bm b}^2,\mu,\zeta/\nu^2)\,.
%=&\sum_{h}\int_0^1dz\,z\int d^2{\bm P}_{h\perp}e^{-i{\bm b}\cdot\frac{{\bm P}_{h\perp}}{z}}\frac{\bm P_{h\perp}^\alpha}{z_hM_h} H_{1,h/q}^{\perp}(z_h,{\bm P}_{h\perp}^2,\mu,\zeta/\nu^2)\nnu
%=&\sum_{h}\int_0^1dz_h\,z_h^3\int d^2{\bm k}_\perp e^{i{\bm b}\cdot{\bm k}_\perp}\left(-\frac{{\bm k}_\perp^\alpha}{M_h}\right)H_{1,h/q}^{\perp}(z_h,z_h^2{\bm k}_{\perp}^2,\mu,\zeta/\nu^2)\nnu
%=&\sum_{h}\int_0^1dz_h\,z_h^3\left(-\frac{\hat{\bm b}^\alpha}{M_h}\right)\int k_\perp^2dk_\perp 2\pi iJ_1(bk_\perp)H_{1,h/q}^{\perp}(z_h,z_h^2{\bm k}_{\perp}^2,\mu,\zeta/\nu^2)\nnu
%=&\sum_{h}\int_0^1dz_h\,z_h^4M_h\left(-i{\bm b}^\alpha\right)H_1^\perp(z,{\bm b}^2,\mu.\zeta/\nu^2)\,.
\,.
\end{align}
Then the azimuthal angle dependent EEC at DIS in Eq.\ \cref{eq:EECazimDISdef2} can be written as~\footnote{Here TMD PDFs $\tilde{f}^{(n)}(x,{\bm b}^2,\mu,\zeta/\nu^2)$, EEC jet functions $\jet_q({\bm b},\mu,\zeta/\nu^2)$ and $\jet_q^\perp({\bm b},\mu,\zeta/\nu^2)$ are written as $\tilde{f}^{(n)},\ \jet_q$ and $\jet_q^\perp$ respectively, for simplification of the notations.}

\begin{align}
\frac{d\Sigma_{\rm DIS}}{dxdyd\tau d\phi}=&\frac{1}{2} \sum_{a}\int d^2\bm{q}_T dz_a z_a \frac{d\sigma}{dxdyd^2\bm{q}_T dz_a} \delta(\tau - \frac{\bm{q}_T^2}{Q^2}) \delta(\phi - \phi_{q_T})\nnu
=&\frac{2\pi\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\sum_qe_q^2\int d^2{\bm q}_T\delta(\tau -\frac{{\bm q}_T^2}{Q^2})\delta(\phi-\phi_{q_T})\int\frac{db\ b}{2\pi}H(Q,\mu)\nnu
&\times S({\bm b}^2,\mu,\nu)\bigg\{J_0(bq_T)\tilde{f}_{1,q}\jet_q+\cos(2\phi_{q_T})\frac{2(1-y)}{1+(1-y)^2}J_2(bq_T)\frac{b^2}{2}\tilde{h}_{1,q}^{\perp(1)}\jet^\perp_q\nnu
&\quad+S_{\parallel}\sin(2\phi_{q_T})\frac{2(1-y)}{1+(1-y)^2}J_2(bq_T)\frac{b^2}{2}\tilde{h}_{1L,q}^{\perp(1)}\jet^\perp_q\nnu
&\quad+|{\bm S}_\perp|\bigg[-\sin(\phi_{q_T}-\phi_s)J_1(bq_T){b}\tilde{f}_{1T,q}^{\perp(1)}\jet_q\nnu
&\quad+\sin(\phi_{q_T}+\phi_s)\frac{2(1-y)}{1+(1-y)^2}\frac{b}{2}J_1(bq_T)\tilde{h}_{1,q}\jet^\perp_q\nnu
&\quad+\sin(3\phi_{q_T}-\phi_s)\frac{2(1-y)}{1+(1-y)^2}\frac{M^2b^3}{8}J_3(bq_T)\tilde{h}_{1T,q}^{\perp(2)}\jet^\perp_q\bigg]\nnu
&+\lambda_e\bigg[S_{\parallel}\frac{y(2-y)}{1+(1-y)^2}J_0(bq_T)\tilde{g}_{1L,q}^q\jet_q
+|{\bm S}_\perp|\cos(\phi_{q_T}-\phi_s)J_1(bq_T){b}\tilde{g}_{1T,q}^{\perp(1)}\jet_q\bigg]\bigg\}\,,\label{eq:EECDIS2}
\end{align}
where the first term appeared already in\ \cite{Li:2021txc}. By defining 
\begin{align}
\sigma_0=2z\frac{\pi\alpha_{em}^2}{zQ^2}\frac{1+(1-y)^2}{y}=\frac{2\pi\alpha_{em}^2}{Q^2}\frac{1+(1-y)^2}{y}=\frac{2\pi\alpha_{em}^2}{Q^2}\frac{y}{1-\epsilon}\,,
\end{align}
where $\epsilon=(1-y)/(1-y+y^2/2)$, one has \cref{eq:EECDIS2} in the form below,
\begin{align}
\frac{d\Sigma_{\rm DIS}}{dxdyd\tau d\phi}=&\sigma_0\sum_qe_q^2\int d^2{\bm q}_T\delta(\tau -\frac{{\bm q}_T^2}{Q^2})\delta(\phi-\phi_{qT})\int\frac{db\ b}{2\pi}H(Q,\mu)\nnu
&\times S({\bm b}^2,\mu,\nu)\bigg\{J_0(bq_T)\tilde{f}_{1,q}\jet_q+\epsilon\cos(2\phi_{q_T})J_2(bq_T)\frac{b^2}{2}\tilde{h}_{1,q}^{\perp(1)}\jet^\perp_q\nnu
&\quad+S_{\parallel}\epsilon\sin(2\phi_{q_T})J_2(bq_T)\frac{b^2}{2}\tilde{h}_{1L,q}^{\perp(1)}\jet^\perp_q+|{\bm S}_\perp|\bigg[-\sin(\phi_{q_T}-\phi_s)J_1(bq_T){b}\tilde{f}_{1T,q}^{\perp(1)}\jet_q\nnu
&\quad+\epsilon\sin(\phi_{q_T}+\phi_s)\frac{b}{2}J_1(bq_T)\tilde{h}_{1,q}\jet^\perp_q+\epsilon\sin(3\phi_{q_T}-\phi_s)\frac{M^2b^3}{8}J_3(bq_T)\tilde{h}_{1T,q}^{\perp(2)}\jet^\perp_q\bigg]\nnu
&+\lambda_e\bigg[S_{\parallel}\sqrt{1-\epsilon^2}J_0(bq_T)\tilde{g}_{1L,q}^q\jet_q
+|{\bm S}_\perp|\sqrt{1-\epsilon^2}\cos(\phi_{q_T}-\phi_s)J_1(bq_T){b}\tilde{g}_{1T,q}^{\perp(1)}\jet_q\bigg]\bigg\}\,,\label{eq:EECDIS4}
\end{align}

Unlike the EEC in $e^+e^-$ annihilation, DIS version of the EEC has only one EEC jet function per term as it measures correlation between one outgoing hadron and the beam. By defining the notation $\mathcal{C}[\tilde{f}^{(m)}\jet_q^{(\perp)}]$ as
\begin{align}
\mathcal{C}[\tilde{f}^{(m)}\jet_q]=&\sum_q e_q^2H(Q,\mu)S({\bm b}^2,\mu,\nu)\jet_q({\bm b}^2,\mu,\zeta/\nu^2) \nnu
&\times b^{m}J_{m}(bq_T){M^m}\tilde{f}^{(m)}_q(x,{\bm b}^2,\mu,\zeta/\nu^2)\,,\label{eq:cdef1}\\
\mathcal{C}[\tilde{f}^{(m)}\jet_q^{\perp}]=&\sum_q e_q^2H(Q,\mu)S({\bm b}^2,\mu,\nu)\jet_q^\perp({\bm b}^2,\mu,\zeta/\nu^2) \nnu
&\times\frac{b^{m+1}}{2}J_{m+1}(bq_T){M^m}(-{M_h})\tilde{f}^{(m)}_q(x,{\bm b}^2,\mu,\zeta/\nu^2) \,,\label{eq:cdef2}
\end{align}
And define the structure functions $\mathcal{F}_{AB}$ as
\begin{align}
\mathcal{F}_{UU}=&\,\mathcal{C}[\tilde{f}_{1}\jet_q]\,,\\
\mathcal{F}_{UU}^{\cos(2\phi_{q_T})}=&\,-\mathcal{C}[\tilde{h}^{\perp(1)}_{1}{\jet_q^\perp}]\,,\\
\mathcal{F}_{UL}^{\sin(2\phi_{q_T})}=&\,-\mathcal{C}[\tilde{h}^{\perp(1)}_{1L}{\jet_q^\perp}]\,,\\
\mathcal{F}_{UT}^{\sin(\phi_{q_T}-\phi_s)}=&\,-\mathcal{C}[\tilde{f}^{\perp(1)}_{1T}\jet_q]\,,\\
\mathcal{F}_{UT}^{\sin(\phi_{q_T}+\phi_s)}=&\,-\mathcal{C}[\tilde{h}_{1}{\jet_q^\perp}]\,,\\
\mathcal{F}_{UT}^{\sin(3\phi_{q_T}-\phi_s)}=&\,-\frac{1}{4}\mathcal{C}[\tilde{h}^{\perp(2)}_{1T}{\jet_q^\perp}]\,,\\
\mathcal{F}_{LL}=&\,\mathcal{C}[\tilde{g}_{1L}\jet_q]\,,\\
\mathcal{F}_{LT}^{\cos(\phi_{q_T}-\phi_s)}=&\,\mathcal{C}[\tilde{g}^{\perp(1)}_{1T}\jet_q]\,,
\end{align}
one finally obtains the azimuthal angle-dependent EEC at DIS as given in \cref{eq:EECDIS3}.

\subsection{Lab frame}\label{sec:appb}
As introduced in~\cite{Gao:2022bzi}, an optimized observable $q_*$ is defined for probing the transverse momentum of the produced hadron with respect to the photon momentum direction and at leading power $q_*=q_{T}\sin\phi_{q_T} $. Namely one has
\begin{align}
\frac{d\sigma}{dxdydz_ad{q_*}}=&\int d^2{\bm q}_{T}\delta\left(q_*-q_{T}\sin\phi_{q_T} \right) \frac{d\sigma}{dxdydz_ad^2{\bm q}_{T}}\,.\label{eq:lab1}
\end{align}
Using the identities 
\begin{align}
J_0\left({bq_{T}}\right):\ &\int d^2{\bm q}_{T}\delta\left(q_*-q_{T}\sin\phi_{q_T} \right)J_0(bq_{T})=\int q_{T}dq_{T}\frac{d\phi_{q_T}}{\sin\phi_{q_T}}\delta\left(\frac{q_*}{\sin\phi_{q_T}}-{q_{T}}\right)J_0\left({bq_{T}}\right)\nnu
=&\int \frac{\phi_{q_T}}{\sin^2\phi_{q_T}}q_*\Theta\left(\frac{q_*}{\sin\phi_{q_T}}\right)J_0\left(\frac{bq_*}{\sin\phi_{q_T}}\right)=\,\frac{2\cos\left(bq_*\right)}{b}\,,\label{eq:qs_int_1}\\
J_1\left({bq_{T}}\right):\ &\int d^2{\bm q}_{T}\delta\left(q_*-q_T\sin\phi_{q_T}\right)\sin\left(\phi_{q_T}\right)J_1({bq_{T}})\nnu
=&\int \frac{\phi_{q_T}}{\sin^2\phi_{q_T}}q_*\Theta\left(\frac{q_*}{\sin\phi_{q_T}}\right)\sin\left(\phi_{q_T}\right)J_1\left(\frac{bq_*}{\sin\phi_{q_T}}\right)=\,\frac{2\sin\left(bq_*\right)}{b}\,,\\
&\int d^2{\bm q}_T\delta\left(q_*-q_T\sin\phi_{q_T}\right)\cos\left(\phi_{q_T}\right)J_1(bq_T)=0\,,\\
J_2\left({bq_{T}}\right):\ &\int d^2{\bm q}_T\delta\left(q_*-q_T\sin\phi_{q_T}\right)\sin\left(2\phi_{q_T}\right)J_2({bq_{T}})=0\,,\label{eq:h1lp}\\
&\int d^2{\bm q}_T\delta\left(q_*-q_T\sin\phi_{q_T}\right)\cos\left(2\phi_{q_T}\right)J_2({bq_{T}})\nnu
=&\int \frac{\phi_{q_T}}{\sin^2\phi_{q_T}}q_*\Theta\left(\frac{q_*}{\sin\phi_{q_T}}\right)\cos\left(2\phi_{q_T}\right)J_2\left(\frac{bq_*}{\sin\phi_{q_T}}\right)=\,\frac{2\cos\left(bq_*\right)}{b}\,,\\
J_3\left({bq_{T}}\right):\ &\int d^2{\bm q}_T\delta\left(q_*-q_T\sin\phi_{q_T}\right)\sin\left(3\phi_{q_T}\right)J_3(bq_T)\nnu
=&\int \frac{\phi_{q_T}}{\sin^2\phi_{q_T}}q_*\Theta\left(\frac{q_*}{\sin\phi_{q_T}}\right)\sin\left(3\phi_{q_T}\right)J_3\left(\frac{bq_*}{\sin\phi_{q_T}}\right)=\,\frac{2\sin\left(bq_*\right)}{b}\,,\\
&\int d^2{\bm q}_T\delta\left(q_*-q_T\sin\phi_{q_T}\right)\cos\left(3\phi_{q_T}\right)J_3(bq_T)=0\,,\label{eq:qs_int_2}
\end{align}
following the DIS differential cross section introduced in App.~\ref{app1} and \cref{eq:lab1}, one obtains
\begin{align}
\frac{d\sigma}{dxdydz_ad{q_*}}=&\frac{2\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\int db\sum_q e_q^2H(Q,\mu)S({\bm b}^2,\mu,\nu)\bigg\{\cos\left(bq_*\right)\bigg[\tilde{f}_{1,q}\tilde{D}_1\nnu
&+\frac{2(1-y)}{1+(1-y)^2}zMM_hb^2\tilde{h}_{1,q}^{\perp (1)}\tilde{H}_1^{\perp (1)}+\lambda_eS_{\parallel}\frac{y(2-y)}{1+(1-y)^2}\tilde{g}_{1L,q}\tilde{D}_1\bigg]\nnu
&+|{\bm S}_\perp|\sin\left(bq_*\right)\cos\phi_s\bigg[-Mb\tilde{f}_{1T,q}^{\perp(1)}\tilde{D}_1+\frac{2(1-y)}{1+(1-y)^2}zM_hb\tilde{h}_{1,q}\tilde{H}_1^{\perp (1)}\nnu
&+\frac{2(1-y)}{1+(1-y)^2}\frac{zM^2M_hb^3}{4}\tilde{h}_{1T,q}^{\perp (2)}\tilde{H}_1^{\perp (1)}\bigg]\nnu
&+\lambda_e|{\bm S}_\perp|\sin\left(bq_*\right)\sin\phi_sM\tilde{g}_{1T,q}^{(1)}\tilde{D}_1\bigg\}\,.
\end{align}
Note that as indicated in \cref{eq:h1lp}, the contribution from $h_{1L}^\perp$ will vanish when measuring $q_*$. Now we define the EEC with $q_*$ measured as
\begin{align}
\frac{d\Sigma_{\rm DIS}}{dxdydq_*}=&\frac{1}{2} \sum_{a}\int d^2\bm{q}_T dz_a z_a \frac{d\sigma}{dxdy dz_ad^2\bm{q}_T} \delta(q_* - q_T\sin\phi_{q_T}) \nnu
%=&\frac{1}{2} \sum_{a}\int dz_a z_a \frac{d\sigma}{dxdy dz_ad^2q_*} \nnu
=&\frac{2\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\int db\sum_qe_q^2H(Q,\mu)S({\bm b}^2,\mu,\nu)\bigg\{\cos\left(bq_*\right)\bigg[\tilde{f}_{1,q}{J}_q\nnu
&+\frac{2(1-y)}{1+(1-y)^2}\frac{Mb^2}{2}\tilde{h}_{1,q}^{\perp (1)}{J}_q^\perp+\lambda_eS_{\parallel}\frac{y(2-y)}{1+(1-y)^2}\tilde{g}_{1L,q}{J}_q\bigg]\nnu
&+|{\bm S}_\perp|\sin\left(bq_*\right)\cos\phi_s\bigg[-Mb\tilde{f}_{1T,q}^{\perp(1)}{J}_q+\frac{2(1-y)}{1+(1-y)^2}\frac{b}{2}\tilde{h}_{1,q}{J}_q^\perp\nnu
&+\frac{2(1-y)}{1+(1-y)^2}\frac{M^2b^3}{8}\tilde{h}_{1T,q}^{\perp (2)}{J}_q^\perp\bigg]\nnu
&+\lambda_e|{\bm S}_\perp|\sin\left(bq_*\right)\sin\phi_sMb\tilde{g}_{1T,q}^{(1)}{J}_q\bigg\}\,,\label{eq:EECDISq2}
\end{align}
By defining the notation $\mathcal{D}[\tilde{f}^{(m)}\jet_q^{(\perp)}]$ as
\begin{align}
\mathcal{D}[\tilde{f}^{(m)}\jet_q]=&\sum_q e_q^2H(Q,\mu)S({\bm b}^2,\mu,\nu)\jet_q({\bm b}^2,\mu,\zeta/\nu^2) \nnu
&\times b^{m}{M^m}\tilde{f}^{(m)}_q(x,{\bm b}^2,\mu,\zeta/\nu^2)\,,\\
\mathcal{D}[\tilde{f}^{(m)}\jet_q^{\perp}]=&\sum_q e_q^2H(Q,\mu)S({\bm b}^2,\mu,\nu)\jet_q^\perp({\bm b}^2,\mu,\zeta/\nu^2) \nnu
&\times\frac{b^{m+1}}{2}{M^m}{(-M_h)}\tilde{f}^{(m)}_q(x,{\bm b}^2,\mu,\zeta/\nu^2) \,.
\end{align}
Compared to $\mathcal{C}[\cdots]$ defined in \cref{eq:cdef1} and~\cref{eq:cdef2}, the notation here $\mathcal{D}[\cdots]$ is not equipped with a Bessel function, since $J_{n+m}(bq_T)$ has been integrated out in \cref{eq:qs_int_1}-\cref{eq:qs_int_2} for measuring $q_*$.

Finally, one obtains the azimuthal angle-dependent EEC at DIS with $q_*$ measured
\begin{align}
\frac{d\Sigma_{\rm DIS}}{dxdydq_*}=&\frac{2\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\int db\bigg\{\cos\left(bq_*\right)\bigg[\mathcal{D}[\tilde{f}_1\jet_q]\nnu
&+\frac{2(1-y)}{1+(1-y)^2}\mathcal{D}[\tilde{h}^{\perp(1)}\jet_q^{\perp}]+\lambda_eS_{\parallel}\frac{y(2-y)}{1+(1-y)^2}\mathcal{D}[\tilde{g}_{1L}\jet_q]\bigg]\nnu
&+|{\bm S}_\perp|\sin\left(bq_*\right)\cos\phi_s\bigg[-\mathcal{D}[\tilde{f}^{\perp(1)}_{1T}\jet_q]+\frac{2(1-y)}{1+(1-y)^2}\mathcal{D}[\tilde{h}_1\jet_q^{\perp}]\nnu
&+\frac{2(1-y)}{1+(1-y)^2}\frac{1}{4}\mathcal{D}[\tilde{h}^{\perp(2)}_{1T}\jet_q^{\perp}]\bigg]\nnu
&+\lambda_e|{\bm S}_\perp|\sin\left(bq_*\right)\sin\phi_s\mathcal{D}[\tilde{g}^{(1)}_{1T}\jet_q]\bigg\}\,,\label{eq:EECDISq22}
\end{align}
Upon closer inspection of \cref{eq:EECDISq22} and Eq.(10) in~\cite{Gao:2022bzi}, the disparity in sign arises from different definitions of the $n$-th order TMD PDFs in $b$-space. Nonetheless, one can successfully harmonize the two works by adroitly factoring in $(-1)^n$ for each structure function in \cref{eq:EECDISq22} that corresponds to $\tilde{f}^{(n)}$, and thereby cancel the divergence in convention.Therefore, one observes a consistency between the structure functions in \cref{eq:EECDISq22} and those in~\cite{Gao:2022bzi}. 

\iffalse
\begin{align}
&\frac{d\Sigma_{\rm SIDIS}}{dxdyd\tau d\phi}=\sum_h\int dzz\frac{d\sigma_{\rm SIDIS}}{dxdydzd\tau d\phi}\nnu
=&\frac{2\pi\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\sum_h\sum_qe_q^2\int d^2{\bm q}_T\delta(\tau -\frac{{\bm q}_T^2}{Q^2})\delta(\phi - \phi_{q_T})\int\frac{bdb}{2\pi}\nnu
&\times\int dzz\bigg[J_0(q_Tb)\big(C_{q\leftarrow i}\otimes f_1^q^i(x,\mu_b)\big)\big(C_{j\leftarrow q}\otimes D_{1,h/j}(z,\mu_b)\big)e^{-S_{\rm pert}\left(Q, b_{*}\right)-S_{\rm NP}^{\rm SIDIS}(Q, b)}\nnu
&+\sin(\phi_{q_T}+\phi_s)\frac{2(1-y)}{1+(1-y)^2}\frac{b}{2z}J_1(q_Tb)\big(\delta C_{q\leftarrow i}\otimes h_1^i(x,\mu_b)\big)\big(\deltaC_{j\leftarrow q}\otimes \hat{H}^{(3)}_{h/j}(z,\mu_b)\big)\nnu
&\quad\times e^{-S_{\rm pert}\left(Q, b_{*}\right)-S_{\rm NP,collins}^{\rm SIDIS}(Q, b)}+\cdots\bigg]\,,\\
=&\frac{2\pi\alpha_{\rm em}^2}{Q^2}\frac{1+(1-y)^2}{y}\sum_qe_q^2\int d^2{\bm q}_T\delta(\tau -\frac{{\bm q}_T^2}{Q^2})\delta(\phi - \phi_{q_T})\int\frac{bdb}{2\pi}\nnu
&\times\bigg[J_0(q_Tb)\big(C_{q\leftarrow i}\otimes f_1^q^i(x,\mu_b)\big)\jet_q({\bm b},\mu,\nu)+\sin(\phi_{q_T}+\phi_s)\frac{2(1-y)}{1+(1-y)^2}\nnu
&\times\frac{b}{2}J_1(q_Tb)\big(\delta C_{q\leftarrow i}\otimes h_1^i(x,\mu_b)\big)\jet_q^\perp({\bm b},\mu,\nu)+\cdots\bigg]\,,\label{eq:EECDIS2}
\end{align}
\fi

%In this work, we investigate the factorization theorem for the energy-energy correlation with Collins asymmetry in the back-to-back region. In the factorization formula we present, this event shape observable is correlated with the Collins function in the back-to-back limit and are sensitive to the azimuthal angle between the two hadrons participated in the collision. With the analytical formalism derived and the non-perturbative corrections fitted from Fragmentation function grids, we defined the Collins EEC jet function and provide predictions for the Collins asymmetry correlated with EEC jet at Belle and EIC kinematics.

\section{Inclusive jet production}\label{app:jet}
In this appendix, we provide the expressions for all the structure functions that appear in \cref{eq:crosssection1}. We start with the squared matrix element of the process $e+p\rightarrow \nu+\mathrm{jet}+X$, where the incoming proton and electron are unpolarized, which is given by
\bea
&|\mathcal{M}|^2=\left(\frac{e^2}{{2}\sin^2\theta_w}\right)^2|V_{ud}|^2\frac{(g^{\mu\nu}-\frac{q^\mu q^\nu}{m_W^2})(g^{\mu'\nu'}-\frac{q^{\mu'} q^{\nu'}}{m_W^2})}{(q^2-m_W^2)^2+(m_W\Gamma_W)^2}\nnu
&\times\mathrm{Tr}\left[{\slashed{P}_D}\gamma^\mu\left(\frac{1-\gamma_5}{2}\right)\slashed{P}_B\gamma^{\mu'}\left(\frac{1-\gamma_5}{2}\right)\right]\nnu
&\times\mathrm{Tr}\left[\hat{\slashed{P}}_C\gamma^\nu\left(\frac{1-\gamma_5}{2}\right)\hat{\slashed{P}}_A\gamma^{\nu'}\left(\frac{1-\gamma_5}{2}\right)\right]\nnu
=&\, 8(G_Fm_W^2)^2|V_{ud}|^2\frac{1}{(\hat{t}-m_W^2)^2+(m_W\Gamma_W)^2}\nnu
&\times\mathrm{Tr}\left[\slashed{P}_D\gamma^\mu\left(\frac{1-\gamma_5}{2}\right)\slashed{P}_B\gamma^{\nu}\left(\frac{1-\gamma_5}{2}\right)\right]\nnu
&\times\mathrm{Tr}\left[\hat{\slashed{P}}_C\gamma_\mu\left(\frac{1-\gamma_5}{2}\right)\hat{\slashed{P}}_A\gamma_{\nu}\left(\frac{1-\gamma_5}{2}\right)\right]\,.
\eea
Here $\hat{{P}}_A=xP_A$ and $\hat{{P}}_C={P}_J$ and we used $4G_F/\sqrt{2}=e^2/(2 m_W^2\sin^2\theta_w)$. For a longitudinally polarized proton with helicity $\lambda_p$, we substitute $\hat{\slashed{P}}_A\rightarrow \gamma_5\hat{\slashed{P}}_A$. For a transversely polarized proton with transverse spin $S_T^i$, we have $\hat{\slashed{P}}_A\rightarrow \gamma_5\gamma_i\hat{\slashed{P}}_A$. However, note that the trace of the hadronic tensor vanishes for a transversely polarized proton.
For a longitudinally polarized electron with helicity $\lambda_e$, one substitutes $\slashed{P}_B\rightarrow\slashed{P}_B+\lambda_e\gamma_5\slashed{P}_B$.
The leptonic tensor is given in terms of the momenta of the electron and the left-handed neutrino:
\bea
L^{\mu\nu}&=\mathrm{Tr}\left[\slashed{P}_D\gamma^\mu(1+\lambda_e\gamma_5)\slashed{P}_B\gamma^\nu\left(\frac{1-\gamma_5}{2}\right)\right]\nnu
&=(1-\lambda_e)\left(P_B^\mu P_D^\nu+P_B^\nu P_D^\mu-g^{\mu\nu}P_B\cdot P_D+i\epsilon^{\mu\nu P_BP_D}\right)\nnu
&=L_u^{\mu\nu}+L_p^{\mu\nu}\, ,
\eea
where 
\bea
L_u^{\mu\nu}&=\left(P_B^\mu P_D^\nu+P_B^\nu P_D^\mu-g^{\mu\nu}P_B\cdot P_D+i\epsilon^{\mu\nu P_BP_D}\right)\, ,\\
L_p^{\mu\nu}&=-\lambda_e\left(P_B^\mu P_D^\nu+P_B^\nu P_D^\mu-g^{\mu\nu}P_B\cdot P_D+i\epsilon^{\mu\nu P_BP_D}\right),\nnu
\eea
represent the polarized and unpolarized components of the leptonic tensor. We can then obtain the differential cross section given in \cref{eq:crosssection1} with the following structure functions
\bea
F_{UU}=&\sum_q \frac{|\overline{\mathcal{M}}_{eq\rightarrow\nu q'}|^2}{16\pi^2\hat{s}^2}H(Q,\mu)\,\mathcal{J}_q(p_T^{\mathrm{jet}}R,\mu)\nnu
&\times\int\frac{{\rm d}b_T b_T}{2\pi}J_0(q_Tb_T)\,f_1^{\mathrm{TMD}}(x,b_T,\mu, \zeta)\nnu
& \qquad\times S_q(b_T,y_{\mathrm{jet}},R,\mu)\, ,\nnu
=&\,\mathcal{C}\left[f_1\right]_{eq\rightarrow\nu q'}\, ,\\
F_{LU}=&\,\mathcal{C}\left[f_1\right]_{e_Lq\rightarrow\nu q'}\, ,\label{eq:flu}\\
F_{UL}=&\,\mathcal{C}\left[g_{1L}\right]_{eq_L\rightarrow\nu q'}\, ,\\
F_{LL}=&\,\mathcal{C}\left[g_{1L}\right]_{e_Lq_L\rightarrow\nu q'}\, ,
\eea
\bea
F_{UT}^{\cos(\phi_{q}-\phi_{S_A})}=&\sum_q \frac{|\overline{\mathcal{M}}_{eq_L\rightarrow\nu q'}|^2}{16\pi^2\hat{s}^2}H(Q,\mu)\,\mathcal{J}_q(p_T^{\mathrm{jet}}R,\mu)\nnu
&\times\int\frac{{\rm d}b_T b_T^2}{4\pi M}J_1(q_Tb_T)\,g_{1T}^{(1),\mathrm{TMD}}(x,b_T,\mu, \zeta)\nnu
& \qquad\times S_q(b_T,y_{\mathrm{jet}},R,\mu)\, ,\nnu
=&\tilde{\mathcal{C}}\left[g_{1T}\right]_{eq_L\rightarrow\nu q'}\, ,\\
F_{LT}^{\cos(\phi_{q}-\phi_{S_A})}=&\,\tilde{\mathcal{C}}\left[g_{1T}\right]_{e_Lq_L\rightarrow\nu q'}\, ,\\
F_{UT}^{\sin(\phi_{q}-\phi_{S_A})}=&\,\tilde{\mathcal{C}}\left[f^\perp_{1T}\right]_{eq\rightarrow\nu q'}\, ,\\
F_{LT}^{\sin(\phi_{q}-\phi_{S_A})}=&\,\tilde{\mathcal{C}}\left[f^\perp_{1T}\right]_{e_Lq\rightarrow\nu q'}\, .
\eea

The relevant leading-order matrix elements squared are given by
\bea
|\overline{\mathcal{M}}_{eu\rightarrow\nu d}|^2
=&\, 8(G_F m_W^2)^2|V_{ud}|^2\frac{\hat{s}^2}{(\hat{t}-m_W^2)^2+m_W^2\Gamma_W^2}\,,\\
|\overline{\mathcal{M}}_{e\bar{d}\rightarrow\nu \bar{u}}|^2
=&\,8(G_F m_W^2)^2|V_{ud}|^2\frac{\hat{u}^2}{(\hat{t}-m_W^2)^2+m_W^2\Gamma_W^2} \,,\\
|\overline{\mathcal{M}}_{e_Lq\rightarrow\nu q'}|^2 =&\,-|\overline{\mathcal{M}}_{eq\rightarrow\nu q'}|^2\,,\\ \label{eq:eLq} 
|\overline{\mathcal{M}}_{eq_L\rightarrow\nu q'}|^2 =&\,-|\overline{\mathcal{M}}_{eq\rightarrow\nu q'}|^2\,,\\
|\overline{\mathcal{M}}_{e_Lq_L\rightarrow\nu q'}|^2 =&\,|\overline{\mathcal{M}}_{eq\rightarrow\nu q'}|^2\,, \label{eq:eLqL} 
\eea
The matrix elements for an unpolarized and polarized electron are related to each other, see \cref{eq:eLq}, \cref{eq:eLqL} due to the factor $(1-\lambda_e)$ in the expression of the leptonic tensor. As a result, we obtain the following relations between the different structure functions:
\bea
F_{LU}&=-F_{UU}\,,\\
F_{LL}&=-F_{UL}\,,\\
F_{LT}^{\cos(\phi_q-\phi_{S_A})}&=-F_{UT}^{\cos(\phi_q-\phi_{S_A})}\,,\\
F_{LT}^{\sin(\phi_q-\phi_{S_A})}&=-F_{UT}^{\sin(\phi_q-\phi_{S_A})}\,.
\eea

\section{Hadron distributions inside the jet~\label{app:h-in-jet}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
For an unpolarized electron collide with a transversely polarized $\bar{d}$-quark from initial proton, one has
Then
\bea
|\overline{\mathcal{M}}_{eu_T\rightarrow\nu d_T}|^2
&=
8(G_F m_W^2)^2|V_{ud}|^2\frac{2\hat{u}\hat{s}}{(\hat{t}-m_W^2)^2+m_W^2\Gamma_W^2}
\,,\\
|\overline{\mathcal{M}}_{e\bar{d}_T\rightarrow\nu \bar{u}_T}|^2 
&=
8(G_F m_W^2)^2|V_{ud}|^2\frac{2\hat{u}\hat{s}}{(\hat{t}-m_W^2)^2+m_W^2\Gamma_W^2}
\,,\\
|\overline{\mathcal{M}}_{e_Lu_T\rightarrow\nu d_T}|^2
&=
|\overline{\mathcal{M}}_{eu_T\rightarrow\nu d_T}|^2
\,,\\
|\overline{\mathcal{M}}_{e_L\bar{d}_T\rightarrow\nu \bar{u}_T}|^2
&=
|\overline{\mathcal{M}}_{e\bar{d}_T\rightarrow\nu \bar{u}_T}|^2
\,.
\eea

The azimuthal angular dependence for $h_1^\perp,\ h_{1L}^\perp,\ h_1$ and $h_{1T}^\perp$ are respectively:
\bea
h_1^\perp:& \frac{1}{Mz_hM_h}\left(\cos(\phi_{q}-\hat{\phi}_h)-i\sin(\phi_{q}-\hat{\phi}_h)\right)\, ,\\
h_{1L}^\perp:& \frac{\lambda_p}{Mz_hM_h}\left(\sin(\phi_{q}-\hat{\phi}_h)+i\cos(\phi_{q}-\hat{\phi}_h)\right)\, ,\\
h_1:& \frac{|S_T|}{z_hM_h}\left(\sin(\phi_{S_A}-\hat{\phi}_h)+i\cos(\phi_{S_A}-\hat{\phi}_h)\right)\, ,\\
h_{1T}^\perp:& \frac{|S_T|}{2M^2z_hM_h}\left(\sin(2\phi_{q}-\phi_{S_A}-\hat{\phi}_h)\right.\nonumber\\
&\left.+i\cos(2\phi_{q}-\phi_{S_A}-\hat{\phi}_h)\right)\, .
\eea
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For an unpolarized final-state hadron, we obtain TMD JFFs $\mathcal{D}_1,\ \mathcal{H}_1^\perp$ at leading-twist~\cite{Kang:2021ffh}. The corresponding correlator can be written as follows
\bea\label{eq:jT_direction_dependent}
\Delta(z_h,\vec{j}_T)=&\mathcal{D}_1^{h/q}(z_h,{j}_T)\frac{\slashed{n}_-}{2}\nnu
&-i\mathcal{H}^{\perp,h/q}_1(z_h,{j}_T)\frac{\slashed{j_T}}{z_hM_h}\frac{\slashed{n}_-}{2}\, ,
\eea
where we suppress the depenence on the renormalization scale $\mu$ and the Collins-Soper scale $\zeta$~\cite{Collins:2011zzd}. The different traces of the correlator are given by
\bea
\Delta^{h/q[\gamma^-]}=&\mathcal{D}_1^{h/q}(z_h,{j}_T)\, ,\\
\Delta^{h/q[i\sigma^{i-}\gamma_5]}=&\frac{\epsilon_T^{ij}{j_T}^j}{z_hM_h}\mathcal{H}^{\perp,h/q}_1(z_h,{j}_T)\, ,
\eea
For an electron colliding with an unpolarized or a longitudinally polarized initial proton, we obtain the same partonic scattering amplitudes as shown in Appendix~\ref{app:jet}.  However, if the electron collides with a transversely polarized quark from the initial proton, the corresponding term in the hadronic tensor is given by 
\bea
H^{\mu\nu}_{\mathcal{H}_1^{\perp h/q}}={\rm Tr}\left[\frac{\slashed{j_T}}{z_hM_h}\hat{\slashed{P}}_C\gamma^\mu\left(\frac{1-\gamma_5}{2}\right)\slashed{v}\hat{\slashed{P}}_A\gamma^\nu\left(\frac{1-\gamma_5}{2}\right)\right]\,
\label{eq:had_tensor}
\eea
where $\hat{{P}}_A=xP_A$ and $\hat{{P}}_C={P}_J$. For different TMD PDFs, the vector $\slashed{v}$ is given by $\big(-\slashed{S}_T\gamma_5\big)$ for $h_1$, $\big(-\lambda_p\slashed{k}_T\gamma_5/M\big)$ for $h_{1L}^\perp$, $\big(-i\slashed{k}_T/M\big)$ for $h_1^\perp$ and $\big((\vec{k}_T\cdot\vec{S}_T\slashed{k}_T-\vec{k}_T^2\slashed{S}_T/2)\gamma_5/M^2\big)$ for $h_{1T}^\perp$. Note that there are always three $\gamma$ matrices between the $(1-\gamma_5)/2$ factors in the expression of the hadronic tensor in \cref{eq:had_tensor}. Thus, we find
\bea\label{eq:g5mat}
&\left(\frac{1-\gamma_5}{2}\right)\gamma_\alpha\gamma_\beta\gamma_\rho\left(\frac{1-\gamma_5}{2}\right)\nnu
&=\gamma_\alpha\gamma_\beta\gamma_\rho\left(\frac{1+\gamma_5}{2}\right)\left(\frac{1-\gamma_5}{2}\right)=0\,.
\eea
Therefore, the expression in \cref{eq:had_tensor} vanishes and spin asymmetries involving transversely polarized quarks in CC DIS are zero. As a result, all contributions related to chiral-odd Collins jet fragmentation function do not appear in the differential cross section for hadron-in-jet production. Here, we show the differential cross section in terms of the remaining non-zero structure functions
\bea
&\frac{{\rm d}\sigma^{ep\rightarrow \nu+\mathrm{jet}X}}{{\rm d}y_J\, {\rm d}^2p_{JT}\, {\rm d}^2q_T\,{\rm d}z_h\,{\rm d}^2{j_T}}=F^h_{UU}+\lambda_p F^h_{UL}\nnu
&+|S_T|\left[\cos(\phi_{q}-\phi_{S_A})F_{UT}^{h,\cos(\phi_{q}-\phi_{S_A})}\right.\nnu
&\hspace{1.2cm}\left.+\sin(\phi_{q} -\phi_{S_A})F_{UT}^{h,\sin(\phi_{q}-\phi_{S_A})}\right]\nnu
&+\lambda_e\left[F^h_{LU}+|S_T|\sin(\phi_{q}-\phi_{S_A})F_{LT}^{h,\sin(\phi_{q}-\phi_{S_A})}\right.\nnu
&\quad+\left.\lambda_pF^h_{LL}+|S_T|\cos(\phi_{q}-\phi_{S_A})F_{LT}^{h,\cos(\phi_{q}-\phi_{S_A})})\right]\,.
\eea
In total there are 8 structure functions, which are given by
\bea
F^h_{UU}=&\sum_q \frac{|\overline{\mathcal{M}}_{eq\rightarrow\nu q'}|^2}{16\pi^2\hat{s}^2}H(Q,\mu)\,\mathcal{D}_{1}(p_T^{\mathrm{jet}}R,\mu)\nnu
&\times\int\frac{{\rm d}b_Tb_T}{2\pi}J_0(q_Tb_T)\,f_1^{\mathrm{TMD}}(x,b_T,\mu, \zeta)\nnu
&\times S_q(b_T,y_{\mathrm{jet}},R,\mu)\, ,\nnu
=&\,\mathcal{C}^h\left[f_1\mathcal{D}_1\right]_{eq\rightarrow\nu q'}\, ,\\
F^h_{LU}=&\,\mathcal{C}^h\left[f_1\mathcal{D}_1\right]_{e_Lq\rightarrow\nu q'}\, ,\\
F^h_{UL}=&\,\mathcal{C}^h\left[g_{1L}\mathcal{D}_1\right]_{eq_L\rightarrow\nu q'}\, ,\\
F^h_{LL}=&\,\mathcal{C}^h\left[g_{1L}\mathcal{D}_1\right]_{e_Lq_L\rightarrow\nu q'}\, ,
\eea
\bea
F_{UT}^{h,\cos(\phi_{q}-\phi_{S_A})}=&\sum_q \frac{|\overline{\mathcal{M}}_{eq_L\rightarrow\nu q'}|^2}{16\pi^2\hat{s}^2}H(Q,\mu)\,\mathcal{D}_{1}(p_T^{\mathrm{jet}}R,\mu)\nnu
&\times\int\frac{{\rm d}b_T b_T^2}{4\pi M}J_1(q_Tb_T)\,g_{1T}^{(1),\mathrm{TMD}}(x,b_T,\mu, \zeta)\nnu
&\times S_q(b_T,y_{\mathrm{jet}},R,\mu)\, ,\nnu
=&\,\tilde{\mathcal{C}}^h\left[g_{1T}\mathcal{D}_1/M\right]_{eq_L\rightarrow\nu q'}\, ,\\
F_{LT}^{h,\cos(\phi_{q}-\phi_{S_A})}=&\,\tilde{\mathcal{C}}^h\left[{g_{1T}\mathcal{D}_1}/{M}\right]_{e_Lq_L\rightarrow\nu q'}\, ,\\
F_{UT}^{h,\sin(\phi_{q}-\phi_{S_A})}=&\,\tilde{\mathcal{C}}^h\left[{f^\perp_{1T}\mathcal{D}_1}/{M}\right]_{eq\rightarrow\nu q'}\, ,\\
F_{LT}^{h,\sin(\phi_{q}-\phi_{S_A})}=&\,\tilde{\mathcal{C}}^h\left[{f^\perp_{1T}\mathcal{D}_1}/{M}\right]_{e_Lq\rightarrow\nu q'}\, .
\eea

\iffalse
\bea
F^{h,\sin(\phi_{S_A}-\hat{\phi}_h)}_{UT}=&{\mathcal{C}}^h\left[\frac{h_1\mathcal{H}_{1}^\perp}{z_hM_h}\right]_{eq_T\rightarrow\nu q'_T}\, ,\\
F^{h,\sin(\phi_{S_A}-\hat{\phi}_h)}_{LT}=&{\mathcal{C}}^h\left[\frac{h_1\mathcal{H}_{1}^\perp}{z_hM_h}\right]_{e_Lq_T\rightarrow\nu q'_T}\, ,\\
F^{h,\cos(\phi_{q}-\hat{\phi}_h)}_{UU}=&\tilde{\mathcal{C}}^h\left[\frac{h^\perp_1\mathcal{H}_{1}^\perp}{Mz_hM_h}\right]_{eq_T\rightarrow\nu q'_T}\, ,\\
F^{h,\sin(\phi_{q}-\hat{\phi}_h)}_{UL}=&\tilde{\mathcal{C}}^h\left[\frac{h^\perp_{1L}\mathcal{H}_{1}^\perp}{Mz_hM_h}\right]_{eq_T\rightarrow\nu q'_T}\, ,\\
F^{h,\cos(\phi_{q}-\hat{\phi}_h)}_{LU}=&\tilde{\mathcal{C}}^h\left[\frac{h^\perp_1\mathcal{H}_{1}^\perp}{Mz_hM_h}\right]_{e_Lq_T\rightarrow\nu q'_T}\, ,\\
F^{h,\sin(\phi_{q}-\hat{\phi}_h)}_{LL}=&\tilde{\mathcal{C}}^h\left[\frac{h^\perp_{1L}\mathcal{H}_{1}^\perp}{Mz_hM_h}\right]_{e_Lq_T\rightarrow\nu q'_T}\, ,\\
&F_{UT}^{h,\cos(2\phi_{q}-\phi_{S_A}-\hat{\phi}_h)}=\sum \frac{|\overline{\mathcal{M}}_{eq_T\rightarrow\nu q'_T}|^2}{16\pi^2\hat{s}^2}H(Q,\mu)\nnu
&\qquad\times\frac{\mathcal{H}^\perp_{1}(p_T^{\mathrm{jet}}R,\mu)}{z_hM_h}\int\frac{b_T^3db_T}{8\pi}J_2(q_Tb_T)\nnu
&\qquad\times\frac{h_{1T}^{\perp,\mathrm{TMD}}(x,b_T,\mu, \zeta)}{2M^2}S_q(b_T,y_{\mathrm{jet}},R,\mu)\, ,\nnu
&=\tilde{\tilde{\mathcal{C}}}^h\left[\frac{h^\perp_{1T}\mathcal{H}_{1}^\perp}{2M^2z_hM_h}\right]_{eq_T\rightarrow\nu q'_T}\, ,\\
&F_{LT}^{h,\cos(2\phi_{q}-\phi_{S_A}-\hat{\phi}_h)}=\tilde{\tilde{\mathcal{C}}}^h\left[\frac{h^\perp_{1T}\mathcal{H}_{1}^\perp}{2M^2z_hM_h}\right]_{e_Lq_T\rightarrow\nu q'_T}\, ,
\eea
\fi

We can obtain relations between the different hadron-in-jet structure functions analogous to inclusive jets production (see Appendix~\ref{app:jet}):

\bea
F^h_{LU} &= -F^h_{UU}\,,\\
F^h_{LL}&=-F^h_{UL}\,,\\
F_{LT}^{h,\cos(\phi_q-\phi_{S_A})}&=-F_{UT}^{h,\cos(\phi_q-\phi_{S_A})}\,,\\
F_{LT}^{h,\sin(\phi_q-\phi_{S_A})}&=-F_{UT}^{h,\sin(\phi_q-\phi_{S_A})}\,.
\eea
\end{subappendices}

==> ch6.5-moreQC.tex <==
\section{Outlook}
Besides studying the thermal behavior of QCD phase diagram, quantum simulations can also be applied to: (1) parton physics, (2) open quantum system, (3) parton shower in a medium, etc. Exploring these topics presents exciting prospects for physics research at the Electron-Ion Collider (EIC), a facility that offers high-energy and high-luminosity beams with a wide range of beam energies, polarizations, and ion species. This versatility provides a unique tool to image quarks and gluons with high precision and to investigate the new QCD frontier of strong color fields in nuclei. Ultimately, these efforts aim to deepen our understanding of how matter is fundamentally composed.

As illustrated in the previous sections, a range of quantum computing applications have arisen in high-energy and nuclear physics in recent years~\cite{Preskill_2018,Jordan1130,kaplan2017ground,Preskill:2019WY,Klco_2019,PhysRevLett.120.210501,PhysRevA.98.032331,PhysRevD.101.074038,PhysRevD.101.074512,Roggero_2020,Chang2019,cloet2019opportunities,Nachman_2021,PhysRevD.102.016007,Wei_2020,Holland_2020,PhysRevLett.124.080501,Shaw_2020,Liu_2020,kreshchuk2020quantum,PhysRevResearch.2.023342,Klco_2020,Di_Matteo_2021,davoudi2020search,Bepari_2021}. In this subsection, we will explain why quantum computing provides a potentially transformative approach for studying and understanding QCD, especially the scientific topics which are relevant to the future Electron-Ion Collider (EIC).

The high-energy and high-luminosity EIC capable of a versatile range of beam energies, polarizations and ion species is the novel tool to precisely image quarks and gluons, and to explore the new QCD frontier of strong color fields in nuclei -- to understand how matter at its most fundamental level is made. 
%Following endorsement by the National Academy of Sciences, 
In early 2020, DOE has selected Brookhaven National Laboratory as the site for building the EIC. The EIC user community developed the EIC yellow report~\cite{AbdulKhalek:2021gbh} in 2020, which lists the key science questions the EIC will address. Among them, the following three important questions are essential to this section:
\begin{itemize}
    \item[i.] How are partons inside the nucleon distributed in both momentum and position space? 
    \item[ii.] How do the confined hadronic states emerge from quarks and gluons?
    \item[iii.] How do color-charged quarks and gluons, and jets, interact with a nuclear medium?
\end{itemize}
All these questions can be answered and understood from the scattering cross section data measured from the future EIC. Questions i is related to the structure of the proton in terms of quarks and gluons (collectively called partons), as encoded in the so-called parton distribution functions (PDFs) and their extensions. Question ii explains how the partons turn themselves into hadrons, the process of fragmentation, which is encoded in various fragmentation functions (FFs). Finally, Question iii would understand quantum many-body physics (a dynamics process) in the nuclear medium. Both PDFs and FFs are correlation functions that are defined in terms of the fundamental field on the light cone. In other words, these correlation functions are not only separated in space but also in real-time. All these three questions involve the description of QCD in real-time and can in principle be studied on quantum computers. 

In the next subsections, we provide possible directions where quantum simulations can be applied for EIC physics: (1) soft function, (2) open quantum system, and (3) parton shower. In each of these sections, for each proposed topic, we provide our preparation and work for a known example, which can further lead to future projects. In ``soft function'', we would deal with Questions i and ii above. Both topics (2) and (3) deal with Question iii. In ``open quantum system'', we treat jet interaction with the nuclear medium as an open quantum system and perform quantum simulation for jet modification in the medium via a Lindblad equation~\cite{KOSSAKOWSKI1972247,GORINI1978149,Lindblad1976}. In ``parton shower'', we compute $1\to 2$ parton helicity amplitudes via a quantum computer, since such  parton branching is the basic element for parton shower. This would hopefully provide insights for parton shower in the nuclear medium. Needless to say, all these studies are exploratory, in the sense they are not for the true QCD, but for some simplified models that mimic QCD and the nuclear medium, to demonstrate the proof of concept in the near-term noisy intermediate quantum (NISQ) era~\cite{Preskill_2018}.

\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Parton Physics}
%%%%%%%%%%%%%%%%%%%%%%%%
Studying the fundamental partonic structure of hadrons and the fragmentation process from partons to hadrons have been essential in QCD calculations for many years~\cite{Ellis:1991qj,Collins:2011zzd}. Such information is encoded in the PDFs and FFs, respectively, whose intrinsic scale is on the order of $\Lambda_{\mathrm QCD}\sim 200$~MeV corresponding to the size of the hadron $1/R$ with $R\sim 1$~fm. QCD strong coupling constant is very large at such a scale and thus the usual perturbation theory fails. Because of their non-perturbative nature, PDFs and FFs are usually extracted from the experimental data through global analysis~\cite{Dulat:2015mca,Butterworth:2015oua,deFlorian:2007aj} within the so-called QCD factorization framework~\cite{Collins:1989gx}. As defined below, PDFs and FFs are light-cone correlators and thus naturally depend on real-time. However, in the formulation of non-perturbative QCD on a Euclidean lattice, one cannot directly calculate time-dependent correlations. A recent breakthrough~\cite{Ji:2013dva} by X.~Ji has enables us to extract the PDFs via the approach of so-called quasi-PDFs within Large-Momentum Effective Theory~\cite{Ji:2020ect}. However, such a method does not apply to the FFs, since the FFs involve the non-inclusive final state and so far there are no lattice QCD computations for the FFs~\cite{Metz:2016swz}. With the exceptional capability in solving real-time evolution problems of field theory and increasing applications found for nuclear and particle physics, quantum algorithms and quantum computers become highly promising in overcoming the difficulties faced by lattice QCD on classical computers.

%%%%%%%%%%%%

%%%%%%%%%%%%
Recently, with the assistance of quantum algorithms, accurately determining an unpolarized parton distribution functions in a meson has been realized in \cite{Li:2021kcs} using $1+1$ dimensional Nambu-Jona-Lasinio (NJL) model~\cite{Nambu:1961tp,Nambu:1961fr}. While simulating real QCD is still unreachable at the moment, the NJL model captures many fundamental features of QCD and provides a unified picture of vacuum, mesons, and nucleons~\cite{Christov:1995vm,Klevansky:1992qe}, and thus would be a great starting point to demonstrate conceptual proof of quantum algorithms. Below we first review the procedure provided in~\cite{Li:2021kcs} and we have prepared and tested our quantum algorithms for unpolarized PDFs using $\mathtt{IBM}$ quantum simulators. 

With the general framework and quantum algorithms ready for unpolarized PDFs, we propose to study longitudinally polarized PDFs (referred to as helicity distribution functions), GPDs, and FFs. We derive the new formula and layout the general procedure for these additional parton distributions and fragmentation functions. 

%\subsubsection{Existing work and our preparation: unpolarized PDFs}
\label{sec:un-pdf}
Recently, the authors of \cite{Li:2021kcs} provide a systematic quantum algorithm to compute unpolarized PDFs in a meson, using $1+1$ dimensional NJL model, 
$\mathcal{L}=\bar{\psi}_\alpha(i\gamma^\mu\partial_\mu-m_\alpha)\psi_\alpha+g(\bar{\psi}_\alpha{\psi}_\alpha)^2$, 
where $g$ is the coupling constant of the strong force, $\alpha$ indicates the flavor of the distributed parton and $m_\alpha$ is the quark mass. For $1+1$ dimension, 
%the light-cone coordinate is given by $n^\mu=(1,-1)$ and 
the quark field of one flavor $\psi_\alpha(0,x)$ can be discretized in $N/2$ lattice sites based on the staggered fermion approach \cite{BOCK1993605,PhysRevD.91.034504} and then further performed with Jordan-Wigner transformation~\cite{Jordan1928,PhysRevLett.63.322,Backens2019}
\begin{align}\label{eq:discrete}
\psi_\alpha(0,x)=
%\begin{pmatrix}
%\phi_{\alpha,2x}\\ \phi_{\alpha,2x+1}\end{pmatrix}=
\begin{pmatrix}
\Xi_{\alpha,2n}^3\sigma_{\alpha,2n}^+\\ \Xi_{\alpha,2n+1}^3\sigma_{\alpha,2n+1}^+\end{pmatrix}\,,\quad 0\le n\le \frac{N}{2}-1\,,
%$\Xi_{\alpha, n}^{3}=\left(\prod_{\beta=1}^{\alpha-1} \prod_{i=0}^{\frac{N}{2}-1}{\sigma}_{\beta, i}^{3}\right) \left(\prod_{j=0}^{n-1}{\sigma}_{\alpha, j}^{3}\right)$
\end{align}
where $\Xi_{\alpha, n}^{3}$ is introduced in \cite{Li:2021kcs}. The unpolarized PDF $f_{q/h}(x)$ in the hadron rest frame is defined by
\begin{align}
\label{eq:pdf}
&f_{q/h}(x)=\int\frac{dx'}{2\pi}e^{-ixM_hx'}\langle h|e^{iHt}\bar{\psi}(0,x')e^{-iHt}\frac{\gamma^+}{2}\psi(0,0)|h\rangle=\sum_{m,n=0}^1\sum_{x'}\frac{e^{-ixM_hx'}}{4\pi}T_{mn,\alpha}\,,
\end{align}
where $x$ is the momentum fraction of the hadron carried by the quark and we have $T_{mn,\alpha}=\langle h|e^{iHt}\Xi_{\alpha,-2x'+m}^{3,\dagger}\sigma_{\alpha,-2x'+m}^+e^{-iHt}\Xi_{\alpha,n}^3\sigma_{\alpha,n}^+|h\rangle$.

The systematic quantum algorithms which allow computing the unpolarized PDFs above are given as follows
\begin{enumerate}
\item {\textit Hadronic state preparation}. To begin with, the hadronic state $|h\rangle$ is prepared by quantum-number-resolving variational quantum eigensolver (VQE), where trial hadronic states $|\psi_{lk}\rangle$ and unitary operator $U(\theta)$ are assumed. The unitary operator $U(\theta)$ is constructed with the quantum alternating operator ansatz (QAOA) as introduced in~\cite{farhi2014quantum,PRXQuantum.1.020319}: $U(\theta)=\prod_{n=1}^{N_{\mathrm cycle}}\prod_{m=1}e^{i\theta_{nm}H_m}$, 
as shown in \cref{fig:njl_circ}. Here $N_{\mathrm cycle}$ is the number of total cycles in the initial state preparation process. To optimize for hadronic states, $U(\theta)$ will be applied to states $|\psi_{lk}\rangle$ repeatedly until the cost function $E_l(\theta)=\sum_i\omega_{li}\langle\psi_{li}|H|\psi_{li}(\theta)\rangle$ takes a minimum value at the parameter set $\theta^*$ \cite{PhysRevResearch.1.033062}. Thus $|h\rangle=U(\theta^*)|\psi_{lk}\rangle$ for the $k$-th excited state.
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.76\textwidth]{QC_figures/njl_circ.png}
    \caption{Quantum circuit for the hadronic preparation using QAOA in one loop. Each dashed-line box represents the operation of $\prod_{m=1}e^{i\theta_{nm}H_m}$ in one cycle.}
    \label{fig:njl_circ}
\end{figure}

\item {\textit Correlation function calculation}. With the initial hadronic states generated, one is able to evaluate PDFs given in \cref{eq:pdf} with the circuit given in \cref{fig:njl_circ_all}. The Hamiltonian can be decomposed into $H=\sum_{i=1}^4H_i$, where $[H_i,H_{i+1}]\ne0$, $H_1$ and $H_3$ form the periodic boundary condition, $H_2$ is diagonal and dependent on the coupling constant~$g$, providing interactions between two quark flavours and $H_4$ is also diagonal and dependent on the quark mass $m_\alpha$ and coupling constant $g$. Specifically, by taking $N=12$, namely $N/2=6$ lattice sites for each flavor, with very large layer number $N'$ and $\Delta t=t/N'$ defined, one obtains $e^{iHt}=\prod_{N'}e^{iH{t}/{N'}}\approx\prod_{N'}\prod_{j=1}^{4}e^{iH_j\Delta t}$ for \cref{eq:pdf} .
%which are easily written in terms of quantum gates by applying universality and properties of Clifford gates $H,\ S,\ $Pauli matrices, etc. More details can be found in \cite{Qiskit-Textbook}. 
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.63\textwidth]{QC_figures/njl_circ_all.png}
    \caption{Quantum circuit for calculating PDFs using $1+1$ NJL model.}
    \label{fig:njl_circ_all}
\end{figure} 
\end{enumerate}
Recently, this quantum algorithm has been proved to give consistent results with theoretical calculation in the $1+1$ dimensional NJL model and the quantum advantages over the classical Euclidean lattice methodology in resolving the intrinsic difficulties of simulating the real-time dynamics is demonstrated in \cite{Li:2021kcs}, indicating the possibility of studying the realistic hadron structures with more qubits in the future. Meanwhile, many applications have the potential to be achieved by extending this algorithm to the corresponding context. In the sections below, we propose three projects as promising applications of the quantum circuit setup introduced above.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Soft function}
%%%%%%%%%%%%
Soft function is usually generated by soft gluon radiation and can be obtained from soft limit of QCD amplitude. Because all momentum components would be small for soft function, the soft function in QCD is usually the most complicated and of course non-perturbative when the momentum scale is at the order of $\Lambda_{\mathrm QCD}$. However, in a large class of QCD factorization formula~\cite{Collins:2011zzd}, soft function is an indispensable ingredient and can be closely connected with the extraction of PDFs and FFs. Because of this, computing soft function from first principle is extremely important in fully understanding the hadron structure. Below we first review existing work and our quantum algorithm set-up, we then propose to use such algorithms to study soft function at the partonic threshold. This so-called threshold soft function is very essential in understanding PDFs $f_{q/h}(x)$ and FFs $D_1^{h/q}(z)$ at large $x\to 1$ (or $z\to 1$) region, which is of extremely practical use for the experimental program at Jefferson Lab~\cite{Dudek:2012vr}.

%\subsubsection{Existing work and our preparation}
\label{sec:soft_1}

Recently, the authors of \cite{Bauer:2021gup} presented a quantum circuit to compute a soft matrix element defined as $\langle X|\mathrm{~T}[Y_{n} Y_{\bar{n}}^{\dagger}]| \Omega\rangle$, where $T$ denotes the time-ordering operator, $|\Omega\rangle$ denotes the ground state and $|X\rangle$ is the final state. $Y_n$ ($Y_{\bar n}$) is a Wilson line representing particles moving in $n$ ($\bar n$) direction. As you will see from our section below, the square of such a matrix element 
\begin{align}
|\langle X|\mathrm{~T}[Y_{n} Y_{\bar{n}}^{\dagger}]| \Omega\rangle|^2\,,
\end{align}
is an indispensable component for defining the soft function in an actual physical process. Since the computation for gauge field is much more involved, the authors made use of the $1+1$ dimensional scalar $\phi$ field to illustrate the conceptual approach. We review and reproduce the results with our own quantum circuits at the $\mathtt{IBM}$ quantum simulators. In the next section, we propose to use this quantum algorithm to compute the threshold soft function. 

To start, the first step would be to prepare the ground state $|\Omega\rangle$ and the final state $|X\rangle$. The ground state $|\Omega\rangle$ of the scalar field theory is given by a multivariate Gaussian distribution, which is provided by $\mathtt{Qiskit}$ circuit library \cite{gadi_aleksandrowicz_2019_2562111}. For a field $\phi_i$ described by $N$ lattice sites, one has $N$ registers $|l_0\rangle,\ \cdots,\ |l_{N-1}\rangle$, where each register might include multiple qubits. Then each register is operated with $U_\Omega$, which creates the multivariate Gaussian vacuum state $|\Omega\rangle$ from the initial state as shown in \cref{fig:soft_circ_2}. After operating $U_Y$, the Wilson line operator, we apply the unitary operator $U_X^\dagger$ to prepare the final state $\langle X|$ for measurements, where $|X\rangle$ can be generated for either the vacuum state $|\Omega\rangle$ or states of definite multiplicity and momentum as presented in~\cite{Jordan:2011ne,Jordan:2011ci}. Besides applying a function from $\mathtt{Qiskit}$, one can also prepare states using the approach of Kitaev and Webb (KW)~\cite{kitaev2009wavefunction}. 
\iffalse
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.45\textwidth]{QC_figures/soft_circ_1.png}
    \caption{Quantum circuit for measuring the  transition rates from the vacuum state $|\Omega\rangle$ of the Wilson line to some state $|X\rangle$. $U_{\Omega}$ prepares initial ground state, $U_{X}^{\dagger}$ prepares final state $|X\rangle$ for measurements and $U_Y$ is the interaction operator.}
    \label{fig:soft_circ_1}
\end{figure}
\fi


%\subsubsection{Wilson expectation values}
Next, we will handle the Wilson line operators. As presented in~\cite{Jordan:2011ci,Klco:2018zqz,Bauer:2021gup}, the continuous field values in field theory can be digitized at each lattice point and further evaluated by digital quantum computers. For a lattice point described by $n_Q$ qubits, the number of possible values on that point is $2^{n_Q}$. In the 1+1 dimensional free scalar field model in~\cite{Bauer:2021gup}, the Wilson line $Y_n = {\mathrm P} \exp\left[ig\int_0^\infty ds\,\phi(x^\mu=n^\mu s)\right]$, and we have the discretized result
\begin{align}
\mathrm{T}[Y_{n} Y_{\bar{n}}^{\dagger}]=&e^{-i H n_{0} \delta x} \exp [i g \delta x(\phi_{x_{2 n_{0}}}-\phi_{x_{0}})]e^{i H \delta x} \exp [i g \delta(\phi_{x_{2n_{0}-1}}-\phi_{x_{1}})]\nonumber \\ 
& \times \cdots \times e^{i H \delta x} \exp [i g \delta x(\phi_{x_{n}}-\phi_{x_{n_{0}}})]\label{eq:soft}\,.
\end{align}
In other words, the Wilson line operator is made up of a series of time-evolution operators for a period that corresponds to the lattice spacing and field exponential. The last operated time evolution $e^{-i H n_{0} \delta x}$ evolves the state back from the largest time $n_0\delta x$ to $t=0$. To test the availability of this field discretization model, one applies $N=3$ lattice sites with $n_Q=2$ qubits for each site. The lattice spacing $\delta x$ is chosen to be 1. Then the expectation value of the Wilson line operator given in \cref{eq:soft} will be reduced to
\begin{align}
|\langle X|\mathrm{~T}[Y_{n} Y_{\bar{n}}^{\dagger}]| \Omega\rangle|^{2}=|\langle X|e^{iHt}e^{i g \delta x (\phi_{x_{2}}-\phi_{x_{0}})}e^{-iHt}| \Omega\rangle|^{2}\,.
\label{eqn:wilson}
\end{align}
Such transition rates from the vacuum state $|\Omega\rangle$ of the Wilson line to the final state $|X\rangle$ can be calculated using the circuit shown in \cref{fig:soft_circ_2}. 
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.75\textwidth]{QC_figures/soft_circ_0.png}
    \caption{Quantum circuit for measuring the transition rates from the vacuum state $|\Omega\rangle$ of the Wilson line to some final state $|X\rangle$. $U_{\Omega}$ prepares initial ground state, $U_{X}^{\dagger}$ prepares final state $|X\rangle$ for measurements and the middle dashed-line block shown is $U_Y$, the Wilson line operator for $N=3$ lattice sites with $n_Q=2$ qubits per site.}
    \label{fig:soft_circ_2}
\end{figure}
Here two examples with $|X\rangle = |\Omega\rangle$ and $|X\rangle = |p_1\rangle$ are shown in \cref{fig:soft_result}, where these soft transition rates are plotted as a function of the strong coupling constant $g$. The solid curves represent the analytical calculations, which are completely worked out for this simple scalar field model. The dashed curve are the perturbative results up to the first non-trivial order, i.e. next-to-leading order (NLO) at $\mathcal{O}(g^2$). It is evident that the quantum simulations agree with the analytical results, while the perturbative NLO results only work well for small $g$ as expected.
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.52\textwidth]{QC_figures/soft_0617.pdf}
    \caption{Results of the transition rate in quantum simulation (squared dots) and analytic calculation (solid lines) from the vacuum state $|\Omega\rangle$ of the Wilson line to vacuum state $|\Omega\rangle$ and one-particle momentum state $|p_1\rangle$ using $N=3$ lattice sites with $n_Q=2$ qubits per site.}
    \label{fig:soft_result}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Open quantum system}
%%%%%%%%%%%%


%%%%%%%%%%%%
%\subsection{Hard probes in hot medium}\label{sec:lind}
%%%%%%%%%%%%
Quantum simulation can be used to investigate the dynamics of large-scale systems that are in principle intractable using traditional methods. Nontrivial quantum computations, e.g. hybrid quantum-classical algorithms such as variational quantum eigensolver~\cite{McClean_2016,Kandala2017,Peruzzo2014,Arute2020,PhysRevX.8.011021,Chong2017} and fully quantum simulations of the unitary time evolution of closed quantum systems, can be carried out with parallel progress in quantum algorithms and executable quantum software. However, many physics systems are open systems that include interactions between the subsystems and the environment. To solve these problems, Refs.~\cite{KOSSAKOWSKI1972247,GORINI1978149,Lindblad1976} showed that the evolution of the subsystem is guided by a generalization of the Shr\"{o}dinger equation known as the Lindblad equation in the Markovian limit, where the environment correlation time is substantially less than the subsystem relaxation time. 

In the nuclear physics community, Lindblad equations have been derived for both heavy quarkonium~\cite{Yao:2021lus,Yao:2020eqy,Yao:2020xwx} and jets~\cite{Vaidya:2020cyi} interacting with the nuclear medium. In the quantum computing community, the authors of \cite{cleve2019efficient} developed efficient quantum algorithms for simulating Lindblad evolution. In~\cite{deJong:2020tvx}, the authors applied such quantum algorithms to describe heavy quarkonium interacting with the nuclear medium. On the other hand, there has been no quantum simulation for jet production in the nuclear medium and we propose to undertake this task. Below we first review the setup for heavy quarkonium in~\cite{deJong:2020tvx} and we reproduce their results with $\mathtt{IBM}$ quantum simulators. We then outline what's needed to study jet interaction in the nuclear medium. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  From slides
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Under weak coupling approximations, the evolution of the sub-system is governed by the Lindblad equation
\bea
\frac{\mathrm{d}}{\mathrm{d} t} \rho_{S}(t)=&-i\left[H_{S 1}(t)+H_{L}, \rho_{S}(t)\right]+\sum_{j=1}^{m}\left(L_{j} \rho_{S}(t) L_{j}^{\dagger}-\frac{1}{2}\left\{L_{j}^{\dagger} L_{j}, \rho_{S}(t)\right\}\right)\,
\eea
where $H_{S1}$ encodes the interaction inside the sub-system (between $c$ and $\bar{c}$), $H_L$ is the thermal correction generated by loop effects of $H_I$, and $L_j$ are Lindblad operators (non-unitary Lindblad evolution). In our toy model, $H_{S1}$ and $H_L$ are simplified to be $0$. The density matrix $\rho(t)$ of the whole system can be written as 
\bea
\rho(t)=\rho_S(t)\otimes\rho_E=|\psi_S(t)\rangle\langle\psi_S(t)|\otimes\rho_E\,.
\eea
with $\rho_S(t)$ representing the sub-system density matrix. Therefore, one can obtain the whole system density matrix at time $t$ by applying a unitary operator $U(t,0)$,
\bea
\rho(t)=U(t,0)\rho_S(0)\otimes\rho_EU^\dagger(t,0)\,.
\eea
Accordingly, one finally obtains the sub-system density matrix by taking a partial trace on the environment space as illustrated in \cref{fig:density-matrix}, namely
\bea
\rho_S(t)={\rm Tr}\left[U(t,0)\rho_S(0)\otimes\rho_EU^\dagger(t,0)\right]\,.
\eea
More specifically, the evolution of $\rho_{S}(t)=|\psi_S(t)\rangle\langle\psi_S(t)|$ can be obtained by the following quantum algorithm~\cite{DeJong:2020riy}
\begin{figure}[hp]
\centering
\includegraphics[width=0.7\textwidth]{QC_figures/openq3.png}
    \caption{Illustration of the whole system and sub-system density matrix.}
    \label{fig:density-matrix}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Existing work and our preparation: heavy quarkonium in medium} \label{sec:lind}

The whole system Hamiltonian, which includes the subsystem and the environment, can be expressed as $
H(t)=H_S(t)+H_E(t)+H_I(t)=H_{S_0}(t)+H_{S_1}(t)+H_E(t)+H_I(t)$, where $H_S(t)$, $H_E(t)$, and $H_I(t)$ are the Hamiltonians of the subsystem, the environment, and their interaction, respectively. $H_{S_0}$ is the free Hamiltonian of the subsystem and $H_{S_1}$ encodes the interaction inside the subsystem. The density matrix of the whole system is written as $\rho(t)=\rho_S(t)\otimes\rho_E$, 
%\begin{align}
%\rho(t)=\rho_S(t)\otimes\rho_E=|\psi_S(t)\rangle\langle\psi_S(t)|\otimes\rho_E\,.
%\end{align}
with $\rho_S(t)$ for the subsystem with dimension $d$. Under weak coupling approximations, the evolution of the subsystem is governed by the Markovian Lindblad equation \cite{KOSSAKOWSKI1972247,GORINI1978149,Lindblad1976}
\begin{align}
\frac{\mathrm{d}}{\mathrm{d} t} \rho_{S}(t)=&-i\left[H_{S 1}(t)+H_{L}, \rho_{S}(t)\right]+\sum_{j=1}^{m}\left(L_{j} \rho_{S}(t) L_{j}^{\dagger}-\frac{1}{2}\left\{L_{j}^{\dagger} L_{j}, \rho_{S}(t)\right\}\right)\,,
\end{align}
where $H_L$ denotes a thermal correction to $H_S$ generated by loop effects of $H_I$ , and the $L_j$ are Lindblad operators. It is well-known that Lindblad evolution is non-unitary and thus ancillary qubits are used in quantum simulations to achieve the results for the subsystem. Ref.~\cite{cleve2019efficient} has provided a quantum circuit to study Lindblad evolution, where the key ingredient, the $J$-operator, is a $d^2\times d^2$ block matrix with non-zero blocks $J_{0i}=L_i^\dagger$ and $J_{i0}=L_i$ $(i=1,\cdots,d^2-1)$. 

In~\cite{deJong:2020tvx}, the set-up for quantum simulation is provided and shown in \cref{fig:lindbladcycle} for one trotterization step, to study heavy quarkonium (subsystem) in the nuclear medium such as quark-gluon plasma (QGP, as environment).
\begin{figure}[hp]
\includegraphics[width=\textwidth]{QC_figures/openq40.png}
\caption{One trotterization evolution cycle for quantum state $|\psi\rangle$.}
\label{fig:lindbladcycle}
\end{figure}
 As a proof of concept, they treat the heavy quarkonium as a two-state system of heavy quark and anti-heavy quark: either bound or unbound state. They further set $H_{S_1}(t)=H_L(t)=0$, and treat the medium as a simple scalar $\phi$ field. Within this model, the dimension of $\rho_S(t)$ is $d=2$, and one needs 2 ancillary qubits. The quantum circuit is described in \cref{fig:lind_circ}, with the main ingredient given by the evolution factor $e^{-iJ\sqrt{t/N}}$, which is decomposed into single qubit rotations $\mathtt{U3}$ and $\mathtt{CNOT}$ gates by $\mathtt{qsearch}$ compiler \cite{davis2019heuristics} for circuit construction. 
As indicated in~\cite{deJong:2020tvx}, in the Markovian limit, two Lindblad operators $j = 0,\ 1$ are given with
\begin{align}
&L_j=\frac{\sqrt{\Gamma_j}}{2}\left(\sigma^X\mp i\sigma^Y\right)\,,\\
&\Gamma_0=\frac{g^2\Delta En_B(\Delta E)}{2\pi}\,,\ \Gamma_1=\Gamma_0+\frac{g^2\Delta E}{2\pi}\,.
\end{align}
Here the Bose-Einstein distribution $n_B(\Delta E)=({\mathrm exp}(\Delta E/T)-1)^{-1}$. 
By assuming no interaction inside the subsystem $H_{S_1}(t)$ and neglecting the loop corrections $H_L(t)$, the quantum algorithm for simulating the Markovian Lindblad equation is given in \cref{fig:lind_circ}. Here, the left dashed-line box corresponds to one cycle of time ${t/N}$. After each cycle, the two ancillary states $q_0$ and $q_1$ are traced out and after $N$ cycles, the subsystem state $q_2$ is measured at the end.
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.73\textwidth]{QC_figures/lindb_circ.png}
    \caption{ Quantum circuit for simulating the Lindblad equation \cite{cleve2019efficient}. %Here we have assumed little effects from $H_{S_1}(t)$ and $H_L(t)$. 
    The left block enclosed by the dashed line corresponds to one cycle of time ${t/N}$. After $N$ cycles, the measurement of the subsystem is performed to the state of the subsystem, namely $q_2$.
    }
    \label{fig:lind_circ}
\end{figure}
Next, using the $\mathtt{qsearch}$ compiler \cite{davis2019heuristics}, we decomposition each cycle of the quantum algorithm in \cref{fig:lind_circ} in terms of single qubit rotations $\mathtt{U3}$ and $\mathtt{CNOT}$ gates. An example is provided in \cref{fig:lind_circ_2}.
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.9\textwidth]{QC_figures/lindblad_g3_t5.png}
    \caption{Decomposition of a one cycle of the quantum algorithm in \cref{fig:lind_circ} in terms of single qubit rotations $\mathtt{U3}$ and $\mathtt{CNOT}$ gates using the $\mathtt{qsearch}$ compiler \cite{davis2019heuristics}. Three qubits $q_0$, $q_1$ and $q_2$ are used, where $q_0$ and $q_1$ are ancillary qubits represented the environment and $q_2$ corresponds to the subsystem.}
    \label{fig:lind_circ_2}
\end{figure}
In \cref{fig:lind_result}, we present the result for this toy model obtained from the $\mathtt{Qiskit}$ simulator at $\mathtt{IBM}$~\cite{gadi_aleksandrowicz_2019_2562111,ibmq} Quantum Experience. Here $P_0(t) \equiv \langle0|\rho_S(t)|0\rangle$ is measured as a function of time $t$ and is simply the surviving probability for the bound quarkonium state in the nuclear medium. The simulations of the quantum algorithm are shown for the coupling $g=0.3$ and $0.5$ with $N = 100$ cycles of $J$-operator. Our quantum simulation results are consistent with numerical solutions from the 4th order Runge-Kutta method, showing correctness of our algorithms, which indicates promising applications in applying quantum circuits for simulating open system physics.
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.57\textwidth]{QC_figures/lindblad_0617.pdf}
    \caption{Results of the quantum simulation using $\mathtt{Qiskit}$ with the number of cycles $N = 100$ for coupling constant $g=0.3$ and $0.5$ compared to numerical calculation with the 4th order Runge-Kutta method.}
    \label{fig:lind_result}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Parton shower in medium}
%%%%%%%%%%%%%%%%%%%%%%%%
The interpretation of measurements of high-energy particle collisions relies heavily on the performance of full event generators. One most important ingredient of an event generator is the parton shower, whose basic elements include the splitting functions, i.e. the probability for a parton to branch into two partons, and Sudakov factors that determine the probability for the system not to change between two shower
times. There are well-established event generators for proton-proton collisions such as Pythia~\cite{Sjostrand:2007gs}, Herwig~\cite{Bahr:2008pv}, and Sherpa~\cite{Gleisberg:2008ta}. On the other hand, a full event generator in heavy ion collisions is still under active developments e.g. within JETSCAPE collaboration~\cite{Putschke:2019yrg,Everett:2020xug}. Since parton shower is an indispensable ingredient for any event generator, we propose to study parton shower in the nuclear medium via quantum simulations. Since one parton branching into two partons is the basic element for developing parton shower, we start with the even basic $1\to 2$ helicity amplitudes. We first review the existing work and our preparation to study $1\to 2$ helicity amplitudes in vacuum. We then outline the steps how to study $1\to 2$ helicity amplitudes in the nuclear medium. The parton branch in the nuclear medium such as quark-gluon plasma should naturally be a dynamic process depending on the interaction between the partons and the medium before and after the branching. We expect that our quantum simulations for $1\to 2$ helicity amplitudes in the medium can offer some insights in this regard. 

As a result of the factorization theorem, the hard interaction and the parton shower are two elements of the event evolution that can be characterized perturbatively. While they are also the most time-consuming components of the event simulation in classical computers~\cite{Sjostrand:2007gs,Bahr:2008pv,Gleisberg:2008ta}. To speed up the event generator processes, the hard interaction is evaluated by the helicity amplitude calculations and a Markov chain algorithm is applied for the parton shower. As found by \cite{Bepari:2020xqi}, quantum algorithms are sufficient to provide reliable results for both hard scattering processes and parton shower.

%\subsection{Existing work and our preparation: $1\rightarrow 2$ helicity amplitude in vacuum} \label{sec:heli_1}
%%%%%%%%%%%%
In Ref.~\cite{Bepari:2020xqi}, the authors provided quantum algorithms for calculations of helicity amplitudes, which exploits the equivalence between spinors and qubits, and the unique features of a quantum computer to compute the helicities of each particle involved simultaneously, thus fully utilising the quantum nature of the computation. We review this method and reproduce the results with $\mathtt{IBM}$ quantum simulators. We start with the $q\rightarrow q+g$ process for a simple example of helicity amplitude calculation, where the vertex $\mathcal{M}^\pm_{gq\bar{q}}$ are given by
\begin{align}
\mathcal{M}_{gq\bar{q}}^+=-\frac{\sqrt{2}\langle p_fq\rangle[p_{\bar{f}}p]}{\langle qp\rangle}\,,\quad \mathcal{M}_{gq\bar{q}}^-= -\frac{\sqrt{2}\langle p_fp\rangle[p_{\bar{f}}q]}{[qp]}\,.
\label{eq:M-}
\end{align}
To calculate the products in each $gq\bar{q}$ vertex, one simply defines unitary operators $U_{p\rangle},\ U_{p]},\ U_{\langle p}$ and $U_{[p}$ as shown in \cite{Bepari:2020xqi}, such that $U_{p\rangle}|0\rangle=|p\rangle\,,\ U_{p]}|0\rangle=|p]\,,\ \langle 0|U_{\langle p}=\langle p|$ and  $\langle 0|U_{[p}=[p|\,.$
\iffalse
\begin{figure}[hbt!]
    \centering
    \includegraphics[width = 0.7\textwidth]{QC_figures/heli_circ.png}
    \caption{Gate decompositions for calculating helicity amplitudes in \cref{eq:M-}.
    \label{fig:hel_circ}
\end{figure}
\fi
For instance, by operating first $U_{q\rangle}$ then $U_{\langle p_f}$ on state $|0\rangle$ and measuring the final state in $\langle 0|$, one obtains $|\langle p_fq\rangle|^2$. For other products, the quantum circuits are shown in \cref{fig:hel_circ_all} for positive and negative helicity amplitudes in \cref{eq:M-}. 
\begin{figure}[hbt!]
    \centering
   \includegraphics[width = 0.4\textwidth]{QC_figures/pos_heli_circ.png}\hspace{0.5cm}
   \includegraphics[width = 0.4\textwidth]{QC_figures/neg_heli_circ.png}
  %\caption{Negative helicity.}
  %\label{fig:nhel_circ_all}
    \caption{Quantum circuit that calculates positive (left) and negative (right) helicity amplitude for the $q\rightarrow q+g$ process in \cref{eq:M-}.}
    \label{fig:hel_circ_all}
\end{figure}

In \cref{fig:hel}, we present the comparison between our quantum simulation results and theoretical calculations for helicity amplitude. The quantum simulations are produced via $\mathtt{IBM}$ quantum simulators with 3 qubits. For the theoretical calculations, we utilized the Mathematica package $\mathtt{Spinors\ @\ Mathematica\ (S@M)}$. We found that our quantum simulations are in good agreement with theoretical results. Along with the same logic, we are able to extend the process to $2\rightarrow n$ process. As $n$ increases, the time-saving advantage of quantum algorithms becomes growingly dominant and shows more superiority over their classical counterparts. 
\begin{figure}[hbt!]
    \centering
        \includegraphics[width = 0.9\textwidth]{QC_figures/pos_heli.png}
        \includegraphics[width = 0.9\textwidth]{QC_figures/neg_heli.png}
    \caption{Positive (top) and negative (bottom) helicity amplitude calculation results for the $q\rightarrow q+g$ process. Quantum simulating results from $\mathtt{IBM}$ quantum simulators are consistent with theoretical results which are calculated by the Mathematica package $\mathtt{S@M}$.}
    \label{fig:hel}
\end{figure}
 In the quantum circuit, each qubit corresponds to one product in \cref{eq:M-}. Therefore, one is able to calculate the amplitudes for more particle scattering by adding qubits and corresponding unitary gates. More over, by tracing out all qubits except one, the measurement equals to the modulus squared value of the product on that qubit. 

To simulate increasingly complicated hard interactions and splitting processes at higher-energy colliders in the future, quantum computing method can circumvent difficulties in generating these pseudo-data as well as consume less time. 

\section{Summary}
In conclusion, we performed a quantum simulation for the chiral phase transition of the 1+1 dimensional NJL model at finite temperature, baryochemical potential and chiral chemical potential using the \texttt{QITE} algorithm. Specifically, we use a 4-qubit quantum circuit to simulate the NJL Hamiltonian and find that the results among the digital quantum simulation, exact diagonalization, and analytical analysis are all consistent, implying that quantum computing will be a promising tool in simulating finite-temperature behaviors in the future for QCD.

The quantum simulations' efficacy has been shown to be insensitive to the chemical potentials $\mu$ and $\mu_5$ (and possibly other external parameters), which opens up new possibilities for studying finite density effects in QCD and other field theories. Owing to technological constraints (nonperturbative dynamics, Monte Carlo failure due to the sign problem, etc.) restricting the use of typical computing methods, this element of quark physics remains substantially unexplored in comparison to other fields. With the development of scalable quantum computing technologies on the horizon, Lattice QCD calculations on quantum computers are becoming not only conceivable, but also practical. 

We also present other directions explored in prior research, which shows that NISQ quantum computers may produce consistent and correct answers to physical issues that cannot be solved efficiently or effectively using classical computing algorithms, reflecting bright prospects for future applications of quantum computing to non-perturbative QCD in the NISQ era and beyond.


==> macros.tex <==

%
% thesis_macros
% Copyright (C) 1995 by John Heidemann, <johnh@isi.edu>
%

% \RequirePackage{johnh_general}

\RequirePackage{ifthen}

% \def\epsfreduction{0.667}
\def\epsfgraphreduction{0.9}

\newcommand\comment[1]{{[\sffamily #1]}}

%
% TeX seems to want to indent after chapters,
% although it shouldn't.  Rather than argue
% with it, I work around it manually by putting this
% hack in the right places:
\newcommand{\noindenthack}{\noindent}


\newcommand{\fwling}{featherweight layering}
\newcommand{\fwls}{featherweight layers}
\newcommand{\fwl}{featherweight layer}

\newcommand{\Fwling}{Featherweight layering}
\newcommand{\Fwls}{Featherweight layers}
\newcommand{\Fwl}{Featherweight layer}

\newcommand{\FwLing}{Featherweight Layering}
\newcommand{\FwLs}{Featherweight Layers}
\newcommand{\FwL}{Featherweight Layer}

\newcommand{\xvop}[2]{{\scomputer {{#1}\_{#2}}}}
\newcommand{\vop}[1]{\xvop{vop}{#1}}

\newcommand{\usec}{$\mu$seconds}
\newcommand{\unix}{Unix}

\newcommand{\dotdot}{\scomputer{..}}

\newenvironment{mycode}%
	{\small
	}{%
	}

\newcommand{\mylangle}{\langle}
\newcommand{\myrangle}{\rangle}
\newcommand{\myrightarrow}{\rightarrow}


%
% Sizes of various things:
%
  \newcommand{\tablesize}{\normalsize}
  \newcommand{\computertablesize}{\small}
  \newcommand{\bibliographysize}{\normalsize}

  %
  % Another space-saver:  shrink the figures and graphs.
  %
 \def\epsfreduction{0.85}
 \def\epsfgraphreduction{0.9}   % should be left at 0.9 with two-column text
% \def\epsfsize#1#2{\epsfreduction#1}

%\newcommand{\appendixnumbering}{
%	\renewcommand{\thechapter}{\Alph{chapter}}
%	\setcounter{chapter}{0}
%	}

\newenvironment{functions}%
	{\begin{description}}%
	{\end{description}}

\makeatletter
  \newcommand{\SubmitSingleSpace}{
    \ifissubmit
      \renewcommand\baselinestretch{\@singlespacing}\@normalsize
    \fi
  }
  \newcommand{\SubmitDoubleSpace}{
    \ifissubmit
      \renewcommand\baselinestretch{\@doublespacing}\@normalsize
    \fi
  }
\makeatother


\iffalse
Figure drawing style guide:

layer labels:
	helvetica 12pt bold
	(short acronyms) helvetica 14pt bold

spacing:  8 pixels
each layers will be 3 high and 7 or 7.5 wide

or spacing: 8 pts
each layer will be 4 high and 10 wide

boxes and vnode links are line #2
\fi



==> main.tex <==

%
% main.tex
% Copyright (C) 1995 by John Heidemann, <johnh@isi.edu>.
% $Id: demo2big.tex,v 1.2 1996/01/16 18:57:04 johnh Exp $
%

\input{include/macros}

\begin{document}

\input{include/titlepages}
\input{include/introduction}
%...
%\input{stacking_model}
%\input{stacking_techniques}
%\input{stacking_implementation}
%\input{stacking_evaluation}
%\input{coherence_architecture}
%\input{coherence_implementation}
%\input{coherence_evaluation}
%\input{fwl_implementation}
%\input{fwl_evaluation}
%\input{related_work}
%\input{conclusion}

%\appendix
%\input{stacking_appendix}
%\input{coherence_appendix}

%\bibliographystyle{uclathes}
%\bibliography{ficus,thesis}

%\input{colophon}

\end{document}



==> titlepages.tex <==

%
% Title pages of the thing
% Copyright (C) 1995 by John Heidemann, <johnh@isi.edu>.
%



\title{Stackable Design of File Systems}
\author{John~Shelby Heidemann}


\department{Computer Science}
\degreemonth{September}
\degreeyear{1995}

\chair{Gerald~J.~Popek}
\chair{D.~Stott Parker}
\member{Richard~Muntz}
\member{Rajive~L.~Bagrodia}
\member{Kirby~A.~Baker}

\dedication{\textsl{Are you dedicated?}}

\acknowledgments{
Ack!  P'tui.
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% vita
%
\vitaitem{1968}{B.S., Computer Science, Caribou University}
\vitaitem{etc.}{etc.}
\vitaitem{1995}{Graduated, UCLA}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% publications
%

\publication{
	Richard~G.\ Guy, John~S.\ Heidemann, Wai Mak, Thomas~W.\ Page,~Jr.,\ 
	  Gerald~J.\ Popek, and Dieter Rothmeier.
	Implementation of the Ficus
	  replicated file system.
	In \emph{USENIX Conference Proceedings}, pages
	  63--71.
	USENIX, June 1990.
}

\publication{
	etc.
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\include{abstract}

%
% I built a custom title page to do what I want.  So sue me.
% NEEDSWORK:  I had to copy some stuff from uclathti.sty.
%
\makeatletter
  \newcommand{\CustomTitlePage}{
    \begin{titlepage}
      \ColumnSave
      \vspace*{1.5in}   % a hacky way to center.  TeX didn't like \vfill.
      \begin{center}
  
      {\bfseries\huge \@title} \\
      \vskip 48pt plus0pt minus18pt
  
      {\large \@author} \\
      \vskip 12pt plus0pt minus3pt
      {\large University of California, Los Angeles} \\
      \vskip 6pt plus0pt minus2pt
      {\large \@degreemonth, \@degreeyear} \\
      \vskip 48pt plus0pt minus18pt
  
      \normalsize A \@thesisname\
      submitted in partial satisfaction \\
      of the requirements for the degree \\
      \@degreename\if@department\ in \@department \fi\\
      \vskip 24pt plus0pt minus6pt

      \normalsize
	UCLA Computer Science Department \\
	Technical Report UCLA-CSD-950032 \\
      \vskip 24pt plus0pt minus6pt

      \textbf{Thesis committee:} \\
      \ifnum\c@chairs<1
        \typeout{No committee chair.}
      \else\ifnum\c@chairs<2
        \@chairA, chair \\
      \else\ifnum\c@chairs<3
        \@chairA, co-chair \\
        \@chairB, co-chair \\
      \else\ifnum\c@chairs<4
        \@chairA, co-chair \\
        \@chairB, co-chair \\
        \@chairC, co-chair \\
      \fi\fi\fi\fi
      \ifnum\c@members<1 \typeout{No non-chair committee members.}\fi
      \ifnum\c@members>0 \@memberA \\ \fi
      \ifnum\c@members>1 \@memberB \\ \fi
      \ifnum\c@members>2 \@memberC \\ \fi
      \ifnum\c@members>3 \@memberD \\ \fi
      \ifnum\c@members>4 \@memberE \\ \fi
      \ifnum\c@members>5 \@memberF \\ \fi

      \end{center}
    \end{titlepage}
  }

  \newcommand{\CustomAcknowledgePage}{
  \chapter*{Acknowledgments}

  \@acknowledgments
  }
\makeatother

\ifissubmit
  \makeintropages
\else
  \makeatletter
    \pagenumbering{roman}
    \CustomTitlePage
    \@makecopyrightpage
    \@makededication
    \tableofcontents
    \listoffigures
    \listoftables
    \cleardoublepage
    \@makeabstractpage{1.0}
    \CustomAcknowledgePage
%    \@makevitapage

    \cleardoublepage
    \pagestyle{headings}
    \pagenumbering{arabic}
    \setcounter{page}{1}
  \makeatother
\fi


% LocalWords:  Stott Muntz Ted Yu Wu Michial Gunter Stovall Salomone Louie Qian
% LocalWords:  Qin Weidner McKusick Pendry Minshall kitrace Ousterhout CSD ftp
% LocalWords:  Administrativia csd ps HyperCard Yarvis Alexy Rudenko pt Los co
% LocalWords:  degreemonth degreeyear thesisname degreename chairA chairB roman
% LocalWords:  chairC memberA memberB memberC memberD memberE memberF arabic
% LocalWords:  makecopyrightpage makededication makeabstractpage Monique http
% LocalWords:  Bennarosh www html

